Breakdown of homoclinic orbits to L3 in the RPC3BP (II). An asymptotic formula

The Restricted 3-Body Problem models the motion of a body of negligible mass under the gravitational influence of two massive bodies called the primaries. If one assumes that the primaries perform circular motions and that all three bodies are coplanar, one has the Restricted Planar Circular 3-Body Problem (RPC3BP). In rotating coordinates, it can be modeled by a two degrees of freedom Hamiltonian, which has five critical points called the Lagrange points L1,.., L5. The Lagrange point L3 is a saddle-center critical point which is collinear with the primaries and beyond the largest of the two. In this paper, we obtain an asymptotic formula for the distance between the stable and unstable manifolds of L3 for small values of the mass ratio $0<\mu\ll 1$. In particular we show that L3 cannot have (one round) homoclinic orbits. If the ratio between the masses of the primaries $\mu$ is small, the hyperbolic eigenvalues of L3 are weaker, by a factor of order $\sqrt\mu$, than the elliptic ones. This rapidly rotating dynamics makes the distance between manifolds exponentially small with respect to $\sqrt\mu$. Thus, classical perturbative methods (i.e the Melnikov-Poincar\'e method) can not be applied. The obtention of this asymptotic formula relies on the results obtained in the prequel paper on the complex singularities of the homoclinic of a certain averaged equation and on the associated inner equation. In this second paper, we relate the solutions of the inner equation to the analytic continuation of the parameterizations of the invariant manifolds of L3 via complex matching techniques. We complete the proof of the asymptotic formula for their distance showing that its dominant term is the one given by the analysis of the inner equation.

==> Article Outer/commands.tex <==
%%%%%%%%%%%%%%%%%%%
% LATEX SHORTCUTS %
%%%%%%%%%%%%%%%%%%%

% EDITION
\def\singlespace{ \renewcommand{\baselinestretch}{1.0}\normalsize }
\def\middlespace{ \renewcommand{\baselinestretch}{1.3}\normalsize }
\def\doublespace{ \renewcommand{\baselinestretch}{2.0}\normalsize }
%\newcommand{\st}{\text{ : }}
\newcommand{\st}{\h:\h}
\newcommand{\stb}{\text{ }\big\rvert \text{ }}
\newcommand{\h}{\hspace{1mm}}
\newcommand{\hh}{\hspace{5mm}}
\newcommand{\pp}{\\[0.6em]}
\newcommand{\dps}{\displaystyle}
\newcommand{\coma}{\text{, \h }}
\newcommand{\dpf}[2]{\left( \frac{#1}{#2} \right)}
\newcommand{\idk}[1]{\mathbf{1}_{\{k=#1\}}}
\newcommand{\efr}[2]{^{\frac{#1}{#2}}}
\newcommand{\mefr}[2]{^{-\frac{#1}{#2}}}

% THEOREMS
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{theorem}[lemma]{Theorem}
%\theoremstyle{remark}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{example}[lemma]{Example}
%\theoremstyle{definition}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{notation}[lemma]{Notation}
\newtheorem{comentary}[lemma]{Comentary}
\def\figlabel#1{\label{#1}}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\beal{\begin{aligned}}
\def\enal{\end{aligned}}

% BASICS
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\normf}[1]{\llbracket#1\rrbracket}
\newcommand{\vabs}[1]{\left| #1 \right|}
\newcommand{\vabsSmall}[1]{| #1 |}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\claus}[1]{\left\{#1\right\}}
\newcommand{\boxClaus}[1]{\left[#1\right]}
\newcommand{\ii}{^{-1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\tl}{\tilde}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\renewcommand{\Re}{\mathrm{Re\, }}
\renewcommand{\Im}{\mathrm{Im\,}}
\renewcommand{\arg}{\mathrm{arg\,}}
\renewcommand{\inf}{\mathrm{inf\,}}

% SPACES
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\complexs}{\mathbb{C}}
\newcommand{\torus}{\mathbb{T}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\field}{\mathbb{F}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\scalarField}{\mathbb{K}}
\newcommand{\disc}{\mathbb{D}}

% TRIGONOMETRY
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\arccsc}{arcCsc}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arcsech}{arcsech}
\DeclareMathOperator{\arccsch}{arcCsch}
\DeclareMathOperator{\arccoth}{arcCoth} 

% GREEK ALPHABET
\newcommand{\al}{\alpha}
\newcommand{\bet}{\beta}
\newcommand{\de}{\delta}
\newcommand{\D}{\Delta}
\newcommand{\e}{\varepsilon}
\newcommand{\ph}{\varphi}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\s}{\sigma}
\newcommand{\Si}{\Sigma}
\newcommand{\tht}{\theta}
\newcommand{\Tht}{\Theta}
\newcommand{\ups}{\upsilon}
\newcommand{\Ups}{\Upsilon}
\newcommand{\bb}{B}
% \newcommand{\kk}{\kappa}
% \newcommand{\rr}{\rho}
%\newcommand{\be}{\beta}
% \newcommand{\om}{\omega}
% \newcommand{\lo}{\gamma}
% \newcommand{\Xxi}{\Xi}
% \newcommand{\ppi}{\phi}
% \newcommand{\Ppi}{\Phi}

% VECTORS
\newcommand{\vect}[1]{{\bm #1}}
\newcommand{\fb}{{\bm f}}
\newcommand{\nb}{{\bm n}}
\newcommand{\sbb}{{\bm s}}
\newcommand{\xb}{{\bm x}}
\newcommand{\zb}{{\bm z}}

% POINT DERIVATIVES
\newcommand{\qd}{\dot{q}}
\newcommand{\pd}{\dot{p}} 
\newcommand{\rd}{\dot{r}}
\newcommand{\ud}{\dot{u}}
\newcommand{\xd}{\dot{x}}
\newcommand{\yd}{\dot{y}}
\newcommand{\zd}{\dot{z}}
\newcommand{\zbd}{\dot{\bm z}}
\newcommand{\ttd}{\dot{\tau}}
\newcommand{\td}{\dot{\theta}}
\newcommand{\Rd}{\dot{R}}
\newcommand{\xdd}{\ddot{x}}
\newcommand{\udd}{\ddot{u}}
\newcommand{\rdd}{\ddot{r}}
\newcommand{\lad}{\dot{\lambda}}
\newcommand{\Lad}{\dot{\Lambda}} 

% OVERLINE VARIABLES
\newcommand{\xl}{\tilde{x}}
\newcommand{\yl}{\tilde{y}} 
\newcommand{\lal}{\tilde{\la}} 
\newcommand{\Lal}{\tilde{\La}} 

% DERIVATIVES
\newcommand{\pa}{\partial}
\newcommand{\Dt}[2]{\dfrac{d #1}{d {#2}}}
\newcommand{\Dx}[2]{\dfrac{\partial #1}{\partial {#2}}}
\newcommand{\Dxx}[2]{\dfrac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\Dxy}[3]{\dfrac{\partial^2 #1}{\partial {#2} \partial {#3}}}
\newcommand{\diff}[2]{\frac{d {#1}}{d {#2}}}
\newcommand{\dx}[2]{\frac{\partial #1}{\partial {#2}}}
\newcommand{\dt}[1]{\frac{d {#1}}{dt}}

% CALIGRAPHIC FONTS
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\GGh}{\widehat{\mathcal{G}}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NNN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\RRR}{\mathcal{R}}
\newcommand{\SSS}{\mathcal{S}}
\newcommand{\TTT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\ZZZ}{\mathcal{Z}}
\newcommand{\tEE}{\widetilde{\mathcal{E}}}


% OPERATORS
%\newcommand{\vect}{\mathrm{vec}}
\newcommand{\trace}{\text{Trace}}
\newcommand{\sgn}{\text{sgn}}
\newcommand{\Lip}{\mathrm{Lip}}
%\newcommand{\El}{\mathrm{El}}
%\newcommand{\Par}{\mathrm{Par}}
%\newcommand{\hyp}{\mathrm{hyp}}
%\newcommand{\el}{\mathrm{ell}}
\newcommand{\mix}{\mathrm{mix}}
\newcommand{\adj}{\mathrm{adj}}
\newcommand{\unc}{\mathrm{unc}}
\newcommand{\coup}{\mathrm{coup}}
\newcommand{\mi}{\mathrm{min}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\glob}{\mathrm{glob}}
\newcommand{\inte}{\mathrm{int}}
\newcommand{\fut}{\mathrm{f}}
\newcommand{\past}{\mathrm{p}}
%\newcommand{\h}{\mathrm{h}}
\newcommand{\ex}{\mathrm{e}}

% COLORS
\definecolor{myGreen}{RGB}{0, 200, 0}
\definecolor{myOrange}{RGB}{255, 100, 0}
\definecolor{myYellow}{RGB}{255, 200, 0}
\definecolor{myBlue}{RGB}{0, 200, 255}
\definecolor{myPurple}{RGB}{200, 0, 200}

% ARROWS
\newcommand{\SAParrow}{\hspace{0.2cm} \makebox[-0.25cm][l]{$\Bumpeq$}\longrightarrow}

% OTHER EXPRESSIONS
\newcommand{\Res}{\mathrm{Res\,}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\lln}{\llfloor}
\newcommand{\rrn}{\rrfloor}

% TRIANGLE
\usepackage{stackengine,scalerel}
\stackMath
\newcommand\that[1]{%
\setbox0=\hbox{$#1$}%
\ensurestackMath{%
	\stackon[2pt]{\copy0}{\,\rotatebox{90}{\stretchto{\triangleright}{\dimexpr\wd0-3pt}}}%
}%
}




==> Article Outer/difference.tex <==

We look for an asymptotic expression for the difference 
\[
\dzHat=(\dxOut,\dyOut)^T
=(\xuOut-\xsOut,\yuOut-\ysOut)^T,
\] 
where $(\xuOut,\yuOut)$ and $(\xsOut,\ysOut)$ are components of the perturbed invariant graphs given in Theorem \ref{theorem:existence}.
%
Recall that, by \eqref{eq:invariantEquationDifference2}, $\dzHat$ satisfies
\begin{equation}\label{eq:invariantEquationDifference3}
	\partial_u {\dzHat}(u) = 
	{\AAA}^{\spl}(u) \dzHat(u)
	+ 
	{\BB}^{\spl}(u) \dzHat(u),
\end{equation} 
with $\AAA^{\spl}$ and $\BB^{\spl}$ as given in \eqref{def:operatorsDifferenceAABB}.
%
%and, by the energy level formula in \eqref{eq:defDwOut}, the expression for $\dwOut$ is immediate from $(\dxOut,\dyOut)$.
%
%The point of writing the system for $\dzHat$ as~\eqref{eq:invariantEquationDifference2} is that, as we shall see, we split it into a dominant part, the one corresponding to the matrix $\AAA^{\spl}$, and a small perturbation,
%which corresponds to the the matrix ${\BB}^{\spl}$.
%%
%This allow us to find an asymptotic expression for $\dzHat$, with a dominant term $\dzHat_0$ given by the solution of the system
%
The equation is split as a dominant part, given by the matrix $\AAA^{\spl}$ and a small perturbation corresponding to the the matrix ${\BB}^{\spl}$.
%
Therefore, it makes sense to look for  $\dzHat$ as $\dzHat = \dzHatO + \textit{h.o.t}$ with a suitable dominant term  $\dzHatO=(\dxOutO,\dyOutO)^T$  satisfying
\begin{equation}\label{eq:invariantEquationDifferenceHomogeneous}
\partial_u {\dzHat_0}(u) = 
\AAA^{\spl}(u)\dzHatO(u).
\end{equation}
%	
A fundamental matrix of \eqref{eq:invariantEquationDifferenceHomogeneous}, for $u \in \DBoomerang$, is given by
\begin{equation}\label{def:fundamentalMatrixDifference}
	\MM(u) = \begin{pmatrix}
		m_x(u) & 0 \\
		0 & m_y(u)
	\end{pmatrix},
\end{equation}
with 
\begin{equation}\label{def:mxmyalxaly}
	\begin{aligned}
		m_x(u) &= e^{\frac{i}{\de^2}u} \bb_x(u), 
% 		\hh \hh 
		&\bb_x(u)=\exp\paren{\int_{u_*}^u \wt{\BB}^{\spl}_{2,2}(s) d s}, \\
		m_y(u)& = e^{-\frac{i}{\de^2}u} \bb_y(u), 
% 		\hh \hh 
		&\bb_y(u)=\exp\paren{\int_{u_*}^u \wt{\BB}^{\spl}_{3,3}(s) d s},
	\end{aligned} 
\end{equation}
and a fixed $u_* \in \DBoomerang \cap \reals$. Then, $\Delta\Phi_0$ must be of form 
\begin{equation}\label{def:dzHatO:0}
	\dzHatO(u)= \begin{pmatrix}
		\Delta x_0(u)\\[0.5em]
		\Delta y_0(u)
	\end{pmatrix}=\begin{pmatrix}
		c_x^0 m_x(u)\\[0.5em]
		c_y^0 m_y(u)
	\end{pmatrix},
\end{equation}
for suitable constants $c_x^0,c_y^0\in\mathbb{C}$ which we now determine.


By Theorems~\ref{theorem:innerComputations} and~\ref{theorem:matching} and using the inner change of coordinates in \eqref{def:changeInner},
we have a  good approximation of $\dyOut (u)$
near the singularity $u=iA$ given by
\[
\dyOut(u) \approx 
\sqrt{2} \al_+ \de^{\frac{1}{3}} \DYInn\paren{\frac{u-iA}{\de^2}}.
\]
%
Then, taking  $u=u_+=i(A-\kappa\de^2)$,  we have that
\begin{equation*}
%\label{eq:heuristicsDifferenceA}
\dyOut(u_+) \approx\dyOut_0(u_+) \approx
\sqrt{2} \al_+ \de^{\frac{1}{3}} \DYInn\paren{\frac{u_+-iA}{\de^2}} =
\sqrt{2} \al_+ \de^{\frac{1}{3}} e^{-\kappa} \CInn (1+\chi_3(-i\kappa)).
\end{equation*}
% and the initial condition $c_y$ satisfies
% \begin{equation}\label{eq:heuristicsDifferenceB}
% c_y = \dyOut(u_+) e^{\frac{i}{\de^2}u_+} 
% \approx 
% \de^{\frac{1}{3}} e^{-\frac{A}{\de^2}} \CInn
% \sqrt{2} \al_+ \beta_y^{-1}(u_+) (1+\chi_3(-i\kappa)).
% \end{equation}
Then, using that $\dyOut(u_+) \approx\dyOut_0(u_+)=c_y^0 m_y(u_+)$,
% (analogously for $\Delta x$ at $u=u_-$), 
and proceeding analogously for the component $\dxOut$ at the point $u_-=-i(A-\kappa\de^2)$ (see Remark~\ref{remark:innerComputationConjugats}),
%
% Then, using that $\dyOut(u_+) \approx\dyOut_0(u_+)=c_y^0 m_y(u_+)$,
% (analogously for $\Delta x$ at $u=u_-$), 
we take 
\begin{equation}\label{def:dzHatO}
% 	\dzHatO(u)= \begin{pmatrix}
% 		c_x^0 m_x(u)\\[0.5em]
% 		c_y^0 m_y(u)
% 	\end{pmatrix},
% 	\qquad \text{where} \quad 
% 	\left\{
% 	\begin{array}{l}
		c_x^0 = \de^{\frac{1}{3}} e^{-\frac{A}{\de^2}}
		\conj{\CInn} \,  \sqrt{2} \al_-  \bb^{-1}_x(u_-)\qquad \text{and}\qquad
% 		\\[0.5em]
		c_y^0 =	\de^{\frac{1}{3}} e^{-\frac{A}{\de^2}}
		{\CInn} \sqrt{2} \al_+  \bb^{-1}_y(u_+).
% 	\end{array} \right.
\end{equation}
To prove Theorem \ref{theorem:mainTheoremPoincare}, we check that $\dzHatO(u)$ is the leading term of  $\dzHat(u)$, for $u \in \reals \cap \DBoomerang$, by estimating  the remainder $\dzHatU=\dzHat-\dzHatO$.
%
%\begin{align}\label{def:dzHatU}
%	\dzHatU = 
%	%(\dxOut_1,\dyOut_1)^T = 
%	\dzHat - \dzHatO.
%\end{align}

% % The rest of this section is devoted to prove Theorem \ref{theorem:mainTheoremPoincare}. 
% 
% Throughout the rest of the document, we denote the components of all the functions and operators by a numerical sub-index $f=(f_1,f_2,..,f_N)$, unless stated otherwise. 
%
In order to simplify the notation, throughout the rest of the document, we denote by $C$ any positive constant independent of $\de$ and $\kappa$ to state estimates.

%
%To do so, we prove that $\dzHatO$ is the leading term of $\dzHat$ by obtaining suitable estimates for $\dzHatU=\dzHat-\dzHatO$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{lemma}\label{lemma:fundamentalMatrixDifference}
%For $u \in \DuOut \cap \DsOut$, a fundamental matrix of the homogeneous system~\eqref{eq:invariantEquationDifferenceHomogeneous} is:
%\begin{equation*}%\label{def:fundamentalMatrixDifference}
%\MM(u) = \begin{pmatrix}
%m_x(u) & 0 \\
%0 & m_y(u)
%\end{pmatrix},
%\end{equation*}
%with 
%\begin{equation}\label{def:mxmyalxaly}
%\begin{split}
%m_x(u) = e^{\frac{i}{\de^2}u} \al_x(u), 
%\hh \hh 
%\al_x(u)=\exp\paren{\int_0^u \beta_x(s) d s}, \\
%m_y(u) = e^{-\frac{i}{\de^2}u} \al_y(u), 
%\hh \hh 
%\al_y(u)=\exp\paren{\int_0^u \beta_y(s) d s}.
%\end{split} 
%\end{equation}
%Moreover, for $u \in \DuOut \cap \DsOut$, and $\de$ small enough, we have
%\begin{align}\label{eq:alxalyEstimates}
%C^{-1} \leq \vabs{\al_x(u)} \leq C, \hh
%C^{-1} \leq \vabs{\al_y(u)} \leq C.
%\end{align}
%\end{lemma}
%We postpone the proof of Lemma~\ref{lemma:fundamentalMatrixDifference} until Section~\ref{section:proofDifference}.
%
%In the following we shall give an heuristic idea of how the asymptotic formula for $\dzHat$ can be found. For simplicity, we will focus just on the second component
%of $\dzOut$, that is $\dyOut$. Let us omit the influence of ${\BB}^{\spl}$. Then,
%any solution $\dyOut$ can be written as
%\[
%\dyOut(u) = c_y \h \al_y(u) \h e^{-\frac{i}{\de^2}u},
%\]
%for a certain constant $c_y$. Let us take into account that when $u \sim iA$, then $\dyOut \sim c_y e^{\frac{A}{\de^2}}$. The main idea comes from $\dyOut$ being bounded in $\DuOut \cap \DsOut$. Then $c_y$ must be exponentially small, 
%\[
%c_y \sim e^{-\frac{A}{\de^2}}
%\]
%for $\dyOut$ to be bounded. As a consequence, when $u \in \reals$ we have that $\dyOut$ is exponentially small.
%%
%However, we do not want a bound of $\dyOut$ but an asymptotic formula. Thus we have to find the constant $c_y$, or more concretely a good approximation $c_y^0$ of it. We recall that near the singularity $iA$ we have a good approximation $\DYInn$ of $\dyOut$ given by the study of the inner equation in Theorem~\ref{theorem:innerComputations}. Let us consider the point:
%\begin{align*}
%u_{+} = i\paren{ A - \kappa \de^2},
%\end{align*}
%then
%\[
%\dyOut(u_+) \approx 
%\sqrt{2} \al_+ \de^{\frac{1}{3}} \DYInn\paren{\frac{u_+-iA}{\de^2}} =
%\sqrt{2} \al_+ \de^{\frac{1}{3}} C^{\Inn} e^{-\kappa}(1+\xi_y(-i\kappa)),
%\]
%and the initial condition $c_y$ satisfies
%\[
%c_y = \dyOut(u_+) \al^{-1}_y(u_+) e^{\frac{i}{\de^2}u_+} 
%\approx 
%\sqrt{2} \al_+ \de^{\frac{1}{3}} \al^{-1}_y(u_+) C^{\Inn} e^{-\frac{A}{\de^2}} (1+\xi_y(-i\kappa)).
%\]
%For the first component, $\dxOut$, we can repeat the same arguments, but using the point $u_-=-i(A-\kappa\de^2)$ and the results in Remark~\ref{remark:innerComputationConjugats}. Therefore, following this scheme, to prove Theorem~\ref{theo:difference}, we define the term
%%obtain an asymptotic expression of $\dzOut$, we define the term 
%\begin{equation}\label{def:dzOutO}
%\dzHatO(u)=  \begin{pmatrix}
%c_x^0 m_x(u)
%\\[0.5em]
%c_y^0 m_y(u)
%\end{pmatrix},
%\text{ where } \h \left\{
%%\end{equation}
%%where
%%\begin{equation}
%\begin{array}{l}
%c_x^0 = \sqrt{2} \al_- \de^{\frac{1}{3}} \al^{-1}_x(u_-) \conj{C^{\Inn}} e^{-\frac{A}{\de^2}} , \\[0.5em]
%c_y^0 = \sqrt{2} \al_+ \de^{\frac{1}{3}} \al^{-1}_y(u_+) C^{\Inn} e^{-\frac{A}{\de^2}}.
%\end{array} \right.
%\end{equation}
%Then, using the bound of the matching error given in Proposition~\ref{proposition:matching} and that ${\BB}^{\spl}$, is small, it can be proved that $\dzHatO$ is the dominant part of $\dzHat$. 

%\begin{proof}[End of the proof of Theorem \ref{theorem:mainTheoremPoincare}]

%Since $\al_+^3=\frac12$ and the real-analyticity of the system (see Remark \ref{remark:realAnalytic}), the module of the dominant term $\dzHatO(u_0)$, as given in \eqref{def:dzHatO}, is
%\begin{align*}
%	\vabs{\dyOut_0(u_0)} 
%	= \sqrt[6]{2}
%	\vabs{\CInn}
%	\de^{\frac13}
%	e^{-\frac{A}{\de^2}}
%	\vabs{\beta_y^{-1}(u_+)},
%	\qquad
%	\vabs{\dxOut_0(u_0)} = 
%	\vabs{\dyOut_0(u_0)} 
%\end{align*}
%
%The following lemma provides estimates for $\vabs{\beta_x(u_-)}$ and $\vabs{\beta_y(u_+)}$.
%



==> Article Outer/differenceInner.tex <==

Let us consider the difference 
\begin{equation*}
%\label{def:dzOut}
	\dzOut = (\dwOut,\dxOut,\dyOut)^T = \zuOut - \zsOut,
\end{equation*}
where $\zuOut$ and $\zsOut$ are the perturbed invariant graphs given in Theorem \ref{theorem:existence}.
%
%We analyze this difference in the boomerang domain $\DBoomerang$ (see \eqref{def:dominiBoomerang}).
%
Since $\zuOut$ and $\zsOut$ satisfy the invariance equation \eqref{eq:invariantEquationOuter}, the difference $\dzOut$ satisfies the linear equation
\begin{equation}\label{eq:invariantEquationDifference1}
	\partial_u \dzOut(u)  = 
	\AAA^{\out} \dzOut(u) + 
	\wt{\BB}^{\spl}(u) \dzOut(u),
\end{equation}
where $\AAA^{\out}$ is as given in \eqref{def:matrixAAAOuter} and
\begin{equation}\label{def:Bspl1}
	\wt{\BB}^{\spl}(u) = \int_0^1 
	D_z\RRR^{\out}[\sigma\zuOut + (1-\sigma) \zsOut](u) d \sigma.
\end{equation}
Since  $\zuOut$ and $\zsOut$ are already defined in $\DBoomerang$,  $\wt{\BB}^{\spl}(u)$ can be considered as a  ``known'' function.

In addition, since the graphs of $\zuOut$ and $\zsOut$ belong to the same energy level of $H^{\out}$ (see \eqref{def:hamiltonianOuter}), we have that
\begin{align*}
%\label{eq:energyLevelHout}
	H^{\out}(u,\zuOut(u);\de) - H^{\out}(u,\zsOut(u);\de) =0,
	\quad \text{for } u \in \DBoomerang.
\end{align*}
%
Therefore, we can reduce~\eqref{eq:invariantEquationDifference1} to a two dimensional equation.
%
Indeed, defining $\Ups = 
\paren{\Ups_1,\Ups_2,\Ups_3}$ such that
\begin{align}\label{def:operatorPPdifference}
	\Ups(u) = 
	\int_0^1 D_z H^{\out} 
	\paren{u, \sigma \zuOut(u) + (1-\sigma) \zsOut(u)} d \sigma,
\end{align}
and applying the mean value theorem we have that
\begin{align*}
	\Ups_1(u) \dwOut(u) +
	\Ups_2(u) \dxOut(u) +
	\Ups_3(u) \dyOut(u) = 0.
\end{align*}
Notice that $\Upsilon_1(u)=1+\int_0^1 \partial_w H_1^{\out} \paren{u, \sigma \zuOut(u) + (1-\sigma) \zsOut(u)} d\sigma$ and therefore $\Upsilon_1(u)\neq 0$ for $u \in \DBoomerang$ (see Remark \ref{remark:derivadaH1w}).
%
% Therefore, since $H_1^{\out}$ is analytic, by Remark \ref{remark:derivadaH1w} and taking $\de$ small enough, $\Ups_1(u) \neq 0$ for $u \in\DBoomerangTilde$.
%
Therefore, writing
\begin{equation}\label{eq:defDwOut}
	\dwOut(u) = 
	-\frac{\Ups_2(u)}{\Ups_1(u)} \dxOut(u) 
	-\frac{\Ups_3(u)}{\Ups_1(u)} \dyOut(u)
\end{equation}
% As a result, it is not necessary to study the difference in the first coordinate $\dwOut$.
% Let us consider 
and defining $\dzHat=(\dxOut,\dyOut)^T$, the last two components of \eqref{eq:invariantEquationDifference1} are equivalent to
\begin{equation}\label{eq:invariantEquationDifference2}
	\partial_u {\dzHat}(u) = 
	{\AAA}^{\spl}(u) \dzHat(u)
	+ 
	{\BB}^{\spl}(u) \dzHat(u),
\end{equation} 
where
\begin{align} \label{def:operatorsDifferenceAABB}
	&\AAA^{\spl}=
	\begin{pmatrix}
		\frac{i}{\de^2} + \wt{\BB}^{\spl}_{2,2} & 0 \\
		0 & -\frac{i}{\de^2} + \wt{\BB}^{\spl}_{3,3}
	\end{pmatrix}, 
	%
	&{\BB}^{\spl}=
	\begin{pmatrix} 
		-\frac{	\Ups_2}{	\Ups_1} \wt{\BB}^{\spl}_{2,1} &
		%
		\wt{\BB}^{\spl}_{2,3} 
		-\frac{	\Ups_3}{	\Ups_1} \wt{\BB}^{\spl}_{2,1} \\[0.6em]
		%
		\wt{\BB}^{\spl}_{3,2} 
		-\frac{	\Ups_2}{	\Ups_1} \wt{\BB}^{\spl}_{3,1} &
		%
		-\frac{	\Ups_3}{	\Ups_1} \wt{\BB}^{\spl}_{3,1}
	\end{pmatrix}. 
\end{align}

Next, we give an heuristic idea of how to obtain an exponentially small bound for $\dyOut(u)$ for $u \in \DBoomerang$.
%
The case for $\dxOut$ is analogous. 
%
If we omit the influence of $\wt{\BB}^{\spl}$,
then there exists  $c_y\in\mathbb{C}$ such that $\dyOut$ is of the form
\[
\dyOut(u) = c_y \, e^{-\frac{i}{\de^2}u}.
\]
Evaluating this function at the points
\begin{align*}
%\label{def:uMesuMenysDiff}
	u_+ = i(A-\kappa \de^2), \qquad
	u_- =-i(A-\kappa \de^2),
\end{align*}
one has $\dyOut(u_+) \sim c_y e^{\frac{A}{\de^2}-\kappa}$. 
%
Then, since $\dyOut(u_+) \sim 1$, it implies that
$
c_y \sim e^{-\frac{A}{\de^2}+\kappa}
$
and, as a consequence, $\dyOut$ is exponentially small for  $u \in \reals$.
%
However, we are not interested in an upper bound of $\dyOut$ but in an asymptotic formula. 
%
Thus we have to find the constant $c_y$, or more precisely a good approximation of it. 
%

To this end, we need to give the main terms of $\dyOut$ at $u=u_+$.
% up to distance of order $\de^2$ of $u=iA$.
%
Likewise we need to analyze $\dxOut(u)\sim c_x \, e^{\frac{i}{\de^2}u}$ at $u=u_-$.
% 
% with the singularity $u=-iA$ and, for $\dwOut$, we use the energy conservation by means of \eqref{eq:defDwOut}.
%
%To this end, we derive the inner equation of the system.
%
% In particular, first we have to provide a better first approximation of $\zusOut=(\wusOut,\xusOut,\yusOut)$ around $\pm iA$.
%
To perform this analysis we proceed as follows:

\begin{enumerate}
	\item We provide suitable solutions $\ZusInn(U)$ of the so-called inner equation.
	%
	The inner equation, see \cite{Bal06, BalSea08}, describes the dominant behavior of the functions $\zuOut$ and $\zsOut$ close to (one of) the singularities $u=\pm iA$.
	%
	In particular, it involves the first order of the Hamiltonian $H^{\out}$ close to a singularity and it is independent of the small parameter $\de$.
	%
	See Section \ref{subsection:innerHeuristics}.
	%
	\item We check how well $\zusOut(u)$ are approximated by $\ZusInn(U)$ around the singularities $u=\pm iA$ by means of a complex matching procedure.
	%
	See Section \ref{subsection:matching}.
	%
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Due to the slow-fast character of our system, the difference between the unstable and stable manifolds, $\WW^{\unstable}(\de)$ and $\WW^{\stable}(\de)$, is exponentially small with respect to $\de$.
%%
%Indeed, for the parametrizations $\zuOut$ and $\zsOut$ given in Theorem \ref{theorem:existence} and $u \in \DBoomerang$ it can be seen that
%\[
%\dzOut=(\dwOut,\dxOut,\dyOut)
%\quad \text{with} \qquad
%\dxOut(u) \sim C_x e^{\frac{i}{\de^2}u},
%\qquad
%\dyOut(u) \sim C_y e^{-\frac{i}{\de^2}u}.
%\]
%%
%Since by Theorem \ref{theorem:existence} $\dzOut$ is bounded in $\DBoomerang$, to observe the exponentially small behavior in the reals we evaluate the difference near the singularities of the unperturbed separatrix.
%%
%Namely,
%\[
%C_x \sim \dxOut(-i(A-\kappa \de^2) ) 
%e^{-\frac{A}{\de^2}+\kappa}, 
%\qquad
%C_x \sim \dyOut(i(A-\kappa \de^2) ) 
%e^{-\frac{A}{\de^2}+\kappa}. 
%\]
%in particular, up to up to distance of order $\de^2$ of $u=\pm iA$.
%


==> Article Outer/innerHeuristics.tex <==

In this section we summarize the results on the derivation and study of the inner equation obtained in \cite{articleInner}.
%
We focus on the inner equation around the singularity $u=iA$, but analogous results hold near $u=-iA$. 
%

%
%Due to the slow-fast character of our system, to capture the asymptotic first order of the difference $\dzOut = \zuOut-\zsOut$, we need to give the main terms of this difference up to distance of order $\de^2$ of the singularities, see \cite{Bal06, BalSea08}. 

To derive the inner equation, we look for a new Hamiltonian which is a good approximation of $H^{\out}$, given in~\eqref{def:hamiltonianOuter}, in a suitable neighborhood of $u=iA$.
%
First, we scale the variables $(u,w,x,y)$ so that the graphs $\zusOut(u)$ become $\OO(1)$-functions when $u-iA=\OO(\de^2)$.
%
Since, by Theorem \ref{theorem:existence}, we have that
\begin{align*}
\wdOut(u) = \OO(\de^{-\frac43}), 
\qquad
\xdOut(u) = \OO(\de^{\frac13}),
\qquad
\ydOut(u) = \OO(\de^{\frac13}), 
\qquad 
\text{for } \diamond=\unstable,\stable,
\end{align*}
we consider the symplectic scaling
%
%Since the inner equation is independent of $\de$, we introduce a symplectic scaling such that the graphs $\zuOut$ and $\zsOut$ are of order $\OO(1)$ when $\de^{-2}(u-iA)=\OO(1)$.
%%
%Namely,
$
	\phi_{\Inner}:(U,W,X,Y) \to (u,w,x,y),
$
given by
\begin{equation}\label{def:changeInner}
	U=\frac{u-iA}{\de^2}, \hh
	W=\de^{\frac{4}{3}}\frac{w}{2 \al_+^2}, \hh
	X=\frac{x}{\de^{\frac{1}{3}} \sqrt{2} \al_+ } , \hh
	Y=\frac{y}{\de^{\frac{1}{3}}\sqrt{2} {\al_+}},
\end{equation}
%
where  $\al_+ \in \complexs$ is the constant given by in Theorem~\ref{theorem:singularities}, which is added to avoid the dependence of the inner equation on it.
%
Moreover,  we also perform the time scaling $\tau=\de^2 T$.
%
We refer to $(U,W,X,Y)$ as the \emph{inner coordinates}.

%In the next proposition, we express the Hamiltonian $H^{\out}$ in inner coordinates.


\begin{proposition}\label{proposition:innerDerivation}
The Hamiltonian system associated to~\eqref{def:hamiltonianOuter} expressed in the inner coordinates  is Hamiltonian with respect to the symplectic form $dU \wedge dW + i dX \wedge dY$ and
\begin{equation}\label{def:hamiltonianInnerComplete}
	H^{\Inner} = \HH + H_1^{\Inner},
\end{equation}
where 
\begin{equation*}
	%\label{def:hamiltonianInner}
\HH(U,W,X,Y) = 
H^{\inn}(U,W,X,Y;\de) |_{\de=0} =
W + XY + \KK(U,W,X,Y),
\end{equation*}
with
\begin{align*}
\KK(U,W,X,Y) =& \,
-\frac{3}{4}U^{\frac{2}{3}} W^2 
- \frac{1}{3 U^{\frac{2}{3}}}
\paren{\frac{1}{\sqrt{1+\JJ(U,W,X,Y)}} - 1 }, %\label{def:hamiltonianK} 
\\
%\end{align*}
%and
%\begin{align*}
\begin{split}	
\JJ(U,W,X,Y) =& \,
\frac{4 W^2}{9 U^{\frac{2}{3}} }
-\frac{16 W}{27 U^{\frac{4}{3}}} 
+\frac{16}{81 U^{2}}
%
+\frac{4(X+Y)}{9 U} \paren{W 
-\frac{2}{3 U^{\frac23}}} \\[0.6em]
%
&-\frac{4i(X-Y)}{3 U^{\frac{2}{3}}} 
%
-\frac{X^2 + Y^2}{3 U^{\frac{4}{3}}}
+\frac{10 X Y}{9 U^{\frac{4}{3}}} .
\end{split} \nonumber
\end{align*}
%
Moreover, if 
$\cttInnDerA^{-1} \leq \vabs{U} \leq \cttInnDerA$ and 
$\vabs{(W,X,Y)} \leq \cttInnDerB$ 
for some $\cttInnDerA>1$  and $0<\cttInnDerB<1$,
there exist
$\cttInnDerC,\cttInnDerAA,\cttInnDerBB>0$
independent of 
$\de, \cttInnDerA, \cttInnDerB$ such that
\begin{equation}\label{eq:boundsH1Inn}
|H_1^{\Inner}(U,W,X,Y;\de)|
\leq 
\cttInnDerC \cttInnDerA^{\cttInnDerAA}
\cttInnDerB^{\cttInnDerBB}
\de^{\frac{4}{3}}.
\end{equation} 
\end{proposition}

This result is proven in \cite{articleInner} in Proposition 2.5.

Now, we present the study of the inner Hamiltonian $\HH$.
%
%In particular, we study the solutions of the inner equation that approximate $\zuOut$ and $\zsOut$ given in Theorem \ref{theorem:existence} near the singularities and after the inner change of variables. 
Denoting $Z=(W,X,Y)^T$, the equations associated to the Hamiltonian $\HH$, can be written as
\begin{equation*}
%\label{eq:systemEDOsInner}
	\left\{ \begin{array}{l}
		\dot{U} = 1 + g^{\Inner}(U,Z),\\
		\dot{Z} = \AAA^{\Inn} Z + f^{\Inner}(U,Z),
	\end{array} \right.
\end{equation*}
where 
\begin{equation}\label{def:matrixAAA}
	\AAA^{\Inner}= \begin{pmatrix}
		0 & 0 & 0 \\
		0 & i & 0 \\
		0 & 0 & -i
	\end{pmatrix},
\end{equation}
and
$f^{\Inn} = \paren{-\partial_U \KK, 
	i \partial_Y \KK, -i\partial_X \KK }^T$ 
and
$g^{\inn} = \partial_{W} \KK$.
%
%with $\KK$ given in~\eqref{def:hamiltonianK}.
%
We look for invariant graphs $Z=\ZuInn(U)$ and $Z=\ZsInn(U)$ of this equation, that  satisfy the invariance equation also called \emph{inner equation},
\begin{equation}\label{eq:invariantEquationInner}
	\partial_U \ZdInn(U) = 
	\AAA^{\Inner} \ZdInn + \RRR^{\Inner}[\ZdInn](U),
	\qquad \text{for } 
	\diamond=\unstable, \stable,
\end{equation}
with
\begin{equation}\label{def:operatorRRRInner}
\RRR^{\Inn}[\varphi](U)= 
	\frac{f^{\Inner}(U,\varphi)- g^{\Inner}(U,\varphi) \AAA^{\Inner} \varphi }{1+g^{\Inner}(U,\varphi)}.
\end{equation}
%
%In order to ``select'' the solutions we are  interested in we need some uniformity with respect to $\de$ and $U=\de^{-2}(u-iA)$.
%%
%Notice that $\Re U \to \pm \infty$ as $\de \to 0$, depending on the sign of $\Re U$.
%%
%Moreover,
%\begin{align*}
%\de^{\frac43} \vabs{\wdOut(\de^2 U + iA)}
%\sim
%\frac1{\vabs{U}^{\frac83}} + 
%\frac{\de^{\frac43}}{\vabs{U}}, 
%\quad
%\de^{-\frac13} \vabs{\xdOut(\de^2 U + iA)},
%\de^{-\frac13} \vabs{\ydOut(\de^2 U + iA)}
%\sim
%\frac1{\vabs{U}^{\frac43}}.
%\end{align*}
%%
%For that reason, we look for the solutions $\ZdInn$ satisfying the asymptotic conditions
%\begin{equation}\label{eq:asymptoticConditionsInner}
%\begin{split}
%\lim_{\Re U \to -\infty} \ZuInn(U) = 0, 
%\qquad
%\lim_{\Re U \to +\infty} \ZsInn(U) = 0.
%\end{split}
%\end{equation} 
%
\begin{figure}[t] 
	\centering
	\vspace{5mm}
	\begin{overpic}[scale=0.8]{dominiInnerUnstable.png}
		\put(10,60){$\DuInn$}
		\put(32,44){{$\betaInner$}}
		%\put(16,35){$\frac{\rhoInn}{\gamma}$}
		\put(44,54){{$\rhoInn$}}
		\put(102,41){$\Re U$}
		\put(46,86){$\Im U$}
	\end{overpic}
	\bigskip
	\caption{The inner domain $\DuInn$ for the unstable case.}
	\label{fig:dominiInnerUnstable}
\end{figure} 
%
These functions $\ZuInn$ and $\ZsInn$ will be defined 
in the domains
\begin{equation*}%\label{def:domainInnner}
\DuInn = \claus{ U \in \complexs \text{ : }
|\Im U| \geq \tan \betaInner \Re U + \rhoInn}, 
\qquad
 \DsInn = -\DuInn,
\end{equation*}
respectively, for some $\rhoInn>0$ and 
with $\betaBow$ as given in Theorem~\ref{theorem:existence} (see Figure~\ref{fig:dominiInnerUnstable}).
%
%\begin{remark}\label{remark:innerDomains}
%Let us consider the inner domain $\DuInn$ in separatrix coordinates as given in \eqref{def:changeOuter}.
%%
%That is, 
%\begin{equation*}
%\DuInnOut = 
%%\phi_{\Inner} \paren{\DuInn} =
%\claus{
%u \in \complexs \h \mathrm{ : } \h
%\vabs{ \Im(u - iA)} \geq
%\tan \betaInner \Re u + \rhoInn \de^2
%}.
%\end{equation*}
%Let us consider the outer domain $\DuOut$ as defined on~\eqref{def:domainsOuter}. Then, by~\eqref{def:beta0}, it can be checked that for $0<\beta<\frac{\pi}{2}$ one has that $\DuOut \subset \DuInnOut$.
%%
%Analogously, we also have that $\DsOut \subset \DsInnOut$, where $\DsInnOut = - \DuInnOut$.
%\end{remark}
%
Moreover, we analyze the difference $\DZInn=\ZuInn-\ZsInn$ in the overlapping domain
%
\begin{equation*}%\label{def:domainInnnerDifference}
\EInn = \DuInn \cap \DsInn \cap 
	\claus{ U \in \complexs \st \Im U < 0}.
\end{equation*}

%Let us consider the functions
%\begin{equation}\label{def:graphInner}
%	\ZdInn(U) = \big(\WdInn(U),\XdInn(U),\YdInn(U)\big)^T,
%	\qquad
%	\text{for } \diamond=\unstable,\stable,
%\end{equation}

\begin{theorem}\label{theorem:innerComputations}
There exist $\kappaInner, \cttInnExist>0$
such that for $\rhoInn\geq\kappaInner$,	
the equation~\eqref{eq:invariantEquationInner} has analytic solutions
$
\ZdInn(U) =(\WdInn(U),\XdInn(U),\YdInn(U))^T, 
$ for $U \in \DdInn$, $\diamond=\unstable,\stable$, satisfying
\begin{equation*}
%\label{result:innerExistence}
	| U^{\frac{8}{3}} \WdInn(U)| \leq \cttInnExist, \qquad
	| U^{\frac{4}{3}} \XdInn(U) | \leq \cttInnExist, \qquad
	| U^{\frac{4}{3}} \YdInn(U) | \leq \cttInnExist.
	%\text{for }	U \in \DdInn.
\end{equation*}
In addition, there exist $\CInn \in \complexs$, $\cttInnDiff>0$ independent of $\rhoInn$, and an analytic function $\chi=(\chi_1,\chi_2,\chi_3)^T$ 
such that, for $U \in \EInn$,
\begin{equation*}
%\label{result:innerDifference}
	\DZInn(U) = \ZuInn(U)-\ZsInn(U) =
	\CInn e^{-iU} \Big(
	(0,0,1)^T + \chi(U) \Big),
\end{equation*}
with $|(U^{\frac{7}{3}} \chi_1(U), 
U^{2} \chi_2(U),U \chi_3(U))|
\leq \cttInnDiff$.
%
%\begin{align*}
%	| U^{\frac{7}{3}} \chi_1(U)| \leq \cttInnDiff, \qquad
%	| U^{2} \chi_2(U) | \leq \cttInnDiff, \qquad
%	| U \chi_3(U) | \leq \cttInnDiff.
%	%\text{for } U \in \EInn.
%\end{align*}
\end{theorem}

This result is  Theorem 2.7 of \cite{articleInner}.


\begin{remark}\label{remark:innerComputationConjugats}
%
To obtain the analogous result to Theorem \ref{theorem:innerComputations} near the singularity $u=-iA$, one must perform the change of coordinates
%
\begin{equation*}
{V}=\frac{u+iA}{\de^2}, \qquad
\widehat{W}=\de^{\frac{4}{3}}\frac{w}{2 \al_-^2}, \qquad
\widehat{X}=\frac{x}{\de^{\frac{1}{3}} \sqrt{2} \al_- }, 
\qquad
\widehat{Y}=\frac{y}{\de^{\frac{1}{3}}\sqrt{2} {\al_-}},
\end{equation*}
where  $\al_- \in \complexs$ is $\al_- =\conj{\al_+}$ (see Theorem \ref{theorem:singularities}). 	
%	
Then, for $V \in \conj{\DdInn}$, one can prove the existence of the corresponding solutions 
\[
\ZdInnN(V)=(\WdInnN(V),\XdInnN(V),\YdInnN(V))^T, \qquad
\text{where } \diamond = \mathrm{u, s}.
\]
Due to the real-analyticity of the problem (see Remark \ref{remark:realAnalytic}) we have that $\widehat{X}^{\diamond}(V) = \conj{Y^{\diamond}(U)}$. 
%
Therefore, the difference $\DZInnN = \ZuInnN - \ZsInnN$, is given asymptotically for $U \in \conj{\EInn}$ by
\begin{equation*}
%\label{result:innerDifferenceNegative}
	\DZInnN(V) = \conj{\CInn} e^{iV} \Big(
	(0,1,0)^T + \zeta(V) \Big),
\end{equation*}
%where $\conj{\CInn}$ is the conjugate of the constant $\CInn$ given in Theorem~\ref{theorem:innerComputations} and 
where $\zeta=(\zeta_1,\zeta_2,\zeta_3)^T$ satisfies 
$|(V^{\frac{7}{3}} \zeta_1(V),
V \zeta_2(V),
V^{2} \zeta_3(V)| \leq C$, for a constant $C$ independent of $\kappa$.
\end{remark}
% 
% 
% \begin{remark}
% We can obtain a numerical approximation of the constant $\CInn$.
% %
% Taking into account expression~\eqref{result:innerDifference}, for $U \in \EInn$, we have
% \begin{align*}
% 	{\CInn} = \lim_{\Im U \to -\infty} {\DYInn(U) e^{iU}}.
% \end{align*}
% %
% In \cite{articleInner} we show that $\vabs{\CInn}\approx 1.63$.
% %
% However, a more accurate approximation for $\CInn$ is not straightforward, since $\DYInn$ is exponentially small.
% %
% We expect that a rigorous computation method can be applied, see \cite{BCGS21}.
% \end{remark}


==> Article Outer/introductionOuter.tex <==
% 
% The present work is the natural continuation of \cite{articleInner}.
% %
% However, all the results presented in this article are contextualized in such a manner that it can be read independently of its first part.

The Restricted Circular $3$-Body Problem 
models the motion of a body of negligible mass under the gravitational influence of two massive bodies, called the primaries, which perform a circular motion.
%
If one also assumes that the massless body moves on the same plane as the primaries one has the Restricted Planar Circular $3$-Body Problem (RPC$3$BP).

Let us name the two primaries $S$ (star) and $P$ (planet) and
%
normalize their masses so that $m_S=1-\mu$ and $m_P=\mu$, with $\mu \in \left( 0, \frac{1}{2} \right]$. 
%
Choosing a suitable rotating coordinate system, the positions of the primaries can be fixed at $q_S=(\mu,0)$ and  $q_P=(\mu-1, 0)$.
%
Then, the position and momenta of the third body, $(q,p) \in \reals^2 \times \reals^2$, are governed by the Hamiltonian system associated to the Hamiltonian
%
\begin{equation}\label{def:hamiltonianInitialNotSplit} 
	\begin{split}
		\HInicial(q,p;\mu) &= \frac{||p||^2}{2} 
		- q^t \left( \begin{matrix} 0 & 1 \\ -1 & 0 \end{matrix} \right) p 
		-\frac{(1-\mu)}{||q-(\mu,0)||} 
		- \frac{\mu}{||q-(\mu-1,0)||}.
	\end{split}
\end{equation}
% This Hamiltonian is that the system is singular when the third body collides with one of the primaries at $q=q_S$ or $q=q_J$.
%
Note that this Hamiltonian is autonomous. The conservation of $h$ corresponds to the preservation of the classical Jacobi constant.

For $\mu>0$, it is a well known fact that \eqref{def:hamiltonianInitialNotSplit}  has five critical points, usually called Lagrange points
%
(see Figure~\ref{fig:L3Outer}). 
%
On an inertial (non-rotating) system of coordinates, the Lagrange points correspond to periodic dynamics with the same period as the two primaries, i.e on a 1:1 mean motion resonance.
%
The three collinear Lagrange points, $L_1$, $L_2$ and $L_3$, are of center-saddle type whereas, for small $\mu$, the triangular ones, $L_4$ and $L_5$, are of center-center type  (see, for instance, \cite{Szebehely}).

Due to its interest in astrodynamics, a lot of attention has been paid to the study of the invariant manifolds associated to  the points $L_1$ and $L_2$ (see \cite{KLMR00, GLMS01v1, CGMM04}).
%
The dynamics around the points $L_4$ and $L_5$ has also been heavily studied since, due to its stability, it is common to find objects orbiting around these points (for instance the Trojan and Greek Asteroids associated to the pair Sun-Jupiter, see \cite{GDFGS89, CelGio90, RobGab06}).
%
Since the point $L_3$ is located ``at the other side'' of the massive primary, it has received somewhat less attention. However, the associated invariant manifolds (more precisely its center-stable and center-unstable invariant manifolds) play an important role in the dynamics of the RPC3BP  since they act as boundaries of \emph{effective stability} of the stability domains around $L_4$ and $L_5$ 
(see \cite{GJMS01v4, SSST13}). 
%
The invariant manifolds of $L_3$ play also a fundamental role in creating transfer orbits from the small primary to $L_3$ in the RPC$3$BP (see \cite{HTL07, TFRPGM10})  or between primaries in the Bicircular 4-Body Problem (see \cite{JorNic20, JorNic21}).

% \textcolor{red}{(Posar alguna cita?).}

Moreover, being far from collision, the dynamics close to the Lagrange point $L_3$ and its invariant manifolds for small $\mu$ are rather similar to that of other mean motion resonances which play an important role in creating instabilities in the Solar system, see \cite{FGKR16}. On the contrary, since the points $L_1$ and $L_2$ are close to collision for small $\mu$, the analysis of the associated dynamics is quite different.
%\begin{figure}
%	\subfloat[$\mu>0$]{%
%		\begin{overpic}[scale=0.7]{lagrangePointsPerturbedEsquema.png}
%			\put(43,38){{\color{blue} $q_S$ }}
%			\put(14,38){{\color{blue} $q_P$ }}
%			\put(23,45){{\color{red} $L_1$ }}
%			\put(10,45){{\color{red} $L_2$ }}
%			\put(63.5,45){{\color{red} $L_3$ }}
%			\put(27,69){{\color{red} $L_5$ }}	
%			\put(27,14){{\color{red} $L_4$ }}
%			\put(89,42){$q_2$}
%			\put(37.5,82.5){$q_1$}
%		\end{overpic}
%		\vspace{1cm}	
%	}\hfill
%	\subfloat[$\mu=0.003$]{%
%		\begin{overpic}[width=7.5cm]{L3manifoldsm003.png}
%			\put(50,1){$q_1$}
%			\put(12,38){$q_2$}
%			\put(71.5,37.5){{\color{red} $ L_3 \h \bullet$ }}
%			\put(37,58){{\color{red} $\bullet$ }}
%			\put(28,61){{\color{red} $L_5$ }}
%			\put(37,17){{\color{red} $\bullet$ }}	
%			\put(28,12){{\color{red} $L_4$ }}
%			\put(50.5,37.5){{\color{blue} $\bullet$ }}
%			\put(50.5,34){{\color{blue} $q_S$ }}
%			\put(23,37.5){{\color{blue} $\bullet$ }}
%			\put(23,34){{\color{blue} $q_P$ }}
%		\end{overpic}
%	}
%	\caption{(a) Projection onto the $q$-plane of the equilibrium points for the RPC$3$BP on rotating coordinates. (b) Plot of the stable (green) and unstable (blue) manifolds of $L_3$ projected onto the $q$-plane for $\mu=0.003$. }
%	\label{fig:L3perturbed}
%\end{figure}

\begin{figure}
\centering
\begin{overpic}[scale=0.3]{lagrangePointsOuter2.png}
	\put(50,35){\footnotesize{\color{blue} $q_S$ }}
	\put(29,35){\footnotesize{\color{blue} $q_P$ }}
	\put(32,41){{\color{red} $L_1$ }}
	\put(24,41){{\color{red} $L_2$ }}
	\put(75,38){{\color{red} $L_3$ }}
	\put(38,62){{\color{red} $L_5$ }}	
	\put(38,13){{\color{red} $L_4$ }}
	\put(53,64.5){{\color{orange} $\Sigma$ }}
\end{overpic}
	\caption{Projection onto the $q$-plane of the Lagrange points (red) and the unstable (blue) and stable (green) manifolds of $L_3$, for $\mu=0.0028$. }
	\label{fig:L3Outer}
\end{figure}

Over the past years, one of the main focus of study of the  dynamics ``close''  to  $L_3$ and its invariant manifolds has been  the so called ``horseshoe-shaped orbits'', first considered in~\cite{Brown1911},
which are quasi-periodic orbits that encompass the critical points $L_4$, $L_3$ and $L_5$.
%
The interest on these types of orbits arise when modeling the motion of co-orbital satellites, the most famous being Saturn's satellites Janus and Epimetheus, and near Earth asteroids.
%
Recently, in~\cite{NPR20}, the authors have proved the existence of $2$-dimensional elliptic invariant tori on which the trajectories mimic the motions followed by Janus and Epimetheus
%
(see also \cite{DerMur81a, DerMur81b, LlibreOlle01, CorsHall03, BarrabesMikkola05, BarrabesOlle2006, BFPC13, CPY19}).
%
%%%%%%%%%%
%

%%%%

Rather than looking at stable motions ``close to'' $L_3$ as \cite{NPR20}, the goal of this paper (and its prequel \cite{articleInner}) is rather different: its objective is to prove the breakdown of homoclinic connections to $L_3$. Indeed, since  $L_3$ is a center-saddle critical point, it possesses $1$-dimensional unstable and stable manifolds, which we denote by $W^{\unstable}(\mu)$ and $W^{\stable}(\mu)$, respectively, and a $2$-dimensional center manifold.
Theorem \ref{theorem:mainTheorem} below gives an asymptotic formula for the distance between the stable and unstable invariant manifolds (at a suitable transverse section) for mass ratio $\mu>0$ small enough.


% An asymptotic formula for t
\subsection{The distance between the invariant manifolds of \texorpdfstring{$L_3$}{L3}}

%
The one dimensional unstable and stable invariant manifolds of $L_3$ have two branches each (see Figure~\ref{fig:L3Outer}).
% 
One pair circumvents $L_5$, which we denote by $W^{\unstable,+}(\mu)$ and $W^{\stable,+}(\mu)$, and the other,  $W^{\unstable,-}(\mu)$ and $W^{\stable,-}(\mu)$, circumvents $L_4$.
%
Since the Hamiltonian system associated to the Hamiltonian $\HInicial$ is reversible with respect to the involution
\begin{equation*}
%\label{def:involutionCartesians}
	\Phi(q,p;t)=(q_1,-q_2,-p_1,p_2;-t),
\end{equation*}
the $+$ branches of the invariant manifolds are symmetric with respect to the $-$ branches. Thus, we restrict our analysis  to the positive branches.
% $W^{\unstable/\stable,+}(\mu)$.
% since the negative branches are symmetric.

% In this paper, we finish the study (which we started in \cite{articleInner}) of the $1$-dimensional invariant manifolds of $L_3$ to obtain an asymptotic formula for the distance between $W^{\unstable,+}(\mu)$ and $W^{\stable,+}(\mu)$, for $0<\mu\ll 1$.

To measure the distance between $W^{\unstable/\stable,+}(\mu)$, we consider the symplectic polar change of coordinates
\begin{align}\label{def:changePolars}
	q= 
	%	\begin{pmatrix}
	%		q_1 \\ 
	%		q_2
	%	\end{pmatrix} =
	r \begin{pmatrix}
		\cos \tht \\ 
		\sin \tht
	\end{pmatrix},
	\qquad
	p = 
	%	\begin{pmatrix}
	%		p_1 \\ 
	%		p_2
	%	\end{pmatrix} =
	R
	\begin{pmatrix}
		\cos \tht \\ 
		\sin \tht
	\end{pmatrix} 
	- \frac{G}{r} \begin{pmatrix}
		\sin \tht \\ 
		-\cos \tht
	\end{pmatrix},
\end{align} 
where 
% $r$ is the radius, $\tht$ the argument of $q$, 
$R$ is the radial linear momentum  and $G$ is the angular momentum.
%

We consider the $3$-dimensional section 
\[
\Sigma = \claus{(r,\tht,R,G) \in \reals \times \torus \times \reals^2 
\st r>1, \, \tht=\frac{\pi}2 \,}
\]
and denote by $(r^{\unstable}_*,\frac{\pi}2, R^{\unstable}_*,G^{\unstable}_*)$ and $(r^{\stable}_*,\frac{\pi}2,R^{\stable}_*,G^{\stable}_*)$ the first crossing of the invariant manifolds with this section. 

% 
% 	= \max_{t \in \reals} \boxClaus{ W^{\stable,+}(\mu) \cap \Sigma(\tht_*)}.
% \end{align*}	
% 
% \begin{align*}%\label{def:firstCrossingPolars}
% 	(r^{\unstable},\tht_*,R^{\unstable},G^{\unstable})
% 	= \min_{t \in \reals} \boxClaus{ W^{\unstable,+}(\mu) \cap \Sigma(\tht_*)}, 
% 	\quad
% 	(r^{\stable},\tht_*,R^{\stable},G^{\stable}) 
% 	= \max_{t \in \reals} \boxClaus{ W^{\stable,+}(\mu) \cap \Sigma(\tht_*)}.
% \end{align*}	

% Now, we introduce the main result of this paper and \cite{articleInner}.
The next theorem measures the distance between these points for $0< \mu\ll 1$.

\begin{theorem}\label{theorem:mainTheorem}
There exists $\mu_0>0$ such that, for $\mu \in (0,\mu_0)$,
\[
\norm{(r^{\unstable}_*,R^{\unstable}_*,G^{\unstable}_*)-(r^{\stable}_*,R^{\stable}_*,G^{\stable}_*)}
=
\sqrt[3]{4} \,
\mu^{\frac13} e^{-\frac{A}{\sqrt{\mu}}} 
\boxClaus{\vabs{\CInn}+\OO\paren{\frac1{\vabs{\log \mu}}}},
\]
where:
\begin{itemize}
	\item The constant $A>0$ is the real-valued integral
	\begin{equation}\label{def:integralA}
		A= \int_0^{\frac{\sqrt{2}-1}{2}} \frac{2}{1-x}\sqrt\frac{x}{3(x+1)(1-4x-4x^2)}  dx\approx 0.177744.
	\end{equation}
	\item The constant $\CInn \in \complexs$ is the Stokes constant associated to the inner equation analyzed in \cite{articleInner} and in Theorem \ref{theorem:innerComputations} below.
% 		by the result of the inner equation in Theorem 2.7 in \cite{articleInner} (see Section \ref{subsection:innerHeuristics} for an overview of the result).	
	\end{itemize}
\end{theorem}

\begin{remark}\label{remark:sectiontheta}
We can prove the same result for any section 
\[
\Sigma(\tht_*) = \claus{(r,\tht,R,G) 
\in \reals \times \torus \times \reals^2 
\st r>1, \, \tht=\tht_* \,},
\]
with $\tht_* \in
% [\tht_1,\tht_2] \subset 
(0,\tht_0)$ and $\tht_0=\arccos\paren{\frac12-\sqrt2}$ (the value of $\mu_0$ depends on how close to the endpoints of the interval $\tht_*$ is).
The section $\tht=\tht_0$ is close to the ``turning point'' of the invariant manifolds (see Figure \ref{fig:L3Outer}).
\end{remark}

The constant $A$ in \eqref{def:integralA} is derived from the values of the complex singularities of the separatrix of certain integrable averaged system, which is studied in the prequel paper \cite{articleInner}. 
%
The results obtained in  \cite{articleInner} about this separatrix are summarized in Theorem \ref{theorem:singularities} below.
% the whole result is layed out and the proof is given in the prequel \cite{articleInner} of the present paper. 

The origin of the constant $\Theta$ appearing in Theorem \ref{theorem:mainTheorem} is explained in Theorem \ref{theorem:innerComputations}, which analyzes the so-called inner equation. This theorem  is also proven in  \cite{articleInner}. 
%
Moreover, in that paper it is seen, by a numerical computation,  that $\vabs{\CInn}\approx 1.63$. We expect that  one should be able to prove that $\vabs{\CInn}\neq 0$ by  means of  rigorous computer computations (see \cite{BCGS21}). Note that $\vabs{\CInn}\neq 0$ implies that there are not primary (i.e. one round) homoclinic orbits to $L_3$.

% The study of the inner equation  Stokes constant $\Theta$ by the result of the inner equation in Theorem 2.7 in \cite{articleInner} (see Section \ref{subsection:innerHeuristics} for an overview of the result).	


% That is, the difference between manifolds cannot be detected in the truncation of their normal form at any finite order. 
%

%%%%%%%
A fundamental problem in dynamical systems is to prove whether a given model has chaotic dynamics (for instance a Smale horseshoe). 
For many physically relevant models this is usually   remarkably difficult. This is the case of many Celestial Mechanics models, where most of the known chaotic motions have been found in nearly integrable regimes where there is an unperturbed problem which already presents some form of ``hyperbolicity''. This is the case  in the vicinity of collision orbits (see for example \cite{Moe89, BolMac06, Bol06, Moe07}) or close to parabolic orbits (which allows to construct chaotic/oscillatory motions), see~\cite{Sitnikov1960, Alekseev1976, LlibSim80, Moser2001, GMS16, GMSS17, GPSV21}. 
%
There are also several results in regimes far from integrable which rely on computer assisted proofs \cite{Ari02, WilcZgli03, Cap12, GierZgli19}. The problem tackled in this paper and \cite{articleInner} is radically different. Indeed, if one takes the  limit $\mu\to 0$ in \eqref{def:hamiltonianInitialNotSplit} one obtains the classical integrable Kepler problem in the elliptic regime, where  no hyperbolicity is present. Instead, the (weak) hyperbolicity is created by the $\mathcal{O}(\mu)$ perturbation, which can be captured considering an integrable averaged Hamiltonian along the $1:1$ mean motion resonance\footnote{The $1:1$ averaged Hamiltonian has been also studied to obtain ``good'' approximations for the global dynamics in the $1:1$ resonant zone, see for example \cite{RNP16, AlePou21} and the references therein.}.
% , as it was seen in \cite{articleInner}, for $\mu=0$, the unstable and stable manifolds of $L_3$ collapse into a circle of equilibrium points.


One of the classical methods  to construct chaotic dynamics is the Smale-Birkhoff homoclinic theorem   by proving the existence of  transverse homoclinic orbits to invariant objects, most commonly,  periodic orbits.
%
% Then,  implies the existence of chaotic motions in a neighborhood of the corresponding hyperbolic point.
%%%%%
%
Certainly the breakdown of homoclinic orbits to the critical point $L_3$ given by Theorem~\ref{theorem:mainTheorem} does not lead to the existence of chaotic orbits. However, one should expect that Theorem~\ref{theorem:mainTheorem} implies that there exist Lyapunov periodic orbits exponentially close to $L_3$ whose stable and unstable invariant manifolds intersect transversally. This would create chaotic motions ``exponentially close'' to $L_3$ and its invariant manifolds (see \cite{articleChaos}).
% 
% Since the Hamiltonian $\HInicial$ is autonomous and the stable and unstable manifolds of $L_3$ are $1$-dimensional, the branches $W^{\unstable,+}(\mu)$ and $W^{\stable,+}(\mu)$ may coincide (forming an homoclinic connection) or not, but they cannot intersect.
%
% Therefore, by Theorem \ref{theorem:mainTheorem}, an homoclinic connection can exist only if $\CInn = 0$.
% 
% In \cite{articleInner}, by a numerical approximation, it is seen that $\vabs{\CInn}\approx 1.63$.
% %
% However, this is a rough estimate, since the exponentially small character of the difference complicates obtaining a better estimate.
% %
% We expect that a rigorous computation method can be applied, see \cite{BCGS21}.

%%%%%%%%%

% 
% In celestial mechanics models, proving the existence of chaotic motions is a notably difficult problem with very few results.
%
%%%%%%
%
% However, even though $L_3$ remains for the unperturbed problem, it does not maintain its hyperbolic character.
%

%%%%%%%
% 
% Let us notice that, since $W^{\unstable/\stable}(\mu)$  cannot intersect transversally, Theorem \ref{theorem:mainTheorem} does not directly imply the existence of chaotic motions in a neighborhood of $L_3$.
% %
% However, we expect Theorem \ref{theorem:mainTheorem} to be key to understand the motions of some of the different objects surrounding $L_3$.
% %
% One course of action may be studying the unstable and stable manifolds of small Lyapunov periodic orbits of $L_3$.
% %
% Then, due to their higher dimension, if they behave ``similar'' to $W^{\unstable/\stable}(\mu)$ we expect to be able to prove the existence of chaotic motions.
% %
% \textcolor{red}{(Posar alguna cita?).}


%%%%%%%%%%%

% 
% An important question regarding the study of the invariant manifolds of $L_3$ is to understand how these objects confine regions of effective stability around $L_4$ and $L_5$ for the general restricted $3$-Body Problem, see \cite{SSST13}.

% In the case of the RPC$3$BP, on an averaged first order (see Sections 2.1 and 2.2 in \cite{articleInner} for the details), the stable and unstable manifolds coincide and separate the regions of the phase space where the horseshoe-shaped orbits take place with the region where ``tadpole orbits'' (trajectories surrounding $L_4$ or $L_5$) occur.
% %
% For the full problem, due to their low dimension, $W^{\unstable}(\mu)$ and $W^{\stable}(\mu)$ cannot fulfill this role.
% %
% However, the study of the center-stable and center-unstable manifolds of $L_3$, since they are of higher dimension, may provide some results.

%%%%%%%%%%%

%In conclusion, one of the interests behind the study of the breakdown of the $1$-dimensional invariant manifolds of $L_3$ is to prove the none existence of primary homoclinic connections of $L_3$.
%%
%Additionally, it make sense to claim that this result would be an important first step to understand some of the dynamic motions and chaotic phenomena surrounding different objects of $L_3$ (Lyapunov periodic orbits, for example).

%%%%%%%%
As already mentioned, Theorem \ref{theorem:mainTheorem} rules out the existence of primary homoclinic connections to $L_3$ in the RPC$3$BP for $0< \mu\ll 1$. However, it does not prevent the existence of multiround homoclinic orbits, that is homoclinic orbits which pass close to $L_3$ multiple times.
% 
% Another important object related to the dynamics of the invariant manifolds of $L_3$
% are symmetric homoclinic connections, which are connections between the opposed branches $W^{\unstable,+}(\mu)$ and $W^{\stable,-}(\mu)$ (accordingly $W^{\unstable,-}(\mu)$ with $W^{\stable,+}(\mu)$).
%
It has been conjectured (see for instance~\cite{BMO09}, where the authors analyze this problem numerically) that  multi-round homoclinic connections to $L_3$ should exist for a sequence of values $\claus{\mu_k}_{k \in \naturals}$ satisfying $\mu_k\to 0$ as $k \to \infty$. 

% \textcolor{blue}{JO HO TREURIA One of the features of our system is the degeneracy of the unperturbed system. 
% %
% Indeed, notice that for $\mu=0$, the stable and unstable manifolds of $L_3$ become a circle of critical points (see \eqref{def:hamiltonianInitialNotSplit}). 
% %
% Thus, it is necessary to reformulate the system in order to obtain a new first order Hamiltonian with saddle and a separatrix (see Section \ref{section:introductionPoincare}).}
%

%In the following, we denote by $d(\mu)$ the distance between the ``upper branches'' of the one-dimensional invariant manifolds, computed on a section of the phase space.
%
%\textcolor{red}{S'ha d'escriure b\'e aquest teorema.}
%
%In this work and~\cite{?} we 
%analyze the distance betweeen the $1$-dimensional invariant manifolds of $L_3$ and give an asymptotic formula for its difference.
%
%Indeed, in~\cite{?} we give asymptotic formulas for the distance between the stable and unstable manifolds of $L_3$.
%

%%%%%%%%%
\paragraph{A first step towards proving Arnold diffusion along the $1:1$ mean motion resonance in the $3$-Body Problem?}
Consider the $3$-Body Problem in the planetary regime, that is one massive body (the Sun) and two small bodies (the planets) performing approximate ellipses (including the ``Restricted limit'' when one of planets has mass zero).  A fundamental problem is to assert whether such configuration is stable (i.e. is the Solar system stable?). Thanks to Arnold-Herman-F\'ejoz KAM Theorem, many of such configurations are stable, see  \cite{Arnold63,Fejoz04}. However, it is widely expected that there should be strong instabilities created by Arnold diffusion mechanisms (as conjectured by Arnold in \cite{Arnold64}). In particular, it is widely believed that one of the main sources of such instabilities dynamics are the mean motion resonances, where the period of the two planets is resonant (i.e. rationally dependent) \cite{FGKR16}.

The RPC$3$BP has too low dimension (2 degrees of freedom) to possess Arnold diffusion. However, since it can be seen as a first order for higher dimensional models, the analysis performed in this paper can be seen as a humble first step towards constructing Arnold diffusion in the $1:1$ mean motion resonance. In this resonance,  the RPC$3$BP  has a normally hyperbolic invariant manifold given by the center manifold of the Lagrange point $L_3$. This normally hyperbolic invariant manifold is foliated by the classical Lyapunov periodic orbits. One should expect that the techniques developed in the present paper would allow to prove that the invariant manifolds of these periodic orbits intersect transversally within the corresponding energy level of \eqref{def:hamiltonianInitialNotSplit}. Still, this is a much harder problem than the one considered in this paper and the technicalities involved would be considerable. 

This transversality would not lead to Arnold diffusion due to the low dimension of the RPC3BP. However, if one considers either the Restricted Spatial Circular $3$-Body Problem with small $\mu>0$ which has three degrees of freedom, the Restricted Planar Elliptic $3$-Body Problem with small $\mu>0$ and eccentricity of the primaries $e_0>0$, which has two and a half degrees of freedom, or the ``full'' planar $3$-Body Problem (i.e. all three masses positive, two small) which has three degrees of freedom (after the symplectic reduction by the classical first integrals) one should be able to construct orbits with a drastic change in angular momentum (or inclination in the spatial setting). 

In the Restricted Planar Elliptic $3$-Body Problem the change of angular momentum would imply   the transition of the zero mass body orbit from a close to circular ellipse to a more eccentric one. In the full 3BP, due to total angular momentum conservation, the angular momentum would be transferred from one body to the other changing both osculating ellipses.
% \textcolor{red}{Citar Simo-SousaSilva-Terra. Evidences of diffusion in the SRP3BP \cite{SSST14}.}
This behavior would be analogous to that of \cite{FGKR16} for the $3:1$ and $1:7$ resonances. In that paper, the transversality between the invariant manifolds of the normally hyperbolic invariant manifold was checked numerically for the realistic Sun-Jupiter mass ratio $\mu=10^{-3}$. 
% As far as the authors know, no analytic prove for small $\mu$
Arnold diffusion instabilities have been analyzed numerically for the  Restricted Spatial Circular $3$-Body Problem  in \cite{SSST14}.


% 
% 
% From this perspective, the analysis performed in this paper (and \cite{innerArticle}) can be seen as a (very humble) first step towards proving Arnold diffusion along the $1:1$ mean motion resonance.
% 
% 
% , which leads 
% One of the fundamental problems is understand the unstable motions that by  
% 
% 
% One of the fundamental problems in Celestial Mechanics is to understand the unstable motions that the $3$ body problem may possess, specially in the planetary regime (one massive bodies and $N-1$ small bodies) which models the Solar system. In particular, one wants to analyze the global instabilities usually called Arnold diffusion. 
% 
% It is well known that one of the main sources of instabilities are the mean motion resonances where the periods of the small bodies are resonant. In particular the $1:1$ mean motion resonance analyzed in the present paper.
% Still the
% 
% 
% The simplest model that may have \emph{global instabilities} (drift 
% 
% Theorem \ref{theorem:mainTheorem} can be seen as a very humble step towards proving Arnold Diffusion for  Restricted Planar Elliptic 3 Body Problem with small $\mu>0$ and $e_0$

\subsection{The strategy to prove Theorem \ref{theorem:mainTheorem}}

The main difficulty in proving Theorem \ref{theorem:mainTheorem} is that the 
distance between the stable and unstable manifolds of $L_3$ is exponentially small with respect to $\sqrt\mu$ (this is also  usually known as a \emph{beyond all orders} phenomenon). This implies that the classical Melnikov Method \cite{GuckenheimerHolmes} to detect the breakdown of homoclinics cannot be applied.
%

To prove Theorem \ref{theorem:mainTheorem}, we follow the strategy of exponentially small splitting of separatrices (already outlined in \cite{articleInner}) which goes back to the seminal work by Lazutkin \cite{Laz84, Laz05}. See \cite{articleInner} for a list of references on the recent developments in the field of exponentially small splitting of separatrices. In particular, we follow similar strategies of those in  \cite{BFGS12,BCS13}.
% %
% For the analysis of other exponentially small phenomena, see \cite{HMS88, FS90a, FS90b, DelSea92, DelSea97, Gel97a, Tre97, DelRRR98, Gel99, GGM99, Gel00, Lom00, Sau01, GS01, OSS03, BF04, BF05,  Bal06, BalSea08,GOS10, GaiGel10, MSS11, BM12, BCS18a, BCS18b, GGS20} and, in particular, \cite{BFGS12,BCS13} for similar strategies (see  \cite{articleInner} for more details).


%In addition, the separatrix of the system does not have a known explicit parametrization.
%%
%Therefore, in order to obtain its complex singularities, we need to perform a detailed analysis of the first order of the Hamiltonian (see Section \ref{section:singularitiesOuter}).

In the present work the first order of the difference between manifolds is not given by the Melnikov function.
%
Instead, we must  derive and analyze an inner equation which provides the dominant term of this distance. As a consequence, we need to ``match'' (i.e. compare) certain  solutions of the inner equation  with the parameterizations of the perturbed invariant manifolds.
% those of the original system.
%
% For some results on inner equations see \cite{Gel97a, GS01, OSS03, Bal06, BalSea08,BM12}.



The first part of the proof, that was completed in the prequel \cite{articleInner}, dealt with the following steps:
\begin{enumerate}[label*=\Alph*.]
	\item
% 	Due to the degeneracy of the unperturbed problem, w
	We perform a change of coordinates to capture the slow-fast dynamics of the system. 
	%
	The first order of the  new Hamiltonian has a saddle point with an homoclinic connection (also known as separatrix) and  a fast harmonic oscillator.
	%
	%See Section~\ref{section:introductionPoincare}.
	%
	\item We study the analytical continuation of the time-parametrization of the	separatrix of this first order. 
	%
	In particular, we obtain its maximal strip of analyticity and the singularities at the boundary of this strip.
	%
	%See Section \ref{section:singularitiesOuter}.
	%
	\item We derive the inner equation.
	\item We study  two special solutions which will be ``good approximation'' of the perturbed invariant manifolds near the singularities of the unperturbed separatrix (see Step F below).
	%
	%See Section \ref{subsection:innerHeuristics}.
\end{enumerate}

The remaining steps necessary to complete the proof of Theorem~\ref{theorem:mainTheorem} are the following:
\begin{enumerate}[label*=\Alph*.]
	%
	\item[E] We prove the existence of the analytic continuation of the parametrizations of the invariant manifolds of $L_3$, $W^{\unstable,+}(\de)$ and $W^{\stable,+}(\de)$, in an appropriate complex domain called boomerang domain.
	%
	This domain contains a segment of the real line and intersects a sufficiently small neighborhood of the singularities of the unperturbed separatrix.
	%
	%See Section \ref{section:outer}.
	%
	\item[F.] By using complex matching techniques, we show that, close to the singularities of the unperturbed separatrix, the solutions of the inner equation obtained in Step D are ``good approximations'' of the parameterizations of the perturbed invariant manifolds obtained in Step E.
% 	We check that they are ``close enough'' approximations 
	%
	%See Section \ref{subsection:matching}.
	%
	\item[G.] We obtain an asymptotic formula for the difference between the perturbed invariant manifolds by proving that the dominant term comes from the difference between the solutions of the inner equation.
	%
	%See Section \ref{section:difference}.
	%
\end{enumerate}

The structure of this paper goes as follows. 
%
In Section \ref{section:introductionPoincare} we perform the change of coordinates introduced in Step A and state Theorem \ref{theorem:mainTheoremPoincare}, which is a reformulation of Theorem \ref{theorem:mainTheorem} in this new set of variables.
%
Then, in Section \ref{section:resultsOuter}, we state the results concerning Steps B, C and D above  (which are proven in \cite{articleInner}) and we carry out Steps E, F and G. These steps lead to the proof of  Theorem \ref{theorem:mainTheoremPoincare}.
% and finish the proof.
%
Sections \ref{section:proofH-existence} and \ref{section:proofG-matching} are devoted to proving the results in Section \ref{section:resultsOuter} which concern Steps E and F.
% (that were not proved in \cite{articleInner}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{The RPC$3$BP and the Lagrange point $L_3$}
%
%%%%% THE MODEL %%%%%
%
%We briefly present the equations of the motions we study. %see~\cite{Szebehely} for the details.
%
%Let us name the two primaries $S$ (star) and $P$ (planet). Normalizing their masses, we can assume that $m_S=1-\mu$ and $m_P=\mu$, with $\mu \in \left( 0, \frac{1}{2} \right]$. 
%%
%%We consider a synodic reference system. 
%%
%Since the primaries follow circular orbits, choosing a suitable synodic (rotating) coordinate system, their positions can be fixed at $q_S=(\mu,0)$ and  $q_P=(\mu-1, 0)$.
%
%Let us consider $(q,p) \in \reals^2 \times \reals^2$ as the position and momenta of the third body.
%%
%Then, taking appropriate units, the RCP$3$BP is a $2$-degrees of freedom Hamiltonian system with Hamiltonian
%\begin{equation}\label{eq:RShamiltonianInitial}
%\HInicial(q,p;\mu) = 
%\HInicial_0(q,p) 
%+ \mu \HInicial_1(q;\mu),
%\end{equation}
%where
%\begin{equation}\label{eq:RShamiltonianInitial01} 
%\begin{split}
%\HInicial_0(q,p) &= \frac{||p||^2}{2} - q^t K p - \frac{1}{||q||}, 
%\qquad \text{with} \qquad 
%K= \left( \begin{smallmatrix} 0 & 1 \\ -1 & 0 \end{smallmatrix} \right). \\
%	%\end{equation}
%	%and 
%	%\begin{equation}\label{eq:RShamiltonianInitial1}
%\mu \HInicial_1(q;\mu) &= \frac{1}{||q||} - \frac{(1-\mu)}{||q-(\mu,0)||}
%%, \qquad
%%
%%\mu \HInicial^P_1(q;\mu) = 
%- \frac{\mu}{||q-(\mu-1,0)||}.
%\end{split}
%\end{equation}
%%
%%Notice that, in the rotating reference system, the Hamiltonian system modeling the RCP$3$BP is autonomous. 
%%
%Notice that the system has a symmetry with respect to the involution 
%\begin{equation}\label{def:involutionCartesians}
%	\wt{\Phi}(q,p;t)=(q_1,-q_2,-p_1,p_2;-t).
%\end{equation}
%
%For $\mu>0$, it is a well known fact that the system has five equilibrium points: $L_1$, $L_2$, $L_3$, $L_4$ and $L_5$, called Lagrange points.
%%
%The Lagrange point $L_3$ lies collinear with the primaries and it is on the ``opposite side'' of the primary $P$, with respect to $S$.
%%
%It is a center-saddle critical point and, hence, it has $1$-dimensional stable and unstable manifolds (namely $W^{\stable}$ and $W^{\unstable}$, respectively) and a $2$-dimensional center manifold.
%
%The stable and unstable invariant manifolds have two branches each.
%% 
%One pair initially approaches $L_4$ (that is with $\claus{q_2>0}$), we denote them by $W^{\stable,+}$ and $W^{\unstable,+}$, respectively. 
%%
%Accordingly, $W^{\stable,-}$ and $W^{\unstable,-}$ are the pair of branches that approach $L_5$.
%%
%Notice that, by the involution $\wt{\Phi}$, it is only necessary to compute the upper branches since the inferior branches are symmetric.
%
%
%\subsection{Main Result}
%
%
%%In the following, we denote by $d(\mu)$ the distance between the ``upper branches'' of the one-dimensional invariant manifolds, computed on a section of the phase space.
%%
%%\textcolor{red}{S'ha d'escriure b\'e aquest teorema.}
%%
%\begin{theorem}\label{theorem:mainTheorem}
%Consider the Hamiltonian system given by~\eqref{eq:RShamiltonianInitial}.
%%
%Let $d^{\unstable,\stable}$ be the distance between the one-dimensional unstable $W^{\unstable,+}$ and the stable $W^{\stable,+}$ manifolds of $L_3$ \textcolor{red}{on an appropriate section of the phase space}. 
%%
%There exists $\mu_0>0$ such that for $\mu \in (0,\mu_0)$ the  distance is given by
%\[
%d^{\unstable,\stable}(\mu) \sim 
%\mu^{-\frac{2}{3}} e^{-\frac{A}{\sqrt{\mu}}} 
%\paren{ 
%C^{\unstable,\stable} +
%\OO\paren{\frac{1}{\vabs{\log(\mu)}} }
%},
%\]
%where
%\begin{equation}\label{def:integralA}
%A= \int_0^{\frac{\sqrt{2}-1}{2}} \frac{2}{1-x}\sqrt\frac{x}{3(x+1)(1-4x-4x^2)}  dx\approx 0.177744.
%\end{equation}
%\end{theorem}
%
%\subsection{Outline of the proof}
%\label{subsection:stepsProof}
%
%%In this work and~\cite{?} we 
%%analyze the distance betweeen the $1$-dimensional invariant manifolds of $L_3$ and give an asymptotic formula for its difference.
%%
%%Indeed, in~\cite{?} we give asymptotic formulas for the distance between the stable and unstable manifolds of $L_3$.
%%
%The method we use follows the approaches described, for example, in~\cite{BFGS12, BCS13}.
%%
%On~\cite{?} we have obtained results for the steps:
%\begin{enumerate}[label*=\Alph*.]
%\item To perform a change of coordinates which captures the slow-fast dynamics of the system.
%%
%The new Hamiltonian becomes a (fast) oscillator weakly coupled to a $1$-degree of freedom Hamiltonian with a saddle and an homoclinic connection (also know as separatrix).
%%
%%To obtain this new system, we use the Poincar\'e planar elements (see~\cite{MeyerHallOffin}).
%%These variables do not have an explicit expression, which difficults the analysis of the new Hamiltonian.
%%
%\item To analyze the analytical continuation of the time-parametrization of the unperturbed separatrix.
%%
%%In particular, we obtain the maximal strip of analyticity (centered at the real line) for the parametrization.
%%%
%%We also describe the singularities and its character at the boundaries of this region.
%%
%\item To derive the inner equation, which gives the first order of the original system close to the singularities,
%%
%%This equation is independent of the perturbative parameter and possess two special solutions which are approximations of the perturbed invariant manifolds near the singularities.
%%
%and provide an asymptotic formula for the difference between the two solutions of the inner equation.
%%
%%We follow the approach presented in~\cite{BalSea08}.
%\end{enumerate}
%
%To prove Theorem~\ref{theorem:mainTheorem}, it remains:
%\begin{enumerate}[label*=\Alph*.]
%%
%\item[D.] To prove the existence of the analytic continuation of the parametrizations of the invariant manifolds of $L_3$, $W^{\unstable}$ and $W^{\stable}$, in appropriate complex domains, the so called outer domains.
%%
%These domains contain a segment of	the real line and intersects a neighborhood sufficiently close to the singularities of the separatrix.
%%
%\item[E.] By using complex matching techniques, we compare the solutions of the inner equation with the perturbed invariant manifolds on the outer domain.
%%
%\item[F.] Finally, we prove that the dominant term of the difference between manifolds is given by the term obtained from the difference of the solutions of the inner equation.
%\end{enumerate}
%
%\textcolor{red}{Explicar que passa amb $+,-$ de $W^{\unstable,\stable}$.}
%
%
%\textcolor{red}{Comentar $\CInn$}
%
%%The structure of this paper goes as follows...


==> Article Outer/introductionPoincare.tex <==

The Lagrange point $L_3$ is a centre-saddle equilibrium point of the Hamiltonian $h$ in \eqref{def:hamiltonianInitialNotSplit} whose eigenvalues,  as $\mu \to 0$, satisfy 
%
\begin{equation*}
	%\label{eq:specRot}
	\mathrm{Spec}  = \claus{\pm \sqrt{\mu} \, \rho(\mu), \pm i  \, \omega(\mu) },
	\quad
	\text{with} \quad \left\{
	\begin{array}{l}
		\rho(\mu)=\sqrt{\frac{21}{8}}  + \OO(\mu),\\[0.4em]
		\omega(\mu)=1 + \frac{7}{8}\mu + \OO(\mu^2).
	\end{array}\right.
\end{equation*}
% , its associated eigenvalues are

The center and saddle eigenvalues are found at different time-scales. Moreover, when $\mu=0$, the unstable and stable manifolds of $L_3$ ``collapse'' to a circle of critical points.
%
%The singular character of the problem obstructs the application of methods of splitting of separatrices (see \cite{BFGS12} for example).
%, since it does not exist an homoclinic connection for the unperturbed case.
%
Applying a suitable singular change of coordinates, the Hamiltonian $h$ can be written as a perturbation of a pendulum-like Hamiltonian weakly coupled with a fast oscillator.
%
The construction of this change of variables is presented in detail in Section 2.1 in \cite{articleInner}. 
%
In this section, we summarize the most important properties of this set of coordinates.
% and we rewrite  Theorem \ref{theorem:mainTheorem}.


%When studying close to integrable system around resonances it is usual to ``blow-up'' the singularity to capture the slow-fast time scales.
%%
%Indeed, applying an adequate singular change of coordinates, the Hamiltonian $h$ in \eqref{eq:RShamiltonianInitial} becomes a pendulum-like Hamiltonian weakly coupled with a fast oscillator.

%The first step is to consider the Poincar\'e change of coordinates,
%$
%\phi_{\Poi}: (\la,L,\eta,\xi) \to (q,p).
%$
%
The Hamiltonian $h$ expressed in the classical (rotating) Poincar\'e coordinates,
$
\phi_{\Poi}: (\la,L,\eta,\xi) \to (q,p),
$ 
defines a Hamiltonian system with respect to the symplectic form $d\la \wedge dL + i \h d\eta \wedge d\xi$ and the Hamiltonian
\begin{equation} \label{def:hamiltonianPoincare}
H^{\Poi} = H_0^{\Poi}	+ \mu H_1^{\Poi},
\end{equation}
with
\begin{equation}\label{def:hamiltonianPoincare01}
\begin{split}
H_0^{\Poi}(L,\eta,\xi) &= -\frac{1}{2L^2} - L +  \eta \xi 
%
\qquad \text{and} \qquad
%
H_1^{\Poi} = h_1 \circ \phi_{\Poi}.
\end{split}
\end{equation}
Moreover, the critical point $L_3$ satisfies
\begin{equation*}
\la=0, \qquad \quad(L,\eta,\xi) = (1,0,0) + \OO(\mu)
\end{equation*}
and the linearization of the vector field at this point has, at first order, an uncoupled nilpotent and center blocks,
\begin{equation*}
\begin{pmatrix}
0 & -3 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & i & 0 \\
0 & 0 & 0 & -i 
\end{pmatrix}
+ \OO(\mu).
\end{equation*}
Since $\phi_{\Poi}$ is an implicit change of coordinates, there is no explicit expression for $H_1^{\Poi}$.
%
However, it is possible to obtain series expansion in powers of $(L-1,\eta,\xi)$,
(see Lemma 4.1 in \cite{articleInner} and also Appendix \ref{appendix:proofH-technical}).



To capture the slow-fast dynamics of the system,
%
renaming
\[
\de= \mu^{\frac{1}{4}},
\]
we perform the singular symplectic scaling 
\begin{equation}\label{def:changeScaling}
	\phi_{\sca}:
	(\la, \La, x,  y) 
	\mapsto 
	(\la,L,\eta,\xi),
	\qquad
	L = 1 + \de^2 \La , \quad
	\eta = \de x , \quad
	\xi = \de y 
\end{equation}
and the time {reparametrization $t = \de^{-2} \tau$}. 
%
Defining the potential
\begin{equation}\label{def:potentialV}
\begin{split}
V(\la) 
&=  H_1^{\Poi}(\la,1,0,0;0)
= 1 - \cos \la - \frac{1}{\sqrt{2+2\cos \la}},
\end{split}
\end{equation}
the Hamiltonian system associated to $H^{\Poi}$, expressed in scaled coordinates,
defines a Hamiltonian system with respect to the symplectic form $d\la \wedge d\La + i dx \wedge dy$ 
%
and the Hamiltonian
\begin{equation} \label{def:hamiltonianScaling}
	\begin{split}
		{H} = {H}_{\pend} + {H}_{\osc} + H_1,
	\end{split}
\end{equation}
where
\begin{align} 
	{H}_{\pend}(\la,\La) &= -\frac{3}{2} \La^2  + V(\la), \qquad
	% 
	{H}_{\osc}(x,y; \de) = \frac{x y}{\de^2},
	\label{def:HpendHosc} \\
	%
	H_1(\la,\La,x,y;\de) &=
	H_1^{\Poi}(\la,1+\de^2\La,\de x,\de y;\de^4)  - V(\la) +
	\frac{1}{\de^4} F_{\pend}(\de^2\La)
	\label{def:hamiltonianScalingH1}
\end{align}
and
\begin{equation}\label{def:Fpend}
	F_{\pend}(z) = \paren{-\frac{1}{2(1+z)^2}-(1+z)}+\frac{3}{2} + \frac{3}{2}z^2 = \OO(z^3).
\end{equation}
%
Therefore, we can define the ``new'' first order
\begin{equation}\label{def:hamiltonianScalingH0}
	H_0 = H_{\pend} + H_{\osc}.
\end{equation}
From now on, we refer to $H_0$ as the unperturbed Hamiltonian and we identify $H_1$ as the perturbation.

%
The next proposition, proven in \cite[Theorem 2.1]{articleInner}, gives some properties of the Hamiltonian $H$.

\begin{proposition}\label{proposition:HamiltonianScaling}
The Hamiltonian $H$,
away from collision with the primaries,
 is real-analytic  in the sense of $\conj{H(\la,\La,x,y;\de)}= H(\conj{\la},\conj{\La},y,x;\conj{\de}).$ 

Moreover, for $\de > 0$ small enough, 
\begin{itemize}
\item The critical point $L_3$ expressed in  coordinates $(\la,\La,x,y)$ is given by
\begin{equation}\label{def:pointL3sca}
	\Ltres(\de)=\paren{0,
		\de^2 \LtresLa(\de),
		\de^3 \Ltresx(\de),
		\de^3 \Ltresy(\de)},
\end{equation}
with $\vabs{\LtresLa(\de)}$, $\vabs{\Ltresx(\de)}$, $\vabs{\Ltresy(\de)} \leq C$, for some constant $C>0$ independent of $\de$.
%
\item The point $\Ltres(\de)$ is a saddle-center equilibrium point and its linearization is
\begin{equation*}
	\begin{pmatrix}
		0 & -3 & 0 & 0 \\
		-\frac{7}{8} & 0 & 0 & 0 \\
		0 & 0 & \frac{i}{\de^2} & 0 \\
		0 & 0 & 0 & -\frac{i}{\de^2}
	\end{pmatrix} + \OO(\de).
\end{equation*}
Therefore, it possesses a one-dimensional unstable and stable manifolds, $\WW^{\unstable}(\de)$ and  $\WW^{\stable}(\de)$. 
%
%given the at energy level 
%\[
%H^*_{\Ltres}(\de) = H(\Ltres(\de)) 
%\]
\end{itemize}
\end{proposition}	

%The Hamiltonian $H$ is reversible with respect to the involution 
%\begin{equation*}%\label{def:involutionScaling}
%	\Phi(\la,\La,x,y) = (-\la,\La,y,x).
%\end{equation*}
%
%We define the first order
%\begin{equation}\label{def:hamiltonianScalingH0}
%	{H}_0(\la,\La,\xh,\yh;\de) = {H}_{\pend}(\la,\La) + {H}_{\osc}(\xh,\yh; \de),
%\end{equation}
%which corresponds to a uncoupled pendulum-like ${H}_{\pend}$ and an oscillator ${H}_{\osc}$ Hamiltonian.
%
%We define the stable and unstable manifolds of  in scaling coordinates as
%\begin{align*}
%	\WW^{\unstable} = \phi_{\sca} \circ \phi_{\Poi} (W^{\unstable})
%	\WW^{\stable}
%\end{align*}
%
%From now on, we refer to $\WW^{\unstable}(\de)$ and $\WW^{\stable}(\de)$ as the one-dimensional unstable and stable manifolds of $\Ltres(\de)$, respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

The unperturbed system given by $H_0$ in \eqref{def:hamiltonianScalingH0} has two homoclinic connections in the $(\la,\La)$-plane associated to the saddle point $(0,0)$ and described by the energy level $H_{\pend}(\la,\La)=-\frac12$ (see Figure \ref{fig:separatrix}).
%
\begin{figure}[t] 
	\centering
	\begin{overpic}[scale=0.7]{mainSeparatrixPicture.png}
		\put(93,31){{$\pi$}}
		\put(77,28.5){{$\frac{2}{3}\pi$}}
		\put(49,29){{$0$}}
		\put(17,28.5){{$-\frac{2}{3}\pi$}}
		\put(-2,31){{ $-\pi$}}
		\put(98,34){{$\la$}}
		\put(5,70){{$\La$}}
	\end{overpic}
	\caption{Phase portrait of the system given by Hamiltonian ${H}_{\pend}(\la,\La)$ on~\eqref{def:HpendHosc}. On blue the two separatrices.}
	\label{fig:separatrix}
\end{figure}
%
We define 
\begin{equation}\label{def:lambda0}
\la_0 = \arccos\paren{\frac12-\sqrt2},
\end{equation}
which satisfies $H_{\pend}(\la_0,0)=-\frac12$ so that, for the unperturbed system, $\la_0$ is the ``turning point'' in the $(\la,\La)$ variables. 
%
We will see that, in our regime, $\tht \approx \la$ and thus the value of $\tht_0$ introduced in Remark \ref{remark:sectiontheta} is indeed close to the ``turning point'' of the invariant manifolds (see Figure \ref{fig:L3Outer}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We rewrite Theorem \ref{theorem:mainTheorem}, in fact the more general result in Remark \ref{remark:sectiontheta}, in the  set of coordinates $(\la,\La,x,y)$.
%
% The invariant manifolds $\WW^{\unstable}(\de)$ and $\WW^{\stable}(\de)$ are found at the same energy level
% \[
% H^*_{\de} = 
% H(\Ltres(\de);\de).
% %H(\WW^{\unstable}(\de)) = 
% %H(\WW^{\stable}(\de)).
% \]
% %
% This allows us to restrict to a $3$-dimensional problem.
%
% We define the energy level as
%
For $\la_* \in (0,\la_0)$, we consider the $3$-dimensional section
\begin{align*} %\label{def:sectionScaling}
\SSS(\la_*) = \claus{(\la,\La,x,y) \in \reals^2 \times \complexs^2 \st \la = 
\la_*,\, \La>0, \, {x}=\conj{y}
% , \,
% H(\la,\La,x,y;\de) = H^*_{\de}
},
\end{align*}
which is transverse to the flow of $H$, and we define the first crossings of the invariant manifolds $\WW^{\unstable,\stable}(\de)$ with this section as
$(\la_*, \La^{\unstable}_{*},x^{\unstable}_{*},y^{\unstable}_{*})$
and 
$(\la_*, \La^{\stable}_{*},x^{\stable}_{*},y^{\stable}_{*})$.
%
%The distance in the $\La$-direction is recovered by the energy conservation.


\begin{theorem}\label{theorem:mainTheoremPoincare}
%
Fix an interval $[\la_1,\la_2] \subset (0,\la_0)$ with $\la_0$ as given in \eqref{def:lambda0}.
%
Then, there exists $\de_0>0$  and $\cttTheorem>0$ such that, 
%
for $\de \in (0,\de_0)$ 
and $\la_* \in [\la_1,\la_2]$,  the first crossings are analytic with 
respect to $\lambda^*$ and 
\begin{equation}\label{def:estimatesInvMan}
|\La^{\diamond}_{*}|\leq \cttTheorem,
\qquad |x^{\diamond}_{*}|,|y^{\diamond}_{*}|\leq \cttTheorem \delta^3,\qquad 
\diamond=\unstable, \stable.
\end{equation}
Moreover,
%
%
\begin{align*}
\vabs{x^{\unstable}_{*}-x^{\stable}_{*}} = 
\vabs{y^{\unstable}_{*}-y^{\stable}_{*}} 
&= 
\sqrt[6]{2} \,
\de^{\frac{1}{3}}  e^{-\frac{A}{\de^2}} 
	\boxClaus{ \vabs{\CInn}
	+ \OO\paren{\frac{1}{\vabs{\log \de}}}},\\
\vabs{\La^{\unstable}_*-\La^{\stable}_{*}} &= \OO(\de^{\frac43}e^{-\frac{A}{\de^2}}),
\end{align*}
where  $A$ and  $\CInn$ are the constants introduced in Theorem \ref{theorem:mainTheorem}.

% Moreover, $\vabs{\La^{\unstable}_*-\La^{\stable}_{*}} = \OO(\de^{\frac43}e^{-\frac{A}{\de^2}})$.
\end{theorem}
	


==> Article Outer/matching.tex <==

We now study how well the solutions of the inner equation approximate the solutions of the original system given by by Proposition \ref{proposition:existenceComecocos} in an appropriate domain.
%
% To make this comparison, we use the parametrizations $\zuOut$ and $\zsOut$ provided . 
%
%Let us recall that Theorem~\ref{theorem:existence} provides parameterizations of the invariant manifolds, $\zuOut(u)$ and $\zsOut(u)$.
%
%In particular, we will use the parametrizations given in the intermediate result: Proposition \ref{proposition:existenceComecocos}.
%
%Nevertheless, it does not give enough information about the behavior of these manifolds near the singularities $u=\pm iA$. 
%
%To obtain the dominant behavior near the singularity $u=iA$ we use the solutions $\ZuInn(U)$ and $\ZsInn(U)$ of the inner equation given in Theorem~\ref{theorem:innerComputations}.
%
%\textcolor{red}{Analogously, for the negative singularity $u=-iA$, we use the solutions $\ZuInnN$ and $\ZsInnN$ given by Remark~\ref{remark:innerComputationConjugats}.}  
%
As in the previous section, we focus on the singularity $u=iA$, but analogous results can be proven for $u=-iA$ (see Remark \ref{remark:innerComputationConjugats}).
Let us recall that the functions $\zusOut$ are expressed in the separatrix coordinates (see \eqref{def:changeOuter}) 
%
while the functions $\ZusInn$ are expressed in inner coordinates (see \eqref{def:changeInner}).
%
%Therefore, in order to prove that $\ZusInn(U)$ is a good approximation for $\zusOut(u)$, we need to introduce some suitable domains, in both separatrix and inner coordinates where to compare them. 
%
%\paragraph{Matching domains in the separatrix coordinates.}
%

We first define the matching domains in separatrix coordinates and, later, we translate them to the inner coordinates. Let us consider $\betaMchA$, $\betaMchB$,
and $\gamma$  independent of $\de$ and $\kappa$, such that
\begin{equation*}
%\label{def:beta12}
0< \betaMchA < \betaOutA < \betaMchB < \frac{\pi}{2},
\qquad \text{and} \qquad
\g \in \left[\frac35 ,1\right),
\end{equation*}
with $\betaOutA$ as given in Theorem \ref{theorem:singularities}.
%
Then, we define $u_j \in \complexs$ $j=2,3$ (see Figure \ref{fig:matchingDomains}), as the points satisfying:
\begin{itemize}
	\item $\Im u_j = -\tan \beta_{j} \Re u_j + A - \kappa \de^2$.
	\item $\vabs{u_j- u_+} = \de^{2\gamma}$, where $u_+=i(A-\kappa\de^2)$.
	\item $\Re u_2<0$ and $\Re u_3>0$.
\end{itemize}
%
\begin{figure}[t] 
	\centering
	\vspace{5mm}
	\begin{overpic}[scale=0.9]{dominiMatching.png}
		\put(11,8){\textcolor{myGreen}{{\footnotesize $\DuMchOut$}}}
		\put(91,7){\textcolor{myGreen}{{\footnotesize $\DsMchOut$}}}
		\put(29,4.5){{\footnotesize $\betaMchB$}}
		\put(38.5,4.5){{\footnotesize $\betaOutA$}}
		\put(50.5,4.5){{\footnotesize $\betaMchA$}}
		\put(21.5,26.5){{\footnotesize $iA$}}
		\put(83,26.5){{\footnotesize $iA$}}
		\put(27,24){{\footnotesize $\kappa \de^2$}}
		\put(16.5,16.5){{\footnotesize $\de^{2\g}$}}
		\put(11.5,24.5){\textcolor{myGreen}{{\footnotesize $u_2$}}}
		\put(31,10){\textcolor{myGreen}{{\footnotesize $u_3$}}}
		\put(26.25,20.25){\textcolor{myGreen}{{\footnotesize $u_+$}}}
		\put(22,39){{\footnotesize $\Im u$}}
		\put(84,39){{\footnotesize $\Im u$}}
		\put(61,3){{\footnotesize$\Re u$}}
		\put(101,3){{\footnotesize$\Re u$}}
		\put(97,25){\textcolor{myGreen}{{\footnotesize $-\conj{u}_2$}}}
		\put(76,10){\textcolor{myGreen}{{\footnotesize $-\conj{u}_3$}}}
		\put(83,21){\textcolor{myGreen}{{\footnotesize $u_+$}}}
	\end{overpic}
	%	\bigskip
	\caption{The matching domains $\DuMchOut$ and $\DsMchOut$ in the outer variables.}
	\label{fig:matchingDomains}
\end{figure} 
%
We define the matching domains in the separatrix coordinates as the triangular domains
\begin{align*}
%\label{def:matchingDomainOuter}
	\DuMchOut = 
	\that{u_+ \, u_2 \, u_3},
	\qquad
	\DsMchOut =
	\that{u_+ \, (-\conj{u_2}) \, (-\conj{u_3})}.
\end{align*}
%
%\begin{align}%\label{def:matchingDomainOuter}
%\begin{split}
%\DuMchOut = \left\{
%u \in \complexs \st \right.
%&\Im u < -\tan \betaMchA\Re u + A -\kappa \de^2, \\
%&\Im u < -\tan\betaMchB\Re u + A -\kappa \de^2, \\
%&\Im u > \Im u_1 - \tan\paren{\textstyle\frac{\betaMchA+\betaMchB}{2}} \paren{\Re u-\Re u_1} 
%\left. \right\},  \\
%\DsMchOut = \left\{
%u \in \complexs \st \right. & \left.
%- \conj{u} \in \DuMchOut \right\}.
%\end{split}
%\end{align}
%
%We note that there exists a constant $C$ independent of $\de$ such that
%\[
%C^{-1} \de^{2\g} \leq \vabs{u_j - iA} \leq C \de^{2\g},
%\hh
%\text{ for } j=1,2.
%\]
%Moreover, for all $u \in \DuMchOut \cup \DsMchOut$, we have
%\begin{equation}\label{eq:boundsDomainMchOuter}
%\kappa \de^2 \cos \betaMchA  \leq
%\vabs{u -iA} \leq
%C \de^{2\g}.
%\end{equation}
%
%
Let $\dOuter$, $\rhoOuter$ and $\kappaOuter$ be as given in Proposition \ref{proposition:existenceComecocos}. 
%
Then, for $\kappa\geq \kappaOuter$ and $\de>0$ small enough, the  matching domains satisfy
\begin{equation}\label{eq:domainsMatchingOuterSubset}
\DuMchOut \subset \DuOut \qquad \text{ and } \qquad
\DsMchOut \subset \DsOut,
\end{equation}
and, as a result, $\zuOut$ and $\zsOut$ are well defined in $\DuMchOut$ and $\DsMchOut$, respectively. 

%\paragraph{Matching domains in the inner coordinates.}
%
%Next, we introduce some suitable matching domains for $\ZuInn$ and $\ZsInn$.
%
%Let us recall that, by Theorem \ref{theorem:innerComputations}, the solutions $\ZuInn$ and $\ZsInn$ are well defined in $\DuInn$ and $\DsInn$ (see~\eqref{def:domainInnner}), respectively, for some  $\rhoInn\geq\kappaInner$.
%

The  matching domains in inner variables are defined by
\begin{equation}\label{def:matchingDomainInner}
\DdMchInn = \left\{
U \in \complexs \st \de^2 U + iA \in \DdMchOut
\right\}, \qquad
\text{ for } \diamond=\unstable,\stable,
\end{equation} 
with
\begin{equation}\label{def:U12}
U_j = \frac{u_j - iA}{\de^2},
\hh
\text{ for } j=2,3.
\end{equation}
%
%
%Then, taking into account~\eqref{eq:domainsMatchingOuterSubset} and Remark~\ref{remark:innerDomains} we have that
%
%Then, it is clear that there exist a constant $C$ independent of $\de$ such that
%\begin{equation}\label{eq:boundsDomainMchInner12}
%	\frac{C^{-1}}{\de^{2(1-\g)}} \leq
%	\vabs{U_j} \leq
%	\frac{C}{\de^{2(1-\g)}},
%	\hh
%	\text{ for } j=1,2,
%\end{equation}
%
Therefore, for $U \in \DdMchInn$, 
\begin{equation*}
%  \label{eq:boundsDomainMchInner}
	\kappa \cos \betaMchA  \leq 
	\vabs{U} \leq 
	\frac{C}{\de^{2(1-\g)}}.
\end{equation*}
%
By definition, 
\begin{equation*}
%\label{eq:domainsMatchingInnerSubset}
\DuMchInn \subset \DuInn \qquad\text{ and } \qquad
\DsMchInn \subset \DsInn,
\end{equation*}
for $\kappa \geq \kappaInner$ (see Theorem \ref{theorem:innerComputations}). Thus, $\ZusInn$ is well defined in $\DusMchInn$.

In order to compare $\zusOut(u)$ and $\ZusInn(U)$, we translate $\zusOut$ to inner coordinates
\begin{equation}\label{def:ZdMchO}
\ZdMchO(U) =
\big(\WdMchO,\XdMchO, \YdMchO\big)^T(U) =
 \paren{
	\de^{\frac43}\frac{ \wdOut}{2 \al_+^2}, \,
	\frac{\xdOut}{\de^{\frac13} \sqrt{2}\al_+}, \,
	\frac{\ydOut}{\de^{\frac13} \sqrt{2}\al_+}
}^T(\de^2 U + iA),
\end{equation}
with $\diamond=\unstable,\stable$ and $\zdOut=(\wdOut, \xdOut, \ydOut)^T$ are given in Proposition \ref{proposition:existenceComecocos}.
%
%Notice that $\ZdMchO(U)$ corresponds with $\zdOut(u)$ expressed in the inner coordinates. 
%
Therefore, by \eqref{eq:domainsMatchingOuterSubset},
$\ZdMchO$ is well defined in the  matching domain $\DdMchInn$ (which is expressed in inner variables).

Next theorem  gives estimates for $\ZusMchO-\ZusInn$.

%
%To this end, we define
%\begin{equation}\label{def:ZMchU}
%	\ZdMchU=(\WdMchU,\XdMchU,\YdMchU)
%	=\ZdMchO - \ZdInn, 
%	\qquad \text{for } \diamond=\unstable,\stable.
%\end{equation}
%such that $\ZdMchU=(\WdMchU,\XdMchU,\YdMchU)$ and with $\ZdMchO$ as defined on~\eqref{def:ZdMchO}.
%
%In the following theorem, we obtain estimates for the difference $\ZuMchU$ and $\ZsMchU$.

\begin{theorem}\label{theorem:matching}
Consider $\kappaOuter$ and $\kappaInner$ as obtained in Proposition~\ref{proposition:existenceComecocos}
and  	
Theorem \ref{theorem:innerComputations}, respectively.
%	
Then, there exist $\g^*\in [\frac35,1)$, 
$\kappaMch \geq \max\claus{\kappaOuter,\kappaInner}$ 
and $\de_0>0$ such that, 
for  $\g \in (\g^*,1)$,
%
there exists $\cttMch>0$ satisfying that, for $U \in \DdMchInn$,
$\kappa\geq \kappaMch$
and 
$\de \in (0,\de_0)$,
\begin{equation*}
|U^{\frac{4}{3}}\WdMchU(U)| \leq \cttMch \de^{\frac{2}{3}(1-\g)}, \qquad
\vabs{U \h \XdMchU(U)} \leq \cttMch \de^{\frac{2}{3}(1-\g)}, \qquad
\vabs{U \h \YdMchU(U)} \leq \cttMch  \de^{\frac{2}{3}(1-\g)},
\end{equation*}
with 
$
(\WdMchU,\XdMchU,\YdMchU)^T=\ZdMchU
=\ZdMchO - \ZdInn$ and $\diamond=\unstable,\stable$.
\end{theorem}

This theorem is proven in Section \ref{section:proofG-matching}.



==> Article Outer/outer.tex <==

In this section, following the approach described in~\cite{BFGS12, BCS13, 
GMS16}, we study the analytic continuation of the parametrizations of the 
perturbed one-dimensional stable and unstable manifolds, $\WW^{\unstable}(\de)$ 
and $\WW^{\stable}(\de)$. 
%in appropriate complex domains and provide estimates for them.
%
%(Notice that these manifolds coincide with the invariant manifolds of $L_3$ in the original coordinates).
%
%\subsubsection{Perturbed invariant manifolds as a graph}

Since we  measure the distance between the invariant manifolds in the 
section $\la=\la_*$ (see Theorem \ref{theorem:mainTheoremPoincare}), 
we parameterize them as graphs with respect to $\la$ (whenever is possible) or, 
more conveniently, 
%
% However, a priori, we do not know the domain of analyticity of the perturbed invariant manifolds (for the component $\la$).
%
% Nonetheless, for $\de=0$, we know that $\la=\la_h(t)$ and can be analytically extended for $t \in \Pi_{A,\betaBow}^{\mathrm{ext}}$ (see Theorem \ref{theorem:singularities}).
%
% In fact, it is more convenient to use parameterize them as graphs 
with respect 
to the independent variable $u$ defined by $\la=\la_h(u)$.


To define these suitable parameterizations we first translate the 
equilibrium point $\Ltres(\de)$ to $\mathbf{0}$ by the change of coordinates
\begin{equation}\label{def:changeEqui}
	\phi_{\equi}:(\la,\La,x,y) \mapsto (\la,\La,x,y) + \Ltres(\de).
\end{equation}
%
Second, we consider the symplectic change of coordinates 
\begin{equation}\label{def:changeOuter}
	\phi_{\out}:(u,w,x,y) \to (\la,\La,x,y),
	%\end{equation}
	%given by
	%\begin{equation}
	\quad 
	{\la}= \la_h(u), \hh  {\La}= \La_h(u) - \frac{w}{3\La_h(u)}.
\end{equation}
%
We refer to $(u,w,x,y)$ as the \emph{separatrix coordinates}.

Let us remark that $\phi_{\out}$ is not defined for $u=0$ since $\La_h(0)=0$ (see Theorem \ref{theorem:singularities}).
%
We deal with this fact later when considering the domain of definition for $u$.

% 
%We consider the section 
%\begin{align} \label{def:sectionOuter}
%	\Sigma(u_*) = \claus{(u,w,x,y) \in \reals^2 \times \complexs^2 \st u = u_*, \, {x}=\conj{y}},
%\end{align}
%where $\la_*=\la_h(u^*)$.
%
%The change of coordinates $\phi_{\out}$ has some useful characteristics:
%\begin{itemize}
%	\item Since in the unperturbed case the invariant manifolds coincide along the separatrix $(\la_h,\La_h,0,0)$ (see \eqref{eq:separatrixParametrization}), then it makes sense to expect the perturbed ones to be close to it.
%	%
%	\item Even though, a priori, we do not have control over the domain of definition of $(\la,\La)=(\la_h(u),\La_h(u))$, we do know that they are well defined for $u \in \Pi_{A,\betaBow}^{\mathrm{ext}}$.
%	%
%	Thus, considering $u$ as a new coordinates, gives us control over its domain.
%	\item Notice that, for $\de=0$, $\dot{u}=1$ and that $\la=\la_h(u)$ is well defined for $u \in \Pi_{A,\betaBow}^{\mathrm{ext}}$.
%\end{itemize}
%
%
 
After these changes of variables, we look for the perturbed invariant manifolds 
as a graph with respect to $u$.
% and measure the difference between the stable and 
% unstable manifolds at the section $u=u^*$ such that $\la_*=\la_h(u_*)$.
%
In other words, we look for functions
\[
\zdOut(u) = \left(\wdOut(u),\xdOut(u),\ydOut(u)\right)^T,
\quad \text{ for } \diamond=\unstable,\stable,
\]
such that the 
invariant manifolds given in Proposition~\ref{proposition:HamiltonianScaling} 
can be expressed as
\begin{equation}\label{eq:invariantManifoldsExpression}
\WW^{\diamond}(\de)= \left\{ \paren{\la_h(u), \La_h(u)-\frac{\wdOut(u)}{3\La_h(u)}, \xdOut(u), \ydOut(u)} + \Ltres(\de)\right\}, \quad \text{for } \diamond=\unstable,\stable,
\end{equation}
%\footnote{In these coordinates, the unperturbed separatrix is  $\{(w,x,y)=(0,0,0)\}$.}
with $u$ belonging to an appropriate domain contained in $\Pi^{\mathrm{ext}}_{A, \betaBow}$ (see \eqref{def:dominiBow}).
%
%Indeed, since by Theorem~\ref{theorem:singularities}, the parametrization of the separatrix $(\la_h,\La_h)$ is well-defined and analytic in $\Pi^{\mathrm{ext}}_{A, \betaBow}$.
%
The graphs $\zuOut$ and $\zsOut$
must satisfy the asymptotic conditions 
%
\begin{equation}\label{eq:asymptoticConditionsOuter}
	\begin{split}
		\lim_{\Re u \to -\infty} \left(\frac{\wuOut(u)}{\La_h(u)},\xuOut(u), \yuOut(u) \right) = %0, \hh
		\lim_{\Re u \to +\infty} \left(\frac{\wsOut(u)}{\La_h(u)},\xsOut(u), \ysOut(u) \right) = 0.
	\end{split}
\end{equation}

\begin{remark}\label{remark:realAnalytic}
Since the Hamiltonian $H$ is real-analytic in the sense of $\conj{H(\la,\La,x,y;\de)}=H(\conj{\la},\conj{\La},y,x;\conj{\de})$ (see Proposition \ref{proposition:HamiltonianScaling}), 
%
then we say that $\zOut(u)=(\wOut(u),\xOut(u),\yOut(u))^T$ is real-analytic if it satisfies
\begin{align*}
	\wOut(\conj{u}) = \conj{\wOut(u)}, \qquad
	\xOut(\conj{u}) = {\yOut(u)}, \qquad
	\yOut(\conj{u}) = {\xOut(u)}.
	%\quad \text{for } \diamond=\unstable,\stable.
\end{align*}
\end{remark}


The classical way to study exponentially small  splitting of separatrices, in this setting, is to look for solutions $\zuOut$ and $\zsOut$ in a certain complex common domain containing a segment of the real line and intersecting a $\OO(\de^2)$ neighborhood of the singularities $u=\pm iA$ of the separatrix.

Recall that the invariant manifolds can not be expressed as a graph in a neighborhood of $u=0$.
% 
To overcome this technical problem, we find solutions $\zuOut$ and $\zsOut$ defined in a complex domain, which we call \emph{boomerang domain} due to its shape (see Figure~\ref{fig:dominiBoomerang}).
%
\begin{figure}[t] 
	\centering
	\begin{overpic}[scale=1]{DominiBoomerang.png}
		\put(60,31){$\DBoomerang$}
		\put(19,29.5){\footnotesize $\betaOutA$}
		\put(48.5,29.5){\footnotesize $\betaOutB$}
		\put(42,49.5){\footnotesize $iA$}
		\put(52,44.5){\footnotesize $i(A-\kappa \de^2)$}
		\put(39.5,4){\footnotesize $-iA$}
		\put(41,35){\footnotesize $\dBoomerang A$}
		\put(102,27){\footnotesize$\Re u$}
		\put(45,58){\footnotesize$\Im u$}
	\end{overpic}
	\bigskip
	\caption{The boomerang domain $\DBoomerang$ defined in~\eqref{def:dominiBoomerang}.}
	\label{fig:dominiBoomerang}
\end{figure}
%
Namely,
\begin{equation}\label{def:dominiBoomerang}
\begin{split}
\DBoomerang = \left\{ u \in \complexs \right. \st 
&\vabs{\Im u} < A - \kappa \de^2 + \tan \betaOutA \Re u,
% \\
% &
\vabs{\Im u} < A - \kappa \de^2 - \tan \betaOutA \Re u,
\\
&\vabs{\Im u} > \left. \dBoomerang A - \tan \betaOutB \Re u 
\right\},
\end{split}
\end{equation}
where $\kappa>0$ is such that $A-\kappa \de^2>0$,
$\betaOutA$ is the constant given in Theorem~\ref{theorem:singularities}
and $\betaOutB \in [\betaOutA,\frac{\pi}{2})$ and $\dBoomerang \in 
(\frac{1}{4},\frac{1}{2})$
are independent of $\de$.

%In the rest of the paper we assume without mentioning it that $\kappa_j$, for $j=1,..,?$, satisfy that $A-\kappa_j \de^2>0$  and might depend on $\de$.
%
%In the rest of the paper, we fix $\betaOutB \in [\betaOutA,\frac{\pi}{2})$ with $\betaOutA$ given in Theorem~\ref{theorem:singularities}.

\begin{theorem}\label{theorem:existence}
% Let $\zuOut$ and $\zsOut$ be the functions in~\eqref{eq:invariantManifoldsExpression} defining
% the parametrization as a graph of the perturbed unstable and stable manifold, $\WW^{\unstable}(\de)$ and $\WW^{\stable}(\de)$, respectively.
%
Fix a constant $\dBoomerang \in (\frac{1}{4},\frac{1}{2})$.
%
Then, there exists $\de_0, \kappaBoomerang>0$ such that,
%
for $\de \in (0,\de_0)$, 
$\kappa\geq\kappaBoomerang$,
%
the graph parameterizations $\zuOut$ and $\zsOut$ introduced 
in~\eqref{eq:invariantManifoldsExpression} can be extended real-analytically to 
the domain $\DBoomerang$.

Moreover, there exists a real constant $\cttOuterA>0$ independent of $\de$ and $\kappa$ such that, for $u \in \DBoomerang$ we have that
\begin{align*}%\label{eq:boundsOuter}
|\wdOut(u)| \leq \frac{\cttOuterA\de^2}
{\vabs{u^2 + A^2}}
+ \frac{\cttOuterA\de^4}{\vabs{u^2 + A^2}^{\frac{8}{3}}}, \quad
%
|\xdOut(u)| \leq \frac{\cttOuterA\de^3}
{\vabs{u^2 + A^2}^{\frac{4}{3}}}, \quad
%
|\ydOut(u)| \leq \frac{\cttOuterA\de^3}
{\vabs{u^2 + A^2}^{\frac{4}{3}}}.
\end{align*}
\end{theorem}

%\begin{remark}
%On Theorem \ref{theorem:existence} we use a compounded weight to estimate $\wdOut(u)$, for $\diamond=\unstable,\stable$. 
%%
%This weight is necessary, since functions $\wdOut(u)$ have different estimates depending on the region where $u$ is found. 
%%
%Indeed, for $u$ in a neighborhood of the real line we have
%\[
%\vabs{\wdOut(u)} \leq \frac{\cttOuterA}{\vabs{u^2+A^2}\efr{4}{3}},
%\qquad
%\text{for }
%\vabs{\Im u} \ll 1.
%\]
%However, in a neighborhood of the singularities $\pm iA$,
%\[
%\vabs{\wdOut(u)} \leq \frac{\cttOuterA \de^2}{\vabs{u^2+A^2}\efr{8}{3}},
%\qquad
%\text{for }
%\vabs{u-iA}, \vabs{u+iA} \ll 1.
%\]
%\end{remark}

Notice that the asymptotic conditions \eqref{eq:asymptoticConditionsOuter} do 
not have any meaning in the domain $\DBoomerang$ since it is bounded.
%
Therefore, to prove the existence of $\zuOut$ and $\zsOut$ in $\DBoomerang$ one has to start with different domains where these asymptotic conditions make sense and then find a way to extend  them real-analytically to $\DBoomerang$.
%
We describe the details of these process in the  following Sections \ref{subsection:outerBasic} and \ref{subsection:outerExtension}.


==> Article Outer/outerGlobal.tex <==

Since by Proposition~\ref{proposition:existenceComecocos} the unstable solution $\zuOut$ is defined in $\DuOutKappa$,
%
To prove Theorem \ref{theorem:existence}
it only remains to extend it to the points in the boomerang domain $\DBoomerangKappa$ which do not belong to the outer unstable domain. 
%
Namely, we extend $\zuOut$ to
\begin{equation}\label{def:domainBoomerangTilde}
\begin{split}
\DBoomerangTilde = \left\{ u \in \complexs \right. \st 
&\vabs{\Im u} < A - \kappa \de^2 - \tan \betaOutA \Re u,
\\
&\vabs{\Im u} < \dBoomerang A + \tan \betaOutB \Re u, \, \,
\vabs{\Im u} > \left. \dBoomerang A - \tan \betaOutB \Re u 
\right\},
\end{split}
\end{equation}
%
for suitable $\kappa$ and $d$ (see Figure~\ref{fig:dominiBoomerangTilde}).
%
Notice that $\DBoomerangTilde \subset \DBoomerang$ and that $\DBoomerangTilde$ only contains points at distance of $u=\pm iA$ of order $1$ with respect to $\de$.
%
\begin{figure} 
\centering
\begin{overpic}[scale=1]{DominiBoomerangTilde.png}
	\put(50,50){$\DBoomerangTilde$}
	%\put(-5,50){\footnotesize $\DuOut$}
	\put(12,30){$\DBoomerang$}
	\put(33,79){\footnotesize $iA$}
	\put(33,10){\footnotesize $-iA$}
	\put(19,57.5){\footnotesize $\dBoomerang A$}
	\put(101,44.5){\footnotesize$\Re u$}
	\put(27,93.5){\footnotesize$\Im u$}
\end{overpic}
\bigskip
\caption{The domain $\DBoomerangTilde$ defined in~\eqref{def:domainBoomerangTilde}.}
\label{fig:dominiBoomerangTilde}
\end{figure}

As we have mentioned, to measure  the difference between the invariant manifolds $\WW^{\unstable}(\de)$ and $\WW^{\stable}(\de)$ it is  convenient to parameterize them as graphs (see \eqref{eq:invariantManifoldsExpression}). 
%
However, these graph parametrizations are not defined at $u=0$.
%
Moreover, since all the fixed point arguments that we apply to obtain the graph parameterizations rely on complex path integration, we are not able to extend them to domains which are not simply connected.
%
Therefore, to reach $\DBoomerangTilde$ from $\DuOut$, we need to switch to a different parametrization that is well defined at $u=0$.

The auxiliary parametrization we consider is the classical time-parametrization which is associated to the Hamiltonian $H$ in \eqref{def:hamiltonianScaling}.
%
(Recall that the graph parametrization $\zuOut$ was associated to the Hamiltonian $H^{\out} = H \circ \phi_{\equi} \circ \phi_{\out}$).

%This auxiliary parametrization is the classical (complex) time-parametrization. 
%%
%Indeed, we consider  \begin{equation*}%\label{def:flowParametrization}
%\Gu = \phi_{\equi} \circ \phi_{\out}(\cdot,\zuOut(\cdot)).
%\end{equation*}
%%
%Then, by \eqref{eq:invariantManifoldsExpression}, it is clear that $\WW^{\unstable}(\de) = \{\Gu(u)\}$ and $\Gu(u)$ is a solution of the Hamiltonian system defined by $H$ (see \eqref{def:hamiltonianScaling}).
%%
%Therefore, to describe $\WW^{\unstable}(\de)$ we switch from parametrization $\zuOut$ to $\Gu$, whenever we need.
%%

This analytic extension procedure 
%through the time-parametrization 
has three steps:
%
\begin{enumerate}
\item We consider the \emph{outer transition domain} (see Figure \ref{fig:dominisTransition})
\begin{equation}\label{def:DOuterTilde}
\begin{split}	
	\DOuterTilde = \left\{ v \in \complexs \right. \st  
	&\vabs{\Im v} < A - \kappaOuterTilde \de^2 - \tan \betaOutA \Re v,
	\\
	&\vabs{\Im v} > \dOuterA A + \tan \betaOutB \Re v, 
	\\ &\left.
	\vabs{\Im v} < \dOuterB A + \tan \betaOutB \Re v
	\right\},
\end{split}
\end{equation}
where
$\dOuter < \dOuterA < \dOuterB < \frac12$
are independent of $\de$
%
and  $\kappaOuterTilde>\kappaOuter$ is such that $A-\kappaOuterTilde \de^2>0$.
%
Notice that $\DOuterTilde \subset \DuOutKappa$.

Since $\dot{u}=1+o(1)$ (see \eqref{eq:systemEDOsOuter}),
we look for a real-analytic and close to the identity change of coordinates $u=v + \uOut(v)$ defined in $\DOuterTilde$ such that the time-parametrization
\begin{equation}\label{eq:equationuOutA}
\Gu(v) = \phi_{\equi} \circ \phi_{\out}(v+\uOut(v),\zuOut(v+\uOut(v)))
\end{equation}	
is a solution of  the Hamiltonian $H$ in \eqref{def:hamiltonianScaling}.
%
That is, $\dot{v}=1$ and $\Gu(v)\in\WW^{\unstable}(\de)$ for $v\in \DOuterTilde$.
%
See the details in Proposition \ref{proposition:changeuOut} and Corollary \ref{corollary:changeuOut} below.
%
%\item First, we prove the existence of a suitable change of variables
%to obtain $\Gh(v)$ in \eqref{def:flowParametrization} from the parametrizations  $\zuOut(u)$ given in Proposition~\ref{proposition:existenceComecocos}.
%
\item We  extend analytically the time-parametrization $\Gu(v)$ to reach the domain $\DBoomerangTilde$.
%
In particular, we extend $\Gu$ to the \emph{flow domain}
%
\begin{equation}\label{def:dominiFlow}
\begin{split}
	\DFlow = \left\{ v \in \complexs \st
	\right. &
	\vabs{\Im v} < A - \kappa \de^2 - \tan \betaOutA \Re v, 
	\\ & \left.
	\vabs{\Im v} < \dFlow A + \tan \beta_1 \Re v
	\right\},
\end{split}
\end{equation}
where
$\dFlow \in (\dOuterA,\dOuterB)$
is independent of $\de$
%
and  $\kappaFlow>\kappaOuterTilde$ is such that $A-\kappaFlow \de^2>0$.
%
Notice that, 
\[
\DOuterTilde \cap \DFlow\neq\emptyset,
\qquad \text{and} \qquad
\DBoomerangTildeProp \subset \DFlow, 
\]
for $\dBoomerangTilde\in(\dOuter,\dFlow)$ and 
$\kappaBoomerangTilde>\kappaFlow$.
%
See the details in Proposition \ref{proposition:existenceFlow}.

\item We prove that there exists a real-analytic close to the identity change of variables of the form $v=u+\vOut(u)$,  $u\in\DBoomerangTildeProp$, such that the function $\zuOut(u)$ defined by
\begin{equation}\label{eq:equationvOut}
	(u,\zuOut(u)) =
	(\phi_{\equi} \circ \phi_{\out})^{-1} \Big( \Gu(u + \vOut(u))\Big) 	
\end{equation}
gives an invariant graph of $H^{\out}$ in \eqref{def:hamiltonianOuter}.
%
%
See the details in Proposition \ref{proposition:changevOut} and Corollary \ref{corollary:changevOut} below.
\end{enumerate}

As a consequence, we have extended analytically $\zuOut$ to $\DBoomerangTildeProp$.

\begin{figure}[t] 
	\centering
	\begin{overpic}[scale=1]{dominiTransition.png}
		\put(-1,25){$\DOuterTilde$}
		\put(5,6){\footnotesize $\DuOut$}
		\put(71,21){$\DFlow$}
		\put(55,9){\footnotesize $\DOuterTilde$}
		\put(22,22){\footnotesize $\dOuterA A$}
		\put(12,27){\footnotesize $\dOuterB A$}
		\put(21.5,32){\footnotesize $iA-\kappaOuterTilde\de^2$}
		\put(6,17){\footnotesize $\rhoOuterTilde$}
		\put(57,26){\footnotesize $\dFlow A$}
		\put(54,30){\footnotesize $iA-\kappaFlow\de^2$}
		\put(71,30){\footnotesize $v_1$}
		\put(71,6){\footnotesize $\conj{v_1}$}
		\put(56,17){\footnotesize $v_0$}
		\put(35,18){\footnotesize $\Re u$}
		\put(101,18){\footnotesize $\Re v$}
		\put(15,39){\footnotesize $\Im u$}
		\put(64,37){\footnotesize $\Im v$}
	\end{overpic}
	\bigskip
	\caption{The domain $\DOuterTilde$ given in \eqref{def:DOuterTilde} (left) and $\DFlow$ in \eqref{def:dominiFlow} (right).}
	\label{fig:dominisTransition}
\end{figure}


%For the first step, we consider the transition domain:
%\begin{equation}\label{def:DOuterTilde}
%\begin{split}	
%\DOuterTilde = \left\{ u \in \complexs \right. \st  
%&\vabs{\Im u} < A - \kappaOuterTilde \de^2 - \tan \betaOutA \Re u,
%\\ &\left.
%\vabs{\Im u} > \dOuterA A + \tan \betaOutB \Re u, 
%\, \,
%\vabs{\Im u} < \dOuterB A + \tan \betaOutB \Re u
%\right\},
%\end{split}
%\end{equation}
%where
%$\dOuterA, \dOuterB \in (\dOuter,\frac{1}{2})$
%are fixed independently of $\de$
%%
%and  $\kappaOuterTilde>\kappaOuter$ are such that $A-\kappaOuterTilde \de^2>0$.
%%
%Moreover, notice that $\DOuterTilde \subset \DuOutKappa$.
%
%Moreover, we consider $\rhoOuterTilde$ as the the smallest real part of the domain.
%(see Figure~\ref{fig:dominisTransition}).
%
%It is natural to look for parametrizations of $W^{\unstable}$ of the form
%\begin{equation}\label{eq:uOutParametrization}
%\Gh(v) =\phi_{\equi} \circ \phi_{\out}
%	\paren{v+\uOut(v), \zuOut(v+\uOut(v))},
%\qquad v \in \DOuterTilde,
%\end{equation}
%
%In this domain, we look for a change $u=v+\uOut(v)$ such that it allow us to obtain parametrization $\Gu(v)$ from the graph solution $\zuOut(u)$ given in Proposition \ref{proposition:existenceComecocos}.

For the first step, we look for a function $\uOut$ such that $\paren{v+\uOut(v), \zuOut(v+\uOut(v))}$ is a solution of the differential equations given by the Hamiltonian $H^{\out}$ in \eqref{def:hamiltonianOuter}.
%
Therefore, $\uOut$ satisfies 
\begin{equation}\label{eq:equationuOutB}
	\partial_v \, {\uOut}(v) = \partial_w H_1^{\out}
	\paren{v + \uOut(v), \zuOut(v+\uOut(v))}.
\end{equation}
%with
%\begin{equation}\label{def:operatorRRRtransition}
%	R[\varphi](v) = \partial_w H_1^{\out}
%	\paren{v + \varphi(v), \zuOut(v+\varphi(v))}.
%\end{equation}
The next proposition ensures that $\uOut$ exists and it is well defined for $v\in\DOuterTilde$.

\begin{proposition}\label{proposition:changeuOut}
Let the function $\zuOut$ and the constants $\rhoOuter$, $\dOuter$ and $\kappaOuter$ be as obtained in Proposition~\ref{proposition:existenceComecocos}
%
and consider constants $\dOuterA,\dOuterB \in(\dOuter,\frac{1}{2})$ such that $\dOuterA<\dOuterB$ and 
$\kappaOuterTilde>\kappaOuter$. 
%
Then, there exists $\de_0$ such that, for $\de \in (0,\de_0)$,
%
the equation \eqref{eq:equationuOutB} has  a real-analytic solution $\uOut: \DOuterTilde \to  \complexs$.

Moreover, for some  constant $\cttOuterD>0$ independent of $\de$ and  for $v \in \DOuterTilde$, $\uOut$ satisfies
\[
\vabs{\uOut(v)} \leq \cttOuterD \de^{2}
\qquad \text{and} \qquad
v + \uOut(v) \in \DuOutKappa.
\]
\end{proposition}

This proposition is proved in Section \ref{subsection:proofH-changeuOut}.
%\item If $v \in \DOuterTilde$, then $v + \uOut(v) \in \DuOutKappa$.
%
%\item Let $\Gu(v)$ be defined as in \eqref{def:flowParametrization}.
%%
%Then, there exists a constant $\cttOuterE>0$ independent of $\de$ such that, for $v \in \DOuterTilde$,
%\begin{align*}
%\vabsSmall{\lah(v)} \leq \cttOuterE \de^2, \qquad
%\vabsSmall{\Lah(v)} \leq \cttOuterE \de^2, \qquad
%\vabsSmall{\xh(v)} \leq \cttOuterE \de^3, \qquad
%\vabsSmall{\yh(v)} \leq \cttOuterE \de^3.
%\end{align*}
%
%For the second step we consider the \textcolor{red}{flow domain (Pensar millor nom)}. Namely,
%\begin{equation}\label{def:dominiFlow}
%\begin{split}
%\DFlow = \left\{ u \in \complexs \st
%\right. &
%\vabs{\Im u} < A - \kappa \de^2 - \tan \betaOutA \Re u, 
%\\ & \left.
%\vabs{\Im u} < \dFlow A + \tan \beta_1 \Re u
%\right\},
%\end{split}
%\end{equation}
%where
%$\dFlow \in (\dOuterA,\dOuterB)$
%is fixed independently of $\de$
%%
%and  $\kappaFlow>\kappaOuterTilde$ is such that $A-\kappaFlow \de^2>0$.
%
%Moreover, we define $v_0$, $v_1$ and $\conj{v_1}$, the vertices of the domain $\DFlow$(see Figure \ref{fig:dominisTransition}).
%
Together with Proposition \ref{proposition:changeuOut} implies the following corollary.
% that the parametrization $\Gu(v)$, introduced in \eqref{eq:equationuOutA}, is well defined for $v \in \DOuterTilde$.
% %
%See next corollary.

\begin{corollary}\label{corollary:changeuOut}
Under the hypothesis of Proposition \ref{proposition:changeuOut}, 
% Let the function $\uOut$ and the constants
% $\dOuterA, \dOuterB$ and $\kappaOuterTilde$ be as obtained in Proposition~\ref{proposition:changeuOut}.
%
% Then 
there exists $\de_0>0$ such that, for $\de \in (0,\de_0)$,  
the function $\Gu$ in \eqref{eq:equationuOutA} is well defined and real-analytic in $\DOuterTilde$.	
%Moreover, there exists constant $\cttOuterE>0$ independent of $\de$ such that, for $v \in \DOuterTilde$,
%\begin{align*}
%	\vabsSmall{\lah(v)} \leq \cttOuterE \de^2, \qquad
%	\vabsSmall{\Lah(v)} \leq \cttOuterE \de^2, \qquad
%	\vabsSmall{\xh(v)} \leq \cttOuterE \de^3, \qquad
%	\vabsSmall{\yh(v)} \leq \cttOuterE \de^3.
%\end{align*}
\end{corollary}

On the following, we use without mention that $\Gu(v)$ can be split as
\begin{align}\label{eq:splitParametrizationGu}
	\Gu(v) = \G_h(v) + \Gh(v),
	\quad \text{with} \quad
	\left\{
	\begin{aligned}
		\G_h &  = (\la_h,\La_h,0,0)^T, \\
		\Gh  & = (\lah, \Lah, \xh,\yh)^T.
	\end{aligned} 
	\right.
\end{align}
%
The next proposition extends the parametrization $\Gu$ to the domain $\DFlow$ (see \eqref{def:dominiFlow}).


\begin{proposition}\label{proposition:existenceFlow}
Let the function $\Gu$ and the constants
$\dOuterA, \dOuterB$ and $\kappaOuterTilde$ be as obtained in Corollary~\ref{corollary:changeuOut} and Proposition \ref{proposition:changeuOut}
%
and fix
$\dFlow \in (\dOuterA,\dOuterB)$ and $\kappaFlow>\kappaOuterTilde$.
%
Then, there exists $\de_0>0$ such that,
for $\de \in (0,\de_0)$, $\Gu$ 
can be real-analytically extended to $\DFlow$. 

Moreover, there exists a constant $\cttOuterF>0$ independent of $\de$ such that, for $v \in \DFlow$,
\begin{align*}
	\vabsSmall{\lah(v)} \leq \cttOuterF \de^2, \qquad
	\vabsSmall{\Lah(v)} \leq \cttOuterF \de^2, \qquad
	\vabsSmall{\xh(v)} \leq \cttOuterF \de^3, \qquad
	\vabsSmall{\yh(v)} \leq \cttOuterF \de^3.
\end{align*}	
\end{proposition}

This proposition is proved in Section \ref{subsection:proofH-existenceFlow}.

%\begin{equation}\label{def:flowParametrizationB}
%	\Gu(v) = 
%	\paren{\la_h(v), \La_h(v),0,0} + \Gh(v),
%	\qquad
%	\Gh = (\lah,\Lah,\xh, \yh)
%\end{equation}


For the third step, we ``go back'' to the graph parametrization $\zuOut(u)$ by looking for a change $v=u+\vOut(u)$ for $u \in \DBoomerangTilde$.
%
Notice that, in order to satisfy equation \eqref{eq:equationvOut} and recalling \eqref{def:pointL3sca}, $\vOut$ must be a solution of
\begin{equation}\label{eq:equationsvOutA}
	\lah(u+\vOut(u)) = 
	\la_h(u)-\la_h(u+\vOut(u)).
\end{equation}
%
% ().
%
Then, one can easily recover the graph parametrization $(\wuOut(u),\xuOut(u),\yuOut(u))$ using the equations
%
\begin{align}
%\left\{
\begin{aligned}\label{eq:equationsvOutB}
\La_h(u) 
-\La_h(u+\vOut(u))
- \frac{\wuOut(u)}{3\La_h(u)} + \de^2 \LtresLa(\de) 
&=
\Lah(u+\vOut(u)), \\
%
\xuOut(u) + \de^3 \Ltresx(\de) &=\xh(u+\vOut(u)), \\
%
\yuOut(u) + \de^3 \Ltresy(\de)
&=	\yh(u+\vOut(u)).
\end{aligned}
%\right.
\end{align}
%where $\Gu=(\la_h,\La_h,0,0)+(\lah,\Lah,\xh,\yh)$.
%
%Therefore, we look for a change of variables $\vOut$ satisfying \eqref{eq:equationsvOutA}.
%
%Then, by \eqref{eq:equationsvOutB}, we obtain the graph parametrization $\zuOut=(\wuOut,\xuOut,\yuOut)$.

The next proposition ensures that $\vOut$ exists and it is well defined in $\DBoomerangTilde$ (see \eqref{def:domainBoomerangTilde}).

\begin{proposition}\label{proposition:changevOut}
Let the function $\Gu$ and the constants
$\dFlow$ and $\kappaFlow$ be as obtained in Proposition~\ref{proposition:existenceFlow}
and the constant $\dOuter$ as obtained in
Proposition~\ref{proposition:existenceComecocos}.
%
Let us consider constants
$\dBoomerangTilde\in(\dOuter,\dFlow)$ and 
$\kappaBoomerangTilde>\kappaFlow$.
%
Then, there exists $\de_0>0$ such that,
for $\de \in (0,\de_0)$, equation \eqref{eq:equationsvOutA} has a real-analytic solution $\vOut: \DBoomerangTildeProp \to \complexs$ 
satisfying 
\[
\vabs{\vOut(u)} \leq \cttOuterG \de^{2}
\qquad \text{and} \qquad
u + \vOut(u) \in \DFlow.
\]
for some  constant $\cttOuterG>0$ independent of $\de$  and  $u \in \DBoomerangTildeProp$.
\end{proposition}

Proposition \ref{proposition:changevOut} is proved in Section \ref{subsection:proofH-changevOut}. Summarizing all the previous results we obtain the following result.

\begin{corollary}\label{corollary:changevOut}
Let the function $\vOut$ and the constants $\dBoomerangTilde$ and $\kappaBoomerangTilde$ be as obtained in Proposition \ref{proposition:changevOut}. 
%
Then, there exists $\de_0>0$ such that,
for $\de \in (0,\de_0)$, 
equation \eqref{eq:equationsvOutB} has a unique solution $\zuOut=(\wuOut,\xuOut,\yuOut)^T: \DBoomerangTildeProp \to \complexs^3$.

Moreover, there exists a constant $\cttOuterH>0$ independent of $\de$ such that, for $u \in \DBoomerangTildeProp$,
\begin{align*}
	\vabsSmall{\wuOut(u)} \leq \cttOuterH \de^2, \qquad
	\vabsSmall{\xuOut(u)} \leq \cttOuterH \de^3, \qquad
	\vabsSmall{\yuOut(u)} \leq \cttOuterH \de^3.
\end{align*}
\end{corollary}


To finish this section, notice that, taking $\rhoOuter$ big enough,
$\dBoomerang \geq \dBoomerangTilde$ and $\kappaBoomerang\geq\kappaBoomerangTilde$
%
we have that
\[
\DBoomerangKappa \subset \DuOutKappa \cup \DBoomerangTildeProp,
\qquad \text{with} \qquad
\DuOutKappa \cap \DBoomerangTildeProp \neq \emptyset,
\] 
%(see \eqref{def:dominiBoomerang}, \eqref{def:dominisComecocos} and \eqref{def:domainBoomerangTilde}).
%
and then, Corollary
\ref{corollary:changevOut} and Proposition \ref{proposition:existenceComecocos} 
%
imply the statements of  Theorem~\ref{theorem:existence} referring to  the unstable manifold $\zuOut$.




==> Article Outer/outerGraph.tex <==

The Hamiltonian $H$ written in separatrix coordinates 
(see~\eqref{def:changeEqui} and \eqref{def:changeOuter}) becomes
%with respect to the symplectic form ${d u \wedge d w} + i \h {d\xp \wedge d\yp}$ with Hamiltonian
\begin{equation}\label{def:hamiltonianOuter}
	H^{\out} =  H^{\out}_0 +  H^{\out}_1,
\end{equation}
with 
\begin{equation}\label{def:hamiltonianOuterSplit}
	\begin{split}
		H^{\out}_0 = 	w  + \frac{xy}{\de^2}, \qquad
		%
		H^{\out}_1 =
		{H} \circ \paren{\phi_{\equi} \circ \phi_{\out}} -H^{\out}_0.
	\end{split}
\end{equation}
%After all these consideration it seems a good strategy to 
%
%To obtain $\zuOut$ and $\zsOut$ in \eqref{eq:invariantManifoldsExpression} we consider the equation given by Hamiltonian $H^{\out}$ on~\eqref{def:hamiltonianOuter}.
%
%
Introducing the notation $z=(w,x,y)^T$ and defining
\begin{equation}\label{def:matrixAAAOuter}
	\AAA^{\out}= \frac{i}{\de^2} \begin{pmatrix}
		0 & 0 & 0 \\
		0 & 1 & 0 \\
		0 & 0 & -1
	\end{pmatrix},
\end{equation}
the equations associated to the Hamiltonian $H^{\out}$ can be written as
\begin{align}\label{eq:systemEDOsOuter}
	\left\{ \begin{array}{l}
		\dot{u} = 1 + g^{\out}(u,z),\\
		\dot{z} = \AAA^{\out} z + f^{\out}(u,z),
	\end{array} \right.
\end{align}
where $g^{\out} = \partial_w H_1^{\out}$  and $f^{\out}=\paren{-\partial_u 
H_1^{\out}, i\partial_y H_1^{\out}, -i\partial_x H_1^{\out} }^T$. Consequently, 
the parameterizations~$\zuOut(u)$ and $\zsOut(u)$ given in 
\eqref{eq:invariantManifoldsExpression} satisfy the invariance equation
\begin{equation}\label{eq:invariantEquationOuter}
	\partial_u \zdOut = 
	\AAA^{\out} \zdOut + \RRR^{\out}[\zdOut], \hh
	\text{ for } \diamond=\unstable,\stable,
\end{equation}
with
\begin{equation}\label{def:operatorRRROuter}
	\RRR^{\out}[\varphi](u)= 
	\frac{f^{\out}(u,\varphi)- g^{\out}(u,\varphi) \AAA^{\out} \varphi }{1+g^{\out}(u,\varphi)}.
\end{equation}

%Since $\zdOut(u)$ parameterize the stable and unstable manifolds in \eqref{eq:invariantManifoldsExpression}, we look for solutions satisfying  the asymptotic conditions 
%\begin{equation}\label{eq:asymptoticConditionsOuter}
%	\begin{split}
%		\lim_{\Re u \to -\infty} \left(\frac{\wuOut(u)}{\La_h(u)},\xuOut(u), \yuOut(u) \right) = %0, \hh
%		\lim_{\Re u \to +\infty} \left(\frac{\wsOut(u)}{\La_h(u)},\xsOut(u), \ysOut(u) \right) = 0.
%	\end{split}
%\end{equation}
%However, these asymptotic conditions do not have any meaning in the domain $\DBoomerang$, since it is bounded.
%
%To prove the existence of $\zuOut$ and $\zsOut$ in $\DBoomerang$ one has to start with different domains where these asymptotic conditions make sense and then find a way to extend  them analytically to $\DBoomerang$.
\begin{remark}\label{remark:derivadaH1w}
Note that one can use this invariance equation whenever 
\[
 1+g^{\out}(u,\varphi)=1+ \partial_w H_1^{\out}(u,\varphi)\neq 0
\]
This condition is satisfied in the different domains that are considered in this section and in the forthcoming ones and it is checked in Appendix \ref{appendix:proofH-technical}  (see \eqref{proof:boundsInftyg} and  \eqref{def:Fitag}). 
% As a consequence of the previous corollary, there exists a constant $C$ independent of $\de$, such that $\zuOut, \zsOut$ (and actually any $z$ with the estimates in Corollary \ref{corollary:changevOut}) satisfy
% \begin{equation}
% 	\vabs{\partial_w H_1^{\out}(u,\zdOut(u))}
% 	\leq C \de^2,
% 	\qquad \text{for } 
% 	u \in \DBoomerangTilde,
% 	\quad
% 	\diamond=\unstable,\stable.
% \end{equation}
This fact is also used later in Section \ref{section:differenceInner}.
\end{remark}


The first step is to look for solutions of this 
equation in the  domains
\begin{equation}\label{def:dominisInfty}
\begin{split}
\DuInfty = \claus{u \in \complexs \st \Re u < -\rhoInfty}, \qquad
\DsInfty = \claus{u \in \complexs \st \Re u > \rhoInfty},
\end{split}
\end{equation}
for some $\rhoInfty>0$, which allows us to take into account the asymptotic 
conditions \eqref{eq:asymptoticConditionsOuter}. 
%
%
% The following proposition proves the existence of $\zuOut$ and $\zsOut$ in these domains.
%

\begin{proposition}\label{proposition:existenceInfty}
%
Fix $\rhoInfty>0$.
%
Then, there exists $\de_0>0$ such that, for $\de \in (0,\de_0)$,
%
the equation~\eqref{eq:invariantEquationOuter} has a unique real-analytic 
solution $\zdOut =(\wdOut,\xdOut,\ydOut)^T$ in  $\DdInfty$ 
(for $\diamond=\unstable, \stable$)
satisfying the corresponding asymptotic condition \eqref{eq:asymptoticConditionsOuter}.

Moreover, there exists  $\cttOuterB>0$ independent of $\de$ such that, for $u 
\in \DdInfty$, 
\begin{align*}%\label{eq:boundsInfinite}
	|\wdOut(u) e^{-2\vap u}| \leq \cttOuterB\de^2, 
	\qquad
	|\xdOut(u) e^{-\vap u}| \leq \cttOuterB\de^3, 
	\qquad
	|\ydOut(u) e^{-\vap u}| \leq \cttOuterB\de^3.
%	\qquad \vap=\textstyle \sqrt{\frac{21}{8}}.
\end{align*}
with $\nu=\sqrt{\frac{21}{8}}$ for $\diamond=\unstable$ and
$\nu=-\sqrt{\frac{21}{8}}$ for $\diamond=\stable$.
\end{proposition}	

This proposition is proved in Section \ref{subsection:proofH-existenceInfinite}.

To extend analytically the invariant manifolds to reach the boomerang domain $\DBoomerang$ we have to face the problem that these parameterizations become undefined at $u=0$. 
%
To overcome it, first we extend the solutions $\zuOut$ and $\zsOut$ of 
Proposition~\ref{proposition:existenceInfty} to the \emph{outer domains} (see 
Figure~\ref{fig:dominisComecocos})
\begin{equation}\label{def:dominisComecocos}
\begin{split}
\DuOut = \left\{ u \in \complexs \right. \st  
&\vabs{\Im u} < A - \kappa \de^2 - \tan \betaOutA \Re u,
\\
&\vabs{\Im u} > \dOuter A + \tan \betaOutB \Re u  , \left. \,
%
{\Re u} > - \rhoOuter \right\}, \\
%
\DsOut = \big\{u \in \complexs \st & %\right. & \left. 
-u \in \DuOut\big\},
\end{split}
\end{equation}
where
$d_1 \in (\frac{1}{4},\frac{1}{2})$ and $\rhoOuter>\rhoInfty$
are fixed independent of $\de$,
%
and  $\kappa>0$ is such that $A-\kappa \de^2>0$.
%
%Moreover, we define $u_1, \conj{u_1}$, the vertices of the domain $\DuOut$ (see Figure~\ref{fig:dominisComecocos}).
%%\begin{equation}\label{def:vertexsDomainComecocos}
%%	u_1 = -\rhoB + i(A-\kappa \de^2) -i\rhoB\tan \beta_0.
%%\end{equation}

\begin{figure}
\centering
\begin{overpic}[scale=0.7]{dominisComecocos.png}
	\put(10,24){$\DuOut$}
	\put(77,24){$\DsOut$}
	\put(3,-2){\footnotesize $\DuInftyRho$}
	\put(90,-2){\footnotesize $\DsInftyRho$}
	\put(87,18){\footnotesize $\rhoInfty$}
	\put(94,18){\footnotesize $\rhoOuter$}
	\put(59,20.3){\footnotesize $\betaOutA$}
	\put(72.5,20.3){\footnotesize $\betaOutB$}
	\put(72,31){\footnotesize $iA$}
	\put(25,29.2){\footnotesize $iA - \kappa \de^2$}
	\put(25,21){\footnotesize $d_1 A$}
	\put(69,7){\footnotesize $-iA$}
	\put(-1.5,0){\footnotesize $\conj{u_1}$}
	\put(-1.5,39){\footnotesize $u_1$}
	\put(100,19){\footnotesize $\Re u$}
	\put(21,40){\footnotesize $\Im u$}
	\put(73,40){\footnotesize $\Im u$}
\end{overpic}
\bigskip
\caption{The outer domains $\DuOut$ and $\DsOut$ defined in~\eqref{def:dominisComecocos}} 
%and $\DuInftyR{0}$ and $\DsInftyR{0}$, given in~\eqref{def:dominisInfty}.}
\label{fig:dominisComecocos}
\end{figure}

\begin{proposition}\label{proposition:existenceComecocos}
Consider the functions $\zuOut$, $\zsOut$ and the constant $\rhoInfty>0$ 
obtained in Proposition~\ref{proposition:existenceInfty}.
%
Fix constants $\rhoOuter>\rhoInfty$ and $\dOuter \in (\frac{1}{4},\frac{1}{2})$.
%
%$\kappaOuter>0$ big enough and $\de_0>0$ small enough. 
%
Then, there exist $\de_0,\kappaOuter>0$
%
such that, for $\de \in (0,\de_0)$,
$\kappa\geq\kappaOuter$,
%
the functions $\zdOut=(\wdOut,\xdOut,\ydOut)^T$, 
$\diamond=\unstable, \stable$, can be extended analytically to 
the domain $\DdOut$

Moreover, there exists  $\cttOuterC>0$ independent of $\de$ and $\kappa$ such 
that, for $u \in \DdOut$,
\begin{align*}%\label{eq:boundsOuter}
|\wdOut(u)| \leq \frac{\cttOuterC\de^2}
{\vabs{u^2 + A^2}}
+ \frac{\cttOuterC\de^4}{\vabs{u^2 + A^2}^{\frac{8}{3}}}, \quad
%
|\xdOut(u)| \leq \frac{\cttOuterC\de^3}
{\vabs{u^2 + A^2}^{\frac{4}{3}}}, \quad
%
|\ydOut(u)| \leq \frac{\cttOuterC\de^3}
{\vabs{u^2 + A^2}^{\frac{4}{3}}}.
\end{align*}
\end{proposition}	

This proposition is proved in Section \ref{subsection:proofH-existenceBounded}.

Notice that taking $\rhoOuter$ big enough, $\dOuter\leq \dBoomerang$ and $\kappaOuter\leq\kappaBoomerang$ we have $\DBoomerangKappa \subset \DsOutKappa$.
%
Therefore, for the stable manifold $\zsOut$,  Proposition~\ref{proposition:existenceComecocos} implies Theorem~\ref{theorem:existence}.
%
However, we still need to extend further $\zuOut$ in order to reach $\DBoomerangKappa$.

%
%Therefore, we look for solutions satisfying  the asymptotic conditions 
%\begin{equation}\label{eq:asymptoticConditionsOuter}
%\begin{split}
%\lim_{\Re(u) \to -\infty} \left(\frac{\wuOut(u)}{\La_h(u)},\xuOut(u), \yuOut(u) \right) = %0, \hh
%\lim_{\Re(u) \to +\infty} \left(\frac{\wsOut(u)}{\La_h(u)},\xsOut(u), \ysOut(u) \right) = 0.
%\end{split}
%\end{equation}
%
%Notice that, by Proposition~\ref{proposition:domainSeparatrix}, the invariant manifolds can not be written as a graph globally, as the change of variables $\phi_{\out}$ is not defined for  $u= 0$.

%The difference $\dzOut=\zuOut-\zsOut$ is exponentially small in $\de$. 
%
%To obtain an asymptotic formula for $\dzOut=\zuOut-\zsOut$, we need to analyze $\zuOut$ and $\zsOut$ in a suitable domain of the complex plane. 
%
%These domains must contain a segment of the real line and must intersect a neighborhood sufficiently close to the singularities $\pm iA$ of $(\la_h(u),\La_h(u))$, see~\cite{BFGS12}. 


==> Article Outer/proofF-Difference.tex <==

%In this section we prove Theorem \ref{theorem:difference}.
%
%Along this section, we denote the components of all the functions and operators by a numerical sub-index $f=(f_1,f_2)$, unless stated otherwise, and we denote by $C$ any positive constant independent of $\de$ and $\kappa$.

% \subsubsection{An integral equation for $\dzHatU$}
\subsubsection{End of the proof of Theorem \ref{theorem:mainTheoremPoincare}}
We look for $\dzHatU$ as the unique solution of an integral equation.
% give an expression for the remainder $\dzHatU=\dzHat-\dzHatO$.
%In other words, we prove suitable estimates for $\dzHatU=\dzHat-\dzHatO$, with $\dzHatO$ as given in \eqref{def:dzHatO} and $\dzHat=(\dxOut, \dyOut)$ (see \eqref{def:dzOut}).
%
Since $\dzHat$ satisfies~\eqref{eq:invariantEquationDifference3}, by the variations of constants formula
%
\begin{align}\label{eq:dzOutDiff}
	\dzHat(u) = 
	\begin{pmatrix}
		c_x m_x(u)\\
		c_y m_y(u)
	\end{pmatrix}
	+
	\begin{pmatrix}
		\displaystyle m_x(u)
		\int_{u_-}^{u} m_x^{-1}(s) \,
		\pi_1 \paren{{\BB}^{\spl}(s) \dzHat(s)} ds \\
		\displaystyle m_y(u) 
		\int_{u_+}^{u} m_y^{-1}(s) \, 
		\pi_2 \paren{{\BB}^{\spl}(s) \dzHat(s)} ds
	\end{pmatrix},
\end{align}
where $\MM(u)$ is the fundamental matrix \eqref{def:fundamentalMatrixDifference}, $s$ belongs to some integration path in $\DBoomerang$ and $c_x$ and $c_y$ are defined as
\begin{align}\label{def:cxcyDifference}
c_x = \dxOut(u_-) m_x^{-1}(u_-), \qquad
c_y = \dyOut(u_+) m_y^{-1}(u_+).
\end{align}
%with $m_x, m_y$ given  in~\eqref{def:mxmyalxaly} and ${\BB}^{\spl}$ in~\eqref{def:operatorsDifferenceAABB}. 
For $k_1, k_2 \in \complexs$, we define 
\begin{equation}\label{def:operatorIIdiff}
\II[k_1,k_2](u) =
\big(k_1 \, m_x(u), k_2 \, m_y(u)\big)^T,
%\II[k_1,k_2](u) = \begin{pmatrix}
%	k_1 \h m_x(u)\\
%	k_2 \h m_y(u)
%\end{pmatrix} ,
\end{equation}
and the operator
\begin{align}\label{def:operatorEEdiff}
	\EE[\phiA](u) = 
%	\begin{pmatrix}
%		\displaystyle
%		\EE_1[\phiA] \\[0.5em]
%		\EE_2[\phiA]
%	\end{pmatrix}	=
	\begin{pmatrix}
		\displaystyle
		m_x(u) \int_{u_-}^{u} m_x^{-1}(s) \,
		\pi_1 \paren{{\BB}^{\spl}(s) \phiA(s)} ds \\
		\displaystyle
		m_y(u) \int_{u_+}^{u} m_y^{-1}(s) \,
		\pi_2 \paren{{\BB}^{\spl}(s) \phiA(s)} ds
	\end{pmatrix}.
\end{align}
Then, with this notation, $\dzHatO = \II[c_x^0,c_y^0]$ (see \eqref{def:dzHatO}) and equation~\eqref{eq:dzOutDiff} is equivalent to $\dzHat = \II[c_x,c_y]+\EE[\dzHat]$. 
%
Since $\EE$ is a linear operator, $\dzHatU = 
\dzHat-\dzHatO$ satisfies
\begin{equation}\label{eq:dzOutU}
	\dzHatU(u) = 
	\II[c_x-c_x^0, c_y-c_y^0](u) + 
	\EE[\dzHatO](u) + \EE[\dzHatU](u).
\end{equation}

To obtain estimates for $\dzHatU$, we first prove that $\Id-\EE$ is invertible in the Banach space $\XSplTotal= \XSpl \times \XSpl$, with 
%
% We consider 
\begin{align*}
	\XSpl = \left\{ \phiA: \DBoomerang \to \complexs \st \normSpl{\phiA}
	= \sup_{u\in \DBoomerang} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}} 
	\phiA(u)}
	<+\infty \right\},
\end{align*}
% with $d \in \paren{\frac14,\frac12}$ fixed independent of $\de$,
% and the product space  
endowed with the norm
\begin{align}\label{def:normexp}
	\normSplTotal{\phiA} = 
	\normSpl{\phiA_1} + \normSpl{\phiA_2},
\end{align}
for $\phiA=(\phiA_1,\phiA_2)$.
%
Therefore, to prove Theorem \ref{theorem:mainTheoremPoincare} it is enough to see that $\dzHatU$  satisfies that $\normSplTotal{\dzHatU} \leq C\de^{\frac13}\vabs{\log \de}^{-1}$.
%\subsubsection{The inverse operator}

First, we state a lemma  whose proof is postponed to Appendix \ref{subappendix:proofH-technicalFirst}.

\begin{lemma}\label{lemma:boundsBspl}
%
Let $\kappaBoomerang, \de_0$ be the constants given in Theorem \ref{theorem:existence}.
%	
Then, there exists a constant $C>0$ such that, for $\kappa\geq\kappaBoomerang$, $\de \in(0,\de_0)$ and  $u \in \DBoomerang$, 
%
the function $\Ups$ in \eqref{def:operatorPPdifference}, 
the matrix $\BB^{\spl}$ in \eqref{def:operatorsDifferenceAABB} and the functions $\bb_x$, $\bb_y$ in \eqref{def:mxmyalxaly} satisfy
% 
for $\kappa\geq\kappaBoomerang$, $\de \in(0,\de_0)$ and $u \in \DBoomerang$,
%
\begin{align}%\label{proof:boundsPPdifference}
	&\vabs{\Ups_1(u)-1}\leq \frac{C}{\kappa^2}, \qquad
	\vabs{\Ups_2(u)}\leq  \frac{C\de}{\vabs{u^2+A^2}^{\frac{4}{3}}}, \qquad
	\vabs{\Ups_3(u)}\leq  \frac{C\de}{\vabs{u^2+A^2}^{\frac{4}{3}}}, \label{proof:boundsUpsilon}
	 %\qquad	\text{for } j=2,3.
	\\[0.4em]
{C}^{-1} &\leq \vabs{\bb_*(u)} \leq C, 
\quad *=x,y, 
\quad \text{and} \quad
|{\BB}^{\spl}_{i,j}(u)| \leq 
\frac{C \, \de^2}{\vabs{u^2 + A^2}^{2}}, 
\quad i,j \in \claus{1,2}. \nonumber
\end{align}
\end{lemma}


%On the following results, we consider $\kappa=\kappa_0 \log(1/\de)$, with $0<\kappa_0<\frac{2}{3}(1-\g)$, as specified in Proposition~\ref{proposition:difference}. 
%

%\begin{lemma}\label{lemma:operatorII}
%Consider the operator $\II$ in \eqref{def:operatorIIdiff}
%and $c_1, c_2 \in \complexs$. 
%%
%Then, for $\de>0$ small enough and $\kappa>0$ big enough, $\II[c_1,c_2] \in \XSplTotal$.
%
%Moreover, there exists a constant $C$ independent of $c_1$, $c_2$ and $\de$ such that 
%\begin{align*}
%\normSplTotal{\II[c_1,c_2]} \leq C
%\paren{\vabs{c_1} + \vabs{c_2}}
%e^{\frac{A}{\de^2}}.
%\end{align*}
%\end{lemma}
%
%\begin{proof}
%By the definition of operator $\II$, we have that
%\begin{align*}
%	\normSplTotal{\II[c_1,c_2]} = \vabs{c_1}\normSpl{m_x} + \vabs{c_2}\normSpl{m_y}.
%\end{align*}
%where $m_x$ and $m_y$ are given in \eqref{def:mxmyalxaly}.
%%
%Then, by Lemma \ref{lemma:boundsBspl},
%\begin{align*}
%	\normSpl{m_y} &= 
%	%
%	%\sup_{u \in E_{\kappa,d}(u_0)} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}}
%		%	e^{-\frac{i}{\de^2}u} \al_y(u) } 
%		%
%		e^{\frac{A}{\de^2}} 
%		\sup_{u \in \DBoomerang} 
%		\boxClaus{e^{\frac{\Im u-\vabs{\Im u}}{\de^2}}  \vabs{\beta_y(u)}}
%		%
%		\leq C e^{\frac{A}{\de^2}}.
%\end{align*}
%An analogous estimate holds for  $\normSpl{m_x}$.
%\end{proof}

%\begin{proof}
%By the definition of operator $\II$ in~\eqref{def:operatorIIdiff} we have that
%\begin{align*}
%\normSplTotal{\II[k_1,k_2]} = \vabs{k_1}\normSpl{m_x} + \vabs{k_2}\normSpl{m_y}.
%\end{align*}
%We prove the expression just for $\normSpl{m_y}$, the other case is analogous.
%\begin{align*}
%\normSpl{m_y} &= 
%%
%\sup_{u \in E} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}}
%e^{-\frac{i}{\de^2}u} \al_y(u) } 
%%
%= e^{\frac{A}{\de^2}} \sup_{u \in E} 
%\claus{e^{\frac{\Im u-\vabs{\Im u}}{\de^2}}  \vabs{\al_y(u)}	}
%%
%\leq e^{\frac{A}{\de^2}} \sup_{u\in E} \vabs{\al_y(u)}.
%\end{align*}
%Then, by~\eqref{eq:alxalyEstimates} $\al_y$ is bounded, thus have that $\normSpl{m_y} \leq C e^{\frac{A}{\de^2}}$, as we needed to prove.
%\end{proof}

%\begin{lemma}
%We have
%	\begin{align*}
%	\vabs{c_x - c_x^0}, \vabs{c_y - c_y^0} \leq 
%	\frac{C \de^{\frac{1}{3}}}{\log(1/\de)}.
%	\end{align*}
%\end{lemma}

In the next lemma we obtain estimates for the linear operator $\EE$ (see \eqref{def:operatorEEdiff}).

\begin{lemma}\label{lemma:operatorEEdiff}
% Consider the operator $\EE$ as defined in \eqref{def:operatorEEdiff} and
%
Let $\kappaBoomerang, \de_0$ be the constants as given in Theorem \ref{theorem:existence}.
%
There exists $\cttDiffA>0$ such that for $\de\in(0,\de_0)$ and 
$\kappa\geq \kappaBoomerang$,
the operator $\EE: \XSplTotal \to \XSplTotal$ in \eqref{def:operatorEEdiff}  is well defined and satisfies that, for $\phiA \in \XSplTotal$,
\begin{align*}
\normSplTotal{\EE[\phiA]} \leq \frac{\cttDiffA}{\kappa} 
\normSplTotal{\phiA}.
\end{align*}
In particular, $\Id - \EE$ is invertible and 
\begin{align*}
\normSplTotal{(\Id - \EE)^{-1}[\phiA]} \leq 2\normSplTotal{\phiA}.
\end{align*}

\end{lemma}

\begin{proof}
Let us consider $\EE=(\EE_1,\EE_2)^T$, $\phiA \in \XSplTotal$ and $u \in \DBoomerang$.
%
We only prove the estimate for $\EE_2[\phiA](u)$.
%
The corresponding one for $\EE_1[\phiA](u)$ follows analogously.

By the definition of $m_y$ in~\eqref{def:mxmyalxaly} and Lemma \ref{lemma:boundsBspl}, we have that
\begin{align*}
\vabs{\EE_2[\phiA](u)} 
%&= \vabs{m_y(u) (u-u_+) \int_{0}^{1} m_y^{-1}(\rho_t) 
%	\pi_2 \paren{{\BB}^{\spl}(\rho_t) \phiA(\rho_t)} dt} \\
%
&\leq
C \de^2 e^{\frac{\Im u}{\de^2}} 
\vabs{\int_{u_+}^{u} 
e^{-\frac{\Im s}{\de^2}} 
\frac{
\vabs{\phiA_1(s)}+\vabs{\phiA_2(s)}
}{\vabs{s^2+A^2}^2} d s } 
\\
&\leq
C \de^2 e^{\frac{\Im u - A}{\de^2}} 
\normSplTotal{\phiA}
\vabs{\int_{u_+}^{u} 
e^{\frac{\vabs{\Im s}-\Im s}{\de^2}} 
\frac{d s}{\vabs{s^2+A^2}^2}}.
\end{align*}
%Since $\phiA \in \XSplTotal$, we have that
%$
%\vabs{\phiA_1(u)} + \vabs{\phiA_2(u)} \leq
%e^{-\frac{A-\vabs{\Im u}}{\de^2}}\normSplTotal{\phiA}.
%$
%
Let us consider the case $\Im u < 0$. Then, for a fixed $u_0 \in \reals \cap \DBoomerang$, we define the integration path $\rho_t \subset \DBoomerang$ as
\begin{align*}
	\rho_t =	
	\begin{cases}
		u_+ + 2t(u_0-u_+)
		&\quad \text{for } t \in (0,\frac12), \\
		%		
		u_0 + (2t-1)(u-u_0)
		&\quad \text{for }  t \in [\frac12,1).
	\end{cases}	
\end{align*}
%
%
Then,
\begin{align*}%\label{proof:equationGGGmch}
\vabs{\EE_2[\phiA](u)} 
%&\leq
%C \de^2  e^{\frac{\Im u-A}{\de^2}} \vabs{u-u_+ }
%\normSplTotal{\phiA}
% \vabs{\int_{0}^{1}  
%e^{\frac{\vabs{\Im \rho_t}-\Im \rho_t}{\de^2}} \frac{dt}{\vabs{\rho_t^2+A^2}^2} } \\
%
&\leq 
C \de^2  e^{-\frac{\vabs{\Im u}+A}{\de^2}} 
\normSplTotal{\phiA}
\vabs{\int_{0}^{\frac12} \frac{dt}{\vabs{\rho_t-iA}^2}
+ \int_{\frac12}^{1} 
\frac{e^{\frac{2\vabs{\Im \rho_t}}{\de^2}}}{\vabs{\rho_t+iA}^2} dt}  
%
%&= C \de^2  e^{\frac{\vabs{\Im u}-A}{\de^2}}
%\normSplTotal{\phiA}
%\boxClaus{
%	\frac{1}{\vabs{u_+-iA}} - 
%	\frac{1}{\vabs{u-iA}}}
%
\leq \frac{C}{\kappa} 
e^{\frac{\vabs{\Im u}-A}{\de^2}}
\normSplTotal{\phiA}.
\end{align*}
%
If $\Im u \geq 0$, we consider the integration path $\rho_t = u_+ + t(u-u_+)$ for $t\in[0,1]$ and we obtain
\begin{align*}
\vabs{\EE_2[\phiA](u)} &\leq 
C \de^2  e^{\frac{\vabs{\Im u}-A}{\de^2}} 
\normSplTotal{\phiA}
\vabs{\int_{0}^{1} \frac{\vabs{u-u_+}}{\vabs{\rho_t-iA}^2} dt} 
%
%&= C \de^2  e^{\frac{\vabs{\Im u}-A}{\de^2}}
%\normSplTotal{\phiA}
%\boxClaus{
%\frac{1}{\vabs{u_+-iA}} - \frac{1}{\vabs{u-iA}}}
%%
\leq \frac{C}{\kappa} 
e^{\frac{\vabs{\Im u}-A}{\de^2}}
\normSplTotal{\phiA}.
\end{align*}
Therefore,
$
\normSpl{\EE_2[\phiA]} \leq \frac{C}{\kappa}\normSplTotal{\phiA}.
$
\end{proof}

Notice that, by  \eqref{eq:dzOutU}, $\dzHatU$ satisfies
\begin{equation}\label{eq:dzOutUInverse}
(\Id - \EE )\dzHatU(u) = \II[c_x-c_x^0, c_y-c_y^0](u) + \EE[\dzHatO](u).
\end{equation}
Since, by Lemma \ref{lemma:operatorEEdiff}, $\Id-\EE$ is invertible in $\XSplTotal$ we have an explicit formula for $\dzHatU$.
%
Nevertheless, we still need good estimates for  the right hand side with respect to the norm \eqref{def:normexp}.



%
%As a result, by \eqref{eq:dzOutU}, $\dzHatU$ satisfies
%\begin{equation}\label{eq:dzOutUInverse}
%\dzHatU(u) = (\Id - \EE )^{-1}\paren{\II[c_x-c_x^0, c_y-c_y^0](u) + \EE[\dzHatO](u)}.
%\end{equation}


% \subsubsection{End of the proof of Theorem \ref{theorem:mainTheoremPoincare}}
% 
% In this section we finish the prove of Theorem \ref{theorem:mainTheoremPoincare} by obtaining suitable estimates for $\dzHatU$ by means of  equation \eqref{eq:dzOutUInverse}.

%In this section we prove Theorem \ref{theorem:differenceBanach} and finish the prove of Theorem \ref{theorem:difference}.

\begin{lemma}\label{lemma:IconstantsDiff}
%
There exist $\kappa_*, \de_0, \cttDiffB>0$ such that, for
$\kappa=\kappa_*\vabs{\log \de}$ and $\de\in(0,\de_0)$, 
%
% there exists constant $>0$ independent of $\de$ such that
\begin{align*}
\normSplTotal{\II[c_x-c_x^0,c_y-c_y^0]}
\leq \frac{\cttDiffB \, \de^{\frac{1}{3}}}{\vabs{\log \de}}\qquad \text{and}\qquad
\normSplTotal{\EE[\dzHatO](u)}\leq \frac{\cttDiffB \, \de^{\frac{1}{3}}}{\vabs{\log \de}},
\end{align*}
%\begin{align*}
%\vabs{c_x-c_x^0}
%\leq \frac{\cttDiffB \, \de^{\frac{1}{3}}}{\vabs{\log \de}} e^{-\frac{A}{\de^2}},
%%\vabs{\beta_x^{-1}(u_-)}
%\qquad
%\vabs{c_y-c_y^0} 
%\leq \frac{\cttDiffB \, \de^{\frac{1}{3}}}{\vabs{\log \de}} 
%e^{-\frac{A}{\de^2}},
%%\vabs{\beta_y^{-1}(u_+)},
%\end{align*}
with  $\II$,  $(c_x^0,c_y^0)$, $(c_x,c_y)$, $\EE$ and $\dzHatO$ defined  in \eqref{def:operatorIIdiff}, \eqref{def:dzHatO}, \eqref{def:cxcyDifference}, \eqref{def:operatorEEdiff}
and
\eqref{def:dzHatO:0}, respectively.

\end{lemma}

\begin{proof}
By the definition of the function $\II$,
\[
\normSplTotal{\II[c_x-c_x^0,c_y-c_y^0]} = \vabs{c_x-c_x^0}\normSpl{m_x} + \vabs{c_y-c_y^0}\normSpl{m_y},
\]
where $m_x$ and $m_y$ are given in \eqref{def:mxmyalxaly}.
%
Then, by Lemma \ref{lemma:boundsBspl},
\begin{align*}
	\normSpl{m_x} = 
	e^{\frac{A}{\de^2}} 
	\sup_{u \in \DBoomerang} 
	\boxClaus{e^{-\frac{\Im u+\vabs{\Im u}}{\de^2}}  \vabs{\bb_x(u)}}
	%
	\leq C e^{\frac{A}{\de^2}},
	\qquad
	\normSpl{m_y} \leq 
	%
	%\sup_{u \in E_{\kappa,d}(u_0)} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}}
	%	e^{-\frac{i}{\de^2}u} \al_y(u) } 
	%
	%e^{\frac{A}{\de^2}} 
	%\sup_{u \in \DBoomerang} 
	%\boxClaus{e^{\frac{\Im u-\vabs{\Im u}}{\de^2}}  \vabs{\beta_y(u)}}
	%
	C e^{\frac{A}{\de^2}},
\end{align*}
and, as a result,
\begin{equation}\label{proof:operatorIIdiff}
\normSplTotal{\II[c_x-c_x^0,c_y-c_y^0]} \leq
C e^{\frac{A}{\de^2}}
\paren{|c_x-c_x^0| + |c_y-c_y^0|}.
\end{equation}
We now obtain an estimate for $|c_y-c_y^0|$.
%
The estimate for $|c_x-c_x^0|$ follows analogously.

By the definition of $m_y$ (see \eqref{def:mxmyalxaly}), one has
\begin{equation}\label{proof:cyMenyscyO}
\begin{split}	
	\vabs{c_y - c_y^0} 
%	&= \vabs{m^{-1}_y(u_+)}
%	\vabs{\dyOut(u_+) - \dyOutO(u_+)} \\
	&= 	e^{-\frac{A}{\de^2}+\kappa} 
	\vabs{\bb_y^{-1}(u_+)}
	\vabs{\dyOut(u_+) - \dyOutO(u_+)}.
\end{split}
\end{equation}
%
%An analogous result holds for $\vabs{c_x-c_x^0}$.
%%
%Therefore, by Lemma \ref{lemma:boundsBspl},
%\begin{equation}\label{proof:eqOperatorII}
%	\normSplTotal{\II[c_x-c_x^0, c_y-c_y^0]} \leq
%	C e^{\kappa} \Big(
%	\vabs{\dxOut(u_-) - \dxOutO(u_-)} +
%	\vabs{\dyOut(u_+) - \dyOutO(u_+)}
%	\Big).
%\end{equation}
%
%We study first the component $\vabs{\dyOut(u_+) - \dyOutO(u_+)}$.
%
Let us denote $\DYInnC = \YuMchO -\YsMchO$ where $\YusMchO$ are given on~\eqref{def:ZdMchO}. 
%
Recall that $\YusMchO=\YusInn + \YusMchU$ where $\YusInn$ is the third component of $\ZusInn$, the solutions of the inner equation (see Theorems \ref{theorem:innerComputations} and \ref{theorem:matching}).
%
We write,
\begin{align*}
\dyOut(u_+) &= \sqrt{2} \al_+ \de^{\frac{1}{3}} 
\DYInnC\paren{\frac{u_+ - iA}{\de^2}} 
%= \sqrt{2} \al_+ \de^{\frac{1}{3}} 
%\DYInnC\paren{-i\kappa} 
%\\
=\sqrt{2} \al_+ \de^{\frac{1}{3}} \left[
\DYInn \paren{-i\kappa} +
\YuMchU \paren{-i\kappa} - \YsMchU \paren{-i\kappa}
\right].
\end{align*}
%
%Recall that $\YusMchO=\YusInn + \YusMchU$ (see \ref{def:ZMchU}) and
%$\DYInn = \YuInn-\YsInn$ (see \eqref{result:innerDifference}).
%%
%Then
%\begin{equation*}\label{proof:operatorIIa}
%	\dyOut(u_+) = 
%	\sqrt{2} \al_+ \de^{\frac{1}{3}} \left[
%	\DYInn \paren{-i\kappa} +
%	\YuMchU \paren{-i\kappa} - \YsMchU \paren{-i\kappa}
%	\right].
%\end{equation*}
%
By the definition of $\dyOutO$ in \eqref{def:dzHatO:0} (see also \eqref{def:dzHatO}), we have
$
	\dyOutO(u_+) = \sqrt{2}\al_+ \de^{\frac{1}{3}}
	\CInn e^{-\kappa} .
$
%
Then, by  \eqref{proof:cyMenyscyO} and Lemma~\ref{lemma:boundsBspl},
\begin{align*}
	\vabs{c_y-c_y^0} \leq
	C \de^{\frac{1}{3}} e^{-\frac{A}{\de^2}+\kappa} 
	\Big[
	\vabs{\DYInn \paren{-i\kappa} - \CInn e^{-\kappa}}
	+ 
	%\sqrt{2} \vabs{\al_+} \de^{\frac{1}{3}} 
	\vabs{\YuMchU \paren{-i\kappa}} + 
	\vabs{\YsMchU \paren{-i\kappa}}
	\Big],
\end{align*}
%
and, applying Theorems~\ref{theorem:innerComputations} and
\ref{theorem:matching}, we obtain
\begin{equation*}%\label{proof:estimatesII}
\begin{split}	
\vabs{c_y-c_y^0}
&\leq
C \de^{\frac{1}{3}} 
e^{-\frac{A}{\de^2}+\kappa} 
\boxClaus{
\vabs{\chi_3(-i\kappa)  e^{-\kappa} }
+
\frac{C}{\kappa} \de^{\frac23(1-\g)} } 
\leq 
\frac{C}{\kappa} \de^{\frac13} e^{-\frac{A}{\de^2}} 
\paren{1 + 
\de^{\frac23(1-\g)} e^{\kappa}},
\end{split}
\end{equation*}
where $\g \in (\g^*,1)$ with $\g^*\in [\frac{3}{5},1)$ given in Theorem \ref{theorem:matching}.
%
%
%Lastly, applying the estimates in \eqref{proof:estimatesII} to equation \eqref{proof:eqOperatorII} we obtain
%\[
%\normSplTotal{\II[c_x-c_x^0, c_y-c_y^0]} \leq
%\frac{C}{\kappa} \de^{\frac13} \paren{
%	1 + e^{\kappa} \de^{\frac23(1-\g)}} .
%\]
%
Taking $\kappa=\kappa_* \vabs{\log \de}$ with $0<\kappa_*<\frac{2}{3}(1-\g)$, we obtain
\begin{equation*}%\label{proof:estimatesII}
\begin{split}	
\vabs{c_y-c_y^0}
&\leq 
\frac{C\de^{\frac13} }{\vabs{\log \de}} 
e^{-\frac{A}{\de^2}} 
%\vabs{\beta_y^{-1}(u_+)}
\paren{1 +	\de^{\frac23(1-\g)-\kappa_*}}
\leq
\frac{C \de^{\frac13} }{\vabs{\log \de}}
e^{-\frac{A}{\de^2}}.
\end{split}
\end{equation*}
%
This bound and  \eqref{proof:operatorIIdiff} prove the first estimate of the lemma.

For the second estimate, it only remains to bound  $\dzHatO$ and apply Lemma~\ref{lemma:operatorEEdiff}.
%
Indeed, by the definition of $\dzHatO$  in \eqref{def:dzHatO}, Lemma \ref{lemma:boundsBspl} and \eqref{proof:operatorIIdiff}, we have that
\begin{align*}
%\label{proof:dzOutObound}
\normSplTotal{\dzHatO} 
=
\normSplTotal{\II[c_x^0,c_y^0]} 
\leq
C e^{\frac{A}{\de^2}} \paren{\vabs{c_x^0}+\vabs{c_y^0}}
\leq
C \de^{\frac13}.
%\big(\vabs{\beta_x(u_-)} + 
%\vabs{\beta_y(u_+)} \big),
\end{align*}	
%
%and, by Lemma \ref{lemma:boundsBspl}, $\normSplTotal{\dzHatO}<+\infty$.
%	
Since $\kappa=\kappa_* \vabs{\log \de}$ with  $0<\kappa_*<\frac{2}{3}(1-\g)$,
 Lemma \ref{lemma:operatorEEdiff} implies $\normSplTotal{\EE[\dzHatO]} \leq \frac{C  \de^{\frac13}}{\vabs{\log \de}}$. 
\end{proof}

With this lemma, we can give sharp estimates for $\dzHatU$ by using equation
\eqref{eq:dzOutUInverse}. 
%
Indeed, since the right hand side of this equation belongs to  $\XSplTotal$, by Lemma \ref{lemma:operatorEEdiff},
\[
\dzHatU(u) = (\Id - \EE )^{-1}\left( \II[c_x-c_x^0, c_y-c_y^0](u) + \EE[\dzHatO](u)\right).
\]
Then, Lemmas \ref{lemma:operatorEEdiff} and \ref{lemma:IconstantsDiff}	imply
% 
% 
% \begin{proof}
% %	
% First, we check that $\dzHatO \in \XSplTotal$.
% %
% Indeed, by its definition in \eqref{def:dzHatO}, Lemmas \ref{lemma:boundsBspl} and \eqref{proof:operatorIIdiff}, we have that
% \begin{align}\label{proof:dzOutObound}
% \normSplTotal{\dzHatO} 
% =
% \normSplTotal{\II[c_x^0,c_y^0]} 
% \leq
% C e^{\frac{A}{\de^2}} \paren{\vabs{c_x^0}+\vabs{c_y^0}}
% \leq
% C \de^{\frac13}.
% %\big(\vabs{\beta_x(u_-)} + 
% %\vabs{\beta_y(u_+)} \big),
% \end{align}	
% %
% %and, by Lemma \ref{lemma:boundsBspl}, $\normSplTotal{\dzHatO}<+\infty$.
% %	
% We check that $\dzHatU \in \XSplTotal$. 
% %
% By Theorem~\ref{theorem:existence}, we have that
% \begin{align*}
% \normSplTotal{\dzHat} 
% %\sup_{u\in E_{\kappa,d}(u_0)} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}} 
% %	\paren{\xuOut-\xsOut}(u)}
% %+\sup_{u\in E_{\kappa,d}(u_0)} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}} 
% %	\paren{\yuOut-\ysOut}(u)} \\
% %
% &= \normSpl{\xuOut} + \normSpl{\xsOut}
% + \normSpl{\yuOut} + \normSpl{\ysOut} \\
% %
% &\leq \sup_{u\in\DBoomerang} \vabs{e^{\frac{A-\vabs{\Im u}}{\de^2}} 
% \frac{4 \cttOuterA \de^3}{\vabs{u^2+A^2}^{\frac43}}}
% \leq C \de^{\frac{1}{3}}e^{\frac{A}{\de^2}},
% \end{align*}
% Therefore, $\dzHatU=\dzHat-\dzHatO \in \XSplTotal$. 
% %
% Although we note that, a priori, its norm its exponentially large with respect to $\de$. 
% 
% To improve this result, we consider equation~\eqref{eq:dzOutUInverse}.
% %
% %\begin{align*}
% %(\Id - \EE )\dzHatU = \II[c_x-c_x^0, c_y-c_y^0](u) + 
% %\EE[\dzHatO](u).
% %\end{align*}
%
% Let us take
% $\kappa=\kappa_* \vabs{\log \de}$ with $\kappa_*$ as given in Lemma \ref{lemma:IconstantsDiff}.
% %
% Then, taking $\phiA \in \XSplTotal$ and $\de$ small enough, by Lemma \ref{lemma:operatorEEdiff}, 
% \begin{align*}
% \normSplTotal{\EE[\phiA]} \leq \frac{C}{\vabs{\log \de}} 
% \normSplTotal{\phiA}
% < \normSplTotal{\phiA},
% \end{align*}
% and, as a result, the operator $\Id-\EE$ is invertible in $\XSplTotal$. Then, applying \eqref{proof:dzOutObound} and Lemmas
% \ref{lemma:operatorEEdiff} and
% \ref{lemma:IconstantsDiff} to equation~\eqref{eq:dzOutUInverse} one has
\begin{align}\label{def:fitaDeltaphi1}
\normSplTotal{\dzHatU}
% &\leq 
% %
% \frac{\cttDiffB \, \de^{\frac{1}{3}}}{\vabs{\log \de}}
%  +
% \frac{\cttDiffA \normSplTotal{\dzHatO}}{\vabs{\log \de}}
% %
\leq \frac{C \de^{\frac{1}{3}}}{\vabs{\log \de}}.
%\big(\vabs{\beta_x(u_-)} + 
%\vabs{\beta_y(u_+)} \big).
\end{align}
% \end{proof}
%Then, using the bound of the matching error given in Theorem~\ref{theorem:matching} and that $\wt{\BB}^{\spl}$ is small, we prove that $\dzHatO$ is the dominant part of $\dzHat$.
%%
%Indeed, in the following Theorem we obtain estimates for
%\begin{align}\label{def:dzHatU}
%	\dzHatU = (\dxOut_1,\dyOut_1)^T = \dzHat - \dzHatO.
%\end{align}
%
%\begin{theorem}\label{theorem:difference}
%	Let constant $d \in (\frac14,\frac12)$ be as given in Theorem \ref{theorem:existence} and $\dzHatU$ in \eqref{def:dzHatU}.
%	%	
%	Then, there exists $\de_0>0$ and $\kappa_*>0$ such that,
%	%
%	for $\de \in (0,\de_0)$ and
%	$\kappa=\kappa_* \vabs{\log\de}$,
%	%
%	there exists a real constant $\cttDiff>0$ independent of $\de$ such that, 
%	%
%	for $u \in \DBoomerang$,
%	\begin{align*}
%		\vabs{\dxOut_1(u)} 
%		\leq  
%		\cttDiff \,
%		e^{\frac{\vabs{\Im u}-A}{\de^2}}
%		\frac{ \de^{\frac{1}{3}} }{\vabs{\log\de}}
%		,
%		\qquad
%		\vabs{\dyOut_1(u) } 
%		\leq  
%		\cttDiff \,
%		e^{\frac{\vabs{\Im u}-A}{\de^2}}
%		\frac{\de^{\frac{1}{3}}}{\vabs{\log\de}}.
%	\end{align*}
%\end{theorem}
%
%This theorem is proved in Section \ref{section:proofF-Difference}.
To prove Theorem \ref{theorem:mainTheoremPoincare}, it only remains to analyze  $\bb_x(u_-)$ and $\bb_y(u_+)$.

\begin{lemma}\label{lemma:boundsBonsBeta}
%
Let $\kappa_*$ be as given in Lemma \ref{lemma:IconstantsDiff}.
%
Then, there exists $\de_0>0$ such that, for $\de \in (0,\de_0)$ and $\kappa=\kappa_*\vabs{\log \de}$, the  functions $\bb_{x}, \bb_y$ defined in \eqref{def:mxmyalxaly} satisfy
	\begin{align*}
		\bb_x^{-1}(u_-) &= e^{-\frac{4i}9(\pi-\la_h(u_*))}
		\paren{1+\OO\paren{\frac1{\vabs{\log \de}}}},
		\\	
		\bb_y^{-1}(u_+) &= e^{\frac{4i}9(\pi-\la_h(u_*))}
		\paren{1+\OO\paren{\frac1{\vabs{\log \de}}}},
	\end{align*}
	where  $u_{\pm}=\pm i(A-\kappa\de^2)$.
\end{lemma}

This lemma is proven in Appendix \ref{subappendix:proofH-technicalSecond}.

% \begin{proof}[End of proof of Theorem \ref{theorem:mainTheoremPoincare}]

Let $u_* \in \DBoomerang \cap \reals$.
%
We compute the first order of $\dzHatO(u_*)=(\dxOutO(u_*),\dyOutO(u_*))^T$.
%
Since, by Theorem \ref{theorem:singularities}, $(\al_+)^3=(\al_-)^3=\frac12$, and applying Lemma \ref{lemma:boundsBonsBeta} and \eqref{def:dzHatO}, we obtain
\begin{align*}
\vabs{\D x_0(u_*)} =
\vabs{\D y_0(u_*)} =
\sqrt[6]{2}
\vabs{\CInn}
\de^{\frac13} e^{-\frac{A}{\de^2}} 
\paren{1+\OO\paren{\frac1{\vabs{\log \de}}}}.
\end{align*}
% where $\CInn$ is given in Theorem \ref{theorem:innerComputations}.
%
Moreover, by \eqref{def:fitaDeltaphi1}, 
\begin{align*}
\vabs{\D x(u_*) - \D x_0(u_*)},
\vabs{\D y(u_*) - \D y_0(u_*)} 
\leq 
 \frac{C \de^{\frac13} e^{-\frac{A}{\de^2}}}{\vabs{\log \de}}.
\end{align*}
%
Finally, notice that the section $u=u_* \in \DBoomerang \cap \reals$  translates to $\la= \la^* :=\la_h(u_*)$ (see \eqref{def:changeOuter}).
%
Moreover, since $\lad_h=-3\La_h$ (see \eqref{eq:separatrixParametrization}), one deduces that $\La_h(u)>0$ for $u>0$.
%
Therefore, by the change of coordinates \eqref{def:changeOuter}, Theorem \ref{theorem:existence} and taking $\de$ small enough,
\begin{align*}
	\La_*^{\diamond} = \La_h(u_*) - \frac{\wdOut(u_*)}{3\La_h(u_*)}
	= 
	\La_h(u_*) + \OO(\de^2) > 0,
	\qquad
	\text{with }\diamond=\unstable,\stable, 
\end{align*}
and, therefore using formula \eqref{eq:defDwOut} for $\dwOut$ and Lemma \ref{lemma:boundsBspl}, we obtain that
\[
\vabs{\La_*^{\unstable}-\La_*^{\stable}} \leq 
C \vabs{\dwOut(u_*)} 	
\leq 
C \de \vabs{\dxOut(u_*)} +
C \de \vabs{\dyOut(u_*)}
\leq 
C \de^{\frac43} e^{-\frac{A}{\de^2}}.
\]


% Notice that, $\DBoomerang \cap \reals \subset (0,+\infty)$. 
% %
% Therefore, since $\la_h(0)=\la_0$ and $\lim_{\Re u\to+\infty} \la_h(u)=0$, we see that $(\la_1,\la_2) \subset (0,\la_0)$.
% \end{proof}




==> Article Outer/proofF-differenceTechnical.tex <==

In this section we prove
Lemmas \ref{lemma:boundsBspl} and \ref{lemma:boundsBonsBeta}.

\subsection{Proof of Lemma \ref{lemma:boundsBspl}}
\label{subappendix:proofH-technicalFirst}

First, we prove the estimates for the operator $\Ups$ given in \eqref{def:operatorPPdifference}.
%
%\begin{lemma}\label{lemma:estimatesPP}
%%
%%Let the operator $\Ups$ given in \eqref{def:operatorPPdifference}.
%%
%Let the constants $\kappaBoomerang, \de_0$ be as given in Theorem \ref{theorem:existence}.
%%	
%Then, there exists a constant $C>0$ such that, for $\kappa\geq\kappaBoomerang$, $\de \in(0,\de_0)$ and $u \in \DBoomerang$,
%%
%\begin{align*}%\label{proof:boundsPPdifference}
% 	\vabs{\Ups_1(u)-1}\leq \frac{C}{\kappa^2}, \qquad
% 	\vabs{\Ups_j(u)} \leq  \frac{C\de}{\vabs{u^2+A^2}^{\frac{4}{3}}}, \qquad	\text{for } j=2,3.
%\end{align*}
% 
%\end{lemma}
%
For $\sigma \in [0,1]$, we define
$z_{\sigma}=\sigma\zuOut + (1-\sigma) \zsOut$ 
with $z_{\sigma}=(w_{\sigma},x_{\sigma},y_{\sigma})^T$.
%
%\begin{equation*}
%	z_{\tau}=\tau\zuOut + (1-\tau) \zsOut, 
%	\quad \text{with} \quad
%	z_{\tau}=(w_{\tau},x_{\tau},y_{\tau}).
%\end{equation*}
%
Then, by Theorem \ref{theorem:existence}, for $u \in \DBoomerang$, we have that
\begin{equation}\label{proof:ztauBounds}
	\vabs{w_{\sigma}(u)}\leq \frac{C\de^2}{\vabs{u^2+A^2}} +
	\frac{C\de^4}{\vabs{u^2+A^2}^{\frac83}}, \qquad
	\vabs{x_{\sigma}(u)},\vabs{y_{\sigma}(u)}\leq \frac{C\de^3}{\vabs{u^2+A^2}^{\frac43}}.
\end{equation}		
Recalling that $H^{\out} = w + \frac{xy}{\de^2} + H_1^{\out}$ (see \eqref{def:hamiltonianOuter}), one has
%
\begin{equation*}
	\begin{split}
		\vabs{\Ups_1(u)-1}& \leq
		\sup_{\sigma \in[0,1]} \vabs{\partial_w H_1^{\out}(u,z_{\sigma}(u))},\\
		\vabs{\Ups_2(u)}&\leq 
		\frac{\vabs{y_{\sigma}(u)}}{\de^2}
		+
		\sup_{\sigma \in[0,1]} \vabs{
			\partial_x H_1^{\out}(u,z_{\sigma}(u))},
		\\ 
		\vabs{\Ups_3(u)} 
		&\leq 
		\frac{\vabs{x_{\sigma}(u)}}{\de^2}
		+
		\sup_{\sigma \in[0,1]} \vabs{
			\partial_y H_1^{\out}(u,z_{\sigma}(u))}.
	\end{split}
\end{equation*}
Then, by \eqref{proof:ztauBounds} and applying 
 \eqref{def:Fitag} and \eqref{proof:estimatef2f3Out} in the proof of
Lemma \ref{lemma:computationsRRROut} we obtain the estimates for $\Ups_1, \Ups_2$ and $\Ups_3$.

% \begin{proof}[Proof of Lemma \ref{lemma:boundsBspl}]
We also need estimates for the matrix $\wt{\BB}^{\spl}$ given in \eqref{def:Bspl1}, which  satisfies 
\begin{align*}
|\wt{\BB}^{\spl}_{i,j}(u)|
\leq 
\sup_{\sigma \in[0,1]}
\vabs{\paren{D_z \RRR^{\out}
[\zOut_{\sigma}](u)}_{i,j}},
\end{align*}
for $z_{\sigma}= \sigma\zuOut + (1-\sigma) \zsOut$.
%
Then, by \eqref{proof:ztauBounds} and applying Lemma \ref{lemma:computationsRRROut}, for $u \in \DBoomerang$,
% we obtain
%\begin{align}	
%%&\vabs{\wt{\BB}^{\spl}_{1,1}(u)} \leq 
%%\frac{C \de^2}{\vabs{u^2 + A^2}^{\frac{5}{3}}} +
%%\frac{C \de^4}{\vabs{u^2 + A^2}^{3}}, \hh
%%\vabs{\wt{\BB}^{\spl}_{1,2}(u)} \leq 
%%\frac{C\de}{\vabs{u^2 + A^2}^{\frac{7}{3}}}, \hh
%%\vabs{\wt{\BB}^{\spl}_{1,3}(u)} \leq 
%%\frac{C\de}{\vabs{u^2 + A^2}^{\frac{7}{3}}}, \\
%&\vabs{\wt{\BB}^{\spl}_{2,1}(u)} \leq 
%\frac{C\de}{\vabs{u^2 + A^2}^{\frac{2}{3}}}, \,
%\vabs{\wt{\BB}^{\spl}_{2,2}(u)} \leq 
%\frac{C}{\vabs{u^2 + A^2}^{\frac{2}{3}}} +
%\frac{C \de^2}{\vabs{u^2 + A^2}^{2}}, \,
%\vabs{\wt{\BB}^{\spl}_{2,3}(u)} \leq 
%\frac{C\de^2}{\vabs{u^2 + A^2}^{2}}, \\
%&\vabs{\wt{\BB}^{\spl}_{3,1}(u)} \leq 
%\frac{C\de}{\vabs{u^2 + A^2}^{\frac{2}{3}}}, \,
%\vabs{\wt{\BB}^{\spl}_{3,2}(u)} \leq 
%\frac{C\de^2}{\vabs{u^2 + A^2}^{2}}, \,
%\vabs{\wt{\BB}^{\spl}_{3,3}(u)} \leq 
%\frac{C}{\vabs{u^2 + A^2}^{\frac{2}{3}}} +
%\frac{C \de^2}{\vabs{u^2 + A^2}^{2}}.
%\end{align}
\begin{equation} \label{proof:boundsBsplTilde}	
\begin{aligned}
\vabs{\wt{\BB}^{\spl}_{2,1}(u)} &\leq 
\frac{C\de}{\vabs{u^2 + A^2}^{\frac{2}{3}}},
& 
\vabs{\wt{\BB}^{\spl}_{3,1}(u)} &\leq 
\frac{C\de}{\vabs{u^2 + A^2}^{\frac{2}{3}}}, 
\\
\vabs{\wt{\BB}^{\spl}_{2,2}(u)} &\leq 
\frac{C}{\vabs{u^2 + A^2}^{\frac13}} +
\frac{C \de^2}{\vabs{u^2 + A^2}^{2}}, 
&
\vabs{\wt{\BB}^{\spl}_{3,2}(u)} &\leq 
\frac{C\de^2}{\vabs{u^2 + A^2}^{2}}, 
\\
\vabs{\wt{\BB}^{\spl}_{2,3}(u)} &\leq 
\frac{C\de^2}{\vabs{u^2 + A^2}^{2}}, 
&
\vabs{\wt{\BB}^{\spl}_{3,3}(u)} &\leq 
\frac{C}{\vabs{u^2 + A^2}^{\frac13}} +
\frac{C \de^2}{\vabs{u^2 + A^2}^{2}}.
\end{aligned}
\end{equation}
%
Then, by \eqref{proof:boundsUpsilon} and taking $\kappa$ big enough,
% we obtain 
\begin{align*}
	\vabs{{\BB}^{\spl}_{1,1}(u)} &\leq  
	\frac{\vabs{\Ups_2(u)}}{\vabs{\Ups_1(u)}} \vabs{\wt{\BB}^{\spl}_{2,1}(u)} 
	\leq 
	\frac{C \de^2}{\vabs{u^2 + A^2}^{2}}, \\
%%
	\vabs{{\BB}^{\spl}_{1,2}(u)} &\leq 
	\vabs{\wt{\BB}^{\spl}_{2,3}(u)} +
	\frac{\vabs{\Ups_3(u)}}{\vabs{\Ups_1(u)}} \vabs{\wt{\BB}^{\spl}_{2,1}(u)} 
	\leq 
	\frac{C \de^2}{\vabs{u^2 + A^2}^{2}},	
\end{align*}
and analogous estimates hold for ${\BB}^{\spl}_{2,1}$ and ${\BB}^{\spl}_{2,2}$.

%\textcolor{red}{ARREGLAR:}
%
Finally, we compute estimates for $\bb_y(u)$  (see \eqref{def:mxmyalxaly}) and  $u \in \DBoomerang$. The estimates for  $\bb_x(u)$ can be computed analogously.
%
% We only compute estimates for $\bb_y(u)$ and $\Im(u) \geq 0$, the remaining cases can be proven analogously. 
%
Let us consider the integration path $\rho_t = u_* + (u-u_*)t $, for $t\in[0,1]$. 
%
Then
\begin{align*}
\bb_y(u) = \exp \paren{ 
\int_0^{1}  \wt{\BB}^{\spl}_{2,2}\paren{\rho_t}
(u-u_*) dt}.
\end{align*} 
Using the bounds in \eqref{proof:boundsBsplTilde}, we have that
\begin{align*}
\vabs{\log \bb_y(u)} &\leq
%
C \vabs{u-u_*} \vabs{\int^{1}_0  
 \frac{1}{\vabs{\rho^2_t + A^2}^{\frac{1}{3}}} +
\frac{\de^2}{\vabs{\rho^2_t + A^2}^{2}} dt} 
\leq C,
%
%&\leq C \vabs{u-u_0}  \vabs{ \int^{1}_0 \frac{1}{\vabs{\rho(t)-iA}^{\frac{2}{3}}} +
%\frac{\de^2}{\vabs{\rho(t)-iA}^{2}}  dt }\\
%%
%&\leq C \boxClaus{\paren{u_0^2+A^2}^{\frac{1}{6}} - \vabs{u-iA}^{\frac{1}{3}}}
%+ C \boxClaus{ \frac{\de^2}{\vabs{u-iA}} -\frac{\de^2}{\sqrt{u_0^2+A^2} } }\\
%%
%&\leq C \paren{1 - \kappa^{\frac{1}{3}}\de^{\frac{2}{3}}} 
%+ C \paren{\frac{1}{\kappa}-\de^2 } \leq C .
\end{align*}
which implies $C^{-1} \leq \vabs{\bb_y(u)} \leq C$.
% , for $u \in \DBoomerang$.
%	Then,
%	\begin{align*}
%		C^{-1} \leq 
%		\exp\paren{-\vabs{\int_{\rho} \beta_y }} \leq 
%		\vabs{\al_y(u)} \leq
%		\exp\paren{+\vabs{\int_{\rho} \beta_y}} \leq C.
%	\end{align*}

%\begin{lemma}\label{lemma:alxalyEstimates}
%Consider functions $\al_x$ and $\al_y$ as defined on~\eqref{def:mxmyalxaly}. Then, for $it\in E$ and $\de$ small enough, we have
%\begin{align*}
%C^{-1} \leq \vabs{\al_x(it)} \leq C, \hh
%C^{-1} \leq \vabs{\al_y(it)} \leq C.
%\end{align*}
%\end{lemma}
%
% \end{proof}

\subsection{Proof of Lemma \ref{lemma:boundsBonsBeta}}
\label{subappendix:proofH-technicalSecond}

We only give an expression for $\bb_y(u_+)$. The result for $\bb_x(u_-)$ is analogous. 
%
First, we analyze $\wt{\BB}^{\spl}_{3,3}$.

\begin{lemma}\label{lemma:proofConstantA}
For $\de>0$ small enough, $\kappa>0$ large enough and $u \in \DBoomerang$, the function $\wt{\BB}^{\spl}_{3,3}$  defined in \eqref{def:Bspl1} is of the form 
\begin{align*}
	\wt{\BB}_{3,3}^{\spl}(u) = 
	-\frac{4i}3 \La_h(u)
	+ \de^2 m(u;\de),
\end{align*}
for some function $m$ satisfying
\begin{align*}
	\vabs{m(u;\de)}
	\leq \frac{C}{\vabs{u^2+A^2}^{2}}.
\end{align*}
\end{lemma}	

\begin{proof}
Let us define $z_{\tau}= \tau\zuOut + (1-\tau) \zsOut$ and recall that, for $u \in \DBoomerang$,
\begin{align}\label{proof:B33tildeDef}
\wt{\BB}_{3,3}(u) = 
\int_0^1 \partial_y \RRR_3^{\out}[z_{\tau}](u) d\tau.
\end{align}
Then, by the expression of $\RRR_3^{\out}$ in \eqref{eq:expressionRRRout}, the estimates 
in the proof of Lemma \ref{lemma:computationsRRROut} (see Appendix \ref{subsubsection:proofComputationsRRROut}) and Theorem \ref{theorem:existence}, we have that
% obtain that,
\[
\partial_y \RRR_3^{\out}[z_{\tau}](u) 
=
\frac{i}{\de^2} g^{\out}(u,z_{\tau}(u)) +
\de^2 \wt{m}(u;\de),
\]
%
where
$
\vabs{\wt{m}(u;\de)}
\leq \frac{C}{\vabs{u^2+A^2}^{2}}.
$
%
In the following, to simplify notation, we denote by $\wt{m}(u;\de)$ any function satisfying the previous estimate.
%
Since $g^{\out}=\partial_w H_1^{\out}$, by \eqref{proof:H1outExpressionOuter} one has
\[
g^{\out}(u,z_{\tau}(u)) = \partial_w M_P(u,z_{\tau}(u);\de)+
\partial_w M_S(u,z_{\tau}(u);\de)+
\partial_w M_R(u,z_{\tau}(u);\de),
\]
with $M_P$, $M_S$ and $M_R$ as given in \eqref{def:expressionMJOuter},
\eqref{def:expressionMSOuter} and
\eqref{def:expressionMROuter}, respectively.
%
Then, taking into account that $F_{\pend}(s)=2z^3+\OO(z^4)$ (see \eqref{def:Fpend}) and following the proofs of Lemmas \ref{lemma:boundsMPout} and \ref{lemma:boundsMSout}, it is a tedious but an easy computation to see that,
%
\begin{equation*}
\begin{split}	
	g^{\out}(u,z_{\tau}(u)) =& \,
	\partial_w M_P(u,0,0,0;\de) + 
	\partial_w M_S(u,0,0,0;\de)  \\
	&- \frac{w_{\tau}(u)}{3 \La_h^2(u)}
	-\frac{\de^2 \LtresLa(\de)}{\La_h(u)}
	- 2 \de^2\La_h(u) 
	+
	\de^4\wt{m}(u;\de),
\end{split}
\end{equation*}
%
and, by \eqref{proof:B33tildeDef},
\begin{equation}\label{proof:B33tildeDefB}
\begin{split}
\wt{\BB}_{3,3}(u) =& \, \frac{i}{\de^2} \boxClaus{\partial_w M_P(u,0,0,0;\de) + 
\partial_w M_S(u,0,0,0;\de) } \\
&- i\frac{\wuOut(u)+\wsOut(u)}{6 \de^2\La_h^2(u)}
- i\frac{\LtresLa(\de)}{\La_h(u)}
- 2i \La_h(u) 
+
\de^2\wt{m}(u;\de).
\end{split}
\end{equation}

Next, we study the terms $\wusOut(u)$.
%
Since $H^{\out}=w + \frac{xy}{\de^2} + M_P+M_S+M_R$ (see
\eqref{def:hamiltonianOuter} and \eqref{proof:H1outExpressionOuter}), one can see that
\[
H^{\out}(u,\zuOut(u);\de) 
= 
H^{\out}(u,\zsOut(u);\de) 
= 
\lim_{\Re u \to \pm \infty} H^{\out}(u,0,0,0;\de)
=
\de^4 K(\de),
\]
with $\vabs{K(\de)}\leq C$, for $\de$ small enough.
%
Then, by Theorem \ref{theorem:existence}, for $\diamond=\unstable,\stable$,
%
\begin{align*}
\vabs{\wdOut(u) + M_P(u,\zdOut(u);\de)+
M_S(u,\zdOut(u);\de)+ M_R(u,\zdOut(u);\de)}
\leq 
\frac{C\de^4}{\vabs{u^2+A^2}^{\frac83}}.
\end{align*}
Again, following the proofs of Lemmas \ref{lemma:boundsMPout} and \ref{lemma:boundsMSout}, one obtains
%
\begin{align*}
\vabs{\wdOut(u) + M_P(u,0,0,0;\de) 
+ M_S(u,0,0,0;\de)
+\de^2\La_h(u)(3\LtresLa+2\La_h^2(u))}
\leq \frac{C\de^4}{\vabs{u^2+A^2}^{\frac83}},
\end{align*}
and, by \eqref{proof:B33tildeDefB},
\begin{equation*}%\label{proof:B33tildeDefC}
\begin{split}
\wt{\BB}_{3,3}(u) 
=& \, 
-  \frac{4i}3 \La_h(u)
+
\frac{i}{\de^2} \boxClaus{\partial_w M_P(u,0,0,0;\de) 
+ \frac{M_P(u,0,0,0;\de)}{3\La_h^2(u)}
 }
\\
&+ \frac{i}{\de^2} \boxClaus{\partial_w M_S(u,0,0,0;\de) 
+ \frac{M_S(u,0,0,0;\de)}{3\La_h^2(u)} }
+\de^2\wt{m}(u;\de).
%
\end{split}
\end{equation*}
Therefore, it only remains to check that
\begin{align*}
\vabs{\partial_w M_{P,S}(u,0,0,0;\de) 
+ \frac{M_{P,S}(u,0,0,0;\de)}{3\La_h^2(u)}}
\leq \frac{C\de^4}{\vabs{u^2+A^2}^2}.
\end{align*}

Indeed, by \eqref{def:SerieP} and the definition \eqref{def:expressionMJOuter} of $M_P$, one has 
\begin{align*}
M_P(u,w,0,0;\de) = \MM_P\paren{u,\de^2\La_h(u)-\frac{\de^2 w}{3\La_h(u)}+\de^4\LtresLa(\de)},	
\end{align*}
where $\MM_P(u,\La)$ is an analytic function for $u \in \DBoomerang$ and $\vabs{\La} \ll 1$. 
%
Moreover, following the proof of Lemma  \ref{lemma:boundsMPout}, there exist $a_0$ and $a_1$ such that 
\begin{align*}
\vabs{\MM_P(u,\La)-a_0(u;\de)- a_1(u;\de) \La} \leq 
\frac{C\La^2}{\vabs{u^2+A^2}^2},
\end{align*}
with
\[
\vabs{a_0(u;\de)} \leq \frac{C\de^4}{\vabs{u^2+A^2}^{\frac23}},
\qquad
\vabs{a_1(u;\de)} \leq \frac{C}{\vabs{u^2+A^2}^{\frac23}}.
\]
Therefore,
\begin{align*}
\vabs{\partial_w M_{P}(u,0,0,0;\de) 
+ \frac{M_{P}(u,0,0,0;\de)}{3\La_h^2(u)}}
\leq& \,
\frac{\vabs{a_0(u)}}{3\La_h^2(u)}
+ \frac{\de^4\LtresLa(\de)\vabs{a_1(u)}}{3\La_h^2(u)}
+ \frac{C\de^4}{\vabs{u^2+A^2}^{2}} 
\\
\leq& \,
\frac{C\de^4}{\vabs{u^2+A^2}^{2}} .
\end{align*}
An analogous estimate holds for $M_S$.
\end{proof}

\begin{proof}[End of the proof of Lemma \ref{lemma:boundsBonsBeta}]
%
By Lemma \ref{lemma:proofConstantA} and recalling that  $u_+=iA-\kappa \de^2$,
% (see \eqref{def:uMesuMenysDiff}),
\begin{equation}
	\label{proof:constantDifferenceZ}
\begin{split}	
\log B_y(u_+) 
=&
\int_{u_*}^{u_+} \wt{\BB}_{3,3}^{\spl}(u) du
= 
-\frac{4i}3  \int_{u^*}^{i A} \La_h(u) du 
\\ &+
\frac{4i}3 \int^{i A}_{u_+} \La_h(u) du 
+
\de^2
\int_{u^*}^{u_+} {m}(u;\de).
\end{split}
\end{equation}
Then, by Theorem \ref{theorem:singularities} and taking into account that $\kappa=\kappa_* \vabs{\log \de}$ (see Lemma \ref{lemma:IconstantsDiff}), we obtain
\begin{align*}
\vabs{\log B_y(u_+)  + \frac{4 i}3
\int_{u^*}^{i A} \La_h(u) du}
\leq 
\frac{C}{\kappa} 
+
C \kappa^{\frac23}\de^{\frac43}
+
\frac{C\de^2}{\vabs{u_* - iA}}
\leq 
\frac{C}{\vabs{\log \de}}.
\end{align*}
%
Finally, recalling that $\dot{\la}_h=-3\La_h$, applying the change of coordinates $\la=\la_h(u)$
%
and using that $\la_h(iA) = \pi$, we have that
\begin{align*}
\frac{4i}3 \int_{u^*}^{i A} \La_h(u) du 
=
-\frac{4i}9 \int_{\la_h(u_*)}^{\pi} d\la
=
-\frac{4i}9 \paren{\pi-\la_h(u_*)}.
\end{align*}
%
Joining the last statements with \eqref{proof:constantDifferenceZ}, we obtain the statement of the lemma.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% VERSIO ANTIGA %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Proof of Lemma \ref{lemma:boundsBonsBeta}}
%\label{subappendix:proofH-technicalSecond}
%
%We only give an expression for $\bb_y(u_+)$. The result for $\bb_x(u_-)$ is analogous. 
%%
%First, we analyze $\wt{\BB}^{\spl}_{3,3}$.
%
%\begin{lemma}\label{lemma:proofConstantA}
%	For $\de>0$ small enough, $\kappa>0$ large enough and $u \in \DBoomerang$, the function $\wt{\BB}^{\spl}_{3,3}$  defined in \eqref{def:Bspl1} is of the form 
%	%
%	% Then, for ,
%	\begin{align*}
%		\wt{\BB}^{\spl}_{3,3}(u) =& -
%		\frac{i}{3\La_h(u)\sqrt{2+2\cos\la_h(u)}}
%		-i
%		\frac{4\cos\la_h(u)-2+3\LtresLa(\de)}{3\La_h(u)}
%		-
%		2 i \La_h(u) \\
%		&-
%		\frac{i}{6\La^2_h(u)}
%		% {\left. 
%		\frac{\wuOut(u)+\wsOut(u)}{\de^2} 
%		% \right\vert_{\de=0}}
%		+  \de^2 m(u;\de),
%	\end{align*}
%	%where
%	%\begin{align*}
%	%m_0(u) =& 
%	%{\left. \frac{\wuOut(u)+\wsOut(u)}{6 \, \de^2 \La^2_h(u)} \right\vert_{\de=0}}
%	%+
%	%\frac{1}{3\La_h(u)\sqrt{2+2\cos\la_h(u)}}
%	%+
%	%\frac{1+8\cos\la_h(u)}{6\La_h(u)}
%	%+
%	%2 \La_h(u).
%	%\end{align*}
%	where $\LtresLa(\de)$ is given in \eqref{def:pointL3sca}
%	and for some function $m$ which satisfies
%	% such that, there exists a constant $C$ independent of $\de$ and $\kappa$, such that
%	\begin{align*}
%		\vabs{m(u;\de)} \leq \frac{C}{\vabs{u^2+A^2}^2}.
%	\end{align*}
%\end{lemma}	
%
%\begin{proof}
%	% We expand $\wt{\BB}^{\spl}_{3,3}$ in $\delta$, that is 
%	% \begin{align*}
%	% {\wt{\BB}^{\spl}_{3,3}(u)} = {m}_0(u) + \de \, {m}_1(u) + \de^2 m_2(u;\de).
%	% \end{align*}
%	% Using the estimates in \eqref{proof:boundsBsplTilde}, one can see that
%	% \begin{align*}
%	% \vabs{{m}_0(u)+\de \, {m}_1(u)} \leq \frac{C}{\vabs{u^2+A^2}^{\frac23}},
%	% \qquad
%	% \vabs{m_2(u;\de)} \leq 
%	% \frac{C}{\vabs{u^2+A^2}^2}.
%	% \end{align*}	
%	% %
%	% Therefore, we need to compute the terms ${m}_0$ and ${m}_1$. 
%	% %
%	% We do so by following the notation introduced in the proof of Lemma \ref{lemma:computationsRRROut} in Section \ref{subsubsection:proofComputationsRRROut}.
%	Let us define $z_{\tau}= \tau\zuOut + (1-\tau) \zsOut$ and recall that, for $u \in \DBoomerang$,
%	\begin{align*}
%		\wt{\BB}_{3,3}(u) = 
%		\int_0^1 \partial_y \RRR_3^{\out}[z_{\tau}](u) d\tau.
%	\end{align*}
%	Then, by the expression of $\RRR_3^{\out}$ in \eqref{eq:expressionRRRout}, the estimates 
%	in the proof of Lemma \ref{lemma:computationsRRROut} (see Appendix \ref{subsubsection:proofComputationsRRROut}) and Theorem \ref{theorem:existence}, we have that
%	% obtain that,
%	\[
%	\left|\partial_y \RRR_3^{\out}[z_{\tau}](u) -
%	\frac{i}{\de^2} g^{\out}(u,z_{\tau}(u)) \right|\leq \frac{C\de^2}{\vabs{u^2+A^2}^2}.
%	\]
%	Moreover, since $g^{\out}=\partial_w H_1^{\out}$, by \eqref{proof:H1outExpressionOuter} one has
%	\[
%	g^{\out}(u,z_{\tau}(u)) = \partial_w M_P(u,z_{\tau}(u))+
%	\partial_w M_S(u,z_{\tau}(u))+
%	\partial_w M_R(u,z_{\tau}(u)),
%	\]
%	with $M_P$, $M_S$ and $M_R$ as given in \eqref{def:expressionMJOuter},
%	\eqref{def:expressionMSOuter} and
%	\eqref{def:expressionMROuter}, respectively.
%	To complete the proof of the lemma it is enough to analyze each of these terms.
%	
%	% \begin{equation}\label{proof:constantDifferenceC}
%	% \begin{split}
%	% &\partial_y \RRR_3^{\out}[z_{\tau}](u) =
%	% \frac{i}{\de^2} g^{\out}(u,z_{\tau}(u))
%	% + \OO(\de^2) 
%	% \\
%	% &=
%	% \frac{i}{\de^2} \paren{
%	% 		\partial_w M_P(u,z_{\tau}(u))+
%	% 		\partial_w M_S(u,z_{\tau}(u))+
%	% 		\partial_w M_R(u,z_{\tau}(u))}
%	% + \OO(\de^2). 
%	% \end{split}
%	% \end{equation}
%	%
%	%Let us notice that, by Theorem \ref{theorem:existence}, for $u \in \DBoomerang \cap \reals$ and all $\tau \in [0,1]$, we have that
%	%\begin{align*}
%	%	\vabs{w_{\tau}(u)} \leq C \de^2, 
%	%	\qquad
%	%	\vabs{x_{\tau}(u)} \leq C \de^3,
%	%	\qquad
%	%	\vabs{y_{\tau}(u)} \leq C \de^3.
%	%\end{align*}
%	%
%	Applying Lemma \ref{lemma:changeTotalOuter}, we obtain the first order for $\partial_w M_P$ and $\partial_w M_S$,
%	%
%	\begin{equation}\label{proof:constantDifferenceA}
%		\begin{split}
%			\left|\partial_w M_P(u,z_{\tau}(u))
%			%-\frac{\de^2}{3\La_h(u)} \paren{
%			%\frac{\partial_L B[\de^4-1] }{A[\de^4-1]^{\frac32}} \circ \Tht(u,z_{\tau}(u)) }
%			%\\
%			%=&
%			-\frac{\de^2}{3\La_h(u)\sqrt{2+2\cos\la_h(u)}}\right|
%			&\leq \frac{C\de^4}{\vabs{u^2+A^2}^2},\\
%			%%%
%			\left|\partial_w M_S(u,z_{\tau}(u))
%			-\frac{2 \de^2(1-2\cos\la_h(u))}{3 \La_h(u)}\right|&
%			\leq C\de^4.
%		\end{split}	
%	\end{equation}
%	%
%	For the term $M_R$ (see \eqref{def:expressionMROuter}), let us notice that
%	%
%	$F_{\pend}(s)=2z^3+\OO(z^4)$ (see \eqref{def:Fpend}).
%	%
%	Then,
%	\begin{align*}
%		\left|\partial_w M_R(u,z_{\tau}(u))+ \frac{w_{\tau}(u)}{3 \La_h^2(u)}
%		+\frac{\de^2 \LtresLa(\de)}{\La_h(u)}
%		+ 2 \de^2\La_h(u)\right|\leq\frac{C \de^4}{\vabs{u^2+A^2}^{\frac43}}.
%	\end{align*}
%	%Lastly, by following the results in Section 2.1 of \cite{articleInner}, we see that
%	%\begin{equation}\label{def:LLambda}
%	%\LtresLa(\de) = \frac56 + \OO(\de^4).
%	%\end{equation}
%	%\textcolor{red}{No faria falta calcular $\LtresLa$ si no es vol, ja que s'elimina amb les altres derivades.}
%	Then,
%	\begin{align}\label{proof:constantDifferenceB}
%		\left|\int_0^1 \partial_w M_R(u,z_{\tau}(u)) d\tau
%		+\frac{\wuOut(u)+\wsOut(u)}{6\La^2_h(u)} -\frac{\de^2\LtresLa(\de)}{\La_h(u)} 
%		+2\de^2\La_h(u)\right|\leq\frac{C\de^4}{\vabs{u^2+A^2}^{\frac23}}.
%	\end{align}
%	% Finally, applying the results in \eqref{proof:constantDifferenceA} and \eqref{proof:constantDifferenceB} to \eqref{proof:constantDifferenceC}, we obtain that ${m}_0(u)$ is as stated in the lemma and ${m}_1\equiv0$.
%\end{proof}
%
%To give an expression  for $\bb_y(u_+)$ from Lemma \ref{lemma:proofConstantA} we need to give a first order for 
%$\wuOut(u)$ and $\wsOut(u)$.
%
%\begin{lemma}\label{lemma:proofConstantB}
%	Let the functions $\wuOut$ and $\wsOut$ be as given in Theorem \ref{theorem:existence} and constants
%	$\kappa$ and $\de$ as given in in Lemma \ref{lemma:IconstantsDiff}.
%	%
%	Then, for $\diamond=\unstable, \stable$ and $u \in \DBoomerang$, they satisfy
%	\begin{align*}
%		\wdOut(u) = -\de^2 \La_h(u) \paren{ 4\cos\la_h(u)
%			+ 2 \La^2_h(u) + 3\LtresLa(\de)-2 + \frac{1}{\sqrt{2+2\cos\la_h(u)}}
%		} + \de^4 \widetilde w^{\diamond}(u;\de),
%	\end{align*} 
%	where $\LtresLa(\de)$ is given in \eqref{def:pointL3sca} and
%	for some functions
%	\begin{align*}
%		\vabs{ \widetilde  w^{\diamond}(u;\de)} \leq \frac{C}{\vabs{u^2+A^2}^{\frac83}}.
%	\end{align*}
%\end{lemma}
%
%\begin{proof}
%	%
%	We prove the -$\unstable$- case. The stable -$\stable$-  case is analogous.
%	% %
%	% By Theorem \ref{theorem:existence}, we have that, for $u \in \DBoomerang$, 
%	% \begin{align*}
%	% \wuOut(u) = 
%	% \de^2 w_2(u)
%	% + \de^3 w_3(u)
%	% + \de^4 w_4(u;\de),
%	% \end{align*}
%	% such that
%	% \begin{align*}
%	% \vabs{w_2(u)+\de w_3(u)} \leq \frac{C}{\vabs{u^2+A^2}},
%	% \qquad
%	% \vabs{w_4(u;\de)} \leq 
%	% \frac{C}{\vabs{u^2+A^2}^{\frac{8}3}}.
%	% \end{align*}
%	% %
%	% Therefore, we need to compute the terms $w_2(u)$ and $w_3(u)$. 
%	% %
%	% We do so by following the notation introduced in the proof of Lemma \ref{lemma:computationsRRROut} in Section \ref{subsubsection:proofComputationsRRROut}.
%	
%	Let us recall that $\partial_u \wuOut = \RRR^{\out}_1[\zuOut]$ (see \eqref{eq:invariantEquationOuter}).
%	%
%	By the expression of $\RRR_1^{\out}$ in \eqref{eq:expressionRRRout} and the proof of Lemma \ref{lemma:computationsRRROut} in Appendix \eqref{subsubsection:proofComputationsRRROut}
%	we obtain that, 
%	\begin{align*}
%		\left|\partial_u \wuOut(u) -f_1^{\out}(u,\zuOut(u))\right|\leq
%		% 	+ \OO(\de^2) 
%		C\left(\frac{\de^4}{\vabs{u^2+A^2}^{\frac53}}+\frac{\de^8}{{\vabs{u^2+A^2}^{\frac{17}{3}}}}\right).
%	\end{align*}
%	Then, it only remains to obtain a first order for $f_1^\out=-\partial_u 
%	H_1^{\out}$. Using \eqref{proof:H1outExpressionOuter}, one has
%	% \\
%	\[
%	f_1^{\out}(u,\zuOut(u))=-\partial_u M_P(u,\zuOut(u))
%	-\partial_u M_S(u,\zuOut(u))
%	-\partial_u M_R(u,\zuOut(u)),
%	\]
%	% \end{align*}
%	with $M_P$, $M_S$ and $M_R$ as given in \eqref{def:expressionMJOuter},
%	\eqref{def:expressionMSOuter} and
%	\eqref{def:expressionMSOuter}, respectively.
%	%
%	Then, applying Lemma \ref{lemma:changeTotalOuter} and Theorem \ref{theorem:existence}, we obtain the first orders
%	%
%	\begin{equation*}\label{proof:constantwA}
%		\begin{split}
%			\left|	M_P(u,\zuOut(u))-
%			\frac{\de^2 \La_h(u)}{\sqrt{2+2\cos\la_h(u)}}\right|&
%			\leq \frac{C\de^4}{\vabs{u^2+A^2}^{\frac83}},\\
%			%%%
%			\left|M_S(u,\zuOut(u))-2 \de^2 \La_h(u)(1-2\cos\la_h(u))\right|&
%			\leq C\de^4, \\[0.4em]
%			%%%%
%			\left|M_R(u,\zuOut(u))+
%			\de^2 \La_h(u)(3\LtresLa(\de)+2\La_h^2(u))\right|&\leq
%			C\left( \frac{\de^4}{\vabs{u^2+A^2}^{\frac43}}+ \frac{\de^8}{\vabs{u^2+A^2}^{\frac{14}3}}\right).
%		\end{split}	
%	\end{equation*}
%	% As a result, $w_3 \equiv 0$ and
%	% \begin{align*}
%	% \partial_u w_2(u) =
%	% \partial_u \boxClaus{
%	% -\de^2 \La_h(u) \paren{\frac12 + 4\cos\la_h(u)
%	% 	+ 2 \La^2_h(u) + \frac{1}{\sqrt{2+2\cos\la_h(u)}}
%	% }}.
%	% \end{align*}
%	To complete the proof of the lemma it is enough to integrate (see Lemma \ref{lemma:GlipschitzOuter}).
%\end{proof}
%
%\begin{proof}[End of the proof of Lemma \ref{lemma:boundsBonsBeta}]
%	By Lemmas \ref{lemma:proofConstantA} and \ref{lemma:proofConstantB}, we obtain that
%	\begin{align*}
%		\wt{\BB}_{3,3}^{\spl}(u) = 
%		-\frac{4i}3 \La_h(u)
%		+ \de^2 \wt{m}(u;\de),
%		%\quad \text{ where }
%		%\wt{m}_2(u;\de) =
%		%\de^2 \paren{ m_2(u;\de)
%		%- i \frac{w_4^{\unstable}(u;\de) + w_4^{\stable}(u;\de)}{6 \La^2_h(u)}},
%	\end{align*}
%	with
%	\begin{align*}
%		\vabs{\wt{m}(u;\de)}
%		=
%		\vabs{m(u;\de)
%			- i \frac{\wt w^{\unstable}(u;\de) +\wt w^{\stable}(u;\de)}{6 \La^2_h(u)}}
%		\leq \frac{C}{\vabs{u^2+A^2}^{2}}.
%	\end{align*}
%	Recalling that  $u_+=iA-\kappa \de^2$,
%	% (see \eqref{def:uMesuMenysDiff}),
%	\begin{align}\label{proof:constantDifferenceZ}
%		\ln \beta(u_+) 
%		= 
%		-\frac{4i}3  \int_{u^*}^{i A} \La_h(u) du 
%		+
%		\frac{4i}3 \int^{i A}_{u_+} \La_h(u) du 
%		+
%		\de^2
%		\int_{u^*}^{u_+} \wt{m}(u;\de),
%	\end{align}
%	and, by Theorem \ref{theorem:singularities} and taking into account that $\kappa=\kappa_* \vabs{\log \de}$ (see Lemma \ref{lemma:IconstantsDiff}), we obtain
%	\begin{align*}
%		\vabs{\ln \beta(u_+) + \frac{4 i}3
%			\int_{u^*}^{i A} \La_h(u) du}
%		\leq 
%		\frac{C}{\kappa} 
%		+
%		C \kappa^{\frac23}\de^{\frac43}
%		+
%		\frac{C\de^2}{\vabs{u_* - iA}}
%		\leq 
%		\frac{C}{\vabs{\log \de}}.
%	\end{align*}
%	%
%	Lastly, recalling that $\dot{\la}_h=-3\La_h$, applying the change of coordinates $\la=\la_h(u)$.
%	%
%	and using that $\la_h(iA) = \pi$, we have that
%	\begin{align*}
%		\frac{4i}3 \int_{u^*}^{i A} \La_h(u) du 
%		=
%		-\frac{4i}9 \int_{\la_h(u_*)}^{\pi} d\la
%		=
%		-\frac{4i}9 \paren{\pi-\la_h(u_*)}.
%	\end{align*}
%	%
%	Joining the last statements with \eqref{proof:constantDifferenceZ}, we obtain the statement of the lemma.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Moreover, we can compute an expression for $c_x$ and $c_y$. Indeed,
%\begin{align*}
%	c_y(u_0) = \frac{i}{3} \int_{u_0}^{iA} 
%	\frac{d u}{\La_h(u) \sqrt{2+2\la_h(u)}}.
%\end{align*}	
%	%
%Then, for $\la_*= \la_h(u_0) \in (0,\la_0)$, we have that
%\begin{align*}
%c_y(\la_*) = \frac{i}{6}\int_{\la_*}^{\pi} \frac{d \la}{5\cos(\frac{\la}2)-4\cos^3(\frac{\la}2)
%-1}
%\end{align*}
%
%By Theorem \ref{theorem:singularities}, we have that
%$(\la_h,\La_h)$ is analytic at $u=0$ and $(\la_h(0),\La_h(0))=(\la_0,0)$.
%%
%Then,
%\begin{align*}
%\la_h(u) = \la_0 + c_{\la} u^2 + \OO(u^3), 
%\qquad \text{for }
%0 \leq \vabs{u} \ll 1.
%\end{align*}
%Moreover,  since $(\la_h,\La_h)$ is found at the energy level $H_{\pend}=-\frac12$, replacing  the previous expression at the Hamiltonian $H_{\pend}$ it can be seen that
%\begin{align*}
%	c_{\la} = - \frac{(15\sqrt2+18)\sqrt{4\sqrt2-5}}4
%	\approx -7.9452.
%\end{align*}
%
%
%
%We have that, $L_3$ point in the Poincar\'e coordinate $L$ is given by
%\begin{align*}
%	L = \sqrt{\frac{d_{\mu}}{2-d^3_{\mu}}}
%	\qquad \text{with} \qquad
%	d_{\mu} = 1 + \frac5{12} \mu + \OO(\mu^2).
%\end{align*}
%Then
%\begin{align*}
%	\LtresLa(\de)= \frac56 + \OO(\de^4).
%\end{align*}




==> Article Outer/proofG-matching.tex <==

This section is devoted to prove Theorem \ref{theorem:matching} which provides estimates for $\ZusMchU= \ZusMchO - \ZusInn$
in the matching domains $\DuMchInn$ and $\DsMchInn$, given in \eqref{def:matchingDomainInner}.
%
We only prove the theorem for $\ZuMchU$, being the proof for $\ZsMchU$ analogous.

%Let us recall that $\ZdInn$ is given in Theorem \ref{theorem:innerComputations} and 
%\begin{equation}\label{def:ZdMchOProof}
%\ZdMchO(U) = \paren{
%\frac{\de^{\frac43}}{2 \al_+^2}, \,
%\frac{1}{\de^{\frac13} \sqrt{2}\al_+}, \,
%\frac{1}{\de^{\frac13} \sqrt{2}\al_+}
%}\zdOut(\de^2 U + iA), 
%\end{equation}
%where $\zdOut$ is given in Proposition \ref{proposition:existenceComecocos}.
%
%Moreover, by \eqref{eq:domainsMatchingOuterSubset} and \eqref{eq:domainsMatchingInnerSubset}, $\ZdMchO$ and $\ZdInn$ are well defined in the matching domains 
%$\DdMchInn$ for $\kappa \geq \claus{\kappaOuter, \kappaInner}$.
%
%
%Along this section, we denote the components of all the functions and operators by a numerical sub-index $f=(f_1,f_2,f_3)$, unless stated otherwise, and we denote by $C$ any positive constant independent of $\de$ and $\kappa$.

\subsection{Preliminaries and set up}

Proposition \eqref{proposition:innerDerivation} shows that the Hamiltonian $H^{\out}$ expressed in inner coordinates, that is $H^{\inn}$ as given in \eqref{def:hamiltonianInnerComplete},
%
is of the form $H^{\inn}=W+XY+ \KK+H_1^{\inn}$.
%
Then, the equation associated to $H^{\inn}$ can be written as
\begin{equation}\label{eq:systemEDOsInnerComplete}
	\left\{ \begin{array}{l}
		\dot{U} = 1 + g^{\Inner}(U,Z) + g^{\mch}(U,Z),\\
		\dot{Z} = \AAA^{\Inn} Z + f^{\Inner}(U,Z) +  f^{\mch}(U,Z),
	\end{array} \right.
\end{equation}
where $\AAA^{\Inner}$ is given in \eqref{def:matrixAAA} and
\begin{equation}\label{def:fgInnfgMch}
\begin{aligned}	
f^{\Inn} &= \paren{-\partial_U \KK, 
	i \partial_Y \KK, -i\partial_X \KK}^T,
 & \quad
g^{\inn} &= \partial_{W} \KK, 
\\
f^{\mch} &= \paren{-\partial_U H_1^{\inn}, 
	i \partial_Y H_1^{\inn}, -i\partial_X H_1^{\inn} }^T,
 & \quad
g^{\mch} &= \partial_{W} H_1^{\inn}.
\end{aligned}
\end{equation}	
Notice that, since $(u,\zuOut(u))=\phi_{\Inner}(U,\ZuMchO(U))$ (see \eqref{def:ZdMchO}),
%
$(U,\ZuMchO(U))$ is an  invariant graph of equation  \eqref{eq:systemEDOsInnerComplete}.
%
Therefore, $\ZuMchO$ satisfies the invariance equation
\begin{equation*}%\label{eq:invariantEquationInnMchO}
\begin{split}	
%\Dx{\ZuInn}{U} &= 
%\AAA^{\Inner} \ZuInn 
%+ \RRR^{\Inner}[\ZuInn], \\	
\partial_U {\ZuMchO} &= 
	\AAA^{\Inner} \ZuMchO 
	+ \RRR^{\Inner}[\ZuMchO]
	+ \RRR^{\mch}[\ZuMchO],
\end{split}
\end{equation*}
with $\RRR^{\Inner}$ as defined in \eqref{def:operatorRRRInner} and
\begin{equation}\label{def:operatorRRRmch}
	\RRR^{\mch}[\phiA] = 
	\frac{\AAA^{\Inner} \phiA
		+ f^{\Inn}(U, \phiA) 
		+ f^{\mch}(U, \phiA)  }
	{1+ g^{\Inn}(U, \phiA) + g^{\mch}(U, \phiA) } 
	- \AAA^{\Inner} \phiA 
	- \RRR^{\Inner}[\phiA].
\end{equation}
Similarly $\ZuInn$ satisfies the invariance equation 
$
\partial_U \ZuInn =
\AAA^{\Inner} \ZuInn 
+ \RRR^{\Inner}[\ZuInn]
$ (see  Theorem \ref{theorem:innerComputations}) and, 
therefore, the difference $\ZuMchU = \ZuMchO - \ZuInn$ must be a solution of
\begin{equation}\label{eq:invariantEquationMchU1}
	\partial_U {\ZuMchU}  =
	\AAA^{\inn} \ZuMchU +
	\BB(U) \ZuMchU + \RRR^{\mch}[\ZuMchO],
\end{equation}
with
\begin{equation}\label{def:operatorBBmch}
	\BB(U) = \int_{0}^{1} D_{Z}\RRR^{\Inn}
	[(1-s)\ZuInn + s \ZuMchO](U) ds.
\end{equation}
%
The key point is that, since the existence of both $\ZuInn$ and $\ZuMchO$ is already been proven,
we can think of   $\BB(U)$ and
$\RRR^{\mch}[\ZuMchO](U)$ as known functions. Therefore,  equation~\eqref{eq:invariantEquationMchU1} can be understood as  a non homogeneous linear equation with independent term $\RRR^{\mch}[\ZuMchO](U)$.
%
Moreover, defining the linear operator 
%\begin{equation}\label{def:operatorLLmch}
	$\LL^{\inn} \phiA = (\partial_U-\AAA^{\inn})\phiA$,
%\end{equation}
equation~\eqref{eq:invariantEquationMchU1} is equivalent to
\begin{equation}\label{eq:invariantEquationMchU2}
\LL^{\inn}{\ZuMchU}(U) =
 \BB(U)\ZuMchU(U) 
+\RRR^{\mch}[\ZuMchO](U).
\end{equation}
%Let us consider the linear operator $\LL\phiA= (\partial_U - \AAA^{\inn})\phiA$.
%
We prove Theorem \ref{theorem:matching} by solving this equation (with suitable initial conditions).
% showing that the linear operator $\LL^{\inn}-\BB(U)$ 
To this end, we define  the  Banach space 
$
\XcalMchTotal = \XcalMch_{\frac{4}{3}} \times \XcalMch_1 \times \XcalMch_1
$
with
% %
% Given $\al \in \reals$, we consider 
%\begin{equation*}
%	\normMch{\phiA}_{\al} = \sup_{U \in \DuMchInn} \vabs{U^{\al}\phiA(U)},
%\end{equation*}
% the Banach space
\begin{equation*}
	\XcalMch_{\al}= 
	\Bigg\{ \phiA: \DuMchInn \to \complexs  \st  
	\phiA \text{ real-analytic, } 
	\normMch{\phiA}_{\al}=\sup_{U \in \DuMchInn} \vabs{U^{\al}\phiA(U)} < \infty \Bigg\},
\end{equation*}
% and the product space 
endowed with the product norm
$
\normMchTotal{\phiA} = \normMch{\phiA_1}_{\frac{4}{3}} + \normMch{\phiA_2}_{1} + \normMch{\phiA_3}_{1}.
$

Next lemma gives some properties of these Banach spaces.
%
%We use this lemma throughout the section  without mentioning it.
%
%We will work with Lemma 4.3 in~\cite{Bal06}.
%
\begin{lemma}\label{lemma:sumNormsMch}
Let $\g \in [\frac{3}{5},1)$ and $\al, \beta \in \reals$. The following statements hold:
\begin{enumerate}
%\item If $\al < \beta$, then $\XcalMch_{\al} \subset \XcalMch_{\beta}$ and
%$
%\normMch{\varphi}_{\beta} \leq
%C \de^{2(\al-\beta)(1-\g)}
%\normMch{\varphi}_{\al}.
%$
\item If $\varphi \in \XcalMch_{\al}$, then $\varphi \in \XcalMch_{\beta}$ for any $\beta \in \reals$.
%
Moreover,
\begin{align*}
	\begin{cases}
		\normMch{\varphi}_{\beta} \leq 
		C \kappa^{\beta-\al} 
		\normMch{\varphi}_{\al}, 
		&\quad \text{for } \al  > \beta, \\
		%		
		\normMch{\varphi}_{\beta} \leq 
		C \de^{2(\al-\beta)(1-\g)} 
		\normMch{\varphi}_{\al},
		&\quad \text{for } \al  < \beta.
	\end{cases}	
\end{align*}
\item If $\varphi \in \XcalMch_{\al}$ and 
$\zeta \in \XcalMch_{\beta}$, then
$\varphi \zeta \in \XcalMch_{\al+\beta}$ and
	$
	\normMch{\varphi \zeta}_{\al+\beta} \leq \normMch{\varphi}_{\al} \normMch{\zeta}_{\beta}.
	$
\end{enumerate}
%Analogous statements hold for $\XcalInnU$ and $\XcalInnS$.
\end{lemma}

This lemma is a direct consequence of the fact that, as explained in Section \ref{subsection:matching}, $U$ satisfies
\begin{equation}\label{eq:boundsDomainMchInner}
 	\kappa \cos \betaMchA  \leq 
	\vabs{U} \leq 
	\frac{C}{\de^{2(1-\g)}}.
\end{equation}

Now, we present the main result of this section, which implies Theorem~\ref{theorem:matching}.

\begin{proposition}\label{theorem:matchingProof}
%Let us consider constant $\kappaOuter$ obtained in Proposition~\ref{proposition:existenceComecocos}and  constant $\kappaInner$ obtained in Theorem \ref{theorem:innerComputations}.
%
There exist $\g^*\in[\frac35,1)$,
$\kappaMch\geq\max\claus{\kappaOuter,\kappaInner}$,
 $\de_0>0$ and $\cttMchA>0$  such that, 
for  $\g \in (\g^*,1)$,
 $\kappa\geq \kappaMch$
and $\de \in (0,\de_0)$, $\ZuMchU$ satisfies
% \begin{equation*}
	$\normMchTotal{\ZuMchU} \leq \cttMchA \, \de^{\frac{2}{3}(1-\g)}$.
% \end{equation*}
\end{proposition}

%From now on, we will consider that $\kappa$ is big enough and $\de$ is small enough.

\subsection{An integral equation formulation}
\label{subsection:linearOperatorsMch}
% We prove Proposition \ref{theorem:matchingProof} by analyzing $\ZuMchU$ as the solution of a suitable integral equation.

% To obtain a  right-inverse of the operator $\LL^{\inn}-\BB(U)$ (see \eqref{eq:invariantEquationMchU2})
To prove Proposition \ref{theorem:matchingProof}, we first introduce a right-inverse of  $\LL^{\inn}=\partial_U-\AAA^{\inn}$.
%

\begin{lemma}\label{lemma:operadorEEmch}
The operator $\GG^{\inn}[\phiA]=\paren{\GG^{\inn}_1[\phiA_1],\GG^{\inn}_2[\phiA_2],\GG^{\inn}_3[\phiA_3]}^T$
defined as
\begin{equation}\label{def:operatorEEmch}
	\GG^{\inn}[\phiA](U) = \paren{
		\int_{U_3}^U \phiA_1(S) dS, \,
		\int^U_{U_3} e^{-i(S-U)} \phiA_2(S) dS, \,
		\int^U_{U_2} e^{i(S-U)}\phiA_3(S) dS}^T,
\end{equation}
%
where $U_2$ and $U_3$ are introduced in~\eqref{def:U12}, is a right inverse of $\LL^{\inn}$. 

%
Moreover, there exists a constant $C>0$ such that:
%Fix $\eta>1$, $\nu>0$.
%Then, $\GG^{\inn}: \XcalMch_{\eta} \times \XcalMch_{\nu} \times \XcalMch_{\nu} \to \XcalMch_{\eta-1} \times \XcalMch_{\nu} \times \XcalMch_{\nu}$ is a well defined continuous and linear operator. Moreover, it satisfies:
\begin{enumerate}
\item Let $\al>1$. If $\phiA \in \XcalMch_{\al}$, then $\GG^{\inn}_1[\phiA] \in \XcalMch_{\al-1}$ and
$
\normMch{\GG^{\inn}_1[\phiA]}_{\al-1} \leq C \normMch{\phiA}_{\al}.
$
\item Let $\al>0$, $j=2,3$. 
%
If $\phiA \in \XcalMch_{\al}$, 
then $\GG^{\inn}_j[\phiA] \in \XcalMch_{\al}$ and
$
\normMchSmall{\GG^{\inn}_j[\phiA]}_{\al} \leq C  \normMch{\phiA}_{\al}.
$
\end{enumerate}
\end{lemma}

The proof of this lemma  follows the same lines as the proof of Lemma 20 in \cite{BCS13}.
Using the operator $\GG^{\inn}$,  equation~\eqref{eq:invariantEquationMchU2} is equivalent to 
\begin{equation*}
%\label{eq:invariantEquationMchU3}
	\ZMchU(U) = C^{\mch} e^{\AAA^{\inn} U} + 
	\GG^{\inn} \left[ \BB \cdot \ZMchU \right] (U) + 
	\paren{\GG^{\inn} \circ \RRR^{\mch}[Z]} (U),
\end{equation*}
where $C^{\mch}=(C^{\mch}_W,C^{\mch}_X, C^{\mch}_Y)^T$ is defined as
\begin{equation*}
%\label{def:constantMch}
	C_W^{\mch} =\WMchU(U_3), \qquad
	C_X^{\mch} =e^{-i U_3}\XMchU(U_3), \qquad
	C_Y^{\mch} =e^{i U_2}\YMchU(U_2). 
\end{equation*}
Then, defining the operator
$
\TTT[\phiA](U) = 
\GG^{\inn} \left[ \BB \cdot \phiA \right](U),
$
this equation  is equivalent to \begin{equation}\label{eq:invariantEquationMchU4}
	(\Id - \TTT)\ZuMchU = C^{\mch} e^{\AAA^{\inn} U} +  
	\paren{\GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]}
\end{equation}
and  therefore, to estimate $\ZuMchU$, we need to prove that $\Id-\TTT$ is  invertible  in $\XcalMchUTotal$.



% Defining the operator
% $
% \TTT[\phiA](U) = 
% \GG^{\inn} \left[ \BB \cdot \phiA \right](U),
% $
% equation~\eqref{eq:invariantEquationMchU3} is equivalent to \begin{equation}\label{eq:invariantEquationMchU4}
% 	(\Id - \TTT)\ZuMchU = C^{\mch} e^{\AAA^{\inn} U} +  
% 	\paren{\GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]},
% \end{equation}
% and we proceed by proving that $\Id-\TTT$ is an invertible operator in $\XcalMchUTotal$.

\begin{lemma}\label{lemma:operatorTTmch}
Let us consider operators $\BB$ and $\GG^{\inn}$ as given in \eqref{def:operatorBBmch} and \eqref{def:operatorEEmch}.
%
Then, for $\g \in [\frac35,1)$, $\kappa>0$ big enough and $\de>0$ small enough, for $\phiA \in \XcalMchTotal$,
%
\begin{align*}
\normMchTotal{\TTT[\phiA]} 
= \normMchTotal{\GG^{\inn}[\BB\cdot \phiA]}
\leq \frac{1}{2} \normMchTotal{\phiA}
\end{align*}
and therefore
\begin{align*}
\normMchTotal{(\Id-\TTT)^{-1}[\phiA]} \leq 2 \normMchTotal{\phiA}.
\end{align*}
\end{lemma}

To prove this lemma, we use the following estimates, whose proof is a direct result of Lemma 5.5 in \cite{articleInner}.

\begin{lemma}\label{lemma:technicalMatching}
% 
Fix $\varrho>0$ and take $\kappa>0$ big enough. Then, there exists a constant $C$ (depending on $\varrho$ but independent of $\kappa$) such that, for $\phiA \in \XcalMchTotal$ with $\normMchTotal{\phiA}\leq\varrho$, the functions $g^{\inn}$ and $f^{\inn}$ in \eqref{def:operatorRRRInner} and  the operator  $\RRR^{\inn}$ in \eqref{def:fgInnfgMch}  satisfy
%
\begin{align*}
\normMch{g^{\inn}(\cdot,\phiA)}_2  \leq C,
\qquad
\normMch{f_1^{\inn}(\cdot,\phiA)}_{\frac{11}3} \leq C,
\qquad
\normMch{f_j^{\inn}(\cdot,\phiA)}_{\frac43}
\leq C,
\quad j=2,3
\end{align*}
and
\begin{align*}
\normMch{\partial_W \RRR^{\inn}_1[\phiA]}_3 &\leq C, &
%
\normMch{\partial_X \RRR^{\inn}_1[\phiA] }_{\frac73} &\leq C, &
%
\normMch{\partial_Y \RRR^{\inn}_1[\phiA] }_{\frac73} &\leq C, 
\\
\normMch{\partial_W \RRR^{\inn}_j[\phiA]}_{\frac23} &\leq C, &
%
\normMch{\partial_X \RRR^{\inn}_j[\phiA] }_{2} &\leq C, &
%
\normMch{\partial_Y \RRR^{\inn}_j[\phiA] }_{2} &\leq C,
\quad j=2,3.
\end{align*}
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lemma:operatorTTmch}]
% First, we analyze estimates for operator $\BB$.
%	
Let $\ZuMchO$ be as given in \eqref{def:ZdMchO}. Then, by Proposition \ref{proposition:existenceComecocos},
estimates \eqref{eq:boundsDomainMchInner} and taking $\g \in [\frac35,1)$, we have that, for $U \in \DuMchInn$,
\begin{align}\label{eq:boundsZMchO}
	\vabs{\WuMchO(U)} \leq \frac{C}{\vabs{U}^{\frac{8}{3}}}
	+ \frac{C \de^{\frac{4}{3}}}{\vabs{U}}
	\leq
	\frac{C}{\vabs{U}^{\frac{8}{3}}}, \qquad
	%
	\normMch{\XuMchO}_{\frac43} \leq C, \qquad
	%
	\normMch{\YuMchO}_{\frac43} \leq C.
\end{align}		
Then, using also Theorem \ref{theorem:innerComputations}, we obtain that
$(1-s)\ZuInn+s\ZuMchO \in \XcalMchTotal$ for $s \in [0,1]$ and $\g \in [\frac35,1)$ and 
$
\normMchTotal{(1-s)\ZuInn+s\ZuMchO}\leq C.
$
%
As a result, using the definition of $\BB$ in \eqref{def:operatorBBmch} and Lemma \ref{lemma:technicalMatching},
\begin{equation}\label{eq:boundsOperadorBBmch}
\begin{aligned}
\normMch{\BB_{1,1}}_3 &\leq C,  &
%
\normMch{\BB_{1,2}}_{\frac73} &\leq C, &
%
\normMch{\BB_{1,3}}_{\frac73} &\leq C, \\
%
\normMch{\BB_{j,1}}_{\frac23} &\leq C, &
%
\normMch{\BB_{j,2}}_2 &\leq C, &
%
\normMch{\BB_{j,3}}_2 &\leq C, 
%
\quad \text{for } j=2,3.
\end{aligned}	
\end{equation}
% This allows us to  compute estimates for 
% $
% \TTT[\phiA] = \GG^{\inn} \left[\BB  \phiA \right]
% $ for $\phiA \in \XcalMchTotal$.
%
Therefore, by Lemmas~\ref{lemma:operadorEEmch} and \ref{lemma:sumNormsMch} and \eqref{eq:boundsOperadorBBmch}, we obtain
\begin{align*}
	\normMch{\TTT_1[\phiA]}_{\frac{4}{3}} &\leq
	C \normMch{\pi_1 \paren{\BB \phiA} }_{\frac{7}{3}}\\
% \end{align*}
% 
% \begin{align*}
% 	\normMch{\TTT_1[\phiA]}_{\frac{4}{3}}
	&\leq C \boxClaus{\normMch{\BB_{1,1}}_{1} \normMch{\phiA_1}_{\frac{4}{3}}+
		\normMch{\BB_{1,2}}_{\frac{4}{3}} \normMch{\phiA_2}_{1}+
		\normMch{\BB_{1,3}}_{\frac{4}{3}} \normMch{\phiA_3}_{1}} \\
	&\leq 
	\frac{C}{\kappa^2} \normMch{\phiA_1}_{\frac{4}{3}} +
	\frac{C}{\kappa} \normMch{\phiA_2}_{1} +
	\frac{C}{\kappa} \normMch{\phiA_3}_{1}
	%&\leq \sup_{U \in \DuMchInn}\claus{\frac{C}{\vabs{U}} }
	%\normMchTotal{\psi}
	\leq \frac{C}{\kappa} \normMchTotal{\phiA}.
\end{align*}
Proceeding analogously, for $j=2,3$, we have
\begin{align*}
	\normMch{\TTT_j[\phiA]}_{1}
	&\leq C \boxClaus{\normMch{\BB_{j,1}}_{-\frac{1}{3}} 
		\normMch{\phiA_1}_{\frac{4}{3}}+
		\sum_{l=2}^3
		\normMch{\BB_{j,l}}_{0} \normMch{\phiA_l}_{1}}
	%	\normMch{\BB_{j,l}}_{0} \normMch{\phiA_l}_{1}} 
	%\\
	%&\leq 
	%\frac{C}{\kappa} \normMch{\phiA_1}_{\frac{4}{3}} +
	%\frac{C}{\kappa^2} \normMch{\phiA_2}_{1} +
	%\frac{C}{\kappa^2} \normMch{\phiA_3}_{1}
	%
	\leq \frac{C}{\kappa} \normMchTotal{\phiA}.
\end{align*}
Taking $\kappa>0$ big enough, we obtain the statement of the lemma.
%have that
%$
%\normMchTotal{\TTT[\phiA]} \leq \frac{1}{2} \normMchTotal{\phiA}.
%$
%Therefore, $(\Id - \TTT)$ is invertible in $\XcalMchTotal$. 
%
\end{proof}	

%\begin{lemma}\label{lemma:operadorBBmch}
%Let us consider operator $\BB$ as defined in~\eqref{def:operatorBBmch}. 
%%
%Then, for $\g \in (\frac34,1)$, $\kappa>0$ big enough and $\de>0$ small enough, there exists a constant $C$ independent of $\kappa$ and $\de$ such that, for $U \in \DuMchInn$,
%\begin{align*}
%	\normMch{\BB_{1,1}}_3 &\leq C,  &
%	%
%	\normMch{\BB_{1,2}}_{\frac73} &\leq C, &
%	%
%	\normMch{\BB_{1,3}}_{\frac73} &\leq C, \\
%	%
%	\normMch{\BB_{j,1}}_{\frac23} &\leq C, &
%	%
%	\normMch{\BB_{j,2}}_2 &\leq C, &
%	%
%	\normMch{\BB_{j,3}}_2 &\leq C, 
%	%
%	\quad \text{for } j=2,3.
%\end{align*}
%\end{lemma}
%
%\begin{proof}
%%
%To prove this result we need to  obtain estimates for $\ZuMchO$ and $\ZuInn$.
%%
%By Theorem \ref{theorem:innerComputations}, we have that
%\begin{align}\label{eq:boundsZuInn}
%	\normMch{\WuInn}_{\frac83} \leq C, \qquad
%	%
%	\normMch{\XuInn}_{\frac43} \leq C, \qquad
%	%
%	\normMch{\YuInn}_{\frac43} \leq C.
%\end{align}	
%%For $\ZuMchO$, first we notice that, for $U \in \DuMchInn$,  
%%\begin{equation}\label{eq:boundsDomainMchInner}
%%	\kappa \cos \betaMchA  \leq 
%%	\vabs{U} \leq 
%%	\frac{C}{\de^{2(1-\g)}}.
%%\end{equation}
%%
%By Proposition \ref{proposition:existenceComecocos},
%estimates \eqref{eq:boundsDomainMchInner} and taking $\g \in (\frac34,1)$, for $U \in \DuMchInn$, we have that
%\begin{align}\label{eq:boundsZMchO}
%\vabs{\WuMchO(U)} \leq \frac{C}{\vabs{U}^{\frac{8}{3}}}
%+ \frac{C \de^{\frac{2}{3}}}{\vabs{U}^{\frac{4}{3}}}
%\leq
%\frac{C}{\vabs{U}^{\frac{8}{3}}}, \qquad
%%
%\normMch{\XuMchO}_{\frac43} \leq C, \qquad
%%
%\normMch{\YuMchO(U)}_{\frac43} \leq C.
%\end{align}	
%%
%Then, applying Lemma 5.5 in \cite{articleInner}, we obtain the statement of the lemma.
%\end{proof}

\subsection{End of the proof of Proposition \ref{theorem:matchingProof}}

To complete the proof of Proposition \ref{theorem:matchingProof}, we study the right-hand side of equation \eqref{eq:invariantEquationMchU4}.
%
%\begin{lemma}\label{lemma:independentTermsMchA}
%%
%Let $C^{\mch}$ be the constant defined in~\eqref{def:constantMch}. 
%%
%Then, there exist $\g^* \in (\frac34,1)$ such that, for $\g \in (\g^*,1)$ and $\de>0$ small enough, there exists a constant $C$ independent of $\de$ and $\kappa$ such that
%\begin{equation*}
%	\normMchTotalSmall{C^{\mch} e^{\AAA^{\inn} U}}\leq
%	C \de^{\frac{2}{3}(1-\g)}.
%\end{equation*}
%\end{lemma}
%%
%\begin{proof}
 
First, we deal with  the term $C^{\mch} e^{\AAA^{\inn} U}$.
%
Recall that  $U_2$ and $U_3$ in \eqref{def:U12} satisfy
\begin{equation*}%\label{eq:boundsDomainMchInner12}
	\frac{C^{-1}}{\de^{2(1-\g)}} \leq
	\vabs{U_j} \leq
	\frac{C}{\de^{2(1-\g)}},
	\hh
	\text{ for } j=2,3.
\end{equation*}
%
%Next, we consider estimates for $C_W^{\mch}$.
%
Then, taking into account that $\WuMchU= \WuMchO-\WuInn$,  \eqref{eq:boundsZMchO} and Theorem \ref{theorem:innerComputations} imply 
\begin{align*}
|C^{\mch}_W| = \vabs{\WuMchU(U_3)} \leq \vabs{\WuMchO(U_3)}+\vabs{\WuInn(U_3)}
%\leq \vabs{\WuMchO(U_3)} + \vabs{\WuInn(U_2)}
\leq \frac{C}{\vabs{U_3}^{\frac{8}{3}}}
%
\leq 
C \de^{\frac{16}{3}(1-\g)}
\end{align*}
and, as a result, by Lemma \ref{lemma:sumNormsMch},
$	
\normMchSmall{C^{\mch}_W}_{\frac{4}{3}} 
\leq 
C \de^{\frac{8}{3}(1-\g)}.
$
%
Analogously, for $U \in \DuMchInn$,
\begin{align*}
|C^{\mch}_X e^{iU}| 
%
&= |e^{i(U-U_3)} \XuMchU(U_3)| 
\leq \frac{C e^{-\Im(U-U_3)}}{\vabs{U_3}^{\frac{4}{3}}} 
%
\leq C \de^{\frac{8}{3}(1-\g)}
\end{align*}
and then
$
\normMchSmall{C^{\mch}_X e^{iU}}_1
\leq C \de^{\frac{2}{3}(1-\g)}.
$
An analogous result holds for $C^{\mch}_Y e^{-iU}$. Therefore,
\begin{equation}\label{eq:independentTermsMchA}
	\normMchTotalSmall{C^{\mch} e^{\AAA^{\inn} U}}\leq
	C \de^{\frac{2}{3}(1-\g)}.
\end{equation}


%\begin{lemma}\label{lemma:independentTermsMchB}
%%
%Let $\RRR^{\mch}$ and $\GG^{\inn}$ be the operators given in~\eqref{def:operatorRRRmch} and~\eqref{def:operatorEEmch}, respectively. 
%%
%Then, there exist $\g^* \in (\frac34,1)$ such that for $\g \in (\g^*,1)$, $\kappa>0$ big enough and $\de>0$ small enough, there exists a constant $C$ independent of $\de$ and $\kappa$ such that
%\begin{equation*}
%\normMchTotalSmall{\GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]}\leq
%C \de^{\frac{2}{3}(1-\g)}.
%\end{equation*}
%\end{lemma}


Now, we estimate the norm of  $\GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]$. 
%
The operator $\RRR^{\mch}$ in~\eqref{def:operatorRRRmch} can be rewritten as
\begin{align*}
\RRR^{\mch}[\ZuMchO] = \frac{f^{\mch}(1+g^{\Inn})-
	g^{\mch}(\AAA^{\Inn}\ZuMchO+f^{\Inn})}{(1+g^{\Inn})(1+g^{\Inn}+g^{\mch})}.
\end{align*}
%with $f^{\inn}, g^{\inn}, f^{\mch}$ and $g^{\mch}$ as given in \eqref{def:fgInnfgMch}.
%
Then by \eqref{eq:boundsZMchO}, Lemmas \ref{lemma:sumNormsMch} and \ref{lemma:technicalMatching} and  taking $\kappa$ big enough, we obtain
\begin{equation}\label{proof:boundsfgInn}
\begin{aligned}
	\normMch{g^{\inn}(\cdot,\ZuMchO)}_0 &\leq \frac{C}{\kappa^2} \leq \frac12, &\quad 
	%
	\normMch{i\XuMchO + f_2^{\inn}(\cdot,\ZuMchO)}_0 
	&\leq C, \\
	%
	\normMch{f_1^{\inn}(\cdot,\ZuMchO)}_0 &\leq C, 
	&\quad
	%
	\normMch{-i\YuMchO + f_3^{\inn}(\cdot,\ZuMchO)}_0 &\leq C.
\end{aligned}
\end{equation}
%
%Then, taking $\kappa$ big enough, 
%\begin{align}\label{proof:RRRmchOnlyMch}
%|\RRR^{\mch}_i[\ZuMchO](U)| \leq C \,
%\frac{|f_i^{\mch}(U,\ZuMchO)| +
%|g^{\mch}(U,\ZuMchO)|}{|1+g^{\mch}(U,\ZuMchO)|},
%\quad \text{for } i=1,2,3.
%\end{align}
%
To analyze 
$f^{\mch}$ and
$g^{\mch}$ (see \eqref{def:fgInnfgMch}) we rely on the estimates for $H_1^{\inn}$  in \eqref{eq:boundsH1Inn} and its derivatives, which can be easily  obtained by Cauchy estimates.
% there exists a constant $m>0$, such that
Indeed, they can be applied  since  $U \in \DuMchInn$ and, by \eqref{eq:boundsZMchO}, 
% $(\WuMchO(U),\XuMchO(U),\YuMchO(U))$ satisfy
%
\[
\vabs{\WuMchO(U)},\vabs{\XuMchO(U)},\vabs{\YuMchO(U)}\leq C.
\]
% 
% Then, by \eqref{eq:boundsDomainMchInner} and since $\ZuMchO \in \XcalMchTotal$, one has that
% \[
% \vabs{\WuMchO(U),\XuMchO(U),\YuMchO(U)}\leq C.
% \]
%
Then, there exists $m>0$ such that
% $f^{\mch} = \paren{-\partial_U H_1^{\inn}, 
% 	i \partial_Y H_1^{\inn}, -i\partial_X H_1^{\inn} }$,
% $g^{\mch} = \partial_{W} H_1^{\inn}$ (see \eqref{def:fgInnfgMch}) and $H_1^{\inn}$ is analytic, applying the estimates in \eqref{eq:boundsH1Inn} there exists a constant $m>0$, such that
\begin{align}\label{proof:boundsMchA}
|g^{\mch}(U,\ZuMchO)| \leq C 
\de^{\frac43-2 m(1-\g)},
\quad
|f_j^{\mch}(U,\ZuMchO)|\leq C \de^{\frac43-2 m(1-\g)},
\text{ for } j=1,2,3.
\end{align} 
%
We note that,  for $\g \in (\g^*_0,1)$ with $\g^*_0=\max\{\frac{3}{5},\frac{3m-2}{3m}\}$, we have that ${\frac43}-2m(1-\g)>0$.
%
Then, for $\g \in (\g^*_0,1)$, $\de$ small enough and $\kappa$ big enough, using \eqref{proof:boundsfgInn} and
\eqref{proof:boundsMchA} we obtain
\begin{align*}%\label{proof:boundsRmch}
|\RRR^{\mch}_j[\ZuMchO](U)| \leq C \de^{\frac43-2 m(1-\g)}, \qquad
\text{ for }  j=1,2,3. 
\end{align*}
%
Then, by Lemmas \ref{lemma:sumNormsMch} and \ref{lemma:operadorEEmch}, 
\begin{align*}
\normMchTotalSmall{\GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]} &=
\normMchSmall{\GG^{\inn}_1 \circ \RRR_1^{\mch}[\ZuMchO]}_{\frac{4}{3}} 
+
\textstyle\sum_{j=2}^3
\normMchSmall{\GG^{\inn}_j \circ \RRR_j^{\mch}[\ZuMchO]}_{1} \\
&\leq 
C \normMchSmall{\RRR_1^{\mch}[\ZuMchO]}_{\frac{7}{3}} +
\textstyle
\sum_{j=2}^3
C \normMchSmall{\RRR_j^{\mch}[\ZuMchO]}_{1} 
\leq
C \de^{\frac43-2\paren{m+\frac73}(1-\g)}.
\end{align*}
%
If we take  $\g^*=\max\claus{\frac35, \g^*_0, \g^*_1}$
with $\g^*_1=\frac{3m+5}{3m+7}$,
%
and $\g \in (\g^*,1)$, 
%
\begin{align}\label{eq:independentTermsMchB}
\normMchTotalSmall{\GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]}
\leq
C \de^{\frac23(1-\g)}.
\end{align}
To complete the proof of Proposition~\ref{theorem:matchingProof}, we consider
equation~\eqref{eq:invariantEquationMchU4}.  By Lemma \ref{lemma:operatorTTmch}, $(\Id - \TTT)$ is invertible in $\XcalMchTotal$ and moreover
%
% and
% since,  one has that
\begin{equation*}
\begin{split}
\normMchTotal{\ZuMchU}& = 
\normMchTotal{ (\Id - \TTT)^{-1}
\paren{C^{\mch} e^{\AAA^{\inn} U} + \GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]}}\\
&\leq 2 \normMchTotal{ C^{\mch} e^{\AAA^{\inn} U} + \GG^{\inn} \circ \RRR^{\mch}[\ZuMchO]}.
% C \de^{\frac{2}{3}(1-\g)}.
\end{split}
\end{equation*}
Then, it is enough to apply   \eqref{eq:independentTermsMchA} and \eqref{eq:independentTermsMchB}.

\qed


==> Article Outer/proofH-existence.tex <==

In this section, we prove Theorem \ref{theorem:existence} by following the 
scheme detailed in Sections \ref{subsection:outerBasic} and 
\ref{subsection:outerExtension}.
% ,
% %
% that is by proving Propositions \ref{proposition:existenceInfty},
% \ref{proposition:existenceComecocos},
% \ref{proposition:changeuOut},
% \ref{proposition:existenceFlow},
% \ref{proposition:changevOut}.

%we develop the proof of Theorem \ref{theorem:existence}, given in Section \ref{section:outer}. 
%%
%The proof of the theorem is split between Proposition \ref{proposition:existenceInfty} to Proposition \ref{proposition:changevOut}, see Section \ref{subsection:proofH-existenceInfinite} to Section \ref{subsection:proofH-changevOut} for their proofs.
%%
%Lastly, in Section \ref{subsection:proofH-technical}, are proven the technical results that were postponed in the previous sections.

Throughout this section and the following ones, we denote the components of all 
the functions and operators by a numerical sub-index $f=(f_1,f_2,f_3)^T$, unless 
stated otherwise. 
%
%In order to simplify the notation, we denote by $C$ any positive constant  independent of $\de$ and $\kappa$.}
% to state all the bounds.




==> Article Outer/proofH-existenceChangeuOut.tex <==


In this section, by means of a fixed point argument, we prove Proposition 
\ref{proposition:changeuOut}. That is, we obtain a change of 
variables $\uOut$ satisfying \eqref{eq:equationuOutB}, that is
\begin{equation}\label{eq:InvU}
\partial_v \uOut = R[\uOut]\quad \text{ where }\quad 
  R[\uOut]= \partial_w H_1^{\out}
	\paren{v + \uOut(v), \zuOut(v+\uOut(v))}.
\end{equation}
To this end, we consider the Banach space
\begin{equation}\label{def:Yout}
\YcalOuter = \bigg\{\phiA: \DOuterTilde \to \complexs \st \phiA \text{ real-analytic, }
\normSup{\phiA}:=\sup_{v \in \DOuterTilde} \vabs{\uOut(v)}<\infty \bigg\}.
\end{equation}
%where $\normSup{\cdot}$ is the usual supremum norm in $\DOuterTilde$ (see \eqref{def:DOuterTilde}).
%



% First, we state a technical lemma, whose proof is postponed until Section \ref{subsubsection:ProofcomputationsRRRtransitionOuter}.
% 
% \textcolor{red}{Una altra opci\'o:}

First, we state a technical lemma. Its proof is a  direct consequence of the 
proof of Lemma \ref{lemma:computationsRRROut} (see also Remark \ref{rmk:R} 
in Appendix~\ref{subsubsection:proofComputationsRRROut}).
%
%Fix $\varrho>0$ and define
%\[
%\ballOuterTildeDef = \claus{\varphi \in \YcalOuter \st
%	\normSup{\varphi} \leq \varrho \de^2}.
%\]

\begin{lemma}\label{lemma:computationsRRRtransitionOuter}
Fix $\varrho>0$.
% and let $R$ be as defined in \eqref{def:operatorRRRtransition}.
%
For $\de>0$ small enough and $\varphi \in \YcalOuter$ such that 
$\normSup{\varphi} \leq \varrho \de^2$, 
%
there exists a constant $C>0$  such that
% \begin{align*}
		$\normSup{R[\varphi]}\leq C \de^2$ and  
% 		\qquad
		$\normSup{D R[\varphi]} \leq C \de^2$. 
% \end{align*}
\end{lemma}

%\begin{proof}
%Let us notice that, by \eqref{def:hamiltonianOuterSplit} and applying the corresponding change of variables, we have that
%\begin{align*}
%\Dx{H_1^{\out}}{w} =
%-\frac{\de^2}{3\La_h}
%\Dx{H^{\Poi}_1}{L} \circ \phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out}
%-
%\frac1{3\de^2\La_h} F'_{\pend}(\de^2\La_h(u)-\frac{\de^2 \phi_2(u)}{3\La_h(u)} + \de^4\LtresLa)
%\\
%\Dxx{H_1^{\out}}{w} =
%\frac{\de^4}{9\La_h^2}
%\Dxx{H_1^{\Poi}}{L} \circ \phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out}.
%\end{align*}
%Then, since $(\la_h(u),\La_h(u))$ is bounded for $u \in \DOuterTilde$ (see Theorem \ref{theorem:singularities}),
%we obtain
%\begin{align*}
%\vabs{R[\phiA](u)} &\leq C \de^2 \vabs{\partial_{L} H_1^{\Poi}
%\circ \phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out} (u,\phiA(u))}
%, \\
%\quad
%\vabs{D R[\phiA](u)} &\leq C \de^4 \vabs{\partial^2_{\La} H_1^{\Poi} \circ \phi_{\sca}
%\circ \phi_{\equi} \circ \phi_{\out} (u,\phiA(u))}.
%\end{align*}
%Since $\DOuterTilde$ is at distance of order $1$ of the singularities $u=\pm iA$ of the separatrix, then
%$phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out} (u,\phiA(u))$ is far from collision 
%
%Taking into account the definition of $H_1$ in \eqref{def:hamiltonianScalingH1} we have that
%\begin{align}
%\Dx{H_1}{\La}(\la,\La,x,y;\de)	
%=
%\de^2
%\Dx{H_1^{\Poi}}{\La}(\la,1+\de^2\La,\de x, \de y;\de^4) 
%+
%\frac1{\de^2}F_{\pend}(\de^2\La),
%\end{align}
%such that $F_{\pend}(s)=\OO(s^3)$.
%\end{proof}

Let us define the operators
\begin{equation}\label{def:operatorGGtransitionFlow}
G[\varphi](v) = 
\int_{\rhoOuterTilde}^v \varphi(s) ds,
\qquad \text{and} \qquad
F = G \circ R,
\end{equation}
where $\rhoOuterTilde \in \reals$ is the rightmost vertex of the domain $\DOuterTilde$ (see Figure~\ref{fig:dominisTransition}).
%
Then, a solution $\uOut = F[\uOut]$  satisfies  equation 
\eqref{eq:InvU} and the initial condition $\uOut(\rhoOuterTilde)=0$.

% We prove Proposition \ref{proposition:changeuOut} by means of a fixed point argument for the operator $F$.

\begin{proof}[Proof of Proposition \ref{proposition:changeuOut}]

The  operator $G$ in \eqref{def:operatorGGtransitionFlow} satisfies that, for 
$\varphi \in \YcalOuter$, 
\begin{equation}\label{eq:GlipschitzTransitionFlow}
\normSup{G[\phiA]}\leq C \normSup{\phiA}.
\end{equation}
Then, by Lemma
\ref{lemma:computationsRRRtransitionOuter}, 	
there exists $\cttOuterD>0$ independent of $\de$ such that
\begin{align}\label{proof:firstIterationTransitionOuter}
	\normSup{F[0]} \leq C \normSup{R[0]} 	\leq \frac12 \cttOuterD \de^2.
\end{align}
%
Moreover, for $\phiA,\phiB \in B( \cttOuterD \de^2)
% , Now, we compute the 
% Lipschitz constant of $F$ in $B( \cttOuterD \de^2)
= \claus{\varphi \in 
\YcalOuter \st \normSup{\varphi} \leq \cttOuterD \de^2}$,
%
by  the mean value theorem and Lemma 
\ref{lemma:computationsRRRtransitionOuter},  
\begin{align*}
	\normSup{R[\phiA]-R[\phiB]} = 
	\normSupBig{\int_0^1 DR[s\phiA+(1-s)\phiB]ds} \normSup{\phiA-\phiB}
	\leq C \de^2 
	\normSup{\phiA-\phiB}.
\end{align*}
Then, by Lemma \ref{lemma:computationsRRRtransitionOuter}, 
\eqref{eq:GlipschitzTransitionFlow},  
\eqref{proof:firstIterationTransitionOuter}
and taking $\de$ small enough, 
% we obtain
% \begin{equation}\label{proof:contractiveTransitionOuter}
% 	\begin{split}	
% 		\normSup{F[\phiA]-F[\phiB]}
% 		\leq \frac{1}{2}
% 		\normSup{\phiA-\phiB}.
% 	\end{split}
% \end{equation}	
% Therefore, by \eqref{proof:firstIterationTransitionOuter} and
% \eqref{proof:contractiveTransitionOuter},
$F$ is well defined and contractive in $B( \cttOuterD \de^2)$ and, as a result, 
has a fixed point $\uOut \in B( \cttOuterD \de^2)$.

It only remains to check that 
$v+\uOut(v) \in \DuOutKappa$ for $v \in \DOuterTilde$.
%
Indeed, since $\normSup{\uOut}  \leq  \cttOuterD\de^2$ and ${\DOuterTilde} 
\subset \DuOut$, taking $\de$ small enough the statement is proved.

\end{proof}	

%% THIRD STATEMENT %%%
	
%Now we consider the third statement.
%%
%Let $\Gu=(\la_h+\lah,\La_h+\Lah,\xh,\yh)$.
%%
%Then, applying the changes of coordinates $\phi_{\equi}$ and $\phi_{\out}$ (see \eqref{def:changeEqui} and \eqref{def:changeOuter}) in equation \eqref{eq:uOutParametrizationA}, we obtain
%\begin{align*}
%\lah(v) &= \la_h(v+\uOut(v))-\la_h(v) , 
%\\
%\Lah(v) &=
%\La_h(v+\uOut(v)) - \La_h(v)
%-\frac{\wuOut(v+\uOut(v))}{3 \La_h(v+\uOut(v))}
%+ \de^2 \LtresLa(\de),
%\\
%\xh(v) &= \xuOut(v+\uOut(v)) + \de^3 \Ltresx(\de) 
%\\
%\yh(v) &= \yuOut(v+\uOut(v)) + \de^3 \Ltresy(\de).
%\end{align*}
%Then, since Proposition \ref{proposition:existenceComecocos} implies that $\normSup{\wuOut}\leq C\de^2$ and $\normSup{\xuOut},\normSup{\yuOut}\leq C\de^3$, 
%one can easily obtain the estimates of the third statement.




==> Article Outer/proofH-existenceChangevOut.tex <==

Now we prove Proposition \ref{proposition:changevOut} by obtaining the change of variables $\vOut: \DBoomerangTildeProp \to \complexs$  as a solution of equation \eqref{eq:equationsvOutA}. This equation is equivalent to  $\vOut=\NNN[\vOut]$  with
%
%Let us take into account equation \eqref{eq:equationsvOutA} and that $\dot{\la}_h = -3 \La_h$.
%
\begin{equation*}
\NNN[\phiA](u) =
\frac{1}{3\La_h(u)}
\left[
\lah(u+\phiA(u)) + 
\la_h(u+\phiA(u)) -
\la_h(u)
+3\La_h(u) \phiA(u)
\right].
\end{equation*}
%
We obtain $\vOut$ by means of a fixed point argument in the Banach space
\begin{align*}
\YcalBoom = \bigg\{\phiA: \DBoomerangTildeProp \to \complexs \st \phiA \text{ real-analytic, }
\normSup{\phiA} := \sup_{u\in\DBoomerangTildeProp} \vabs{\phiA(u)}<\infty\bigg\}.
\end{align*}
%
%Thus, in the next proposition, we prove the existence of the change of coordinates $\vOut$ in terms of a fixed point equation of the operator $\NNN$.

%\begin{proposition}\label{proposition:changevOutBanach}
%There exists $\de_0>0$ small enough, such that for $\de \in (0,\de_0)$ 
%%
%the fixed point equation $\vOut=\NNN[\vOut]$ has a unique solution $\vOut \in \YcalBoom$.
%%
%Moreover, there exists a constant $\cttBoomerangTilde>0$ independent of $\de$ such that
%\begin{align*}
%\normSup{\vOut} \leq \cttBoomerangTilde \de^2.
%\end{align*}
%\end{proposition}

\begin{proof}[Proof of Proposition \ref{proposition:changevOut}]
%	
Let us first notice  that, by Theorem \ref{theorem:singularities},
\begin{align}\label{proof:boundsHomoclinicVchange}
C^{-1} \leq \normSup{\La_h}  \leq C.
%\qquad
%\sup_{v \in \DFlow}|\dot{\La}_h(v)| \leq C.
\end{align}

% Next, we obtain an estimate for $\NNN[0]$. 
%
Since $\dBoomerangTilde<\dFlow$ and
$\kappaBoomerangTilde>\kappaFlow$, we have that
$
{\DBoomerangTildeProp} \subset \DFlow,
$
%
(see \eqref{def:domainBoomerangTilde} and \eqref{def:dominiFlow}).	
%
Then,  applying Proposition \ref{proposition:existenceFlow},
%
 there exists $b_6>0$ independent of $\de$ such that
\begin{align*}
%\label{proof:firstIterationTransitionBoomerang}
\normSup{\NNN[0]} 
%= \normSupBig{\frac{\lah(u)}{3 \La_h(u)}}
\leq \frac13 \normSup{(\La_h)^{-1}} \normSup{\lah} \leq \frac12 b_6 \de^2.
\end{align*} 	
%
Next, we compute the Lipschitz constant of $\NNN$ in $B(b_6\delta^2) = \{\phiA \in \YcalBoom \st \normSup{\phiA}\leq b_6 \de^2\big\}$.
%
By the mean value theorem, for $\phiA,\phiB \in B(b_6\delta^2)$ and $\phiA_s=(1-s)\phiA+s\phiB$, we have that
\begin{align*}
\normSup{\NNN[\phiA]-\NNN[\phiB]} 
\leq&
% \sup_{s \in [0,1]}
\sup_{u \in \DBoomerangTildeProp}
\vabs{\int_0^1 D\NNN[\phiA_s](u) ds} 
\normSup{\phiA-\phiB}.	
\end{align*}
For $u \in \DBoomerangTildeProp$ and $\de$ small enough, we have that $u+\phiA_s(u) \in \DFlow$.
%
Therefore, by Proposition \ref{proposition:existenceFlow}, \eqref{proof:boundsHomoclinicVchange}
and recalling that $\dot{\la}_h=-3\La_h$,
\begin{align*}
\vabs{D\NNN[\phiA_s](u)}
&\leq
\frac{1}{3\vabs{\La_h(u)}}
\claus{
|\partial_v \lah(u + \phiA_s(u))|
+
\vabs{\La_h(u + \phiA_s(u))-\La_h(u)}
} 
%\\
%&\leq
%C \sup_{v \in \DFlow} 
%|\partial_v \lah(v)| +
%C 
%\sup_{v \in \DFlow} |\dot{\La}_h(v)| \,
%\normSup{\phiA_s} 
%
\leq C\de^2,
\end{align*}
and, taking $\de$ small enough,
$\normSup{\NNN[\phiA]-\NNN[\phiB]}\leq \frac{1}{2}  \normSup{\phiA - \phiB}$.
%
%\begin{align}\label{proof:contractiveTransitionBoomerang}
%\normSup{\NNN[\phiA]-\NNN[\phiB]} 
%\leq C \de^2  \normSup{\phiA - \phiB}
%\leq \frac{1}{2}  \normSup{\phiA - \phiB}.
%\end{align}
%
Therefore, the operator $\NNN$ is well defined and contractive in $B(b_6\delta^2)$ and, as a result, has a fixed point $\vOut \in B(b_6\delta^2)$.

Besides, since 
$
{\DBoomerangTildeProp} \subset \DFlow,
$
%
we obtain that $u+\vOut(u) \in \DFlow$ for $u \in \DBoomerangTildeProp$ and $\de$ small enough.

%
%\begin{equation}\label{proof:changevOutStatement2}
%u+\vOut(u) \in \DFlow, 
%\quad \text{for} \quad
%v \in \DOuterTilde.
%\end{equation}
\end{proof}


==> Article Outer/proofH-existenceFlow.tex <==


In this section, we  extend analytically the parametrization $\Gu$ given in Corollary \ref{corollary:changeuOut} from the transition domain $\DuOut$ to the flow domain  $\DFlow$ (see \eqref{def:dominiFlow}).

Since $\Gu$ satisfies the equations given by $H$ in \eqref{def:hamiltonianScaling}, $\Gh=\Gu-\G_h$ (see \eqref{eq:splitParametrizationGu}) satisfies
\begin{align*}
%\label{eq:diffEquationFlow}
\left\{
\begin{aligned}	
\partial_v \lah &= -3\Lah 
+ \partial_{\La} H_1 (\G_h + \Gh;\de), \\
%
\partial_v \Lah &= 
-V'(\la_h+\lah)
+V'(\la_h)
- \partial_{\la} H_1 (\G_h + \Gh;\de), \\
%
\partial_v \xh &= 
i \frac{\xh}{\de^2}
+ i\partial_{y} H_1 (\G_h + \Gh;\de), \\
%
\partial_v \yh &= 
-i \frac{\yh}{\de^2}
- i\partial_{x} H_1 (\G_h + \Gh;\de),
\end{aligned}
\right.
\end{align*} 
%Along this section, we denote the components of all the functions and operators by a numerical sub-index $f=(f_1,f_2,f_3, f_4)$, unless stated otherwise. 
%
which can be rewritten as
% Then $\Gh$ satisfies \eqref{eq:diffEquationFlow},
%  if and only if 
 $\LL^{\flow} \, \Gh = \RRR^{\flow}[\Gh]$,
where
% Let us define the operators,
\begin{equation}\label{def:operatorLLFlow}
\LL^{\flow} \phiA = 
\paren{\partial_v - \AAA^{\flow}(v)} \phiA,
%	
\qquad
\AAA^{\flow}(v) = \begin{pmatrix}
	0 & -3 & 0 & 0 \\
	-V''(\la_h(v)) & 0 & 0 & 0 \\
	0 & 0 & \frac{i}{\de^2} & 0  \\
	0 & 0 & 0 & -\frac{i}{\de^2} 
\end{pmatrix},
\end{equation}
and
\begin{equation}\label{def:operatorRFlow}
%	
\RRR^{\flow}[\phiA](v) = 
\begin{pmatrix}
	\partial_{\La} H_1 (\G_h(v)+\phiA(v);\de) \\ 
	T[\phiA_1](v)-\partial_{\la} H_1 (\G_h(v)+\phiA(v);\de) 
	\\
	i\partial_{y} H_1 (\G_h(v)+\phiA(v);\de) 
	\\
	-i\partial_{x} H_1 (\G_h(v)+\phiA(v);\de) \\
\end{pmatrix},	
\end{equation}
with
$T[\phiA_1] = -V'(\la_h+\phiA_1) +V'(\la_h)
+ V''(\la_h)\phiA_1 $.
%
%\begin{align}\label{def:operatorGFlow}
%T[\phiA_1] = 
%-V'(\la_h+\phiA_1)
%+V'(\la_h)
%+ V''(\la_h)\phiA_1.
%\end{align}
%
%


We look for $\Gh$ through fixed point argument in the Banach space $\XcalFlowTotal = \paren{\XcalFlow}^4
$, where 
%
%Let us consider the norm:
%\begin{align}
%\normFlow{\phiA} = \sup_{v \in \DFlow} \vabs{\phiA(v)},
%\end{align}
%%Let us consider the Banach space,
\begin{align*}
\XcalFlow = \bigg\{\phiA: \DFlow \to \complexs \st
 \phiA \text{ real-analytic, }
 \normFlow{\phiA}:=\sup_{v\in\DFlow}\vabs{\phiA(v)} < \infty \bigg\},
\end{align*}
endowed with the norm
\[
\normFlowTotal{\phiA} = \de \normFlow{\phiA_1}
+ \de \normFlow{\phiA_2}
+ \normFlow{\phiA_3} + \normFlow{\phiA_4}.
\]
%
% First, we consider .
%
A fundamental matrix of the linear equation $\dot{\xi} = \AAA^{\flow}(v) \xi$ is
\begin{align*}
	%\label{eq:fundamentalMatrixFlow}
\MoveEqLeft 	
\Phi(v) = \begin{pmatrix}
	3\La_h(v) & 3f_h(v) & 0 & 0  \\
	-\dot{\La}_h(v) & -\dot{f}_h(v) & 0 & 0 \\
	0 & 0 & e^{\frac{i}{\de^2} v} & 0 \\
	0 & 0 & 0 & e^{-\frac{i}{\de^2} v}
\end{pmatrix}
\, \text{with } \,
f_h(v) = \La_h(v) \int_{v_0}^{v} \frac{1}{\La_h^2(s)} ds.
\end{align*}
Note that $f_h(v)$ is analytic at $v=0$.
%Moreover, for $v \in \DFlow$, the inverse $\Phi^{-1}(v)$ is well defined and
%\begin{align*}
%	\normFlow{\Phi_{j,l}} \leq C, \qquad
%	\normFlow{(\Phi)^{-1}_{j,l}} \leq C, \qquad
%	\text{for } j,l \in \claus{1,2}.
%\end{align*}

To look for a right inverse of operator $\LL^{\flow}$ in \eqref{def:operatorLLFlow}, 
%
let us consider the linear operator
\begin{align*}
\GG^{\flow}[\phiA](v) = \paren{
	\int_{v_0}^v \phiA_1(s) ds,
	\int_{v_0}^v \phiA_2(s) ds,
	\int_{\conj{v}_1}^v \phiA_3(s) ds,
	\int_{{v}_1}^v \phiA_4(s) ds
}^T,
\end{align*}
where $v_0$, $v_1$ and $\conj{v}_1$ are the vertexs of the domain $\DFlow$ 
%
(see Figure \ref{fig:dominisTransition}).
%
Then, the linear operator
% \begin{align*}%\label{def:operatorGGhFlow}
$\GGh[\phiA] =  \Phi \GG[\Phi^{-1}\phiA]$
% \end{align*}
is a right inverse of the operator $\LL^{\flow}$,
and, 
for $\phiA \in \XcalFlowTotal$, satisfies 
\begin{align}\label{eq:operatorGGhFlow}
\normFlow{\GGh_1[\phiA]} + \normFlow{\GGh_2[\phiA]} \leq C \paren{
\normFlow{\phiA_1} + \normFlow{\phiA_2}},
\quad
\normFlow{\GGh_j[\phiA]} \leq C\de^2\normFlow{\phiA_j} \,
\text{for } j=3,4.	
\end{align}

%
Next, we state a technical lemma providing estimates for $\RRR^{\flow}$.
%
% Its proof is postponed until Section~\ref{subsubsection:ProofComputationsRFlow}.
% 
% \textcolor{red}{O tamb\'e podem dir:}
Its proof is a direct consequence of the definition of the operator in \eqref{def:operatorRFlow} and Corollary \ref{corollary:seriesH1Poi}, which gives estimates for $H_1^{\Poi}$ in \eqref{def:hamiltonianPoincare} (see also the change of coordinates \eqref{def:changeScaling} which relates  $H_1^{\Poi}$ and $H_1$).
%
%First, for a fixed $\varrho>0$, we define
%\begin{align*}
%	\ballFlowDef = \claus{\phiA \in \XcalFlowTotal \st \normFlowTotal{\phiA} \leq \varrho}.
%\end{align*}

\begin{lemma}\label{lemma:computationsRFlow}
Fix $\varrho>0$ and consider $\phiA \in \XcalFlowTotal$ with $\normFlowTotal{\phiA} \leq \varrho \de^3$. Then, for $\de>0$ small enough , there exists a constant $C>0$  such that  the  operator $\RRR^{\flow}$  in \eqref{def:operatorRFlow} satisfies
	\begin{align*}
		\normFlow{\RRR^{\flow}_1[\phiA]},\normFlow{\RRR^{\flow}_2[\phiA]} &\leq C \de^2,
		 \qquad
		%
		\normFlow{\RRR^{\flow}_3[\phiA]},\normFlow{\RRR^{\flow}_4[\phiA]} \leq C \de,\\
		%
		\normFlow{D_j \RRR^{\flow}_l[\phiA]} &\leq C \de, 
		\qquad
		j,l \in \claus{1,2,3,4}.
	\end{align*}
\end{lemma}


Denote by $\mathbf{e}_j$, $j=1,2,3,4$, the canonical basis in $\mathbb{R}^4$. Noticing that, by Corollary~\ref{corollary:changeuOut}, the function $\Gh=(\lah,\Lah,\xh,\yh)$ is already defined at $\claus{v_0,v_1,\conj{v}_1} \in \DOuterTilde$, we can consider the function
% \begin{equation}\label{eq:initialConditionFlow}
\[
\begin{split}
	F^0(v) = \Phi(v)  \left[
	\Phi^{-1}(v_0)\left(
	\lah(v_0)\mathbf{e}_1+ \Lah(v_0)\mathbf{e}_2\right)
	+\xh(\conj{v}_1) \Phi^{-1}(\conj{v}_1) \mathbf{e}_3
	+ \yh({v_1})\Phi^{-1}({v_1}) 
	\mathbf{e}_4
	\right].
\end{split}
\]
% \end{equation}
Then, since $\GGh(F^0)=0$, 
 it only remains to check that
% \begin{equation}\label{def:operatorFFflow}
$\FF = F^0 + \GGh \circ \RRR^{\flow}$
% \end{equation}
is contractive in a suitable ball of $\XcalFlowTotal$.

%The solution $\Gh = \FF[\Gh]$	satisfies  equation \eqref{eq:diffEquationFlow} and it is an analytic continuation of the solution obtained in Proposition~\ref{proposition:changeuOut}.
%
%Thus, we can rewrite Proposition \ref{proposition:existenceFlow} in terms of the operator $\FF$ defined on the Banach space $\XcalFlowTotal$.
%
%\begin{proposition}\label{proposition:existenceFlowBanach}
%There exists $\de_0>0$ such that for $\de \in (0,\de_0)$ and $\kappa>0$ the fixed point equation $\Gh = \FF[\Gh]$ has a unique solution $\Gh \in \XcalFlowTotal$.
%
%Moreover, there exists a real constant $\cttFlowA>0$ independent of $\de$ such that
%\begin{align*}
%\normFlowTotal{\Gh} \leq \cttFlowA \de^3.
%\end{align*}
%\end{proposition}

%We prove Proposition~\ref{proposition:existenceFlowBanach} through a fixed point argument.

\begin{proof}[End of proof of Proposition~\ref{proposition:existenceFlow}]
%
First, we obtain a suitable estimate for $\FF[0]$. 
%
Applying  Propositions \ref{proposition:existenceComecocos} and  \ref{proposition:changeuOut} and using  \eqref{eq:equationuOutA} we obtain that,
for $v \in \DOuterTilde$,
\begin{align*}
	\vabsSmall{\lah(v)} \leq C \de^2, \qquad
	\vabsSmall{\Lah(v)} \leq C \de^2, \qquad
	\vabsSmall{\xh(v)} \leq C \de^3, \qquad
	\vabsSmall{\yh(v)} \leq C \de^3.
\end{align*}
Therefore, since $\claus{v_0,v_1,\conj{v}_1} \in \DOuterTilde$,
\begin{align*}
%\label{proof:initialConditionBoundFlow}
	\normFlowTotal{F^0} &\leq
	%
	C\de \vabsSmall{\lah(v_0)}+
	C\de \vabsSmall{\Lah(v_0)}+
	C \vabs{\xh(\conj{v}_1)}+
	C \vabs{\yh({v_1})} \leq C \de^3,
\end{align*}
%
%We are looking for fixed points of $\varphi=\FF[\varphi]$.
%
%Then, we obtain an estimate for $\FF[0]$. 
%
and, applying \eqref{eq:operatorGGhFlow} and Lemma \ref{lemma:computationsRFlow}, there exists $\cttOuterF>0$ independent of $\de$ such that 
\begin{align}\label{proof:operadorFF0Flow}
	\normFlowTotal{\FF[0]} \leq 
	\normFlowTotal{F^0} +
	\normFlowTotal{\GG \circ \RRR^{\flow}[0]} \leq \frac12 \cttOuterF \de^3.
\end{align}
%
%Moreover, we fix constant $\varrho>0$ such that $\normSup{\FF[0]}\leq \frac{1}{2}\varrho\de^3$.
Let us define $B(\cttOuterF \de^3)= \claus{\phiA \in \XcalFlowTotal \st \normFlowTotal{\phiA} \leq \cttOuterF \de^3}$.
%
%Then, we compute the Lipschitz constant of $\FF$ in $\ballFlow$.
%
By the mean value theorem and Lemma~\ref{lemma:computationsRFlow}, for $\phiA, \phiB \in B(\cttOuterF \de^3)$ and $j=1,..,4$, we obtain
%
%\begin{align*}
%\RRR^{\flow}[\phiA]-\RRR^{\flow}[\phiB] 
%= \boxClaus{\int_0^1 D\RRR^{\flow}[s {\phiA} + (1-s) \phiB] d s} (\phiA - \phiB),
%\end{align*}
%and applying Lemma~\ref{lemma:computationsRFlow}, for $j=1,..,4$, we obtain
\begin{align*}
\normFlow{\RRR^{\flow}_j[\phiA]-\RRR^{\flow}_j[\phiB]}&\leq
%
\sum_{l=1}^4 \boxClaus{
\sup_{\zeta \in B(\cttOuterF \de^3)} \claus{
\normFlow{D_l \RRR^{\flow}_j[\zeta]} }
\normFlow{\phiA_l-\phiB_l}
} 
%&\leq 
%C \de \normFlow{\phiA_1-\phiB_1} +
%C \de \normFlow{\phiA_2-\phiB_2} +
%C \normFlow{\phiA_3-\phiB_3} +
%C \de \normFlow{\phiA_4-\phiB_4} +
\leq C  \normFlowTotal{\phiA-\phiB}.
\end{align*}
%and applying Lemma~\ref{lemma:computationsRFlow}, we obtain
%\begin{align*}
%\normFlow{R_1[\phiA]-R_1[\phiB]}
%&\leq C \de \normFlowTotal{\phiA-\phiB}, &
%%
%\normFlow{R_2[\phiA]-R_2[\phiB]}
%&\leq C \de \normFlowTotal{\phiA-\phiB}, \\
%%
%\normFlow{R_3[\phiA]-R_3[\phiB]}
%&\leq C \normFlowTotal{\phiA-\phiB}, &
%%
%\normFlow{R_4[\phiA]-R_4[\phiB]}
%&\leq C \normFlowTotal{\phiA-\phiB}. 
%\end{align*}
Then, by \eqref{eq:operatorGGhFlow} and taking $\de$ small enough,  
\begin{equation}\label{proof:operadorFFLipschitzFlow}
\begin{split}
\normFlowTotal{\FF[\phiA]-\FF[\phiB]}
\leq& \, 
C\de \boxClaus{ \sum_{j=1}^2 \normFlow{\RRR^{\flow}_j[\phiA]-\RRR^{\flow}_j[\phiB]}}
%\\ &+
+ C\de^2 \boxClaus{ \sum_{l=3}^4 \normFlow{\RRR^{\flow}_l[\phiA]-\RRR^{\flow}_l[\phiB]}}
\\
\leq& \, 
C \de\normFlowTotal{\phiA-\phiB} \leq
\frac{1}{2}\normFlowTotal{\phiA-\phiB}.
\end{split}
\end{equation}

Therefore, by \eqref{proof:operadorFF0Flow} and
\eqref{proof:operadorFFLipschitzFlow},
$\FF$ is well defined and contractive in $B(\cttOuterF \de^3)$ and, as a result, has a fixed point $\Gh \in B(\cttOuterF \de^3)$.
\end{proof}



==> Article Outer/proofH-existenceInfinite.tex <==

The first step is to prove 
Proposition~\ref{proposition:existenceInfty}, which deals with the proof of the existence of 
parameterizations $\zuOut$ and $\zsOut$ satisfying the invariance equation 
\eqref{eq:invariantEquationOuter} and the asymptotic conditions 
\eqref{eq:asymptoticConditionsOuter}.
%
We only consider the $-\unstable-$ case, being the $-\stable-$ case analogous.

Consider the invariance equation \eqref{eq:invariantEquationOuter},
% \begin{equation}\label{eq:invariantEquationInftyA}
$\partial_u \zuOut = 	\AAA^{\out} \zuOut + \RRR^{\out}[\zuOut]$,
% \end{equation}
with $\AAA^{\out}$ and $\RRR^{\out}$ defined in \eqref{def:matrixAAAOuter} and \eqref{def:operatorRRROuter}, respectively.
%
%Introducing the linear operator
%\begin{equation}\label{def:operatorL}
%	\LL \phiA = (\partial_u-\AAA^{\out})\phiA ,
%\end{equation}
This equation can be written as
\begin{equation}\label{eq:invariantEquationInftyB}
	\LL \zuOut = \RRR^{\out}[\zuOut],
	\qquad \text{with} \qquad
	\LL \phiA = (\partial_u-\AAA^{\out})\phiA.
\end{equation}
%
In order to obtain a fixed point equation from 
\eqref{eq:invariantEquationInftyB}, we look for a left 
inverse of $\LL$ in a suitable Banach space.
%
To this end, for a fixed $\rhoInfty>0$ and a  given $\al \in \reals$, we introduce
\[
\XcalInfty_{\al} = \bigg\{ \varphi:\DuInfty  \to \complexs \st \varphi \text{ real-analytic, } 
\normInfty{\varphi}_{\al} := \sup_{u \in \DuInfty} 
|e^{-\al u} \varphi(u)| < \infty \bigg\},
\]
%\[
%\normInfty{\varphi}_{\al} = \sup_{u \in \DuInfty} 
%|e^{-\al u} \varphi(u)|,
%\]
and the product space
$
\XcalInftyTotal= 
\XcalInfty_{2\vap} \times 
\XcalInfty_{\vap} \times 
\XcalInfty_{\vap},
$
with $\nu = \sqrt\frac{21}{8}$
endowed with the weighted product norm
\[
\normInftyTotal{\varphi}= 
\de \normInfty{\varphi_1}_{2\vap} + \normInfty{\varphi_2}_{\vap} + 
\normInfty{\varphi_3}_{\vap}.
\]

Next lemmas, proven in \cite{BFGS12}, give some properties of these Banach 
spaces and provide a left inverse operator of $\mathcal L$. 
%
\begin{lemma}\label{lemma:sumNormsOutInf}
Let $\al, \beta \in \reals$. Then, the following statements hold:
\begin{enumerate}
	\item If $\al>\beta\geq 0$, then $\XcalInfty_{\al} \subset \XcalInfty_{\beta}$. Moreover
	$
	\normInfty{\varphi}_{\beta} \leq \normInfty{\varphi}_{\al}.
	$
	\item If  $\varphi \in \XcalInfty_{\al}$ and $\zeta \in \XcalInfty_{\beta}$, then
	$\varphi \zeta  \in \XcalInfty_{\al+\beta}$ and
	$
	\normInfty{\varphi\zeta}_{\al+\beta} \leq \normInfty{\varphi}_{\al} \normInfty{\zeta}_{\beta}.
	$
\end{enumerate}
\end{lemma}
%\begin{proof}
%	It follows the same lines as the proof of Lemma 6.1 in~\cite{BFGS12}.
%\end{proof}
%Let us consider the singular problem given by Hamiltonian $H_{\pend}(\la,\La)$, as defined on~\eqref{def:HpendHosc}.
%

% In the following lemma we introduce a left-inverse operator of $\LL$.
%

\begin{lemma}\label{lemma:GlipschitzInfinity}
The linear operator $\GG: \XcalInftyTotal \to \XcalInftyTotal$ given by
\[
\GG[\varphi](u) = \left(\int_{-\infty}^u \varphi_1(s) ds, 
\int_{-\infty}^u e^{-\frac{i}{\de^2} (s-u)} \varphi_2(s) ds , 
\int_{-\infty}^u e^{\frac{i}{\de^2} (s-u)} \varphi_3(s) ds \right)^T
\]
%
is continuous, injective and is a left inverse of the operator $\LL$. 

Moreover, there exists a constant $C$ independent of $\de$ and $\rhoInfty$ such that, for $\varphi \in \XcalInftyTotal$, 
%\begin{align*}
%\norm{\GG_1 [h]}_{2\vap} \leq 	C_{\vap} \norm{h_1}_{2\vap}, \qquad
%%
%\norm{\GG_2 [h]}_{\vap} \leq C_{\vap}
%\de^2 \norm{h_2}_{\vap}, \qquad
%%
%\norm{\GG_3 [h]}_{\vap} \leq C_{\vap}
%\de^2 \norm{h_3}_{\vap}.
%\end{align*} 
\begin{align*}
\normInftyTotal{\GG[\phiA]} \leq C
\paren{\normInfty{\varphi_1}_{2\vap} +
\de^2 \normInfty{\varphi_2}_{\vap} +
\de^2 \normInfty{\varphi_3}_{\vap}}.
\end{align*}
\end{lemma}

% \begin{proof}
% It follows the same lines as the proof of Lemma 6.2 in~\cite{BFGS12}.
% \end{proof}

%\begin{proof}
%	Let us assume $z, h \in \XX$ such that $\LL z = h$. Hence, 
%	\begin{align*}
%		\partial_u w = h_1,\hh
%		\partial_u x + \frac{i}{\de^2} x = h_2,  \hh
%		\partial_u y -\frac{i}{\de^2} y = h_3.
%	\end{align*}
%	On the first equation, using that $h_1 \in \XX_{2\rho}$ (and thus decays exponentially) and that we want $\GG_1[h_1]\in \XX_{2\rho}$ one can define
%	%From the first equation we obtain
%	%\[
%	% w(u) = w_0 + \int_{\G_1(u)} h_1(s) ds,
%	%\]
%	%where $\G_1(u) \subset \Dinfty$ is a complex path from infinity to $u$. From equation~\eqref{eq:stableuncondition} the graph for the unstable invariant manifold has to satisfy
%	%\[
%	%\lim_{\Re(u) \to -\infty } |w(u)| = 0 \implies w_0=0.
%	%\]
%	%Then
%	\[
%	\GG_1[h_1](u) =\int_{-\infty}^u h_1(s) ds.
%	\]
%	%On the second equation we can apply the method of variation of parameters, then
%	%\[
%	% x(u) = x_0 e^{-\frac{i}{\de^2} u} + \int_{\G_2(u)} e^{\frac{i}{\de^2} (s-u)} h_2(s) ds.
%	%\]
%	%where $\G_2(u) \subset \Dinfty$ is a complex path from infinity to $u$. Considering we are computing the operator for the unstable invariant manifold, it has to satisfy
%	%\[
%	%\lim_{\Re(u) \to -\infty } |x(u)| = |x_0| e^{\frac{1}{\de^2} \Im(u)} = 0 \implies x_0 = 0.
%	%\]
%	%Then,
%	On the second equation, using the same argument as before and the method of variation of parameters one can define 
%	\[
%	\GG_2[h_2](u) = \int_{-\infty}^u e^{\frac{i}{\de^2} (s-u)} h_2(s) ds.
%	\]
%	Analogously for the third equation. 
%	%\[
%	% \GG_3[h_3](u) = y(u) = \int_{\G_3(u)} e^{-\frac{i}{\de^2} (s-u)} h_3(s) ds,
%	%\]
%	%where $\G_3(u) \subset \Dinfty$ is a complex path from infinity to $u$. To sum it up, we have that
%	% \[
%	%  \LL z = \left(\partial_u w, \partial_u x + \frac{i}{\de^2} x , \partial_u y -\frac{i}{\de^2} y\right).
%	% \]
%	% and
%	%\[
%	% \GG[h] = \left(\int_{\G_1(u)} h_1(s) ds, 
%	% \int_{\G_2(u)} e^{\frac{i}{\de^2} (s-u)} h_2(s) ds , 
%	% \int_{\G_3(u)} e^{-\frac{i}{\de^2} (s-u)} h_3(s) ds \right).
%	%\]
%	%which is a linear and continuous operator. 
%	Now, we proceed by checking the bounds of operators $\GG_1,\GG_2$ and $\GG_3$. Let us assume $h_1 \in \XX_{2\rho}$, then 
%	\begin{align*}
%		|| \GG_1[h_1] ||_{2\rho} =&  \sup_{u \in \DOutInf} \left| e^{-2\rho u}  \int_{-\infty}^u h_1(s) ds \right| 
%		\leq  \norm{h_1}_{2\rho} \sup_{u \in \DOutInf}  \left| e^{-2\rho \Re(u)} \int_{-\infty}^u e^{2\rho s} ds \right|
%		= \frac{\norm{h_1}_{2\rho}}{2\rho}.  
%	\end{align*}
%	%we apply the the change of variables $v=\varphi_u(s):=s-u$, then
%	%\[
%	% \GG_1 [h](u) =  \int_{\G_1(0)} h(v+u) dv,
%	% \]
%	%where $\G_1(0) \subset \varphi_u(\Dinfty)$ is a complex path from infinity to $0$. 
%	%Because $h \in \XX_{2\rho}$, there are no singularities on the region $\Dinfty$ where the function is evaluated. Therefore, all the paths will give the same integral, thus we can select the following path
%	%\[
%	% \ol{\G}_1^R:= \left\{ v \in \complexs \text{ : } v = r, \h r\in[R,0] \right\},
%	%\]
%	%to compute the integral. Then, operator $\GG_1$ can be rewritten as
%	%\begin{align*}
%	% \GG_1 [h](u) = \int_{-\infty}^0 h(u+r) dr. 
%	%\end{align*}
%	%Then, to find its norm
%	% \begin{align*}
%	% || \GG_1[h] ||_{2\rho} =&
%	%  \sup_{u \in \Dinfty} \left| e^{-2\rho u}  \int_{-\infty}^0 h(u+r) dr \right| =
%	%  \sup_{u \in \Dinfty} \left| \int_{-\infty}^{0} e^{2\rho r} e^{-2\rho (u+r)} h(u+r) dr \right| \\[0.6em]  
%	% =& || h ||_{2\rho} \sup_{u \in \Dinfty} \left| \int_{-\infty}^{0} e^{2\rho r} \right|  %\\[0.6em]
%	% = \frac{1}{2\rho} || h ||_{2\rho}. %= \sqrt{\frac{2}{21}} || h ||_{2\rho} \leq || h ||_{2\rho}.
%	% \end{align*}
%	For $\GG_2$, let $R>0$ be a constant big enough and $h_2 \in \XX_{\rho}$. We define the complex path
%	\[
%	\G_2^R:= \left\{ v \in \complexs \st v=r e^{i(\pi-\frac{\beta}{2})}, \h r \in [0,R] \right\}.
%	\]
%	Then, the linear operator $\GG_2$,  can be rewritten as
%	\[
%	\GG_2 [h_2](u) = - \lim_{R \to \infty} \int_{\G_2^R}  e^{\frac{i}{\de^2} v} h_2(v+u) dv ,
%	\]
%	for $u \in \DOutInf$. Now, parametrizing curve $\G_2^R$, we can bound the operator as
%	\begin{align*}
%		|| \GG_2 [h_2] ||_{\rho} 
%		%
%		=& \sup_{\DOutInf} \left| e^{-\rho u}  \int_{0}^{+\infty}  e^{\frac{i}{\de^2} r e^{i(\pi-\frac{\beta}{2})} } h_2(u+r e^{i(\pi-\frac{\beta}{2})}) e^{i(\pi-\frac{\beta}{2})} dr \right| \leq \\
%		%
%		\leq& \sup_{u \in \DOutInf} \left\{ \norm{h_2}_{\rho}  \left| \int_{0}^{+\infty}  e^{-\frac{r}{\de^2} \sin(\frac{\beta}{2})} \left|e^{\rho r e^{i(\pi-\frac{\beta}{2})}} \right| dr \right| \right\} \leq \\
%		%
%		\leq& \sup_{u \in \DOutInf} \left\{ \norm{h_2}_{\rho} \left| \int_{0}^{+\infty}  e^{-\frac{r}{\de^2} \sin(\frac{\beta}{2})} dr \right| \right\}
%		%
%		=  \frac{\de^2}{\sin(\beta/2)} \norm{h_2}_{\rho}. \\
%	\end{align*}
%	Analogously for operator $\GG_3$.
%\end{proof}


Notice that the eigenvalues of the saddle point $(0,0)$ of $H_{\pend}(\la,\La)$ (see \eqref{def:HpendHosc}) are 
$
\pm \sqrt{\frac{21}{8}}.
$
Then, the parametrization of the separatrix  $\sigma =(\la_h,\La_h)$ (see 
\eqref{eq:separatrixParametrization}) satisfies 
\begin{equation}\label{eq:separatrixBanachSpace}
	\la_h \in \XcalInfty_{\vap}
	\quad \text{ and } \quad
	\La_h \in \XcalInfty_{\vap}.
\end{equation}
Therefore, $\zuOut$ is a solution of \eqref{eq:invariantEquationInftyB} 
satisfying the asymptotic conditions \eqref{eq:asymptoticConditionsOuter} if 
and only if $\zuOut \in \XcalInftyTotal$ and satisfies the fixed point equation
\begin{equation*}
%\label{def:operatorFFInf}
	\phiA = \FF[\phiA] = \GG \circ \RRR^{\out}[\phiA].
\end{equation*}
%where the operator $\RRR^{\out}$ is defined in~\eqref{def:operatorRRROuter}.
%
%Then, a solution of $\zuOut = \FF[\zuOut]$ satisfies  equation \eqref{eq:invariantEquationOuter} and the asymptotic condition~\eqref{eq:asymptoticConditionsOuter}. 
%
Thus, Proposition~\ref{proposition:existenceInfty} is a 
straightforward consequence of the following proposition.

\begin{proposition}\label{proposition:existenceInftyBanach}	
There exists $\de_0>0$ such that, for $\de \in (0,\de_0)$, equation $\phiA = 
\FF[\phiA]$  has a  solution $\zuOut \in \XcalInftyTotal$. 	
%
Moreover, there exists a real constant $\cttOutInftyA>0$ independent of $\de$ such that
$
\normInftyTotal{\zuOut} \leq \, \cttOutInftyA \de^3.
$
\end{proposition}

To see that $\FF$ is a contractive operator, we have to pay attention to the 
nonlinear terms $\RRR^{\out}$.
%
% The nonlinear operator $\RRR^{\out}$ satisfies the following properties.


\begin{lemma}\label{lemma:computationsRRRInf}
Fix $\varrho>0$ and let $\RRR^{\out}$ be the operator defined in~\eqref{def:operatorRRROuter}.
%  
Then, for $\de>0$ small enough\footnote{To simplify the exposition, in this 
lemma and in the  technical lemmas from now on,  we avoid referring 
to the existence of $\de_0$ and just mention that $\delta$ must be small 
enough. We follow the same convention for $\kappa$ whenever is needed.}
and $\normInftyTotal{\varphi}\leq \varrho 
\de^3$, there exists a constant $C>0$ such that
\begin{align*}
\normInfty{\RRR^{\out}_1[\varphi]}_{2\vap} \leq C \de^2, \qquad
%
\normInftySmall{\RRR^{\out}_j[\varphi]}_{\vap} \leq C \de, \qquad
%
j= 2,3,
%\normInfty{\RRR^{\out}_3[\varphi]}_{\vap} \leq C_{\varrho} \de.
\end{align*}
and
\begin{align*}
%\begin{array}{lll}
\normInfty{\partial_w {\RRR^{\out}_1} [\varphi]}_0 &\leq C \de^2, &
\normInfty{\partial_x {\RRR^{\out}_1} [\varphi]}_{\vap} &\leq C \de, &
\normInfty{\partial_y {\RRR^{\out}_1} [\varphi]}_{\vap} &\leq C \de, \\
%
\normInftySmall{\partial_w {\RRR^{\out}_j} [\varphi]}_{-\vap} &\leq C \de, &
\normInftySmall{\partial_x {\RRR^{\out}_j} [\varphi]}_0 &\leq C, &
\normInftySmall{\partial_y{\RRR^{\out}_j} [\varphi]}_0 &\leq C, \quad j=2,3.
%\end{array}
%\normInftySmall{\partial_w {\RRR^{\out}_3} [\varphi]}_{-\vap} &\leq C \de, &
%\normInftySmall{\partial_x {\RRR^{\out}_3} [\varphi]}_0 &\leq C \de, &
%\normInftySmall{\partial_y{\RRR^{\out}_3} [\varphi]}_0 &\leq C, 
\end{align*}
\end{lemma}

The proof of this lemma is postponed to 
Appendix~\ref{subsubsection:ProofComputationsRRRInf}.

\begin{proof}[Proof of Proposition~\ref{proposition:existenceInftyBanach}]

Consider the closed ball
\begin{equation*}
%\label{def:ballInfty}
	\ballInftyDef= \claus{\varphi \in \XcalInftyTotal \st \normInftyTotal{\varphi} \leq \varrho}.
\end{equation*}
%
First,  we obtain an estimate for $\FF[0]$. By Lemmas 
\ref{lemma:GlipschitzInfinity} and \ref{lemma:computationsRRRInf}, if $\delta$ 
is small enough,
\begin{align}\label{eq:firstIterationInfty}
\normInftyTotal{\FF[0]} \leq
C \de   \normInfty{\RRR^{\out}_1[0]}_{2\nu} +
C \de^2 \normInfty{\RRR^{\out}_2[0]}_{\nu} +
C \de^2 \normInfty{\RRR^{\out}_3[0]}_{\nu}
\leq \frac12 \cttOutInftyA \de^3,
\end{align}
for some $\cttOutInftyA>0$.

Then, it only remains to check that the operator $\FF$ is contractive in 
$B(\cttOutInftyA\de^3)$.
%
Let $\phiA, \phiB \in B(\cttOutInftyA\de^3)$.  
%
Then, by the mean value theorem, 
\begin{align*}
\RRR_j^{\out}[\varphi]-\RRR_j^{\out}[\wt{\varphi}] 
= \boxClaus{\int_0^1 D{\RRR_j^{\out}}[s {\varphi} + (1-s) \wt{\varphi}] d s} ({\varphi} - \wt{\varphi}),
\qquad j=1,2,3.
\end{align*}
%
Applying Lemmas
\ref{lemma:sumNormsOutInf} and 
\ref{lemma:computationsRRRInf} and the above equality, we obtain
\begin{align*}
\begin{multlined}
\normInfty{\RRR_1^{\out}[{\varphi}]-\RRR_1^{\out}[\wt{\varphi}]}_{2\vap}
\leq
\sup_{\zeta \in B(\cttOutInftyA\de^3)} \Big[
\normInfty{{\varphi}_1-\wt{\varphi}_1}_{2\vap}
 \normInfty{\partial_w{\RRR^{\out}_1}[\zeta]}_{0} \\
+
\normInfty{{\varphi}_2-\wt{\varphi}_2}_{\vap}   
\normInfty{\partial_x{\RRR^{\out}_1}[\zeta]}_{\vap} 
+
\normInfty{{\varphi}_3-\wt{\varphi}_3}_{\vap}
 \normInfty{\partial_y{\RRR^{\out}_1}[\zeta]}_{\vap}
 \Big] 
\leq
C \de \normInftyTotal{{\varphi} -\wt{\varphi}},
\end{multlined}
\\
\begin{multlined}
% \end{multline*}
% Analogously, for $j=2,3$, we obtain
% \begin{multline*}
\normInftySmall{\RRR_j^{\out}[{\varphi}]-\RRR_j^{\out}[\wt{\varphi}]}_{\vap}
%
\leq
\sup_{\zeta \in B(\cttOutInftyA\de^3)} \Big[
\normInfty{{\varphi}_1-\wt{\varphi}_1}_{2\vap}
\normInftySmall{\partial_w{\RRR^{\out}_j}[\zeta]}_{-\vap} \\ 
+
\normInfty{{\varphi}_2-\wt{\varphi}_2}_{\vap} \normInftySmall{\partial_x{\RRR^{\out}_j}[\zeta]}_{0} 
+
\normInfty{{\varphi}_3-\wt{\varphi}_3}_{\vap} \normInftySmall{\partial_y{\RRR^{\out}_j}[\zeta]}_{0} 
\Big] 
%
\leq
C \normInftyTotal{{\varphi} -\wt{\varphi}}.
\end{multlined}
\end{align*}
for $j=2,3$. Then, by Lemma~\ref{lemma:GlipschitzInfinity}
and taking $\de$ small enough,
\begin{equation}\label{eq:FFcontractivaInfty}
\begin{split}
\normInftyTotal{\FF[{\varphi}]-\FF[\wt{\varphi}]} \leq& \,
%
C \de
\normInfty{\RRR_1^{\out}[{\varphi}]-\RRR_1^{\out}[\wt{\varphi}]}_{2\vap}+
%
C\de^2 \sum_{j=2}^3
\normInftySmall{\RRR_j^{\out}[{\varphi}]-\RRR_j^{\out}[\wt{\varphi}]}_{\vap} \\
%\\ &+
%%
%C\de^2 
%\normInfty{\RRR_3^{\out}[{\varphi}]-\RRR_3^{\out}[\wt{\varphi}]}_{\vap} \\
%
\leq& \, C\de^2 \normInftyTotal{{\varphi}-\wt{\varphi}}
\leq \frac{1}{2} \normInftyTotal{{\varphi}-\wt{\varphi}}.
\end{split}
\end{equation}
%
Then, by the definition of $\varrho$ in  \eqref{eq:firstIterationInfty} and 
\eqref{eq:FFcontractivaInfty},
$\FF: B(\cttOutInftyA\de^3) \to B(\cttOutInftyA\de^3)$
is well defined and contractive.
%
Therefore, $\FF$ has a fixed point $\zuOut\in B(\cttOutInftyA\de^3)$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%For $j=2,3$, we have
%\begin{align*}
%&\normInfty{\RRR_1^{\out}[{\varphi}]-\RRR_1^{\out}[\wt{\varphi}]}_{2\vap}
%\leq
%\normInfty{{\varphi}_1-\wt{\varphi}_1}_{2\vap}
%\sup_{\zeta \in \ballInfty} \normInfty{\partial_w{\RRR^{\out}_1}[\zeta]}_{0} \\
%&+
%\normInfty{{\varphi}_2-\wt{\varphi}_2}_{\vap} 
%\sup_{\zeta \in \ballInfty} \normInfty{\partial_x{\RRR^{\out}_1}[\zeta]}_{\vap}
%+
%\normInfty{{\varphi}_3-\wt{\varphi}_3}_{\vap}
%\sup_{\zeta \in \ballInfty} \normInfty{\partial_y{\RRR^{\out}_1}[\zeta]}_{\vap}, \\
%%%%%
%&\normInftySmall{\RRR_j^{\out}[{\varphi}]-\RRR_j^{\out}[\wt{\varphi}]}_{\vap}
%\leq
%\normInfty{{\varphi}_1-\wt{\varphi}_1}_{2\vap}
%\sup_{\zeta \in \ballInfty} \normInftySmall{\partial_w{\RRR^{\out}_j}[\zeta]}_{-\vap} \\
%&+
%\normInfty{{\varphi}_2-\wt{\varphi}_2}_{\vap}
%\sup_{\zeta \in \ballInfty} \normInftySmall{\partial_x{\RRR^{\out}_j}[\zeta]}_{0}
%+
%\normInfty{{\varphi}_3-\wt{\varphi}_3}_{\vap}
%\sup_{\zeta \in \ballInfty} \normInftySmall{\partial_y{\RRR^{\out}_j}[\zeta]}_{0}.
%\end{align*}
%Applying  Lemma~\ref{lemma:computationsRRRInf} we obtain
%\begin{equation*}%\label{proof:boundsR1Inf}
%\begin{split}
%\normInfty{\RRR_1^{\out}[{\varphi}]-\RRR_1^{\out}[\wt{\varphi}]}_{2\vap}	
%&\leq 
%C \de^2 \normInfty{{\varphi}_1 -\wt{\varphi}_1}_{2\vap} +
%C \de \normInfty{{\varphi}_2 -\wt{\varphi}_2}_{\vap} +
%C \de \normInfty{{\varphi}_3 -\wt{\varphi}_3}_{\vap} \\
%&\leq
%C \de \normInftyTotal{{\varphi} -\wt{\varphi}}, \\
%%%%
%\normInftySmall{\RRR_j^{\out}[{\varphi}]-\RRR_j^{\out}[\wt{\varphi}]}_{\vap}	
%&\leq 
%C \de \normInfty{{\varphi}_1 -\wt{\varphi}_1}_{2\vap} +
%C \de \normInfty{{\varphi}_2 -\wt{\varphi}_2}_{\vap} +
%C \de \normInfty{{\varphi}_3 -\wt{\varphi}_3}_{\vap} \\
%&\leq
%C \normInftyTotal{{\varphi} -\wt{\varphi}},
%\end{split}
%\end{equation*}



%\begin{proof}
%We start by studying function $g(u,0)$. Indeed, by~\eqref{eq:H1outerBetter}, we have
%\[
%g(u,0) = \Dx{H_1^{\out}}{w}(u,0,0,0;\de)
%= -\frac{1}{3\La_h(u)}\Dx{H_1^{\equi}}{\La}(\la_h(u),\La_h(u),0,0;\de)
%\]
%Therefore, to compute its norm, it is necessary to compute the first term on $\de$ for $f_1(u,0)$. Applying the results in Lemma~\ref{lemma:derivativesQcomplexs} and the change of variables $\phi_{\out}$ we obtain
%\begin{align*}
%f_1(u,0) =& -\frac{\partial \HH}{\partial u}(u,0,0,0;\de)  = - \Dx{\HH_1}{u}(u,0,0,0;\de)  \\
%%
%=& -\Dx{\wt{H}_1}{\la}(\la_h(u),\La_h(u),0,0) \lad_h(u) - \Dx{\wt{H}_1}{\La}(\la_h(u),\La_h(u),0,0) \Lad_h(u)\\
%%
%=& \lad_h(u) \la_h(u) \h Q_{\la}^{\la}(\la_h(u),\La_h(u); \de) 
%+ \lad_h(u) \La_h(u) \h Q_{\la}^{\La}(\la_h(u),\La_h(u); \de) \\
%+& \Lad_h(u) \la_h(u) \h Q_{\La}^{\la}(\la_h(u),\La_h(u); \de)
%+ \Lad_h(u) \La_h(u) \h Q_{\La}^{\La}(\la_h(u),\La_h(u); \de).
%\end{align*}
%By Lemma~\ref{lemma:fromeqtohomoclinic0} we have that $(\la_h(u), \La_h(u),0,0) \in B_4(\nu)$, thus we can apply the results from Lemma~\ref{lemma:derivativesQcomplexs}. Let us assume $u \in \DOutInf$, then
%\begin{align*}
%|f_1(u,0)| &\leq  |\lad_h(u) \la_h(u)|  \norm{Q_{\la}^{\la}}_{\CC^0(B_2(\nu))}
%+ |\lad_h(u) \La_h(u)| \norm{Q_{\la}^{\La}}_{\CC^0(B_2(\nu))} \\
%&+ |\Lad_h(u) \la_h(u)| \norm{Q_{\La}^{\la}}_{\CC^0(B_2(\nu))}
%+ |\Lad_h(u) \La_h(u)| \norm{Q_{\la}^{\la}}_{\CC^0(B_2(\nu))} \\
%&\leq C \de^2 \left(|\lad_h(u) \la_h(u)| +|\lad_h(u) \La_h(u)| + |\Lad_h(u) \la_h(u)| + |\Lad_h(u) \La_h(u)| \right).
%\end{align*}
%Then, by Lemmas~\ref{lemma:rhoComplexs} and~\ref{lemma:sumNorms} we have that
%\begin{align*}
%\norm{f_1(\cdot,0)}_{2\rho} &\leq C \de^2 \left( \norm{\lad_h \la_h}_{2 \rho} +  \norm{\lad_h \La_h}_{2 \rho} +  \norm{\Lad_h \la_h}_{2 \rho} +  \norm{\Lad_h \La_h}_{2 \rho}\right)
%\leq C \de^2,
%\end{align*}
%and as a consequence
%\[
%\norm{F_1[0]}_{2\rho} \leq C \de^2. 
%\]
%To compute $F_2[0]$ we follow a similar procedure. Thus
%%\[
%%F_2[0](u) = \frac{f_2(u,0)}{g(u,0)} = \frac{O(\de)}{1+O(\de)}.
%%\]
%%Then
%\begin{align*}
%f_2(u,0) =& i\frac{\partial \HH}{\partial y}(u,0,0,0;\de)  = i \Dx{\HH_1}{y}(u,0,0,0;\de)  
%= i \Dx{\wt{H}_1}{x}(\la_h(u),\La_h(u),0,0) \\
%=& i \la_h(u)\h  Q_y^{\la}(\la_h(u),\La_h(u),0,0; \de) + i \La_h(u) \h Q_y^{\la}(\la_h(u),\La_h(u),0,0; \de).
%\end{align*}
%Then
%\begin{align*}
%|f_2(u,0)| &\leq  |\la_h(u)|  \norm{Q_{y}^{\la}}_{\CC^0(B_4(\nu))}
%+ |\La_h(u)| \norm{Q_{\la}^{\La}}_{\CC^0(B_4(\nu))} \\
%&\leq C \de (|\la_h(u)| + |\La_h(u)|),
%\end{align*}
%and applying Lemma~\ref{lemma:rhoComplexs}, 
%\[
%\norm{f_2(\cdot,0)}_{\rho} \leq C \de \left( \norm{\la_h}_{\rho} + \norm{\La_h}_{\rho} \right) \leq C \de .
%\]
%Therefore,
%\[
%\norm{F_2[0]}_{\rho} \leq C \de. 
%\]
%Analogously, we can find the norm for $\norm{F_3[0]}_{\rho}$. Now,  computing the norm of operator $\FF[0]$, we obtain
%\begin{align*}
%\norm{\FF[0]}_{\XX} &= \norm{(\GG \circ \EE) [0]}_{\XX} = \norm{(\GG \circ F) [0] }_{\XX} \\
%%
%&= \de \norm{(\GG_1 \circ F_1)[0]}_{2\rho} + \norm{(\GG_2 \circ F_2)[0]}_{\rho} + \norm{(\GG_3 \circ F_3)[0]}_{\rho}.
%\end{align*}
%And applying the results from Lemma~\ref{lemma:Glipschitz} about operator $\GG$ we obtain
%\begin{align*}
%\norm{\FF[0]}_{\XX} 
%%
%\leq C_1 \de \norm{F_1[0]}_{2\rho} + 
%C_2 \de^2\norm{F_2[0]}_{\rho} + C_3 \de^2\norm{F_3[0]}_{\rho} \leq C \de^3.
%\end{align*}
%\end{proof}

==> Article Outer/proofH-existenceOuter.tex <==

To prove Proposition~\ref{proposition:existenceComecocos}, we must extend 
analytically the parameterizations  $\zuOut$ and $\zsOut$ given in Proposition 
\ref{proposition:existenceInfty} to the outer domains, $\DuOut$ and $\DsOut$, 
respectively.
%
Again, we only deal with the unstable -$\unstable$- case, being the -$\stable$- case analogous.
%
We prove the existence of $\zuOut$ by means of a fixed point argument in a suitable Banach space.

%Let us consider constant $\rhoInfty>0$, as given in Proposition~\ref{proposition:existenceInfty}, and fix constants $\rho>\rhoInfty$ and $d \in (\frac{1}{4},\frac{1}{2})$.
%

%Let us consider the invariance equation
%\begin{equation}
%\LL \zuOut = \RRR^{\out}[\zuOut],
%\end{equation}
%(see \eqref{eq:invariantEquationInftyA}). 
%%
%Then, we prove the existence of $\zuOut$ by means of a fixed point argument in a suitable Banach space.

%First, we introduce the auxiliary function $g_{\de}(u)$ as
%\begin{align}\label{def:gdelta}
%	g_{\de}(u) = \frac{1}{\vabs{u^2+A^2}} + \frac{\de^2}{\vabs{u^2+A^2}^{\frac{8}{3}}}.
%\end{align}
Given $\al, \beta \in \reals$, we consider the norm
\begin{align*}
	&\normOut{\varphi}_{\al,\beta}= 
	\sup_{u\in \DuOut} 
	\vabs{g_{\de}^{-\al}(u) \paren{u^2+A^2}^{\beta}  \varphi(u)},
	\quad
	g_{\de}(u) = \frac{1}{\vabs{u^2+A^2}} + \frac{\de^2}{\vabs{u^2+A^2}^{\frac{8}{3}}},
\end{align*}
and the  associated Banach space
\begin{align}\label{def:XcalOut}
&\XcalOut_{\al, \beta}= \left\{ \varphi: \DuOut \to \complexs  \st  \varphi \text{ real-analytic, } \normOut{\varphi}_{\al,\beta}
 < \infty \right\}. 
\end{align}

These Banach spaces have the following properties, which we use without 
mentioning along the section. Their proof follows the same lines as the proof 
of Lemma 7.1 in \cite{BFGS12}.

%In the next lemma, we state some properties of these Banach spaces.
%%
%We use the results in it without mentioning them along the section.
\begin{lemma}\label{lemma:sumNormsOuter}
% There exists a constant $C$ independent of $\de$  and $\kappa$ such that t
The following statements hold:
\begin{enumerate}
\item If $\varphi \in \XcalOut_{\al,\beta_1}$, then $\varphi \in 
\XcalOut_{\al,\beta_2}$ for any $\beta_2 \in \reals$ and
%
% Moreover,
\begin{align*}
\begin{cases}
\normOut{\varphi}_{\al,\beta_2} \leq C \normOut{\varphi}_{\al,\beta_1}, 
&\quad \text{for } \beta_2 - \beta_1 > 0, \\
%		
\normOut{\varphi}_{\al,\beta_2} \leq C 
(\kappa \de^2)^{\beta_2-\beta_1} \normOut{\varphi}_{\al,\beta_1},
&\quad \text{for } \beta_2-\beta_1 \leq 0.
\end{cases}
\end{align*}
%%%%%%%%%
\item If $\varphi \in \XcalOut_{\al,\beta_1}$, then $\varphi \in 
\XcalOut_{\al-1,\beta_2}$ for any $\beta_2 \in \reals$ and 
%
% Moreover,
\begin{align*}
\begin{cases}
\normOut{\varphi}_{\al-1,\beta_2} \leq C \normOut{\varphi}_{\al,\beta_1}, 
&\quad \text{for } \beta_2 - \beta_1 > \frac53, \\[0.5em]
%		
\normOut{\varphi}_{\al-1,\beta_2} \leq 
C \de^2 (\kappa \de^2)^{(\beta_2-\beta_1)-\frac83} 
 \normOut{\varphi}_{\al,\beta_1},
&\quad \text{for } \beta_2 - \beta_1 \leq \frac53.
\end{cases}
\end{align*}
\item If $\varphi \in \XcalOut_{\al_1,\beta_1}$ and 
$\zeta \in \XcalOut_{\al_2,\beta_2}$, then 
$\varphi \zeta \in \XcalOut_{\al_1+\al_2,\beta_1+\beta_2}$ and
\[
\normOut{\varphi\zeta}_{\al_1+\al_2,\beta_1+\beta_2} \leq \normOut{\varphi}_{\al_1,\beta_1} \normOut{\zeta}_{\al_2,\beta_2}.
\]
%%%%%%%%%
\item If 
$\varphi \in \XcalOut_{0,\beta+1}$ and $\zeta \in 
\XcalOut_{0,\beta+\frac{8}{3}}$, then
$\varphi + \de^2\zeta \in \XcalOut_{1,\beta}$ and 
%
% Moreover,
\begin{align*}
	\normOutSmall{\varphi + \de^2\zeta}_{1,\beta}
	\leq 
	\normOut{\varphi}_{0,\beta+1} +
	\normOut{\zeta}_{0,\beta + \frac{8}{3} }.
\end{align*}
%%%%%%%%%
%%%%%%%%%
\end{enumerate}
\end{lemma}
% \begin{proof}	
% 
% \end{proof}

Let us recall that, by Proposition~\ref{proposition:existenceInfty}, 
the invariance equation~\eqref{eq:invariantEquationOuter}
has a unique solution $\zuOut$ 
in the domain $\DuInfty$ satisfying the asymptotic condition~\eqref{eq:asymptoticConditionsOuter}.
%
Our objective is to extend analytically $\zuOut$  to the outer domain 
$\DuOut$. Notice that, since $\rhoInfty<\rhoOuter$,   $\DuInfty \cap \DuOut 
\neq \emptyset$ (see definitions \eqref{def:dominisInfty} and 
\eqref{def:dominisComecocos} of $\DuInfty$ and $\DuOut$).

As explained in Section \ref{subsection:proofH-existenceInfinite}, equation \eqref{eq:invariantEquationOuter} is equivalent to  $\LL \zuOut = \RRR^{\out}[\zuOut]$ with $\LL\phiA=(\partial_u-\AAA^{\out})\phiA$ and $\RRR^{\out}$ given in \eqref{def:operatorRRROuter}.
%
%We proceed by defining the following linear operator
%\begin{equation}\label{def:operatorLouter}
%	\LL \varphi = (\partial_u-\AAA^{\out})\varphi .
%\end{equation}
%
%The invariance equation~\eqref{eq:invariantEquationOuter} is equivalent to $\LL \zuOut = \RRR^{\out}[\zuOut]$ (see \eqref{def:operatorL}). 
%
In the following lemma we introduce a right-inverse operator of $\LL$ defined on $\XcalOut_{\al,\beta}$. 
%

\begin{lemma}\label{lemma:GlipschitzOuter}
Let us consider the operator $\GG[\varphi]=\paren{\GG_1[\phiA_1],\GG_2[\phiA_2],\GG_3[\phiA_3]}^T$, such that
\begin{equation*}
%\label{def:operatorGGouter}
\GG[\varphi](u) = \paren{
\int_{-\rhoOuter}^u \varphi_1(s) ds,
%
\int_{\conj{u}_1}^u e^{-\frac{i}{\de^2}(s-u) } \varphi_2(s) ds , 
%
\int_{u_1}^u e^{\frac{i}{\de^2}(s-u) } \varphi_3(s) ds }^T,
\end{equation*}
where $u_1$ and $\conj{u}_1$ are the vertices of the domain $\DuOut$ (see Figure~\ref{fig:dominisComecocos}).
%
%Fix $\beta_1, \beta_2>0$, then 
%$
%\GG: \XcalOut_{1,\beta_1} \times 
%\XcalOut_{0,\beta_2} \times \XcalOut_{0,\beta_2}
%\to \XcalOut_{1,\beta_1-1} \times 
%\XcalOut_{0,\beta_2} \times \XcalOut_{0,\beta_2},
%$
%is a continuous and linear operator and is a left-inverse of the operator $\LL$. 
Fix $\beta > 0$. There exists a constant $C$ such that:
\begin{enumerate}
\item If $\varphi \in \XcalOut_{1,\beta}$, then $\GG_1[\varphi] \in 
\XcalOut_{1,\beta-1}$ and
$
\normOut{\GG_1[\varphi]}_{1,\beta-1} \leq C \normOut{\varphi}_{1,\beta}$.
\item If $\varphi \in \XcalOut_{0,\beta}$, then $\GG_j[\varphi] \in 
\XcalOut_{0,\beta}$, $j=2,3$, and
$
\normOut{\GG_j[\varphi]}_{0,\beta} \leq C \de^2 \normOut{\varphi}_{0,\beta}$.
%
%\item Let $\beta_1,\beta_2>0$. If $\varphi \in \XcalOut_{1,\beta_1} \times \XcalOut_{0,\beta_2}
%\times \XcalOut_{0,\beta_2}$, 
%then
%$
%\paren{\LL \circ \GG}[\varphi] = \varphi
%$
%and
%\[
%\paren{\GG \circ \LL}[\varphi](u) =
%\varphi(u) - 
%\paren{\varphi_1(-\rhoOuter),\,
%\varphi_2(\conj{u_1})
%e^{-\frac{i}{\de^2}(\conj{u_1}-u)}, \,
%\varphi_3({u_1})
%e^{\frac{i}{\de^2}({u_1}-u)}
%}.
%\]
\end{enumerate}
\end{lemma}

% \begin{proof}	
The proof of this lemma follows the same lines as the proof of Lemma 7.3 in 
\cite{BFGS12}.
% \end{proof}


%\begin{remark}\label{remark:Ginverse}
%	Given $h \in \XOutTotal$, if $\zOut \in \XOutTotal$ is a solution of $\LL[\zOut]=h$ such that it satisfies the asymptotic condition~\eqref{eq:asymptoticConditionsOuter}, then it satisifes $\zOut=\GG[h]$.
%\end{remark}

Consider $u_1$ and $\conj{u_1}$ as in Figure \ref{fig:dominisComecocos} and the function
\begin{equation*}
%\label{def:initialConditionOuter}
	F^0(u) = \paren{\wuOut(-\rhoOuter),\,
		\xuOut(\conj{u}_1)
		e^{-\frac{i}{\de^2}(\conj{u}_1-u)}, \,
		\yuOut({u_1})
		e^{\frac{i}{\de^2}({u}_1-u)}
	}^T.
\end{equation*}
Notice that, since $0<\rhoInfty<\rhoOuter$, we have
$\claus{-\rhoOuter, u_1,\conj{u}_1} \in \DuInfty$.
%
Therefore, by Proposition~\ref{proposition:existenceInfty}, 
$\zuOut$ is already defined at these points.
%
%and, accordingly, $F^0(u)$ does not depend on $\zuOut$.
%
We define the fixed point operator
\begin{equation}\label{eq:operatorFFouter}
\FF[\phiA]= F^0 + \GG \circ \RRR^{\out}[\phiA],
\end{equation}
where the operator $\RRR^{\out}$ is given in~\eqref{def:operatorRRROuter}.
%
Since $\LL(F^0)=0$, 
by Lemma~\ref{lemma:GlipschitzOuter}, a solution $\zuOut=\FF[\zuOut]$ satisfies $\LL \zuOut = \RRR^{\out}[\zuOut]$ and by construction is the real-analytic continuation of the function $\zuOut$ obtained in Proposition \ref{proposition:existenceInfty}.

We rewrite Proposition~\ref{proposition:existenceComecocos} in terms of the operator $\FF$ defined in the Banach space
\[
\XcalOutTotal = \XcalOut_{1,0} \times \XcalOut_{0,\frac{4}{3}} \times \XcalOut_{0,\frac{4}{3}},
\] 
endowed with the norm
\[
\normOutTotal{\varphi}= 
\de \normOut{\varphi_1}_{1,0} + 
\normOut{\varphi_2}_{0,\frac{4}{3}} + 
\normOut{\varphi_3}_{0,\frac{4}{3}}.
\]

\begin{proposition}\label{proposition:existenceComecocosBanach}
There exist $\de_0, \kappaOuter>0$ such that, for $\de \in (0,\de_0)$ and $\kappa\geq \kappaOuter$, the fixed point equation $\zuOut = {\FF}[\zuOut]$ has a unique solution $\zuOut \in \XcalOutTotal$. 
%
Moreover, there exists a real constant $\cttOutOutA>0$  independent of $\de$ and $\kappa$ such that
%	
$
\normOutTotal{\zuOut} \leq \cttOutOutA \de^3.
$
\end{proposition}

We prove this proposition through a 
fixed point argument.
%
First, we state a technical lemma, whose proof is postponed until 
Appendix~\ref{subsubsection:proofComputationsRRROut}. Fix $\varrho>0$ and define
\begin{equation*}
	%\label{def:ballOuter}
\ballOuterDef= \claus{\varphi \in \XcalOutTotal \st \normOutTotal{\varphi} \leq \varrho}.
\end{equation*}

\begin{lemma}\label{lemma:computationsRRROut}
Fix $\varrho>0$ and let $\RRR^{\out}$ be the operator defined in~\eqref{def:operatorRRROuter}.
%  
For $\de>0$ small enough and $\kappa>0$ big enough, 
there exists a constant $C>0$
such that, for $\varphi \in \ballOuter$,
\begin{align*}
\normOut{\RRR^{\out}_1[\phiA]}_{1,1} \leq C \de^2, \qquad
%
\normOutSmall{\RRR^{\out}_j[\phiA]}_{0,\frac{4}{3}} \leq C \de, \qquad
%
j= 2,3,
\end{align*}
and,
\begin{align*}
&\normOut{\partial_w {\RRR^{\out}_1} [\phiA]}_{1,\frac13} 
\leq C \de^2,  &
%
&\normOut{\partial_x {\RRR^{\out}_1} [\phiA]}_{0,\frac73} 
\leq C\de, &
%
&\normOut{\partial_y {\RRR^{\out}_1} [\phiA]}_{0,\frac{7}{3}} 
\leq C{\de}, \\
%
&\,\normOutSmall{\partial_w {\RRR^{\out}_2} [\phiA]}_{0,\frac{2}{3}} 
\leq C\de, &
%
&\,\normOutSmall{\partial_x {\RRR^{\out}_2} [\phiA]}_{1,-\frac23} 
\leq C, &
%
&\,\normOutSmall{\partial_y{\RRR^{\out}_2} [\phiA]}_{0,2} 
\leq C\de^2, \\
%
&\,\normOutSmall{\partial_w {\RRR^{\out}_3} [\phiA]}_{0,\frac{2}{3}} 
\leq C\de, &
%
&\,\normOutSmall{\partial_x {\RRR^{\out}_3} [\phiA]}_{0,2} 
\leq C\de^2, &
%
&\,\normOutSmall{\partial_y {\RRR^{\out}_3} [\phiA]}_{1,-\frac23} 
\leq C.
\end{align*}

%\begin{align*}
%\normOut{\partial_w {\RRR^{\out}_1} [\phiA]}_{0,1} 
%&\leq \frac{C}{\kappa^2}, &
%%
%\normOut{\partial_x {\RRR^{\out}_1} [\phiA]}_{1,-\frac{1}{3}} 
%&\leq \frac{C}{\de}, &
%%
%\normOut{\partial_y {\RRR^{\out}_1} [\phiA]}_{1,-\frac{1}{3}} 
%&\leq \frac{C}{\de}, \\
%%
%\normOutSmall{\partial_w {\RRR^{\out}_j} [\phiA]}_{-1,\frac{4}{3}} 
%&\leq \frac{C}{\kappa^2 \de}, &
%%
%\normOutSmall{\partial_x {\RRR^{\out}_j} [\phiA]}_{0,0} 
%&\leq \frac{C}{\kappa^2 \de^2}, &
%%
%\normOutSmall{\partial_y{\RRR^{\out}_j} [\phiA]}_{0,0} 
%&\leq \frac{C}{\kappa^2 \de^2}.
%\end{align*}
\end{lemma}

The next lemma gives properties of the operator $\FF$.
%
%The first one deals with the first iteration, namely $\FF[0]$, and the second lemma is about the Lipschitz constant of $\FF$.

\begin{lemma}\label{lemma:FpropertiesComecococs}
Fix $\varrho>0$ and let $\FF$ be the operator defined in~\eqref{eq:operatorFFouter}.
%
Then, for $\de>0$ small enough and $\kappa>0$ big enough,  there exist 
constants $\cttOutOutB, \cttOutOutC>0$ independent of $\de$ and $\kappa$ such 
that
\[
\normOutTotal{\FF[0]} \leq \cttOutOutB \de^3.
\]
Moreover,
% there exists $\cttOutOutC>0$ independent of $\de$ and $\kappa$ such 
% that, 
for $\phiA, \phiB \in \ballOuter$,
\begin{align*}
\de \normOut{{\FF_1}[\phiA]-{\FF_1}[\phiB]}_{1,0}
&\leq \cttOutOutC \paren{ 
%
\frac{\de}{\kappa^2} 
\normOut{\phiA_1 - \phiB_1}_{1,0} 
+ \normOut{\phiA_2 - \phiB_2}_{0,\frac{4}{3}}
+ \normOut{\phiA_3 - \phiB_3}_{0,\frac{4}{3}} }, \\
%%%%%
\normOut{{\FF_j}[\phiA]-{\FF_j}[\phiB]}_{0,\frac{4}{3}} 
&\leq \frac{\cttOutOutC}{\kappa^2} \normOutTotal{\phiA - \phiB},
\qquad \text{for} \quad j=2,3.
\end{align*}

\end{lemma}

\begin{proof}
First, we obtain the estimates for $\FF[0]$. By 
Proposition~\ref{proposition:existenceInfty}, we have that
\begin{align*}
	\vabs{\wuOut(-\rhoOuter)} \leq C \de^2,
	\quad
	\vabs{\xuOut(\conj{u_1})} \leq C \de^3,
	\quad
	\vabs{\yuOut({u_1})} \leq C \de^3,
\end{align*}
and, as a result, 
$\normOutTotalSmall{F^0} \leq C \de^3$.
%\begin{align*}
%	\normOutTotal{F^0} &\leq
%	%
%	C\de \normOut{F^0_1}_{0,0}+
%	C\normOut{F^0_2}_{0,0} +
%	C\normOut{F^0_3}_{0,0} \leq C \de^3.
%\end{align*}
Then, applying Lemmas~\ref{lemma:GlipschitzOuter} and~\ref{lemma:computationsRRROut}, we obtain
\begin{align*}
\normOutTotal{\FF[0]} \leq
\normOutTotal{F^0} +
C \de \normOut{\RRR^{\out}_1[0]}_{1,1} +
C \de^2 \textstyle \sum_{j=2}^3 \normOutSmall{\RRR^{\out}_j[0]}_{0,\frac43} 
%+C \de^2 \normOut{\RRR^{\out}_3[0]}_{0,\frac43} 
\leq C \de^3.
\end{align*}

For the second statement, since $\FF=F^0+\GG \circ \RRR^{\out}$ and $\GG$ is linear, we need to compute estimates for $\RRR^{\out}[\phiA]-\RRR^{\out}[\phiB]$.
%
Then, by the mean value theorem, 
\begin{align*}
	\RRR_j^{\out}[\phiA]-\RRR_j^{\out}[\phiB] 
	= \boxClaus{\int_0^1 D{\RRR_j^{\out}}[s {\phiA} + (1-s) \phiB] d s} (\phiA - \phiB),
	\qquad j=1,2,3.
\end{align*}	
%
In addition, by Lemmas \ref{lemma:sumNormsOuter} and \ref{lemma:computationsRRROut}, for $j=2,3$, we have the estimates
\begin{equation*}%\label{proof:boundsRRRoutLipschitz}
\begin{aligned}	
\normOut{\partial_w {\RRR^{\out}_1} [\phiA]}_{0,1} 
&\leq \frac{C}{\kappa^2}, &
%
\normOut{\partial_x {\RRR^{\out}_1} [\phiA]}_{1,-\frac{1}{3}} 
&\leq \frac{C}{\de}, &
%
\normOut{\partial_y {\RRR^{\out}_1} [\phiA]}_{1,-\frac{1}{3}} 
&\leq \frac{C}{\de}, \\
%
\normOutSmall{\partial_w {\RRR^{\out}_j} [\phiA]}_{-1,\frac{4}{3}} 
&\leq \frac{C}{\kappa^2 \de}, &
%
\normOutSmall{\partial_x {\RRR^{\out}_j} [\phiA]}_{0,0} 
&\leq \frac{C}{\kappa^2 \de^2}, &
%
\normOutSmall{\partial_y{\RRR^{\out}_j} [\phiA]}_{0,0} 
&\leq \frac{C}{\kappa^2 \de^2}.
\end{aligned}
\end{equation*}
%
We estimate each component separately.
%
For $j=1$, we have that
%
\begin{align*}	
\MoveEqLeft[5] \de \lVert \RRR_1^{\out}[\phiA]-	\RRR_1^{\out}[\phiB] \rVert^{\mathrm{out}}_{1,1}
\leq
%
\sup_{\zeta \in \ballOuter} \de \Big[
\normOut{\phiA_1-\phiB_1}_{1,0}
\normOut{\partial_w{\RRR^{\out}_1}[\zeta]}_{0,1} \\
%
&+
\normOut{\phiA_2-\phiB_2}_{0,\frac{4}{3}}  \normOut{\partial_x{\RRR^{\out}_1}[\zeta]}_{1,-\frac{1}{3}}  
+
\normOut{\phiA_3-\phiB_3}_{0,\frac{4}{3}} \normOut{\partial_y{\RRR^{\out}_1}[\zeta]}_{1,-\frac{1}{3}} \Big] 
\\
%%%%%%%%%
%&\leq
%\sup_{\zeta \in \ballOuter} \bigg[
%\frac{C}{\kappa^2\de}
%\normOut{\phiA_1-\phiB_1}_{1,0}
%\normOut{\partial_w{\RRR^{\out}_1}[\zeta]}_{1,\frac13}
%+\frac{C}{\de}
%\normOut{\phiA_2-\phiB_2}_{0,\frac{4}{3}}  \normOut{\partial_x{\RRR^{\out}_1}[\zeta]}_{0,\frac{7}{3}}  \\
%&+\frac{C}{\de}
%\normOut{\phiA_3-\phiB_3}_{0,\frac{4}{3}} \normOut{\partial_y{\RRR^{\out}_1}[\zeta]}_{0,\frac73} \bigg] 
%%%%%%%%%
\leq& \,
\frac{C \de}{\kappa^2} 
\normOut{{\phiA}_1-{\phiB}_1}_{1,0} 
+		
C \normOut{{\phiA}_2 -{\phiB}_2}_{0,\frac{4}{3}}
+
C \normOut{{\phiA}_3 -{\phiB}_3}_{0,\frac{4}{3}}.
\end{align*}
Analogously, for $j=2,3$, we obtain
\begin{align*}
\MoveEqLeft[7]
\normOutSmall{\RRR_j^{\out}[\phiA]-\RRR_j^{\out}[\phiB]}_{0,\frac{4}{3}}
\leq
\sup_{\zeta \in \ballOuter} \Big[
\normOut{\phiA_1-\phiB_1}_{1,0}
\normOutSmall{\partial_w{\RRR^{\out}_j}[\zeta]}_{-1,\frac{4}{3}} \\
&+
\normOut{\phiA_2-\phiB_2}_{0,\frac{4}{3}} \normOutSmall{\partial_x{\RRR^{\out}_j}[\zeta]}_{0,0}
+
\normOut{\phiA_3-\phiB_3}_{0,\frac{4}{3}}
\normOutSmall{\partial_y{\RRR^{\out}_j}[\zeta]}_{0,0} \Big] \\
%%%%%%%
%&\leq
%\sup_{\zeta \in \ballOuter} \bigg[
%\frac{C}{\kappa^2 \de^2}
%\normOut{\phiA_1-\phiB_1}_{1,0}
%\normOutSmall{\partial_w{\RRR^{\out}_2}[\zeta]}_{0,\frac{2}{3}} 
%+
%\frac{C}{\kappa^2\de^2}
%\normOut{\phiA_2-\phiB_2}_{0,\frac{4}{3}} \normOutSmall{\partial_x{\RRR^{\out}_2}[\zeta]}_{1,-\frac13} \\
%&+
%\frac{C}{\kappa^2\de^4}
%\normOut{\phiA_3-\phiB_3}_{0,\frac{4}{3}}
%\normOutSmall{\partial_y{\RRR^{\out}_2}[\zeta]}_{0,2} \bigg]
%%%%%
\leq& \,
\frac{C}{\kappa^2 \de^2}
\normOutTotal{{\phiA} -{\phiB}},
\end{align*}
and, using Lemma~\ref{lemma:GlipschitzOuter}, we obtain the estimates for the 
second statement. 
\end{proof}
%%%%%%%%%%%%%%
%Then, for $j=2,3$, we have
%	\begin{align*}
%		&\normOut{\RRR_1^{\out}[\phiA]-
%			\RRR_1^{\out}[\phiB]}_{1,1}
%		\leq
%		\normOut{\phiA_1-\phiB_1}_{1,0}
%		\sup_{\zeta \in \ballOuter} \normOut{\partial_w{\RRR^{\out}_1}[\zeta]}_{0,1} \\
%		&+
%		\normOut{\phiA_2-\phiB_2}_{0,\frac{4}{3}} 
%		\sup_{\zeta \in \ballOuter} \normOut{\partial_x{\RRR^{\out}_1}[\zeta]}_{1,-\frac{1}{3}}
%		+
%		\normOut{\phiA_3-\phiB_3}_{0,\frac{4}{3}}
%		\sup_{\zeta \in \ballOuter} \normOut{\partial_y{\RRR^{\out}_1}[\zeta]}_{1,-\frac{1}{3}}, \\
%		%%%%
%		&\normOutSmall{\RRR_j^{\out}[\phiA]-\RRR_j^{\out}[\phiB]}_{0,\frac{4}{3}}
%		\leq
%		\normOut{\phiA_1-\phiB_1}_{1,0}
%		\sup_{\zeta \in \ballOuter} \normOutSmall{\partial_w{\RRR^{\out}_j}[\zeta]}_{-1,\frac{4}{3}} \\
%		&+
%		\normOut{\phiA_2-\phiB_2}_{0,\frac{4}{3}}
%		\sup_{\zeta \in \ballOuter} \normOutSmall{\partial_x{\RRR^{\out}_j}[\zeta]}_{0,0}
%		+
%		\normInfty{\phiA_3-\phiB_3}_{0,\frac{4}{3}}
%		\sup_{\zeta \in \ballOuter} \normOutSmall{\partial_y{\RRR^{\out}_j}[\zeta]}_{0,0}.
%	\end{align*}
%	Applying  Lemma~\ref{lemma:computationsRRROut} we obtain
%	\begin{equation*}%\label{proof:boundsR1Inf}
%		\begin{split}
%			\de\normOut{\RRR_1^{\out}[\phiA]-\RRR_1^{\out}[\phiB]}_{1,1}	
%			&\leq 
%			\frac{C \de}{\kappaOuter^2} 
%			\normOut{{\phiA}_1-{\phiB}_1}_{1,0} 
%			+		
%			C \normOut{{\phiA}_2 -{\phiB}_2}_{0,\frac{4}{3}} 
%			+
%			C \normOut{{\phiA}_3 -{\phiB}_3}_{0,\frac{4}{3}}, \\
%			%%%
%			\de^2 \normOutSmall{\RRR_j^{\out}[{\varphi}]-\RRR_j^{\out}[\wt{\varphi}]}_{0,\frac{4}{3}}	
%			&\leq 
%			\frac{C \de}{\kappaOuter^2}
%			\normOut{{\phiA}_1 -\phiB_1}_{1,0} 
%			+
%			\frac{C}{\kappaOuter^2} \normOut{{\phiA}_2 -{\phiB}_2}_{0,\frac{4}{3}} 
%			+
%			\frac{C}{\kappaOuter^2} \normOut{{\phiA}_3 -{\phiB}_3}_{0,\frac{4}{3}} \\
%			&\leq
%			\frac{C}{\kappaOuter^2}
%			\normOutTotal{{\phiA} -{\phiB}},
%		\end{split}
%	\end{equation*}

Lemma~\ref{lemma:FpropertiesComecococs} shows that, by assuming $\kappa$ big enough, operators $\FF_2$ and $\FF_3$ have Lipschitz constant less than $1$ with the norm in $\XcalOutTotal$.
%
However, we are not able to control the Lipschitz constant of $\FF_1$.
%
To overcome this problem, we apply a Gauss-Seidel argument to define a new operator
\begin{equation*} %\label{def:operatorFGaussSeidelOuter}
\wt{\FF}[\zOut]
= \wt{\FF}[(\wOut,\xOut,\yOut)]
= \begin{pmatrix} 
\FF_1[\wOut,\FF_2[\zOut],\FF_3[\zOut]] \\ 
\FF_2[\zOut] \\
\FF_3[\zOut] \end{pmatrix},
\end{equation*}
which turns out to be contractive in a suitable ball and has the same fixed points as $\FF$.

\begin{proof}[End of the proof of Proposition~\ref{proposition:existenceComecocosBanach}]
%
We look for a fixed point of $\wt{\FF}$.
%
First, we obtain an estimate for $\normOutTotalSmall{\wt{\FF}[0]}$. 
%
We rewrite it as
\begin{align*}%\label{proof:operadorJJ0}
\wt{\FF}[0] = \FF[0] + 
\Big(\FF_1[0,\FF_2[0],\FF_3[0]] - \FF_1[0],
0,0\Big)^T,
\end{align*}
and we notice that, by Lemma~\ref{lemma:FpropertiesComecococs}, 
$
\normOutTotalSmall{(0,\FF_2[0],\FF_3[0])} \leq
\normOutTotal{\FF[0]} \leq C \de^3.
$
Then, applying Lemma~\ref{lemma:FpropertiesComecococs}, there exists constant $ 
\cttOutOutA>0$ such that
\begin{equation}\label{proof:operadorJJ0}
\begin{split}	
\normOutTotalSmall{\wt{\FF}[0]} &\leq 
\normOutTotal{\FF[0]} + 
\normOut{\FF_1[0,\FF_2[0],\FF_3[0]] - \FF_1[0]}_{1,0} \\
%
&\leq 
\normOutTotal{\FF[0]} +
C \normOut{\FF_2[0]}_{0,\frac{4}{3}} + 
C \normOut{\FF_3[0]}_{0,\frac{4}{3}}
\leq \frac12  \cttOutOutA \de^3.
\end{split}
\end{equation}
%
%Let us fix constant $\varrho>0$ such that
%\[
%\normOutTotalSmall{\wt{\FF}[0]} \leq \frac{\varrho}{2} \de^3.
%\]

Now, we prove that the operator $\wt{\FF}$ is contractive in $B( \cttOutOutA 
\delta^3)$.
%
Indeed, by Lemma~\ref{lemma:FpropertiesComecococs}, we have that, for $\phiA, 
\phiB \in B( \cttOutOutA 
\delta^3)$,
\begin{align*}
\de \normOutSmall{\wt{\FF}_1[\phiA]-\wt{\FF}_1[\phiB]}_{1,0} &\leq C \paren{
%
\frac{\de}{\kappa^2} 
\normOut{\phiA_1 - \phiB_1}_{1,0}
+
\normOut{\FF_2[\phiA]-\FF_2[\phiB]}_{0,\frac{4}{3}}
+
\normOut{\FF_3[\phiA]-\FF_3[\phiB]}_{0,\frac{4}{3}}
} \\
%
&\leq  
\frac{C \de}{\kappa^2} 
\normOut{\phiA_1 - \phiB_1}_{1,0} + 
\frac{2 C}{\kappa^2} 
\normOutTotal{\phiA-\phiB}
%
\leq 
\frac{C}{\kappa^2} 
\normOutTotal{\phiA-\phiB}, \\
%%%%
\normOutSmall{\wt{\FF}_j[\phiA]-\wt{\FF}_j[\phiB]}_{0,\frac{4}{3}}
&= 
\normOut{\FF_j[\phiA]-\FF_j[\phiB]}_{0,\frac{4}{3}}
\leq
\frac{C}{\kappa^2} 
\normOutTotal{\phiA-\phiB}, 
\qquad \text{for } j=2,3.
\end{align*}
Then, for $\kappa>0$ big enough, we have that
$
	%\label{proof:GaussSeidelLipschitzOuter}
\normOutTotalSmall{\wt{\FF}[\varphi]-\wt{\FF}[\phiB]} \leq \frac{1}{2} \normOutTotal{\phiA-\phiB}.
$
Together with \eqref{proof:operadorJJ0}, this implies that 
$\wt{\FF}:B( \cttOutOutA 
\delta^3) \to B( \cttOutOutA 
\delta^3)$ is well defined and contractive.
%
Therefore, $\wt{\FF}$ has a fixed point $\zuOut \in B( \cttOutOutA 
\delta^3)$.
\end{proof}


==> Article Outer/proofH-existenceTechnicalChangeuOut.tex <==
\subsection{Proof of Lemma~\ref{lemma:computationsRRRtransitionOuter}}
\label{subsubsection:ProofcomputationsRRRtransitionOuter}

\textcolor{red}{Es podria treure.}

%Let us recall operator $R$ as defined in~\eqref{def:operatorRRRtransition} is	
%$
%	R[\varphi](v) = \partial_w H_1^{\out}
%	\paren{v + \varphi(v), \zuOut(v+\varphi(v))},
%$
%with $\zuOut$ as given in Proposition~\ref{proposition:existenceComecocos} and the Hamiltonian $H_1^{\out}$ in \eqref{def:hamiltonianOuterSplit}.
%
%Then, we need to obtain estimates for $R[\varphi]$.

First, let us notice that, since $\DOuterTilde \subset \DuOut$, we have that $\YcalOuter \subset \XcalOut_{0,0}$ (see \eqref{def:XcalOut}).
%
Therefore, for $\al,\beta \in \reals$, if $\phiA \in \XcalOut_{\al,\beta}$ then $\phiA \in \YcalOuter$ and
\begin{equation*}%\label{proof:normesOutTilde}
	\normSup{\phiA} \leq C \normOut{\phiA}_{\al,\beta}.
\end{equation*}

Let $\phiA \in \YcalOuter$ such that $\normSup{\phiA}\leq \varrho \de^2$ and $v \in \DOuterTilde$
%
then, for $\de$ small enough, $v+\phiA(v) \in \DuOut$. 
%
As a result, we can apply the estimates of the derivatives of $H_1^{\out}$ obtained in the proof of Lemma \ref{lemma:computationsRRROut} to operator $R[\phiA]$ (see \eqref{def:operatorRRRtransition}).
%
Indeed, by \eqref{proof:estimatef1OutDCerivatives},
\begin{align*}
\normSup{R[\phiA]}
\leq
\normOut{\partial_w H_1^{\out}
\paren{\cdot, \zuOut}}_{1,-\frac{2}{3}}
\leq
C\de^2.
\end{align*}
Analogously, we can compute estimates for the derivative $DR[\phiA]$. Indeed, applying the results in Proposition \ref{proposition:existenceComecocos},
\eqref{proof:estimategOutDerivatives} and \eqref{proof:estimatef1OutDCerivatives}, we obtain
\begin{align*}
\normSup{DR[\phiA]} \leq&
\normOut{\partial_{uw} H_1^{\out}(\cdot,\zuOut)}_{1,\frac{1}{3}}
+
\normOut{\partial^2_{w} H_1^{\out}(\cdot,\zuOut)}_{0,-\frac{2}{3}}
	\normOut{\partial_u \wuOut}_{1,1} \\
	&+
	\normOut{\partial_{wx} H_1^{\out}(\cdot,\zuOut)}_{0,\frac53}
	\normOut{\partial_u \xuOut}_{0,\frac53}
	+
	\normOut{\partial_{wy} H_1^{\out}(\cdot,\zuOut)}_{1,-2}
	\normOut{\partial_u \yuOut}_{0,\frac{7}{3}} 
	\leq C \de^2.
%	\\
%	\leq&
%	C\de^2 + 
%	\frac{C}{\de^2} \normOut{\partial_{wx} H_1^{\out}(\cdot,\zuOut)}_{0,\frac{5}{3}}
%	+ 
%	\frac{C}{\de^2} \normOut{\partial_{wy} H_1^{\out}(\cdot,\zuOut)}_{0,\frac{5}{3}}
%	\leq C\de^2.
\end{align*}
\qed






==> Article Outer/proofH-existenceTechnicalFlow.tex <==
\subsection{Proof of Lemma~\ref{lemma:computationsRFlow}}
\label{subsubsection:ProofComputationsRFlow}

\textcolor{red}{Es podria treure.}

By the definition of $\RRR^{\flow}[\phiA]$ in \eqref{def:operatorRFlow}, we need to estimate  the derivatives of $H_1(\G_h(v)+\phiA(v);\de)$ and
\begin{align}\label{proof:functionTopertatorRflow}
T[\phiA_{\la}] = -V'(\la_h+\phiA_{\la}) +V'(\la_h)
+ V''(\la_h)\phiA_{\la},
\end{align}
where the potential $V$ is given in \eqref{def:potentialV}.

Let us consider $\phiA=(\phiA_{\la},\phiA_{\La},\phiA_x,\phiA_y) \in \XcalFlowTotal$ such that $\normFlowTotal{\phiA} \leq \varrho \de^3$.
%
%We define $\Phi=(\Phi_{\la},\Phi_{\La},\Phi_x,\Phi_y) = \G_h + \phiA$.
%%
By Theorem \ref{theorem:singularities}, for $v \in \DFlow$ and $\de$ small 
\begin{align}\label{proof:estimatesFlow}
\vabs{\la_h(v)+\phiA_{\la}(v)} < \pi, \quad
\vabs{\La_h(v)+\phiA_{\La}(v)} < C, \quad
\vabs{\phiA_{x}(v)} < C\de^3, \quad
\vabs{\phiA_{y}(v)} < C\de^3.
\end{align}
%
Then, by definition of $H_1$ in \eqref{def:hamiltonianScalingH1}, we have that
\begin{align*}
H_1(\G_h(v)+\phiA(v);\de) =& \,
H_1^{\Poi}\big(\la_h(v)+\phiA_{\la}(v),
1+\de^2(\La_h(v)+\phiA_{\La}(v)),
\de \phiA_x(v),\de \phiA_y(v);\de \big)  \\
&- V(\la_h(v)+\phiA_{\la}(v)) +
\frac{1}{\de^4} F_{\pend}(\de^2\La_h(v)+\de^2\phiA_{\La}(v)),
\end{align*}
where $H_1^{\Poi}$ is given in \eqref{def:hamiltonianPoincare1} and $F_{\pend}$ in \eqref{def:Fpend}, respectively.
%
(Recall that $F_{\pend}(s)=\OO(s^3)$).
%
By \eqref{proof:estimatesFlow} we have that $\vabs{(\de^2(\La_h(v)+\phiA_{\La}(v)),
\de \phiA_x(v), \de \phiA_y(v))} \ll 1$, 
for $\de$ small enough,  and
$\vabs{\la_h(v)+\phiA_{\la}(v)}<\pi$, as  a result, we can apply the results in Corollary \ref{corollary:seriesH1Poi}.
%
Indeed, for $v \in \DFlow$,
\begin{equation}\label{proof:flowA}
\begin{aligned}	
\vabs{\partial_{\la} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de^2, 
& \quad
\vabs{\partial_{x} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de,
\\
\vabs{\partial_{\La} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de^2, 
& \quad
\vabs{\partial_{y} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de,
\end{aligned}
\end{equation}	
and
\begin{equation}\label{proof:flowB}
\begin{split}
%\vabs{ \partial_{\la\La} H_1(\G_h(v)+\phiA(v);\de)}
%&\leq C \de^2
%\qquad
%\vabs{ \partial^2_{\La} H_1(\G_h(v)+\phiA(v);\de)}
%\leq C \de^2, 
%\\
\vabs{\partial_{i j} H_1(\G_h(v)+\phiA(v);\de)} &\leq C \de, 
\qquad \text{for } i,j \in \claus{\la,\La,x,y}.
\end{split}
\end{equation}

Then, it only remains to compute estimates for  $T[\phiA_{\la}]$.
%
By \eqref{proof:functionTopertatorRflow} and
\eqref{proof:estimatesFlow} we have that, for $v \in \DFlow$,
\begin{equation}\label{proof:flowC}
\begin{split}	
\vabs{T[\phiA](v)} \leq C \vabs{V''(\la_h(v))}
\vabs{\phiA_{\la}(v)} \leq C \de^2, \\
\vabs{D T[\phiA](v)} \leq C \vabs{V'''(\la_h(v))}
\vabs{\phiA_{\la}(v)} \leq C \de^2.
\end{split}
\end{equation}

Lastly, joining the estimates from \eqref{proof:flowA},
\eqref{proof:flowB} and \eqref{proof:flowC} we obtain the statement of the lemma. 

\qed


==> Article Outer/proofH-existenceTechnicalInfty.tex <==


\subsection{Estimates in the infinity domain}
\label{subsubsection:ProofComputationsRRRInf}

To prove Lemma~\ref{lemma:computationsRRRInf}, we need to obtain estimates for $\RRR^{\out}$ and its derivatives.
%
Let us recall that, by its definition in~\eqref{def:operatorRRROuter}, for $z=(w,x,y)$ we have
\begin{align}\label{eq:expressionRRRout}
	\RRR^{\out}[z] = \paren{
		\frac{f_1^{\out}(\cdot,z)}{1+g^{\out}(\cdot,z)},
		\frac{{f_2}^{\out}(\cdot,z) - \frac{i x}{\de^2} \, g^{\out}(\cdot,z)}{1+g^{\out}(\cdot,z)},
		\frac{{f_3}^{\out}(\cdot,z) + \frac{i y}{\de^2} \, g^{\out}(\cdot,z)}{1+g^{\out}(\cdot,z)}
	}^T,
\end{align} 
where $g^{\out} = \partial_w H_1^{\out}$ and $f^{\out}=\paren{-\partial_u H_1^{\out}, i\partial_y H_1^{\out}, -i\partial_x H_1^{\out} }^T$.
%

Therefore, we need to obtain first estimates for the first and second derivatives of $H_1^{\out}$, introduced in~\eqref{def:hamiltonianOuterSplit}, that is
\begin{equation}\label{proof:H1outForM1}
H_1^{\out} = H \circ (\phi_{\equi} \circ \phi_{\out}) - \paren{w + \frac{xy}{\de^2}},
\end{equation}
where $H=H_0+H_1$ with $H_0= H_{\pend}+ H_{\osc}$ (see \eqref{def:hamiltonianScaling},  \eqref{def:hamiltonianScalingH0}).
%and the changes of coordinates $\phi_{\equi}$ and $\phi_{\out}$ are given in \eqref{def:changeEqui} and \eqref{def:changeOuter}, respectively.
%

Since $(\la_h,\La_h)$  is a solution of the Hamiltonian  $H_{\pend}$ and belongs to the energy level $H_{\pend}=-\frac12$,
\begin{align*}
H_0 \circ \phi_{\out}
=
H_{\pend}\paren{\la_h(u),\La_h(u)-\frac{w}{3 \La_h(u)}}
+
H_{\osc}(x,y;\de)
=
-\frac12 
+ w
- \frac{w^2}{6\La_h^2(u)}
+ \frac{x y}{\de^2}.
\end{align*}
%
Therefore, by \eqref{proof:H1outForM1}, the Hamiltonian $H_1^{\out}$ can be expressed (up to a constant) as
\begin{align}\label{eq:expressionHamiltonianInfty}
H_1^{\out} = 
M \circ \phi_{\out}
- \frac{w^2}{6\La_h^2(u)} ,
\end{align}
where 
% $M = H \circ \phi_{\equi}- H_0$.
\begin{align*}
% \label{def:functionM1}
M(\la,\La,x,y;\de) = 
(H \circ \phi_{\equi})(\la,\La,x,y;\de) - 
H_0(\la,\La,x,y).
\end{align*}
%
In the following lemma we give properties of $M$.

\begin{lemma}\label{lemma:expressionHamiltonianInfty}
Fix constants $\varrho>0$ and $\la_0 \in (0,\pi)$.
% and consider
%
Then, there exists $\de_0>0$ such that, 
for $\de \in (0,\de_0)$,
$\vabs{\la}<\la_0$, 
$\vabs{\La}<\varrho$
and 
$\vabs{(x,y)}<\varrho\de$
,
the function $M$ satisfies
\begin{align*}
\vabs{ \partial_{\la} M} &\leq 
C\de^2 \vabs{(\la,\La)} +	C\de \vabs{(x,y)}, &
%
\vabs{ \partial_{x} M} &\leq 
C\de \vabs{(\la,\La,x,y)}, \\
%
\vabs{ \partial_{\La} M} &\leq
C\de^2 \vabs{(\la,\La)} +	C\de \vabs{(x,y)}, &
%
\vabs{ \partial_{y} M} &\leq 
C\de \vabs{(\la,\La,x,y)},
\end{align*}
and
\begin{align*}
\vabs{ \partial^2_{\la} M},
\vabs{ \partial_{\la\La} M},
\vabs{ \partial^2_{\La} M}
&\leq C \de^2, 
\qquad
\vabs{\partial_{i j} M} \leq C \de, 
\quad \text{for } i,j \in \claus{\la,\La,x,y}.
\end{align*}
%for a positive constant $C$ independent of $\de$.
\end{lemma}

\begin{proof}
%Let us analyze now $M_1$ to obtain more accurate estimates of its derivatives.
%
Applying  $\phi_{\equi}$ (see \eqref{def:changeEqui}) to the Hamiltonian $H=H_0 + H_1$,  we have that
\begin{equation}\label{proof:M1expressionLtres}
\begin{split}	
M &= 
\paren{H_0 \circ \phi_{\equi} - H_0}
+ H_1 \circ \phi_{\equi} 
\\
&= 	 \de( x \Ltresy + y\Ltresx) 
+ 3\de^2 \La \LtresLa  
+ \de^4 \paren{-\frac{3}{2}\LtresLa^2 +\Ltresx \Ltresy}
+ H_1 \circ \phi_{\equi}.
\end{split}
\end{equation}
Then,  
%taking into account that $\norm{(\LtresLa(\de),\Ltresx(\de),\Ltresy(\de))} \leq C$, we have that, 
%\begin{equation}\label{proof:estimatesM1B}
%\begin{split}	
%\vabs{\partial_{\la} M_1} &= \vabs{\partial_{\la} H_1 (\la,\La + \de^2\LtresLa, x+ \de \Ltresx, y + \de \Ltresy)},
%\\
%\vabs{\partial_{\La} M_1} &\leq C\de^2 + \vabs{\partial_{\La} H_1 (\la,\La + \de^2\LtresLa, x+ \de \Ltresx, y + \de \Ltresy)},
%\\ 
%\vabs{\partial_{x} M_1} &\leq C\de + \vabs{\partial_{x} H_1 (\la,\La + \de^2\LtresLa, x+ \de \Ltresx, y + \de \Ltresy)}, 
%\\
%\vabs{\partial_{\la} M_1} &\leq C \de + \vabs{\partial_{y} H_1 (\la,\La + \de^2\LtresLa, x+ \de \Ltresx, y + \de \Ltresy)},
%\end{split}
%\end{equation}
%and
\begin{align}\label{proof:estimatesDerivativesM1B}
\vabs{\partial_{i j} M} \leq 
\vabs{\partial_{i j} H_1(\la,\La + \de^2\LtresLa, x+ \de \Ltresx, y + \de \Ltresy;\de)}
, 
\quad \text{for } i,j \in \claus{\la,\La,x,y}.
\end{align}
Since $\vabs{\La}<\varrho$
and $\vabs{(x,y)}<\varrho\de$,
then
$\vabs{\La+\de^2\LtresLa}<2\varrho$
and ${\vabs{(x+\de^3 \Ltresx,y+\de^3\Ltresy)}<2\varrho\de}$,
for $\de$ small.
%
% Therefore, we analyze the derivatives of $H_1$ under these assumptions.
By the definition of $H_1$
in \eqref{def:hamiltonianScalingH1} we have that,
\begin{align*}	
H_1(\la,\La,x,y;\de) &=
H_1^{\Poi}
\paren{\la,1+\de^2\La,\de x, \de y;\de^4} 
- V\paren{\la} 
+ \frac{1}{\de^4} F_{\pend}(\de^2\La),
%%
%H_1(\la,\La,0,0;\de) &=
%\paren{H_1^{\Poi}-V} 
%\paren{\la,1+\de^2\La,0,0;\de^4} 
%+ \frac{1}{\de^4} F_{\pend}(\de^2\La)
%= \OO(\de^2),
\end{align*}
where $H_1^{\Poi}$ is given in \eqref{def:hamiltonianPoincare01} (see also \eqref{def:changeScaling}),
$V$ is given \eqref{def:potentialV}
and $F_{\pend}$ is given \eqref{def:Fpend} and satisfies $F_{\pend}(s)=\OO(s^3)$. 
%
Since $\vabs{(\de^2\La,\de x, \de y)} < 2\varrho \de^2 \ll 1$, we  apply  Lemma \ref{corollary:seriesH1Poi} (recall that $\de=\mu^{\frac14}$) and Cauchy estimates to 
% the derivatives
% %
% Then, differentiating the previous expression for $H_1$ we 
obtain 
%\begin{equation}\label{proof:estimatesM1C}
%\begin{aligned}	
%\vabs{\partial_{\la} H_1(\la,\La,0,0;\de)} 
%&\leq C \de^2, 
% & \quad
%\vabs{\partial_{\la} H_1} 
%&\leq C \de, 
% & \quad
%\vabs{\partial_{x} H_1} 
%&\leq C \de,
%\\
%\vabs{\partial_{\La} H_1(\la,\La,0,0;\de)} 
%&\leq C \de^2, 
% & \quad
%\vabs{\partial_{\La} H_1} 
%&\leq C \de^2, 
% & \quad
%\vabs{\partial_{y} H_1} 
%&\leq C \de,
%\end{aligned}
%\end{equation}	
%and
\begin{align}\label{proof:estimatesDerivativesM1C}
	\vabs{ \partial^2_{\la} H_1}
	\vabs{ \partial_{\la\La} H_1},
	\vabs{ \partial^2_{\La} H_1}
	&\leq C \de^2, 
	\qquad
	\vabs{\partial_{i j} H_1} \leq C \de, 
	\quad \text{for } i,j \in \claus{\la,\La,x,y}.
\end{align}
%\begin{equation}
%\begin{aligned}	
%\vabs{\partial_{\la\La} H_1} 
%&\leq C \de^2, 
%& \quad
%\vabs{\partial^2_{\La} H_1} 
%&\leq C \de^4, 
%& \quad
%\vabs{\partial_{\la x} H_1} 
%&\leq C \de,
%&\quad
%\vabs{\partial_{\la y} H_1} 
%&\leq C \de, 
%\\
%\vabs{\partial^2_{\La x} H_1} 
%&\leq C \de^3, 
%& \quad
%\vabs{\partial_{\La y} H_1} 
%&\leq C \de^3, 
%& \quad
%\vabs{\partial^2_{x} H_1} 
%&\leq C \de^2,
%& \quad
%\vabs{\partial^2_{y} H_1} 
%&\leq C \de^2.
%\end{aligned}
%\end{equation}	
%
Then,   \eqref{proof:estimatesDerivativesM1B} and
\eqref{proof:estimatesDerivativesM1C} give the estimates for the second derivatives of $M$.


For the first derivatives of $M$, let us take into account that, by Theorem~\ref{theorem:singularities},  $0$ is a critical point of both Hamiltonians $(H \circ \phi_{\equi})$ and $H_0$ and,
%
therefore, also of $M= (H \circ \phi_{\equi})- H_0$.
%
This fact and the estimates of the second derivatives, together with the mean value theorem, gives the estimates for the first derivatives of $M$.
%
%\begin{align*}
%	\Dx{M_1}{\la}({0};\de) =
%	\Dx{M_1}{\La}({0};\de) =
%	\Dx{M_1}{x}({0};\de) =
%	\Dx{M_1}{y}({0};\de) = 0.
%\end{align*}
%In particular, 
%\begin{align*}% \label{proof:estimatesM1A}
%	\vabs{ \partial_{\la} M_1},
%	\vabs{ \partial_{\La} M_1},
%	\vabs{ \partial_{x} M_1},
%	\vabs{ \partial_{y} M_1} &\leq 
%	C \paren{
%		\vabs{\la}+ \vabs{\La}+\vabs{x}+\vabs{y}}.
%\end{align*}	
%Therefore, joining this result with the estimates in \eqref{proof:estimatesM1B} and \eqref{proof:estimatesM1C}, we obtain the statement for the first derivatives of $M_1$. 
\end{proof}

%where $H$ is given in~\eqref{def:hamiltonianScaling} and $\phi_{\equi}$ and $\phi_{\out}$ are given in~\eqref{def:changeEqui} and~\eqref{def:changeOuter}, respectively.
%%
%Then, defining $M_1 = (H \circ \phi_{\equi})- H_0$, we have
%\[
%H^{\out}_1 = \paren{H_0 \circ \phi_{\out}  
%-\paren{w + \frac{xy}{\de^2}}} +
%M_1 \circ \phi_{\out} 
%=  - \frac{w^2}{6\La_h^2(u)} +
%M_1 \circ \phi_{\out} .
%\]
% 
%	Let us first consider Hamiltonian $H^{\equi}=H_0+H_1^{\equi}$ as defined on~\eqref{def:hamiltonianEqui}. 
%	%
%	By construction, $\mathbf{0}$ is a fixed point of $H^{\equi}_1$. Therefore,
%	\begin{align*}
%		\Dx{H_1^{\equi}}{\la}(\mathbf{0};\de) =
%		\Dx{H_1^{\equi}}{\La}(\mathbf{0};\de) =
%		\Dx{H_1^{\equi}}{x}(\mathbf{0};\de) =
%		\Dx{H_1^{\equi}}{y}(\mathbf{0};\de) = 0,
%	\end{align*}
%	and the derivatives of $H_1^{\equi}$ are of order $1$ with respect to $(\la,\La,x,y)$. Then, for $(\la,\La,x,y)\sim \mathbf{0}$, we can express these derivatives as
%	\begin{align}\label{proof:linealH1equi}
%		D H_1^{\equi} = Q \cdot (\la,\La,x,y)^T
%	\end{align}
%	where $Q$ is a $4\times4$ functional matrix such that 
%	$Q_{i,j}=Q_{i,j}(\la,\La,x,y)$.
%	%
%	Moreover, since by its definition $H_1^{\equi} \sim \OO(\de)$, we have that
%	\begin{align}\label{proof:matrixQgeneral}
%		\norm{Q_{i,j}(\la,\La,x,y)} \leq C\de.
%	\end{align}
%	Additionally, by the definition of $H_1^{\equi}$, notice that
%	\[
%	H_1^{\equi}(\la,\La,0,0;\de) \sim \OO(\de^2).
%	\]
%	Therefore, we can consider $Q_{i,j}=Q_{i,j}(\la,\La)$ for $i,j\in  \claus{1,2}$ and
%	\begin{align}\label{proof:matrixQlaLa}
%		\norm{Q_{i,j}(\la,\La)} \leq C\de^2, \quad
%		\text { for } i,j \in  \claus{1,2}.
%	\end{align}
%	%Then, the first two derivatives of $H_{1}^{\equi}$, for $(\la,\La,x,y) \sim \mathbf{0}$ can be express as
%	%\[
%	%\begin{pmatrix}
%	%	\partial_{\la} H_1^{\equi} \\
%	%	\partial_{\La} H_1^{\equi} 
%	%\end{pmatrix}
%	%= Q^{a} \cdot 
%	%\begin{pmatrix}
%	%	\la \\
%	%	\La
%	%\end{pmatrix}
%	%+ Q^b \cdot
%	%\begin{pmatrix}
%	%	x \\
%	%	y
%	%\end{pmatrix}
%	%\] 
%	%where $Q^a$ and $Q^b$ are $2\times2$ functional matrices such that
%	%$Q^a_{i,j}=Q^a_{i,j}(\la,\La)$ and
%	%$Q^b_{i,j}=Q^b_{i,j}(\la,\La,x,y)$.
%	%%
%	%Moreover, we have that
%	%\[
%	%\norm{Q^a_{i,j}(\la,\La)} \leq C\de^2 
%	%\quad \text{ and } \quad
%	%\norm{Q^b_{i,j}(\la,\La,x,y)} \leq C\de.
%	%\]
%	%%%%%%%%%%%
%	Then, let us recall the outer change of coordinates $\phi_{\out}:(u,w,x,y) \to (\la,\La,x,y)$, as defined in~\eqref{def:changeOuter}, such that by~\eqref{eq:H1outerBetter} we have that
%	\begin{equation}\label{proof:H1outerBetter}
%		H_1^{\out}(u,w,x,y;\de) = H_1^{\equi}\paren{\la_h,\La_h(u)-\frac{w}{3\La_h(u)},x,y;\de}.
%	\end{equation}
%	where $H_1^{\equi}$ was defined on~\eqref{def:hamiltonianEqui}.


\begin{proof}[End of the proof of Lemma~\ref{lemma:computationsRRRInf}]

Let us consider $\varphi=(\varphi_w,\varphi_x,\varphi_y)^T \in \XcalInftyTotal$ such that
$\normInftyTotal{\phiA} \leq \varrho \de^3$.
%
We estimate the first and second derivatives of $H_1^{\out}$ evaluated at $(u,\phiA(u))$ (recall \eqref{eq:expressionRRRout}), given by
% By \eqref{eq:expressionHamiltonianInfty}, we have that
\begin{align}\label{proof:expressionH1sepInfty}
H_1^{\out}(u,\phiA(u);\de) = M\paren{\la_h(u),\La_h(u)-\frac{\phiA_w(u)}{3\La_h(u)},
\phiA_x(u),\phiA_y(u);\de}
- \frac{\phiA^2_w(u)}{6\La_h^2(u)}. 
\end{align}	
First, let us define
\begin{align*}
{\varphi}_{\la}(u) = \la_h(u), \qquad
{\varphi}_{\La}(u) = \La_h(u)-\frac{\varphi_w(u)}{3\La_h(u)}
\quad \text{and} \quad
\Phi = (\phiA_{\la},\phiA_{\La},\phiA_x,\phiA_y).
\end{align*}
Since $\normInftyTotal{\phiA} \leq \varrho \de^3$ and $\la_h, \La_h \in \XcalInfty_{\vap}$ (see \eqref{eq:separatrixBanachSpace}), 
\begin{equation}\label{proof:estimatesCoordinatesEqui}
%\normInfty{\la_h}_{\vap},
%\normInfty{\La_h}_{\vap} \leq C,
%\quad	
\normInfty{\varphi_{w}}_{2\vap} \leq C \de^2, \qquad
\normInfty{\varphi_{x}}_{\vap},
\normInfty{\varphi_{y}}_{\vap} \leq C \de^3, \qquad
\normInfty{\varphi_{\la}}_{\vap},
\normInfty{\varphi_{\La}}_{\vap} \leq C.
\end{equation}
Moreover since, by Theorem \ref{theorem:singularities}, $\la_h(u)\neq\pi$ for  $u \in \DuInfty$, we have that
\[
\vabs{\phiA_{\la}(u)} = \vabs{\la_h(u)} < \pi,
%
\quad
%
\vabs{\phiA_{\La}(u)}
\leq C e^{-\vap \rhoInfty}
\leq C,
\quad
%
\vabs{(\phiA_{x}(u), \phiA_y(u))}
\leq C\de^3 e^{-\vap \rhoInfty}
\leq C\de^3
\]
and, therefore, we can apply  Lemma~\ref{lemma:expressionHamiltonianInfty} to \eqref{proof:expressionH1sepInfty}.
In the following computations, we use generously Lemma \ref{lemma:sumNormsOutInf} without mentioning it.

\begin{enumerate}
\item First, we consider $g^{\out}=\partial_w H_1^{\out}$.
%
By \eqref{proof:expressionH1sepInfty}, we have that
\begin{align*}
g^{\out}(u,\varphi(u)) 
%
&=-\frac{\partial_{\La} M \circ \Phi(u)}{3\La_h(u)} 
-\frac{\varphi_{w}(u)}{3\La_h^2(u)}.
\end{align*}
Notice that, by Theorem \ref{theorem:singularities}, $\vabs{\La_h(u)}\geq C$ for $u \in \DuInfty$. Then, $\normInftySmall{\La_h^{-1}}_{-\vap} \leq C$.
Therefore, by Lemma \ref{lemma:expressionHamiltonianInfty} and estimates~\eqref{proof:estimatesCoordinatesEqui}, we have that
\begin{equation}\label{proof:boundsInftyg}
\begin{split}	
\normInfty{g^{\out}(\cdot,\varphi)}_0 &\leq
C \de \boxClaus{\de\normInfty{\varphi_{\la}}_{\vap} +
\de\normInfty{\varphi_{\La}}_{\vap}  +
\normInfty{\varphi_{x}}_{\vap} +
\normInfty{\varphi_{y}}_{\vap}} 
+ C \normInfty{\varphi_{w}}_{2\vap} \\
&\leq C \de^2.
\end{split}
\end{equation}
%
To compute its derivative with respect to $w$, by \eqref{proof:expressionH1sepInfty}, we have that
\begin{align*}
\partial_w g^{\out} (u,\varphi(u)) 
%
&=
\frac{\partial^2_{\La} M \circ \Phi(u)}{9\La^2_h(u)} 
-\frac{1}{3\La^2_h(u)},
\end{align*}
and, by Lemma \ref{lemma:expressionHamiltonianInfty} and estimates~\eqref{proof:estimatesCoordinatesEqui}, 
%
% \begin{equation}\label{proof:boundsInftyDerivative1g}
$\normInfty{\partial_w g^{\out}(\cdot,\varphi)}_{-2\vap} \leq C$.
% \end{equation}
Following a similar procedure, we obtain
% \begin{equation}\label{proof:boundsInftyDerivative2g}
$\normInfty{\partial_x g^{\out}(\cdot,\varphi)}_{-\vap} \leq C \de$
% , \qquad
and $\normInfty{\partial_y g^{\out}(\cdot,\varphi)}_{-\vap} \leq C \de$.
% \end{equation}

\item Now, we obtain estimates for $f_1^{\out}=-\partial_u H_1^{\out}$.
%
By \eqref{proof:expressionH1sepInfty}, we have that
\begin{align*}
f_1^{\out}(u,\varphi(u)) =&
%
- \lad_h(u)  \partial_{\la}{M} \circ \Phi(u)
%
-\frac{\Lad_h(u)}{3\La^3_h(u)} \varphi^2_{w}(u) \\
%
&- \paren{\Lad_h(u) + \frac{\Lad_h(u)}{3 \La_h^2(u)} \varphi_{w}(u)} 
\partial_{\La}{M} \circ \Phi(u).
\end{align*}
Then, since $\lad_h, \Lad_h \in \XcalInfty_{\vap}$,  by Lemma \ref{lemma:expressionHamiltonianInfty} and estimates~\eqref{proof:estimatesCoordinatesEqui}, we have that
% \begin{equation}\label{proof:boundsInftyDerivative1f1}
$\normInfty{f_1^{\out}(\cdot,\varphi)}_{2\vap} \leq C\de^2$.
% \end{equation}
To compute its derivative with respect to  $x$, by \eqref{proof:expressionH1sepInfty}, 
\begin{align*}
\partial_x f_1^{\out}(u,\varphi(u)) =&
%
- \lad_h(u) \partial_{x \la} M \circ \Phi(u) 
%
- \paren{\Lad_h(u) + \frac{\Lad_h(u)}{3 \La_h^2(u)} \varphi_{w}(u)} 
\partial_{x \La} M \circ \Phi(u)
\end{align*}
and, therefore,
%
% \begin{equation}\label{proof:boundsInftyDerivative2f1}
$\normInfty{\partial_x f_1^{\out}(\cdot,\varphi)}_{\vap} \leq C\de$.
% \end{equation}
Similarly one can obtain
% \begin{equation}
$\normInfty{\partial_w f_1^{\out}(\cdot,\varphi)}_{0} \leq C\de^2$ and
% \qquad
$\normInfty{\partial_y f_1^{\out}(\cdot,\varphi)}_{\vap} \leq C\de$.
% \end{equation}
\item Analogously to the previous estimates, 
we can obtain bounds for $f^{\out}_2= i \partial_y H_1^{\out}$ and $f^{\out}_3=-i \partial_x H_1^{\out}$.
%
Then, for $j=2,3$, it can be seen that
% \begin{equation}\label{proof:boundsInftyRestA}
% \begin{aligned}
$\normInftySmall{f_j^{\out}(\cdot,\varphi)}_{\vap} \leq C\de$, 
% \end{aligned}
% \end{equation}
and differentiating we obtain
% \begin{equation}\label{proof:boundsInftyRestB}
% \begin{aligned}
$\normInftySmall{\partial_w f_j^{\out}(\cdot,\varphi)}_{-\vap} \leq C\de$,
$\normInftySmall{\partial_x f_j^{\out}(\cdot,\varphi)}_{0} \leq C\de$ and
%
$\normInftySmall{\partial_y f_j^{\out}(\cdot,\varphi)}_{0} \leq C\de$.
% \end{aligned}
% \end{equation}
%We can compute estimates as well for $\wt{f}_j^{\out}$ with $j=2,3$, (see~\eqref{eq:expressionf1f2f3}), 
%\begin{equation}\label{proof:boundsInftyRestTilde}
%\begin{aligned}
%\normInftySmall{\wt{f}_j^{\out}(\cdot,\varphi)}_{\vap}, \,
%%
%\normInftySmall{\partial_w \wt{f}_j^{\out}(\cdot,\varphi)}_{-\vap}, \,
%%
%\normInftySmall{\partial_x \wt{f}_j^{\out}(\cdot,\varphi)}_{0}, \,
%%
%\normInftySmall{\partial_y \wt{f}_j^{\out}(\cdot,\varphi)}_{0} \leq C\de.
%\end{aligned}
%\end{equation}
%%
\end{enumerate}
%
Then, by the definition of $\RRR^{\out}$ in~\eqref{eq:expressionRRRout} and the just obtained  estimates, we complete the proof of the lemma.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{lemma}\label{lemma:expressionHamiltonianInfty}
%	The Hamiltonian $H_1^{\out}$, as given in~\eqref{def:hamiltonianOuterSplit}, can be expressed (up to a constant) as
%	\begin{align}\label{eq:expressionHamiltonianInfty}
%		H_1^{\out}(u,w,x,y;\de) = 
%		- \frac{w^2}{6\La_h^2(u)} +
%		M_1 \paren{\la_h(u),\La_h(u)-\frac{w}{3\La_h(u)},x,y;\de},
%	\end{align}
%	where $M_1 = (H \circ \phi_{\equi})- H_0$ (see~\eqref{def:hamiltonianScaling}, \eqref{def:changeEqui}) and $(\la_h,\La_h)$ are given in~\eqref{eq:separatrixParametrization}.
%	%
%	%Moreover, $D M_1^{\out}(\la,\La,x,y;\de) = Q \cdot (\la,\La,x,y)^T$ 
%	%where $Q$ is a $4\times4$ functional matrix such that 
%	%\begin{itemize}
%	%\item $Q_{i,j}=Q_{i,j}(\la,\La;\de)$ and $\norm{Q_{i,j}(\la,\La;\de)} \leq C\de^2$, for $i,j\in  \claus{1,2}$.
%	%%\begin{align}\label{proof:matrixQlaLa}
%	%%	\norm{Q_{i,j}(\la,\La)} \leq C\de^2, \quad
%	%%		\text { for } i,j \in  \claus{1,2}.
%	%%\end{align}
%	%\item $Q_{i,j}=Q_{i,j}(\la,\La,x,y;\de)$ and
%	%$\norm{Q_{i,j}(\la,\La,x,y)} \leq C\de$, otherwise.
%	%%\begin{align}\label{proof:matrixQgeneral}
%	%%	\norm{Q_{i,j}(\la,\La,x,y)} \leq C\de.
%	%%\end{align}
%	%\end{itemize}
%	
%	Moreover, for $\norm{(\la,\La,x,y)} \ll 1$, $M_1=M_1(\la,\La,x,y;\de)$ is analytic and
%	\begin{align*}
%		\vabs{ \partial_{\la} M_1} &\leq 
%		C\de^2 \paren{\vabs{\la} + \vabs{\La}} +	C\de \paren{\vabs{x} + \vabs{y}}, &
%		%
%		\vabs{ \partial_{x} M_1} &\leq 
%		C \de \paren{\vabs{\la}+\vabs{\La}+
%			\vabs{x}+\vabs{y}}, \\
%		%
%		\vabs{ \partial_{\La} M_1} &\leq
%		C\de^2 \paren{\vabs{\la} + \vabs{\La}} +	C\de \paren{\vabs{x} + \vabs{y}}, &
%		%
%		\vabs{ \partial_{y} M_1} &\leq 
%		C\de \paren{
%			\vabs{\la}+ \vabs{\La}+\vabs{x}+\vabs{y}}. 
%	\end{align*}
%	%and
%	%\begin{align*}
%	%\vabs{ \partial^2_{\la} M_1},
%	%\vabs{ \partial^2_{\La} M_1},
%	%\vabs{ \partial_{\la\La} M_1} \leq C \de^2, 
%	%\quad
%	%\vabs{ \partial_{z_1 z_2} M_1}\leq C \de,
%	%\text{ for }
%	%\end{align*}
%\end{lemma}
%
%\begin{proof}
%	Let us recall the Hamiltonian $H_1^{\out}$ is defined in~\eqref{def:hamiltonianOuterSplit} as
%	\begin{equation}\label{proof:hamiltonianOuter1}
%		H^{\out}_1 =
%		{H} \circ \paren{\phi_{\equi} \circ \phi_{\out}} -\paren{w + \frac{xy}{\de^2}},	
%	\end{equation}
%	where  the change of coordinates (see~\eqref{def:changeEqui} and~\eqref{def:changeOuter}) are
%	\begin{equation}\label{proof:changeOfCoordinatesInfty}
%		\begin{aligned}
%			&\phi_{\equi}:(\la,\La,x,y) \mapsto 
%			\paren{\la,\La + \de^2 \LtresLa(\de),x + \de^3\Ltresx(\de),y + \de^3 \Ltresy(\de)} ,
%			\\
%			&\phi_{\out}:(u,w,\xp,\yp) \mapsto \paren{\la_h(u),\La_h(u) - \frac{w}{3\La_h(u)},\xh,\yh},
%		\end{aligned}
%	\end{equation}
%	and the Hamiltonian $H=H_0 + H_1$ (given in~\eqref{def:hamiltonianScaling}) such that $H_0$ is defined as
%	\begin{equation}\label{proof:H0expressionInfty}
%		H_0 = H_{\pend} + H_{\osc}, 
%		\quad \text{where} \quad
%		H_{\pend}(\la,\La) = -\frac{3}{2}\La^2 + V(\la),
%		\quad
%		H_{\osc}(x,y;\de) = \frac{xy}{\de^2},
%	\end{equation} 
%	where $V$ is the potential given in~\eqref{def:potentialV}. 
%	%
%	Then, since $M_1 = (H \circ \phi_{\equi})- H_0$ and \eqref{proof:hamiltonianOuter1}, we have that
%	\begin{align*}
%		H_1^{\out} &= M_1 \circ \phi_{\out} + H_0 \circ \phi_{\out} -\paren{w + \frac{xy}{\de^2}} \\
%		&= M_1 \circ \phi_{\out}
%		- \frac{3}{2}\La^2_h(u) + V(\la_h(u))  - \frac{w^2}{6\La_h^2(u)}.
%	\end{align*}
%	Since $(\la_h,\La_h)$ is the parametrization of the separatrix of $H_{\pend}$ (see~\eqref{eq:separatrixParametrization}) we have that $H_{\pend}(\la_h(u),\La_h(u))=H_{\pend}(0,0) = -\frac{1}{2}$, and we obtain expression \eqref{eq:expressionHamiltonianInfty}.
%	
%	Notice that, by Theorem~\ref{theorem:singularities},  $\mathbf{0}$ is a fixed point of both Hamiltonians $(H \circ \phi_{\equi})$ and $H_0$.
%	%
%	Therefore, ${0}$ is also a fixed point of $M_1= (H \circ \phi_{\equi})- H_0$ and
%	\begin{align*}
%		\Dx{M_1}{\la}({0};\de) =
%		\Dx{M_1}{\La}({0};\de) =
%		\Dx{M_1}{x}({0};\de) =
%		\Dx{M_1}{y}({0};\de) = 0.
%	\end{align*}
%	In particular, $M_1$ is analytic on a neighborhood of $\mathbf{0}$ and, for $\norm{(\la,\La,x,y)} \ll 1$ we have
%	\begin{align} \label{proof:estimatesM1}
%		\vabs{ \partial_{\la} M_1},
%		\vabs{ \partial_{\La} M_1},
%		\vabs{ \partial_{x} M_1},
%		\vabs{ \partial_{y} M_1} &\leq 
%		C \paren{
%			\vabs{\la}+ \vabs{\La}+\vabs{x}+\vabs{y}}.
%		%\text{ for } \norm{(\la,\La,x,y)} \ll 1.
%	\end{align}	
%	
%	Let us analyze now $M_1$ to obtain more accurate estimates of its derivatives.
%	%
%	Since $H=H_0 + H_1$, taking into account~\eqref{proof:changeOfCoordinatesInfty} and~\eqref{proof:H0expressionInfty}, we have that
%	\begin{align*}
%		M_1 &= (H_0 + H_1) \circ \phi_{\equi} - H_0 \\
%		&= 	H_1 \circ \phi_{\equi} 
%		+ \de( x \Ltresy + y\Ltresx) 
%		+ 3\de^2 \La \LtresLa  
%		+ \de^4 \paren{-\frac{3}{2}\LtresLa^2 +\Ltresx \Ltresy}.
%	\end{align*}
%	%
%	Moreover, by the construction of $H_1$
%	(see~\eqref{def:hamiltonianScalingH1}), we have that, for $\norm{(\la,\La,x,y)} \ll 1$,
%	\begin{align*}	
%		H_1(\la,\La,x,y;\de) &=
%		\paren{H_1^{\Poi}-V} 
%		\paren{\la,1+\de^2\La,\de x, \de y;\de^4} 
%		+ \frac{1}{\de^4} F_{\pend}(\de^2\La)
%		= \OO(\de),
%		\\
%		%
%		H_1(\la,\La,0,0;\de) &=
%		\paren{H_1^{\Poi}-V} 
%		\paren{\la,1+\de^2\La,0,0;\de^4} 
%		+ \frac{1}{\de^4} F_{\pend}(\de^2\La)
%		= \OO(\de^2),
%	\end{align*}
%	where $H_1^{\Poi}$ is given in~\eqref{def:hamiltonianPoincare01} and 
%	$F_{\pend}$ in~\eqref{def:Fpend}. 
%	%
%	Accordingly,
%	\begin{align*}
%		M_1(\la,\La,x,y;\de) = \OO(\de), \qquad
%		M_1(\la,\La,0,0;\de) = \OO(\de^2).
%	\end{align*}
%	Then, joining these results with~\eqref{proof:estimatesM1} we obtain the estimates of the lemma. 
%\end{proof}


==> Article Outer/proofH-existenceTechnicalIntro.tex <==
In this appendix we prove the technical Lemmas \ref{lemma:computationsRRRInf} and
\ref{lemma:computationsRRROut}.
% ,
% \ref{lemma:computationsRRRtransitionOuter}
% and
% \ref{lemma:computationsRFlow} \textcolor{red}{els ultims dos lemmes potser es treuen}.
%
All these results involve, in some sense, estimates for the first and second derivatives of the Hamiltonian $H_1^{\out}$ in \eqref{def:hamiltonianOuterSplit}.
%
However, to obtain estimates for $H_1^{\out}$, we  first obtain some properties of $H_1^{\Poi}$ (see \eqref{def:hamiltonianPoincare01}), which can be written as
\begin{equation}\label{def:hamiltonianPoincare1}
\begin{split}
H_1^{\Poi} = 
\frac1{\mu} \PP[0] - \frac{1-\mu}{\mu}{\PP[\mu]}
	- {\PP[\mu-1]},
\end{split}
\end{equation}
where
\begin{equation}\label{def:functionD}
\PP[\zeta](\la,L,\eta,\xi) = 
\paren{\norm{q-(\zeta,0)}^{-1}}
\circ \phi_{\Poi}.
\end{equation}
%The function $P[\zeta]$ does not have an explicit expression.
%
In \cite{articleInner}, we computed the series expansion of $\PP[\zeta]$ in powers of $(\eta,\xi)$. In particular, $\PP[\zeta]$ can be written as 
\begin{equation}\label{def:functionD2}
 \PP[\zeta](\la,L,\eta,\xi) =\frac{1}{\sqrt{A[\zeta](\la)+	B[\zeta](\la,L,\eta,\xi)}}
\end{equation}
where $A$ and $B$ are of the form 
\begin{align}
A[\zeta](\la) =& \, 
1- 2\zeta \cos \la  +\zeta^2, \label{def:DA} \\
%%%
\begin{split}\label{def:DB}
	B[\zeta](\la,L,\eta,\xi) =& \,
	4 (L-1)(1-\zeta\cos\la) +
	\frac{\eta}{\sqrt2}
	\paren{3 \zeta - 2e^{-i\la}  - \zeta e^{-2i\la}} \\
	%
	&+ \frac{\xi}{\sqrt2}
	\paren{3 \zeta - 2 e^{i\la} - \zeta e^{2 i\la}}
	+ R[\zeta](\la,L,\eta,\xi),
\end{split} 
\end{align}
and, for fixed $\varrho>0$,  $R$ is  analytic and satisfies that
\begin{equation}\label{eq:boundD2mes}
	\vabs{R[\zeta](\la,L,\eta,\xi)} \leq 
	K(\varrho) \vabs{(L-1,\eta,\xi)}^2,
\end{equation}
%\begin{equation}\label{eq:boundRPoi}
%	\vabs{R[\zeta](\la,L,\eta,\xi)} \leq 
%	\vabs{\frac{B[\zeta]}{A[\zeta]}},
%\end{equation}
for $\vabs{\Im \la}\leq \varrho$, $\vabs{(L-1,\eta, \xi)} \ll 1$ and $\zeta\in [-1,1]$.

Then, wherever $|A[\zeta](\la)|>|B[\zeta](\la,L,\eta,\xi)|$, $\PP[\zeta](\la,L,\eta,\xi)$ can be written as 
% %
% The next result is a direct consequence of Lemma 4.1 in \cite{articleInner}.
% 
% \begin{lemma}\label{lemma:seriesH1Poi}
% Fix $\zeta \in [-1,1]$ and define .
% \begin{align}
% A[\zeta](\la) =& \, 
% 1- 2\zeta \cos \la  +\zeta^2, \label{def:DA} \\
% %%%
% \begin{split}\label{def:DB}
% 	B[\zeta](\la,L,\eta,\xi) =& \,
% 	4 (L-1)(1-\zeta\cos\la) +
% 	\frac{\eta}{\sqrt2}
% 	\paren{3 \zeta - 2e^{-i\la}  - \zeta e^{-2i\la}} \\
% 	%
% 	&+ \frac{\xi}{\sqrt2}
% 	\paren{3 \zeta - 2 e^{i\la} - \zeta e^{2 i\la}}
% 	+ R[\zeta](\la,L,\eta,\xi).
% \end{split} 
% \end{align}
% 
% % 
% Then, if 
% 
% for $\vabs{(L-1,\eta, \xi)} \ll 1$, $D[\zeta]$ can be written as
\begin{equation}\label{def:SerieP}
	\PP[\zeta](\la,L,\eta,\xi) =  
	\frac1{\sqrt{A[\zeta]}} +
	\sum_{n=1}^{+\infty}
	\binom{-\frac12}{n}
	\frac{\paren{B[\zeta]}^n }{ \paren{A[\zeta]}^{n+\frac12}}.
\end{equation}
%\begin{align*}
%P[\zeta] =  
%\frac1{\sqrt{A[\zeta]}} +
% \frac{B_1[\zeta]}{2(A[\zeta])^{\frac32}}
%+ B_{\geq 2}[\zeta],
% %\end{align*}
% where 
% %
% In addition, for a fixed $\varrho\geq 0$ such that $\vabs{\Im \la}\leq \varrho$
% %
% the function $R[\zeta]$ is analytic and satisfies that
% \begin{equation}\label{eq:boundD2mes}
% 	\vabs{R[\zeta](\la,L,\eta,\xi)} \leq 
% 	C \vabs{(L-1,\eta,\xi)}^2,
% \end{equation}
% %\begin{equation}\label{eq:boundRPoi}
% %	\vabs{R[\zeta](\la,L,\eta,\xi)} \leq 
% %	\vabs{\frac{B[\zeta]}{A[\zeta]}},
% %\end{equation}
% with $C=C(\varrho)$ a positive constant independent of $\zeta$.
% % \end{lemma}

\begin{remark}\label{remark:collisions}
The Hamiltonian $H^{\Poi} = H_0^{\Poi}	+ \mu H_1^{\Poi}$
 (see \eqref{def:hamiltonianPoincare} and \eqref{def:hamiltonianPoincare1}) is analytic away from the collisions with the primaries, that is zeroes of the denominators of  $\PP[\mu]$ and $\PP[\mu-1]$.
% %
% (which correspond with collision with the primaries $S$ and $P$, respectively).
%
% Notice that, since $A[0]=1$, the function $D[0]$ is analytic.
%
For $0<\mu \ll 1$,  one has
\begin{align*}
A[\mu] = 1 + \OO(\mu), \qquad 
A[\mu-1] = 2 +2 \cos\la + \OO(\mu).
\end{align*}
Therefore, in the regime that we consider, collisions with the primary $S$ are not possible but collisions with $P$ may take place at $\la \sim \pi$. 
%
%As a consequence, in the following, it is necessary to be careful when computing $P[\mu-1]$ near $\la=\pi$.
\end{remark}

We now obtain  estimates for $H_1^{\Poi}$ in domains ``far'' from $\la=\pi$. 
%(which corresponds with $L_3$ and is far from collision).

\begin{lemma}\label{corollary:seriesH1Poi}
Fix $\la_0 \in (0,\pi)$ and $\mu_0\in (0,\frac12)$ and consider the Hamiltonian $H_1^{\Poi}$ and the potential $V$ introduced in \eqref{def:hamiltonianPoincare1} and 
\eqref{def:potentialV}, respectively.	
%
Then, for 
for $\vabs{\la}<\la_0$, $\vabs{(L-1,\eta,\xi)}\ll 1$ and $\mu\in(0,\mu_0)$,
the Hamiltonian $H_1^{\Poi}$ can be written as
\begin{align*}
	H_1^{\Poi}(\la,L,\eta,\xi;\mu)-V(\la) 
	=&
	D_0(\mu,\la) +
	D_{1}(\mu,\la) \big((L-1),\eta,\xi \big) +
	D_2(\la,L,\eta,\xi;\mu),
\end{align*}
such that, for $j=1,2,3$,
\begin{align*}
	&\vabs{D_{0}(\mu,\la)} \leq K \mu,
	\qquad
	\vabs{(D_{1}(\mu,\la))_j} \leq K, 
	\qquad
	\vabs{D_2(\la,L,\eta,\xi;\mu)} \leq 
	K \vabs{(L-1,\eta,\xi)}^2,
\end{align*}
with $K$ a positive constant independent of $\la$ and $\mu$.
\end{lemma}

%\textcolor{red}{In order to simplify the notation, throughout this appendix, we denote by $C$ any positive constant independent of $\de=\mu^{\frac14}$ and $\kappa$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{align*}
%	H_1^{\Poi}(\la,L,\eta,\xi;\mu)-V(\la) 
%	=&
%	D_0(\mu) +
%	D_{1,L}(\mu) (L-1) +
%	D_{1,\eta}(\mu) \eta \\ &+ 
%	D_{1,\xi}(\mu) \xi +
%	D_2(\la,L,\eta,\xi;\mu),
%\end{align*}	
%such that
%\begin{align*}
%	&\vabs{D_{0}(\mu)} \leq C \mu,
%	\qquad
%	\vabs{D_{1,L}(\mu)} \leq C, 
%	\qquad
%	\vabs{D_{1,\eta}(\mu)} \leq C \mu,
%	\qquad
%	\vabs{D_{1,\xi}(\mu)} \leq C \mu, 
%	\\
%	&\vabs{D_2(\la,L,\eta,\xi;\mu)} \leq 
%	C \paren{
%		\mu \vabs{\la}^2 +
%		\vabs{\la}\vabs{(L-1,\eta,\xi)} +
%		\vabs{(L-1,\eta,\xi)}^2
%	},
%\end{align*}


%The first two lemmas involve estimates of the operator $\RRR^{\out}$ and its derivatives in different domains.
%%
%Let us recall that, by its definition in~\eqref{def:operatorRRROuter}, for $z=(w,x,y)$ we have
%\begin{align}\label{eq:expressionRRRout}
%\RRR^{\out}[z](u) = \paren{
%	\frac{f_1^{\out}(u,z)}{1+g^{\out}(u,z)},
%	\frac{{f_2}^{\out} - \frac{i x}{\de^2} \, g^{\out}}{1+g^{\out}(u,z)},
%	\frac{{f_3}^{\out} + \frac{i y}{\de^2} \, g^{\out}}{1+g^{\out}(u,z)}
%},
%\end{align} 
%where $g^{\out} = \partial_w H_1^{\out}$ and $f^{\out}=\paren{-\partial_u H_1^{\out}, i\partial_y H_1^{\out}, -i\partial_x H_1^{\out} }$.

%\begin{equation}\label{eq:expressionf1f2f3}
%\begin{aligned}
%g^{\out} &= \partial_w H_1^{\out}, &
%\quad
%f_2^{\out} &=i\partial_y H_1^{\out},&
%\quad
%f_3^{\out} &=-i\partial_x H_1^{\out}
%\\
%f_1^{\out} &=-\partial_u H_1^{\out}, &
%\quad
%\wt{f}_2^{\out} &= {f_2}^{\out} - \frac{i x}{\de^2} \, g^{\out} &
%\quad
%\wt{f}_3^{\out} &= {f_3}^{\out} - \frac{i y}{\de^2} \, g^{\out}.
%\end{aligned}
%\end{equation}

%Therefore, we need to estimate the first and second derivatives of $H_1^{\out}$ (see~\eqref{def:hamiltonianOuterSplit}).


==> Article Outer/proofH-existenceTechnicalOuter.tex <==
\subsection{Estimates in the outer domain}
\label{subsubsection:proofComputationsRRROut}

% Let us recall that, by the expression in~\eqref{eq:expressionRRRout}, 
To obtain estimates of $\RRR^{\out}$, we write
% we need to estimate the first and second derivatives of $H_1^{\out}$.
%(see~\eqref{def:hamiltonianOuterSplit}).
% We present a suitable expression of 
$H_1^{\out}$ in~\eqref{def:hamiltonianOuterSplit} (up to a constant) as
%
\begin{equation*}
H_1^{\out} = 
%
H_1 \circ \phi_{\equi} \circ \phi_{\out}
%
- \frac{w^2}{6\La_h^2(u)} 
+
\de( x \Ltresy + y\Ltresx) 
+ 3\de^2 \LtresLa  \paren{\La_h(u)-\frac{w}{3\La_h(u)}},
\end{equation*} 
(see \eqref{eq:expressionHamiltonianInfty} and \eqref{proof:M1expressionLtres}).
Then, by the definition of $H_1$ in \eqref{def:hamiltonianScalingH1}, we obtain
\begin{align*}
H_1^{\out} =& \,
%
(H^{\Poi}_1-V) 
\circ \phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out}
%
+ \frac{1}{\de^4} 
F_{\pend}\paren{\de^2\La_h(u) - 
	\frac{\de^2  w}{3 \La_h(u)} + 
	\de^4\LtresLa} \\
%
&- \frac{w^2}{6\La_h^2(u)} 
+
\de( x \Ltresy + y\Ltresx) 
+ 3\de^2 \LtresLa  \paren{\La_h(u)-\frac{w}{3\La_h(u)}},
\end{align*}
where $H_1^{\Poi}$ is given in \eqref{def:hamiltonianPoincare1}, 
the potential $V$ in \eqref{def:potentialV} and $F_{\pend}$ in \eqref{def:Fpend}.
%
The changes of coordinates $\phi_{\sca}$, $\phi_{\equi}$ and $\phi_{\out}$ are given in \eqref{def:changeScaling}, \eqref{def:changeEqui} and \eqref{def:changeOuter}, respectively.

Considering $z=(w,x,y)$, we denote the composition of  change of coordinates as
\begin{equation}\label{def:changeTotalOuter}
	(\la, L, \eta, \xi) =
	\Theta(u,z) = (\phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out})(u,z).
\end{equation}
% 
% In order to simplify the computations, we split $H_1^{\out}$ in three terms.
% %
%
Then, since $\mu=\de^4$, the Hamiltonian $H_1^{\out}$ can be split (up to a constant) as
\begin{equation}\label{proof:H1outExpressionOuter}
	H_1^{\out} = M_P + M_{S} + M_R,
\end{equation}
where
\begin{align}
M_P(u,z;\de) =& 
-\paren{\PP[\de^4-1]
	- \frac{1}{\sqrt{2+2\cos \la}}
}\circ \Theta(u,z), 
\label{def:expressionMJOuter}
\\
%
%M_{S}(u,z;\de) =& \,
%\frac{1}{\sqrt{D[\de^4]\circ\Theta(u,z)}} - 1 , 
%\label{def:expressionMSOuter}
%\\
%
M_{S}(u,z;\de) =& \,
\paren{ 
	\frac{1}{\de^4} \PP[0] -
	\frac{1-\de^4}{\de^4} \PP[\de^4] 
	- 1 + \cos \la} \circ\Theta(u,z), 
\label{def:expressionMSOuter} \\
%%%%
\begin{split}\label{def:expressionMROuter}
	M_R(u,z;\de) =& 
	- \frac{w^2}{6\La_h^2(u)} 
	%
	+ \de^2 \LtresLa \paren{3 \La_h(u)
		- \frac{w}{\La_h(u)} } 
	%
	+ \de (x \Ltresy + y \Ltresx ), \\
	%
	&+ \frac{1}{\de^4} 
	F_{\pend}\paren{\de^2\La_h(u) - 
		\frac{\de^2  w}{3 \La_h(u)} + 
		\de^4\LtresLa},
	%	- \frac{3}{2}\de^4 \LtresLa^2
	%	+ \de^4 \Ltresx \Ltresy
	%	-\frac{1}{2} ,
\end{split}	
\end{align}
%
and  $\PP$ is the function given in~\eqref{def:functionD}.
%
% Therefore, we need to obtain estimates for the first and second derivatives of $M_P$, $M_S$ and $M_R$.
% 
% \begin{remark}
% Notice that, by Theorem \ref{theorem:singularities}, $\la=\la_h(u) \sim \pi$ when $u \sim \pm iA$.
% %
% Therefore, by Remark \ref{remark:collisions}, the domain $\DuOut$ contains points close to collision with the primary $P$, which  are given by the singularities of function $\PP[\de^4-1]$.
% %
% As a result, the function $M_P$ will give the leading term of the estimates for $H_1^{\out}$ and its derivatives (except for $\partial_w^2 H_1^{\out}$).
% %
% This indicates that we need to obtain precise estimates for $M_P$, whereas the estimates for $M_S$ and $M_R$ are rather straightforward. 
% \end{remark}

To obtain estimates for the  derivatives of $M_P$, $M_S$ and $M_R$,  we first analyze  the change of coordinates $\Tht$ in~\eqref{def:changeTotalOuter}. It can be expressed as
\begin{equation}\label{proof:ThtExpression}
\Tht(u,z)=
\Big(\pi + \Tht_{\la}(u), 1 + \Tht_{L}(u,w),
\Tht_{\eta}(x),\Tht_{\xi}(y) \Big),
\end{equation}
where
\begin{equation*}
\begin{aligned}	
\Tht_{\la}(u) &= \la_h(u)-\pi,  &
\Tht_{\eta}(x) &= \de x + \de^4 \Ltresx(\de), \\
%
\Tht_L(u,w) &= \de^2 \La_h(u) 
- \frac{\de^2 w}{3 \La_h(u)} + \de^4 \LtresLa(\de), \quad&
\Tht_{\xi}(x) &= \de y + \de^4 \Ltresy(\de).
\end{aligned}
\end{equation*}
Next lemma, which is a direct consequence of Theorem \ref{theorem:singularities}, gives estimates for this change of coordinates.


\begin{lemma}\label{lemma:changeTotalOuter}
Fix  $\varrho>0$ and $\de>0$ small enough. Then, for
$\phiA \in \ballOuter \subset \XcalOutTotal$,
% one has that
\begin{align*}
\normOut{\Tht_{\la}}_{0,-\frac{2}{3}}&\leq C, &
%%%
\normOut{\Tht_{L}(\cdot,\phiA)}_{0,\frac{1}{3}} 
&\leq C \de^2, &
%%%
\normOut{\Tht_{\eta}(\cdot,\phiA)}_{0,\frac{4}{3}} 
&\leq C \de^4, \\
%%%%%%%%%%
\normOut{\Tht_{\la}^{-1}}_{0,\frac{2}{3}}&\leq C, &
%%%
\normOut{1+\Tht_{L}(\cdot,\phiA)}_{0,0} 
&\leq C, &
%%%%
\normOut{\Tht_{\xi}(\cdot,\phiA)}_{0,\frac{4}{3}} 
&\leq C \de^4.
\end{align*}
Moreover, its derivatives satisfy
\begin{align*}
\normOut{\partial_u \Tht_{\la}}_{0,\frac{1}{3}} &\leq C, 
& 
\normOut{\partial_u \Tht_{L}(\cdot,\phiA)}_{0,\frac{4}{3}} &\leq C \de^2, 
&
\normOut{\partial_w \Tht_{L}(\cdot,\phiA)}_{0,-\frac{1}{3}} &\leq C \de^2,
\\
\normOut{\partial_{uw} \Tht_{L}(\cdot,\phiA)}_{0,\frac{2}{3}} &\leq C\de^2,
& 
\partial_x \Tht_{\eta},
\partial_y \Tht_{\xi} &\equiv \de, 
& 
\partial^2_{w} \Tht_L, 
\partial^2_{x} \Tht_{\eta}, 
\partial^2_y \Tht_{\xi} &\equiv 0. 
\end{align*}
\end{lemma}
%\begin{align*}
%\normOut{\partial_u \Tht_{\la}(\cdot,\phiA)}_{0,\frac{1}{3}} &\leq C, 
%& 
%\normOut{\partial^2_u \Tht_{\la}(\cdot,\phiA)}_{0,\frac{4}{3}} &\leq C, 
%& 
%\normOut{\partial_u \Tht_{L}(\cdot,\phiA)}_{0,\frac{4}{3}} &\leq C \de^2, 
%\\
%\normOut{\partial_w \Tht_{L}(\cdot,\phiA)}_{0,-\frac{1}{3}} &\leq C \de^2,
%& 
%\normOut{\partial^2_u \Tht_{L}(\cdot,\phiA)}_{0,\frac{7}{3}} &\leq C \de^2, 
%&
%\normOut{\partial_{uw} \Tht_{L}(\cdot,\phiA)}_{0,\frac{2}{3}} &\leq C\de^2, 
%\\
%\partial^2_{w} \Tht_L &\equiv 0 
%& 
%\partial_x \Tht_{\eta},
%\partial_y \Tht_{\xi} &\equiv \de, 
%& 
%\partial^2_{x} \Tht_{\eta}, \partial^2_y \Tht_{\xi} &\equiv 0.
%\end{align*}

In the next lemma we obtain estimates for the  derivatives of $M_P$.
% given in \eqref{def:expressionMJOuter}.

\begin{lemma}\label{lemma:boundsMPout}
Fix $\varrho>0$,  $\de>0$ small enough and
$\kappa>0$ big enough. Then, for 
$\phiA \in \ballOuter$ and $*=x,y$, 
\begin{equation*}%\label{proof:estimatesMP}
\begin{aligned}	
\normOut{\partial_u M_P(\cdot,\phiA)
}_{1,1}
&\leq C \de^2, & 
%
\normOut{\partial_w M_P(\cdot,\phiA)
}_{1,-\frac{2}{3}}
&\leq C \de^{2},  & 
%
\normOut{\partial_* M_P(\cdot,\phiA)
}_{0,\frac{4}{3}}
&\leq C \de, \\
%%%%%%
\normOut{\partial_{u w} M_P(\cdot,\phiA)
}_{1,\frac{1}{3}}
&\leq C \de^{2},  &
%
\normOut{\partial_{u *} M_P(\cdot,\phiA)
}_{0,\frac{7}{3}}
&\leq C \de,  &
%
\normOut{\partial^2_{w} M_P(\cdot,\phiA)
}_{0,\frac{4}{3}}
&\leq C \de^4, \\
%
\normOut{\partial_{w *} M_P(\cdot,\phiA)
}_{0,\frac{5}{3}}
&\leq C \de^3, &
%
\normOut{\partial^2_{*} M_P(\cdot,\phiA)
}_{0,2}
&\leq C \de^2,  &
%
\normOut{\partial_{xy} M_P(\cdot,\phiA)
}_{0,2}
&\leq C \de^2.
\end{aligned}
\end{equation*}
\end{lemma}

\begin{proof}

We consider $\phiA \in \ballOuter \subset \XcalOutTotal$
%
and 
% By the definition of $M_P$, we need
we estimate the derivatives of $\PP[\de^4-1] \circ \Tht(u,\phiA(u))$. We
% To apply Lemma \ref{lemma:seriesH1Poi}, 
first we obtain bounds for $A[\de^4-1]$ and $B[\de^4-1]$ (see \eqref{def:DA} and \eqref{def:DB}).
%
To simplify the notation, we define
\begin{align}\label{proof:defABP}
\wt{A}(u) = A[\de^4-1](\pi +\Tht_{\la}(u)), \qquad
\wt{B}(u,z) = B[\de^4-1] \circ \Tht(u,z).
\end{align}

%
%To simplify notation, we consider the auxiliary function
%\[
%\Phi(u)=
%\Theta(u,\varphi(u)), 
%\quad \text{ with } \quad
%\Phi=\paren{\pi+\Phi_{\la},1+\Phi_L, \Phi_{\eta}, \Phi_{\xi}}.
%\] 
%
%with components
%$\Phi=\paren{\Phi_{\la},\Phi_L, \Phi_{\eta}, \Phi_{\xi}}$
%

%Therefore, $M_P$ can be expressed as
%\begin{align}\label{proof:expressionMP}
%M_P(u,z) = -\frac{1}{\sqrt{A(u)+B(u,z)}} + \frac{1}{\sqrt{A(u)}}
%\end{align}
%where
%\begin{equation}\label{proof:defAB}
%A(u) = 2 - 2\cos \Tht_{\la}(u), 
%\qquad
%B = B_0 + B_1 + B_2, 
%\end{equation}
%and
%\begin{equation}\label{proof:defBs}
%\begin{aligned}
%B_0(u,z) &= 
%\paren{D_0[\de^4-1] - (2+2\cos \la)} 
%\circ \Tht(u,z), 
%\\
%%
%B_1(u,z) &= 
%D_1[\de^4-1] \circ \Tht(u,z), 
%\qquad
%B_2(u,z) = 
%D_{\geq 2}[\de^4-1] \circ \Tht(u,z),
%\end{aligned}
%\end{equation}
%where the change $\Tht$ is given in \eqref{proof:ThtExpression}.
%%
%As a result, to estimate the derivatives of $M_P$ we need to estimate first the derivatives of $A$, $B_0$, $B_1$ and $B_2$.


In the following computations we use extensively the results in Lemma~\ref{lemma:sumNormsOuter} without mentioning them.

\begin{enumerate}
\item Estimates of $\wtA(u)$:
%
Defining $\lah=\la-\pi$, by \eqref{def:DA},
\begin{align*}
A[\de^4-1](\lah+\pi) = 2(1-\cos\lah) -2\de^4(1-\cos\lah) + \de^8.
\end{align*}
%
Then, applying Lemma~\ref{lemma:changeTotalOuter}, 
\begin{equation*}\label{proof:estimateTrigoOuter}
\begin{aligned}
\normOut{\sin \Tht_{\la}}_{0,-\frac{2}{3}} 
\leq 
C \normOut{\Tht_{\la}}_{0,-\frac{2}{3}}
\leq C, 	\qquad
%	
\normOut{(1-\cos \Tht_{\la})^{-1}
}_{0,\frac{4}{3}} 
\leq
C \normOut{\Tht_{\la}^{-2}
}_{0,\frac{4}{3}} 
\leq C
\end{aligned}	
\end{equation*}
and, as a result,
\begin{equation}\label{proof:DA}
\begin{split}	
\normOutSmall{\wtA^{-1}}_{0,\frac{4}{3}} 
&\leq 
C \normOut{(1-\cos \Tht_{\la})^{-1}
}_{0,\frac{4}{3}} 
\leq C,
\\
\normOutSmall{\partial_u \wtA}_{0,-\frac{1}{3}}
&\leq C
\normOut{\sin \Tht_{\la}}_{0,-\frac23}
\normOut{\partial_u \Tht_{\la}}_{0,\frac13}
\leq C.
\end{split}
\end{equation}
%We use the estimates in \eqref{proof:estimateTrigoOuter} without mentioning them throughout the rest of the proof.

\item Estimates of $\wtB(u,\phiA(u))$:
%
Considering the auxiliary variables
$(\lah,\Lh)=(\la-\pi,L-1)$,
%
we have that
\begin{equation}\label{proof:D0expansion}
\begin{split}	
B[\de^4-1](\pi+\lah,1+\Lh,\eta,\xi)
= \,& 
4 \Lh (1-\cos \lah + \de^4 \cos \lah) \\ 
&+
\frac{\eta}{\sqrt{2}} 
(-3 +2 e^{-i\lah}+e^{-2i\lah} +\de^4(3+ e^{-2i\lah})) \\
&+
\frac{\xi}{\sqrt{2}} 
(-3 +2 e^{i\lah}+e^{2i\lah} +\de^4(3+ e^{2i\lah})) \\
&+ R[\de^4-1](\pi+\lah,1+\Lh,\eta,\xi).
\end{split}
\end{equation}
%
Then, by the estimates in \eqref{eq:boundD2mes} and Lemma~\ref{lemma:changeTotalOuter},
\begin{equation}\label{proof:DB}
\begin{aligned}
\normOutSmall{\wtB(\cdot,\phiA)}_{1,-2} 
\leq \,&
C \normOut{\Tht_{L}(\cdot,\phiA)
\Tht_{\la}^2}_{0,-1}
+ \frac{C}{\de^2}
\normOut{\Tht_{\eta}(\cdot,\phiA) \Tht_{\la}}_{0,\frac23} \\
&+ \frac{C}{\de^2}
\normOut{\Tht_{\xi}(\cdot,\phiA) \Tht_{\la}}_{0,\frac23}
+ 
\frac{C}{\de^2}
\normOut{(\Tht_{L},\Tht_{\eta},\Tht_{\xi})^2}_{0,\frac23} \leq C \de^2.
\end{aligned}
\end{equation}

Now, we look for estimates of the first derivatives of $\wtB(u,\phiA(u))$.
%
By its definition in \eqref{proof:defABP} and the expression of $\Tht$ in \eqref{proof:ThtExpression}, we have that
\begin{equation}\label{proof:boundsBtildePoincare}
\begin{aligned}	
\partial_u \wtB =& \,
%
\boxClaus{ \partial_{\la} B[\de^4-1] \circ \Tht}
\partial_u  \Tht_{\la}
+
\boxClaus{\partial_{L} B[\de^4-1] \circ \Tht}
\partial_u  \Tht_{L}, \\
%
\partial_w \wtB =& \,
\boxClaus{
\partial_{L} B[\de^4-1] \circ \Tht
}
\partial_w  \Tht_{L}, \\
%
\partial_x \wtB =& \,
\boxClaus{
	\partial_{\eta} B[\de^4-1] \circ \Tht
}
\partial_{x}  \Tht_{\eta}, \qquad
%
\partial_y \wtB = \,
\boxClaus{
	\partial_{\xi} B[\de^4-1] \circ \Tht
}
\partial_y \Tht_{\xi}.
\end{aligned}
\end{equation}
Differentiating \eqref{proof:D0expansion} and applying Lemma~\ref{lemma:changeTotalOuter}, 
\begin{align*}
\normOut{\partial_{\la} B[\de^4-1] \circ \Tht(\cdot,\phiA)}_{1,-\frac43}
\leq& \, 
C \normOut{\Tht_{L}(\cdot,\phiA) \Tht_{\la}}_{-\frac13} +
\frac{C}{\de^2}
\normOut{\Tht_{\eta}(\cdot,\phiA)}_{0,\frac43}
\\
&+ \frac{C}{\de^2}
\normOut{\Tht_{\xi}(\cdot,\phiA)}_{0,\frac43}
+ C\de^2
\leq C \de^2, 
\\
%%%%%%%%
\normOut{\partial_{L} B[\de^4-1] \circ \Tht(\cdot,\phiA)}_{1,-\frac73}
\leq&
C \normOut{\Tht_{\la}^2}_{0,-\frac43} +
\frac{C}{\de^2} \normOut{\Tht_{L}(\cdot,\phiA)}_{0,\frac13}
+ \frac{C}{\kappa} 
\leq C,
\\
%%%%%%%%%
\normOut{\partial_{*} B[\de^4-1] \circ \Tht(\cdot,\phiA)}_{0,-\frac23}
\leq&
C \normOut{\Tht_{\la}}_{0,-\frac23}
+
\frac{C}{\kappa}
\leq C, \quad \text{for } *=\eta,\xi.
\end{align*}
%
Then, using also \eqref{proof:boundsBtildePoincare} and taking $*=x,y$,
%
\begin{align}\label{proof:DBfirst}
\normOutSmall{\partial_u \wtB(\cdot,\phiA)
}_{1,-1}
&\leq C \de^2, & 
%
\normOutSmall{\partial_w \wtB(\cdot,\phiA)
}_{1,-\frac83}
&\leq C \de^2, & 
%
\normOutSmall{\partial_* \wtB(\cdot,\phiA)
}_{0,-\frac23}
&\leq C \de.	
\end{align}
%
Analogously, for the second derivatives, one can obtain the estimates
\begin{equation}\label{proof:DBsecond}
\begin{aligned}	
\normOutSmall{\partial_{u w} \wtB(\cdot,\phiA) }_{1,-\frac53}
&\leq C \de^2, & \hspace{-1mm}
%
\normOutSmall{\partial^2_{w} \wtB(\cdot,\phiA)
}_{0,\frac23}
&\leq C \de^4, & \hspace{-1mm}
%
\normOutSmall{\partial_{u *} \wtB(\cdot,\phiA)
}_{0,\frac13}
&\leq C \de, \\
%
\normOutSmall{\partial_{w *} \wtB(\cdot,\phiA)
}_{0,-\frac13}
&\leq C \de^3,& \hspace{-1mm}
%
\normOutSmall{\partial^2_{*} \wtB(\cdot,\phiA)
}_{0,0}
&\leq C \de^2, & \hspace{-1mm}
%
\normOutSmall{\partial_{xy} \wtB(\cdot,\phiA)
}_{0,0}
&\leq C \de^2.
\end{aligned}
\end{equation}
\end{enumerate}
Now, we are ready to obtain estimates for $M_P(u,\phiA(u))$  by using the series expansion \eqref{def:SerieP}.
% applying the results in Lemma \ref{lemma:seriesH1Poi}.
%
First, we check that it is convergent.
%
Indeed, by \eqref{proof:DA} and \eqref{proof:DB}, for $u \in \DuOut$ and taking $\kappa$ big enough we have that
\begin{align*}
\vabs{\frac{\wtB(u,\phiA(u))}{\wtA(u)}}
&\leq 		
\normOutSmall{\wtB(\cdot,\phiA)}_{0,-\frac{4}{3}}
\normOutSmall{\wtA^{-1}}_{0,\frac{4}{3}} 
%
\leq 
\frac{C}{\kappa^2\de^2}
\normOutSmall{\wtB(\cdot,\phiA)}_{1,-2}
\leq \frac{C}{\kappa^2} \ll 1.
\end{align*}
Therefore, by \eqref{def:functionD2} and  \eqref{def:expressionMJOuter},
\begin{align}\label{proof:expressionMP}
\vabs{M_P(u,\phiA(u))} \leq 
\vabs{\frac1{\textstyle\sqrt{A[\de^4-1](\la_h(u))}} - \frac1{\sqrt{2+2\cos \la_h(u)}}  }
+
C \frac{|\wtB(u,\phiA(u))|}{|\wtA(u)|^{\frac32}}.
\end{align}
% and analogous estimates holds for the first and second derivatives.
Then, to estimate $M_P$ and its derivatives, it only remains to analyze the $u$-derivative of  its first term.
%
Indeed, by the definition of $A[\de^4-1]$ in \eqref{def:DA}.
%we have that
%\begin{align*}
%\frac1{\textstyle\sqrt{A[\de^4-1]}} - \frac1{\sqrt{2+2\cos \la}} 
%= 
%\frac{\de^4(2+2\cos\la)-\de^8}{\sqrt{2+2\cos\la}
%\sqrt{A[\de^4-1]} \paren{\sqrt{2+2\cos \la} +
%\sqrt{A[\de^4-1]} }},
%\end{align*}
% and differentiating, we obtain that
\begin{align}\label{proof:DApotential}
\normOut{\partial_u \paren{\frac1{\textstyle\sqrt{A[\de^4-1](\la_h(u))}} - \frac1{\sqrt{2+2\cos \la_h(u)}} } }_{0,\frac43} \leq C \de^4.
\end{align}
Therefore, applying estimates \eqref{proof:DA}, \eqref{proof:DB}, \eqref{proof:DBfirst}, 
\eqref{proof:DBsecond} and  \eqref{proof:DApotential}, to the derivatives of $M_P$ and using \eqref{proof:expressionMP}, we obtain the statement of the lemma.
\end{proof}
%\begin{equation}\label{proof:estimatesMP}
%\begin{aligned}	
%\normOut{\partial_u M_P(\cdot,\phiA)
%}_{1,1}
%&\leq C \de^2, \hspace{-2.5mm} & 
%%
%\normOut{\partial_w M_P(\cdot,\phiA)
%}_{1,-\frac{2}{3}}
%&\leq C \de^{2}, \hspace{-2.5mm} & 
%%
%\normOut{\partial_* M_P(\cdot,\phiA)
%}_{0,\frac{4}{3}}
%&\leq C \de, \\
%%%%%%%
%\normOut{\partial_{u w} M_P(\cdot,\phiA)
%}_{1,\frac{1}{3}}
%&\leq C \de^{2}, \hspace{-2.5mm} &
%%
%\normOut{\partial_{u *} M_P(\cdot,\phiA)
%}_{0,\frac{7}{3}}
%&\leq C \de, \hspace{-2.5mm} &
%%contenidos...
%\normOut{\partial^2_{w} M_P(\cdot,\phiA)
%}_{0,\frac{8}{3}}
%&\leq C \de^4, \\
%%
%\normOut{\partial_{w *} M_P(\cdot,\phiA)
%}_{0,\frac{5}{3}}
%&\leq C \de^3,\hspace{-2.5mm}  &
%%
%\normOut{\partial^2_{*} M_P(\cdot,\phiA)
%}_{0,2}
%&\leq C \de^2, \hspace{-2.5mm}  &
%%
%\normOut{\partial_{xy} M_P(\cdot,\phiA)
%}_{0,2}
%&\leq C \de^2.
%\end{aligned}
%\end{equation}


Analogously to Lemma \ref{lemma:boundsMPout}, we obtain estimates for the first and second derivatives of $M_S$ and $M_R$ (see \eqref{def:expressionMSOuter} and \eqref{def:expressionMROuter}).

\begin{lemma}\label{lemma:boundsMSout}
Fix $\varrho>0$, 
%  
$\de>0$ small enough
and $\kappa>0$ big enough. Then, for 
$\phiA \in \ballOuter$  and $*=x,y$, we have  
\begin{equation*}%\label{proof:estimatesMS}
\begin{aligned}	
\normOut{\partial_u M_S(\cdot,\phiA)
}_{0,\frac{4}{3}}
&\leq C \de^2, & 
%
\normOut{\partial_w M_S(\cdot,\phiA)
}_{0,-\frac{1}{3}}
&\leq C \de^{2}, & 
%
\normOut{\partial_* M_S(\cdot,\phiA)
}_{0,0}
&\leq C \de, \\
%%%%%%
\normOut{\partial_{u w} M_S(\cdot,\phiA)
}_{0,\frac{2}{3}}
&\leq C \de^{2},  &
%
\normOut{\partial_{u *} M_S(\cdot,\phiA)
}_{0,\frac{1}{3}}
&\leq C \de,  &
%
\normOut{\partial^2_{w} M_S(\cdot,\phiA)
}_{0,-\frac{2}{3}}
&\leq C \de^4, \\
%
\normOut{\partial_{w *} M_S(\cdot,\phiA)
}_{0,-\frac{1}{3}}
&\leq C \de^3,  &
%
\normOut{\partial^2_{*} M_S(\cdot,\phiA)
}_{0,0}
&\leq C \de^2,  &
%
\normOut{\partial_{xy} M_S(\cdot,\phiA)
}_{0,0}
&\leq C \de^2.
\end{aligned}
\end{equation*}
% \end{lemma}
% 
% \begin{lemma}\label{lemma:boundsMRout}
% Fix $\varrho>0$, $\de>0$ small enough and
% $\kappa>0$ big enough,
% $\phiA \in \ballOuter$ (see \eqref{def:ballOuter}) and $*=x,y$, we have 
%
and
\begin{equation*}%\label{proof:estimatesMR}
\begin{aligned}	
\normOut{\partial_u M_R(\cdot,\phiA)
}_{1,1}
&\leq C \de^2,  & 
%
\normOut{\partial_w M_R(\cdot,\phiA)
}_{1,-\frac{2}{3}}
&\leq C \de^{2},  & 
%
\normOut{\partial_* M_R(\cdot,\phiA)
}_{0,0}
&\leq C \de, \\
%%%%%%
\normOut{\partial_{u w} M_R(\cdot,\phiA)
}_{1,\frac{1}{3}}
&\leq C \de^{2},  &
%
\partial_{u *} M_R(\cdot,\phiA)
&\equiv 0,  &
%
\normOut{\partial^2_{w} M_R(\cdot,\phiA)
}_{0,-\frac{2}{3}}
&\leq C, \\
%
\partial_{w *} M_R(\cdot,\phiA)
&\equiv 0,  &
%
\partial^2_{*} M_R(\cdot,\phiA)
&\equiv 0,   &
%
\partial_{xy} M_R(\cdot,\phiA)
&\equiv 0.
\end{aligned}
\end{equation*}
\end{lemma}

%\begin{lemma}\label{lemma:boundsMS}
%Fix $\varrho>0$ and let $M_S$ be the operator defined in~\eqref{def:expressionMSOuter}.
%%  
%Then, for $\de>0$ small enough, $\kappa>0$ big enough and $\phiA \in \XcalOutTotal$ such that $\normOutTotal{\phiA} \leq \varrho \de^3$, there exists a constant $C_{\varrho}>0$ independent of $\de$ and $\kappa$ such that	
%\begin{align*}
%\normOut{\partial_u M_S(\cdot,\phiA) }_{0,\frac{4}{3}} &\leq C \de^2, &
%%
%\normOut{\partial_w M_S(\cdot,\phiA) }_{0,-\frac{1}{3}} &\leq C \de^2, \\
%%
%\normOut{\partial_x M_S(\cdot,\phiA)
%}_{0,0} &\leq C \de, &
%%
%\normOut{\partial_y M_S(\cdot,\phiA)
%}_{0,0} &\leq C \de, 
%\end{align*}
%and
%\begin{align*}
%\normOut{\partial_{uw}M_S(\cdot,\phiA)
%}_{0,\frac{2}{3}} &\leq C \de^2, &
%%
%\normOut{\partial_{ux}M_S(\cdot,\phiA)
%}_{0,-\frac{2}{3}} &\leq C \de, &
%%
%\normOut{\partial_{uy}M_S(\cdot,\phiA) }_{0,-\frac{2}{3}} &\leq C \de, \\
%%%%
%\normOut{\partial^2_{w}M_S(\cdot,\phiA)
%}_{0,-\frac{2}{3}} &\leq C \de^4, &
%%
%\normOut{\partial_{wx}M_S(\cdot,\phiA) }_{0,-\frac{1}{3}} &\leq C \de^3, &
%%
%\normOut{\partial_{wy}M_S(\cdot,\phiA) }_{0,-\frac{1}{3}} &\leq C \de^3, \\
%%%%
%\normOut{\partial^2_{x}M_S(\cdot,\phiA) }_{0,0} &\leq C \de^2, &
%%
%\normOut{\partial^2_{y}M_S(\cdot,\phiA)}_{0,0} &\leq C \de^2, &
%%
%\normOut{\partial_{xy}M_S(\cdot,\phiA)}_{0,0} &\leq C \de^2.
%\end{align*}
%\end{lemma}

%\begin{lemma}\label{lemma:boundsH1out}
%	Fix $\varrho>0$ and let $H_1^{\out}$ be the Hamiltonian given  in~\eqref{def:hamiltonianOuterSplit} and $\ballOuter \subset \XcalOutTotal$ in~\eqref{def:ballOuter}.
%	%  
%	Then, for $\de>0$ small enough and $\kappaOuter>0$ big enough, 
%	there exists a constant $C>0$ independent of $\de$ such that	
%	for $\phiA \in \ballOuter$, we have 
%	\begin{align*}
%		\normOut{\partial_u H_1^{\out}(\cdot,\phiA)}_{1,1} 
%		&\leq C \de^2, &
%		\normOut{\partial_w H_1^{\out}(\cdot,\phiA) }_{1,-\frac{2}{3}} &\leq C \de^2, \\
%		%
%		\normOut{\partial_x H_1^{\out}(\cdot,\phiA)
%		}_{0,\frac{4}{3}} &\leq C \de, &
%		\normOut{\partial_y H_1^{\out}(\cdot,\phiA) }_{0,\frac{4}{3}} &\leq C \de, 
%	\end{align*}
%	and
%	\begin{align*}
%		\normOut{\partial_{uw}H_1^{\out}(\cdot,\phiA)
%		}_{1,\frac{1}{3}} &\leq C \de^2, &
%		%
%		\normOut{\partial_{ux}H_1^{\out}(\cdot,\phiA)
%		}_{0,\frac{7}{3}} &\leq C \de, &
%		%
%		\normOut{\partial_{uy}H_1^{\out}(\cdot,\phiA) }_{0,\frac{7}{3}} &\leq C \de, \\
%		%%%
%		\normOut{\partial^2_{w}H_1^{\out}(\cdot,\phiA)
%		}_{0,-\frac{2}{3}} &\leq C, &
%		%
%		\normOut{\partial_{wx}H_1^{\out}(\cdot,\phiA) }_{0,\frac{5}{3}} &\leq C \de^3, &
%		%
%		\normOut{\partial_{wy}H_1^{\out}(\cdot,\phiA) }_{0,\frac{5}{3}} &\leq C \de^3, \\
%		%%%
%		\normOut{\partial^2_{x}H_1^{\out}(\cdot,\phiA) }_{0,2} &\leq C \de^2, &
%		%
%		\normOut{\partial^2_{y}H_1^{\out}(\cdot,\phiA)}_{0,2} &\leq C \de^2, &
%		%
%		\normOut{\partial_{xy}H_1^{\out}(\cdot,\phiA)}_{0,2} &\leq C \de^2.
%	\end{align*}
%\end{lemma}


\begin{proof}[End of the proof of Lemma~\ref{lemma:computationsRRROut}]

We start by estimating the first and second derivatives of $H_1^{\out}(u,\phiA(u);\de)$ in suitable norms.
%
%
Recall that by \eqref{proof:H1outExpressionOuter}, $H_1^{\out}=M_P+M_S+M_R$. 
%
Therefore, taking $\varphi \in \ballInfty \subset \XcalOutTotal$ and  applying  Lemmas \ref{lemma:boundsMPout} and \ref{lemma:boundsMSout}:

\begin{enumerate}
\item For $g^{\out}=\partial_w H_1^{\out}$ one has
% \begin{equation}\label{proof:estimategOut}
\[
\begin{split}	
\normOut{g^{\out}(\cdot,\phiA)}_{1,-\frac23} \leq&
\normOut{\partial_w M_P(\cdot,\phiA)}_{1,-\frac23} 
+ C
\normOut{\partial_w M_S(\cdot,\phiA)}_{0,-\frac13} +
\normOut{\partial_w M_R(\cdot,\phiA)}_{1,-\frac23} \\ \leq& C \de^2
\end{split}
% \end{equation}
\]
and, in particular, for $\kappa$ big enough
\begin{equation}\label{def:Fitag}
\normOut{g^{\out}(\cdot,\phiA)}_{0,0} \leq C \kappa^{-2} \ll 1.	
\end{equation}
Analogously, 
% \begin{align}\label{proof:estimategOutDerivatives}
$\normOut{\partial_w g^{\out}(\cdot,\phiA)}_{0,-\frac23}
\leq C$ and  
$\normOut{\partial_* g^{\out}(\cdot,\phiA)}_{0,\frac53}
\leq C \de^3$, 
 for $*=x,y$.
% \end{align}

\item For $f_1^{\out}=-\partial_u H_1^{\out}$, one has that
% \begin{equation}\label{proof:estimatef1Out}
\[
% \begin{split}
\normOut{f^{\out}_1(\cdot,\phiA)}_{1,1} 
\leq
\normOut{\partial_u M_P(\cdot,\phiA)}_{1,1}
+
C \normOut{\partial_u M_S(\cdot,\phiA)}_{0,\frac43}+
\normOut{\partial_u M_R(\cdot,\phiA)}_{1,1}
\leq
C \de^2,
% \end{split}
% \end{equation} 
\] 
% \begin{align}\label{proof:estimatef1OutDCerivatives}
$\normOut{\partial_w f_1^{\out}(\cdot,\phiA)}_{1,\frac13}
\leq
C \de^2$ and 
% \qquad
$\normOut{\partial_* f_1^{\out}(\cdot,\phiA)}_{0,\frac73}
\leq 
C \de,
\quad $
for $*=x,y$.
% \end{align}

\item For $f_2^{\out} = i \partial_y H_1^{\out}$ and $f_3^{\out} = -i \partial_x H_1^{\out}$,
%
we can obtain the estimates
\begin{equation}\label{proof:estimatef2f3Out}
\begin{split}	
\normOut{f_2(\cdot,\phiA)}_{0,\frac43} 
\leq&
\normOut{\partial_y M_P(\cdot,\phiA)}_{0,\frac43} 
+ C
\normOut{\partial_y M_S(\cdot,\phiA)
+ 
\partial_y M_R(\cdot,\phiA)}_{0,0}
\leq 
C \de, \\
%%
\normOut{f_3(\cdot,\phiA)}_{0,\frac43} 
\leq&
\normOut{\partial_x M_P(\cdot,\phiA)}_{0,\frac43} 
+ C
\normOut{\partial_x M_S(\cdot,\phiA)
+	
\partial_x M_R(\cdot,\phiA)}_{0,0}
\leq 
C \de.
\end{split}
\end{equation}
Analogously, we have that
% \begin{align}\label{proof:estimatef2f3OutDerivatives}
$\normOutSmall{\partial_w f_j^{\out}(\cdot,\phiA)}_{0,\frac53}
\leq
C \de^3$ and 
% \qquad
$\normOutSmall{\partial_* f_j^{\out}(\cdot,\phiA)}_{0,2}
\leq 
C \de^2$,
for $j=2,3$ and $*=x,y$.
% \end{align}

\end{enumerate}

Joining these estimates  and taking $\kappa$ big enough, we complete the proof of the lemma. 
%
%First, we analyze the denominator. 
%%
%Taking $\kappa$ big enough, we have
%\begin{align*}
%\normOut{g(\cdot,\phiA)}_{0,0}
%\leq
%\leq \frac{C}{\kappa^2} \leq \frac{1}{2},
%%
%\quad \text{and} \quad
%\normOut{1 + g(\cdot,\phiA)}_{0,0} \geq \frac{1}{2}.
%\end{align*}
\end{proof}

\begin{remark}\label{rmk:R} 
Note that that $\DOuterTilde \subset \DuOut$ and  $\YcalOuter \subset 
\XcalOut_{0,0}$ (see \eqref{def:Yout} and \eqref{def:XcalOut}). Then, the proof 
of Lemma~\ref{lemma:computationsRRRtransitionOuter} is a direct consequence of 
the estimates  for $g^{\out}$ and its derivatives in Item 1 above and the 
fact that, by \eqref{eq:systemEDOsOuter} and \eqref{eq:InvU},
\[
R[\uOut](v)= \partial_w H_1^{\out}
	\paren{v + \uOut(v), \zuOut(v+\uOut(v))}= g^{\out}\paren{v + \uOut(v), 
\zuOut(v+\uOut(v))}.
\]
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{lemma}\label{lemma:expressionHamiltonianOuter}
%	Let us consider $z=(w,x,y)$ and the change of variables
%	\begin{equation}\label{def:changeTotalOuter}
%		\Theta(u,z) = (\phi_{\sca} \circ \phi_{\equi} \circ \phi_{\out})(u,z),	
%	\end{equation}
%	where the individual changes are given in \eqref{def:changeScaling}, \eqref{def:changeEqui} and~\eqref{def:changeOuter}, respectively.
%	%
%	Then, the Hamiltonian $H_1^{\out}(u,z;\de)$ (see \eqref{def:hamiltonianOuterSplit}) up to a constant, can be expressed as
%	\begin{equation*}
%		H_1^{\out} = M_P + M_{S} + M_R,
%	\end{equation*}
%	where
%	\begin{align}
%		M_P(u,z;\de) =& 
%		-\paren{\frac{1}{\sqrt{D[\de^4-1] }}
%			+ \frac{1}{\sqrt{2+2\cos \la}}
%		}\circ \Theta(u,z), 
%		\label{def:expressionMJOuter}
%		\\
%		%
%		%M_{S}(u,z;\de) =& \,
%		%\frac{1}{\sqrt{D[\de^4]\circ\Theta(u,z)}} - 1 , 
%		%\label{def:expressionMSOuter}
%		%\\
%		%
%		M_{S}(u,z;\de) =& \,
%		\paren{ 
%			\frac{1}{\de^4 \sqrt{D[0]}} -
%			\frac{1-\de^4}{\de^4\sqrt{D[\de^4]}} 
%			- 1 + \cos \la} \circ\Theta(u,z), 
%		\label{def:expressionMSOuter} \\
%		%%%%
%		\begin{split}\label{def:expressionMROuter}
%			M_R(u,z;\de) =& 
%			- \frac{w^2}{6\La_h^2(u)} 
%			%
%			+ \de^2 \LtresLa \paren{3 \La_h(u)
%				- \frac{w}{\La_h(u)} } 
%			%
%			+ \de (x \Ltresy + y \Ltresx ), \\
%			%
%			&+ \frac{1}{\de^4} 
%			F_{\pend}\paren{\de^2\La_h(u) - 
%				\frac{\de^2  w}{3 \La_h(u)} + 
%				\de^4\LtresLa},
%			%	- \frac{3}{2}\de^4 \LtresLa^2
%			%	+ \de^4 \Ltresx \Ltresy
%			%	-\frac{1}{2} ,
%		\end{split}	
%	\end{align}
%	with function $D[\zeta]$ given in~\eqref{def:functionD},  
%	%
%	$F_{\pend}$ in \eqref{def:Fpend},
%	%
%	$(\LtresLa,\Ltresx,\Ltresy)$ in~\eqref{def:pointL3sca}
%	%
%	and the parametrization of the separatrix
%	$(\la_h,\La_h)$  in~\eqref{eq:separatrixParametrization}.
%\end{lemma}
%
%\begin{proof}
%	The result is a direct consequence of the definition of $H_1^{\out}$ in \eqref{def:hamiltonianOuterSplit}.	
%\end{proof}
%
%\begin{proof}
%Since $H=H_{\pend} + H_{\osc} + H_1$ (see \eqref{def:hamiltonianScaling}),
%the Hamiltonian $H_1^{\out}$ in~\eqref{def:hamiltonianOuterSplit} can be expressed as
%\begin{equation}\label{proof:hamiltonianOuterA}
%H^{\out}_1 =
%\paren{H_{\pend} + H_{\osc} + H_1} \circ \phi_{\equi} \circ \phi_{\out}
% -\paren{w + \frac{xy}{\de^2}},	
%\end{equation}
%where
%the Hamiltonians $H_{\pend}$ and $H_{\osc}$ are given in \eqref{def:HpendHosc} and $H_1$  in~\eqref{def:hamiltonianScalingH1}.
%%
%The change of coordinates (see~\eqref{def:changeEqui} and~\eqref{def:changeOuter}) is
%\begin{equation*}
%%\label{proof:changeOfCoordinatesInfty}
%\begin{aligned}
%&\phi_{\equi} \circ \phi_{\out}
%(u,w,x,y) =
%\paren{\la_h(u),
%\La_h(u) - \frac{w}{3\La_h(u)} 
%+ \de^2 \LtresLa,
%x + \de^3\Ltresx,
%y + \de^3 \Ltresy}.
%\end{aligned}
%\end{equation*}
%Therefore, we analyze each component in~\eqref{proof:hamiltonianOuterA} individually.
%
%First, we analyze $H_{\pend}$.
%%
%Since $(\la_h,\La_h)$ is the parametrization of the separatrix of $H_{\pend}$ we have that $H_{\pend}(\la_h(u),\La_h(u))=H_{\pend}(0,0) = -\frac{1}{2}$.
%%
%Then,
%\begin{align}\label{proof:HpendExpression}
%H_{\pend} \circ \phi_{\equi} \circ \phi_{\out}
%=
%w 
%- \frac{w^2}{6\La_h^2(u)} 
%+ \de^2 \LtresLa \paren{3 \La_h(u)
%- \frac{w}{\La_h(u)} }.
%\end{align}
%In the case of $H_{\osc}$, we have
%\begin{align}\label{proof:HoscExpression}
%H_{\osc} \circ \phi_{\equi} \circ \phi_{\out}
%=
%\frac{x y}{\de^2}
%+ \de (x \Ltresy + y \Ltresx ).
%\end{align}
%For $H_1$ given in~\eqref{def:hamiltonianScalingH1}, we have
%\begin{align*}
%H_1 \circ \phi_{\equi} \circ \phi_{\out}
%=
%H_1^{\Poi} \circ \Tht(u,z)  - V(\la_h(u)) +
%\frac{1}{\de^4} F_{\pend}\paren{
%\de^2\La_h(u) - \frac{\de^2 w}{3\La_h(u)}
%+ \de^4 \LtresLa}.
%\end{align*}
%Then, by the definition of $H_1^{\Poi}$ in~\eqref{def:hamiltonianPoincare01} and since $V(\la_h) = V \circ \Tht$, we obtain the statement of the lemma.
%\end{proof}


==> Article Outer/resultsIntro.tex <==
In this section, we present the main steps necessary to prove Theorem \ref{theorem:mainTheoremPoincare} (see the list in Section \ref{section:introduction}) and complete its proof.
%
In Section \ref{section:singularitiesOuter} we summarize the results concerning the analysis of the separatrix of the unperturbed Hamiltonian $H_{\pend}$ (see \eqref{def:HpendHosc}) done in \cite{articleInner} (Step B).
%
In Section \ref{section:outer}, we prove the existence of parametrizations of the perturbed invariant manifolds in suitable complexs domains (Step E).
%
In Section \ref{section:differenceInner}, we study the difference between the perturbed manifolds near the singularities of the perturbed separatrix.
%
In particular, in Section \ref{subsection:innerHeuristics}, we summarize the results concerning the derivation (Step C) and analysis (Step D) of the inner equation obtained in \cite{articleInner} and, in Section \ref{subsection:matching}, we
compare certain solutions of the inner equation with the parametrizations of the perturbed manifolds by means of complex matching techniques (Step F).
%
Finally, in Section \ref{section:difference}, we combine all the previous results to obtain the dominant term of the difference between the invariant manifolds and prove Theorem \ref{theorem:mainTheoremPoincare} (Step G).


%In the remaining sections we present the rest of necessary results.
%%
%In particular, in Section \ref{section:outer}, we prove the existence of parametrizations of the perturbed invariant manifolds in suitable complexs domains (Step D).
%%
%In Section \ref{section:matching}, we 
%compare the complex parametrizations of the invariant manifolds with the solutions of the inner equation (Step E).
%



==> Article Outer/shortcutsOuter.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LATEX SPECIFIC SHORTCUTS %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% BASICS %%%
\newcommand{\unstable}{{\mathrm{u}}}
\newcommand{\stable}{{\mathrm{s}}}
\newcommand{\stableun}{^{\mathrm{u},\mathrm{s}}}
\newcommand{\phiA}{\varphi}
\newcommand{\phiB}{\tilde{\varphi}}
\newcommand{\wtA}{\widetilde{A}}
\newcommand{\wtB}{\widetilde{B}}

%%%% CHANGE VARIABLES %%%
\newcommand{\HInicial}{h}
\newcommand{\rot}{\mathrm{rot}}
\newcommand{\pol}{\mathrm{pol}}
\newcommand{\Del}{\mathrm{Del}}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\sca}{\mathrm{sc}}
\newcommand{\equi}{\mathrm{eq}}
\newcommand{\osc}{\mathrm{osc}}
\newcommand{\pend}{\mathrm{p}}
\newcommand{\flow}{\mathrm{fl}}
\newcommand{\lah}{\hat{\lambda}}
\newcommand{\Lh}{\hat{L}}
\newcommand{\Lah}{\hat{\Lambda}}
\newcommand{\xh}{\hat{x}}
\newcommand{\xp}{x}
\newcommand{\yh}{\hat{y}}
\newcommand{\yp}{y}
% L3
\newcommand{\Ltres}{\mathfrak{L}}
\newcommand{\LtresLa}{\mathfrak{L}_{\Lambda}}
\newcommand{\Ltresx}{\mathfrak{L}_x}
\newcommand{\Ltresy}{\mathfrak{L}_y}

%%%% SINGULARITIES %%%
\newcommand{\fh}{\hat{f}}
\newcommand{\vap}{\nu}
\newcommand{\proj}{\mathtt{p}}

%%%% INNER SPACE %%%
\newcommand{\inn}{\mathrm{in}}
\newcommand{\Inn}{^{\mathrm{in}}}
\newcommand{\Inner}{{\mathrm{in}}}
\newcommand{\rhoInn}{\kappa}
\newcommand{\kappaInner}{\kappa_5}
\newcommand{\CInn}{\Tht}
% Domain
\newcommand{\DInn}{\mathcal{D}^{\mathrm{in}}_{\rhoInn}}
\newcommand{\DInnR}[1]{\mathcal{D}^{\mathrm{in}}_{\rhoInn_{#1}}}
\newcommand{\DuInn}{\mathcal{D}^{\mathrm{u,in}}_{\rhoInn}}
\newcommand{\DsInn}{\mathcal{D}^{\mathrm{s,in}}_{\rhoInn}}
\newcommand{\DusInn}{\mathcal{D}^{\mathrm{u/s,in}}_{\rhoInn}}
\newcommand{\DdInn}{\mathcal{D}^{\diamond,\mathrm{in}}_{\rhoInn}}
\newcommand{\DusInnR}[1]{\mathcal{D}^{\mathrm{u/s,in}}_{\rhoInn_{#1}}}
\newcommand{\EInn}{\mathcal{E}^{\mathrm{in}}_{\rhoInn}}
\newcommand{\EInnR}[1]{\mathcal{E}^{\mathrm{in}}_{\rhoInn_{#1}}}
% Domain Outer
\newcommand{\DuInnOut}{{D}^{\mathrm{u,in}}_{\rhoInn}}
\newcommand{\DsInnOut}{{D}^{\mathrm{s,in}}_{\rhoInn}}
\newcommand{\DusInnOut}{{D}^{\mathrm{u/s,in}}_{\rhoInn}}
\newcommand{\DdInnOut}{{D}^{\diamond,\mathrm{in}}_{\rhoInn}}
% Banach Spaces
\newcommand{\XcalInn}{\mathcal{X}^{\mathrm{in}}}
\newcommand{\XcalInnS}{\mathcal{X}^{\mathrm{s,in}}}
\newcommand{\XcalInnU}{\mathcal{X}^{\mathrm{u,in}}}
\newcommand{\XcalInnD}{\mathcal{X}^{\diamond,\mathrm{in}}}
\newcommand{\XcalInnUS}{\mathcal{X}^{\mathrm{u/s,in}}}
\newcommand{\YcalInn}{\mathcal{Y}^{\mathrm{in}}}
\newcommand{\ZcalInn}{\mathcal{Z}^{\mathrm{in}}}
\newcommand{\XcalInnTotal}{\mathcal{X}^{\mathrm{in}}_{\times}}
\newcommand{\XcalInnSTotal}{\mathcal{X}^{\mathrm{s,in}}_{\times}}
\newcommand{\XcalInnUTotal}{\mathcal{X}^{\mathrm{u,in}}_{\times}}
\newcommand{\XcalInnDTotal}{\mathcal{X}^{\diamond,\mathrm{in}}_{\times}}
\newcommand{\XcalInnUSTotal}{\mathcal{X}^{\mathrm{u/s,in}}_{\times}}
\newcommand{\YcalInnTotal}{\mathcal{Y}^{\mathrm{in}}_{\times}}
% Norms
\newcommand{\normInn}[1]{\left\lVert#1\right\rVert^{\mathrm{in}}}
\newcommand{\normInnS}[1]{\left\lVert#1\right\rVert^{\mathrm{s,in}}}
\newcommand{\normInnU}[1]{\left\lVert#1\right\rVert^{\mathrm{u,in}}}
\newcommand{\normInnD}[1]{\left\lVert#1\right\rVert^{\diamond,\mathrm{in}}}
\newcommand{\normInnUS}[1]{\left\lVert#1\right\rVert^{\mathrm{u/s,in}}}
\newcommand{\normInnTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{in}}_{\times}}
\newcommand{\normInnUSTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{u/s,in}}_{\times}}
\newcommand{\normInnDTotal}[1]{\left\lVert#1\right\rVert^{\diamond,\mathrm{in}}_{\times}}
\newcommand{\normInnExp}[1]{\left\lVert#1\right\rVert^{\mathrm{in, e}}}
% Variables
\newcommand{\ZInn}{Z_0}
\newcommand{\ZInnB}{\widetilde{Z}_0}
\newcommand{\ZInnN}{\widehat{Z}_0}
\newcommand{\ZuInn}{Z^{\mathrm{u}}_0}
\newcommand{\ZuInnN}{\widehat{Z}^{\mathrm{u}}_0}
\newcommand{\ZsInn}{Z^{\mathrm{s}}_0}
\newcommand{\ZsInnN}{\widehat{Z}^{\mathrm{s}}_0}
\newcommand{\ZusInn}{Z^{\mathrm{u,s}}_0}
\newcommand{\ZdInn}{Z^{\diamond}_0}
\newcommand{\ZdInnN}{\widehat{Z}^{\diamond}_0}
\newcommand{\WInn}{W_0}
\newcommand{\WInnB}{\widetilde{W}_0}
\newcommand{\WInnN}{\widehat{W}_0}
\newcommand{\WuInn}{W^{\mathrm{u}}_0}
\newcommand{\WsInn}{W^{\mathrm{s}}_0}
\newcommand{\WusInn}{W^{\mathrm{u,s}}_0}
\newcommand{\WdInn}{W^{\diamond}_0}
\newcommand{\WdInnN}{\widehat{W}^{\diamond}_0}
\newcommand{\XInn}{X_0}
\newcommand{\XInnB}{\widetilde{X}_0}
\newcommand{\XInnN}{\widehat{X}_0}
\newcommand{\XuInn}{X^{\mathrm{u}}_0}
\newcommand{\XsInn}{X^{\mathrm{s}}_0}
\newcommand{\XusInn}{X^{\mathrm{u,s}}_0}
\newcommand{\XdInn}{X^{\diamond}_0}
\newcommand{\XdInnN}{\widehat{X}^{\diamond}_0}
\newcommand{\YInn}{Y_0}
\newcommand{\YInnB}{\widetilde{Y}_0}
\newcommand{\YInnN}{\widehat{Y}_0}
\newcommand{\YuInn}{Y^{\mathrm{u}}_0}
\newcommand{\YsInn}{Y^{\mathrm{s}}_0}
\newcommand{\YusInn}{Y^{\mathrm{u,s}}_0}
\newcommand{\YdInn}{Y^{\diamond}_0}
\newcommand{\YdInnN}{\widehat{Y}^{\diamond}_0}
% Diference variables
\newcommand{\DZInn}{\Delta Z_0}
\newcommand{\DWInn}{\Delta W_0}
\newcommand{\DXInn}{\Delta X_0}
\newcommand{\DYInn}{\Delta Y_0}
\newcommand{\DZInnN}{\Delta \widehat{Z}_0}
\newcommand{\DWInnN}{\Delta \widehat{W}_0}
\newcommand{\DXInnN}{\Delta \widehat{X}_0}
\newcommand{\DYInnN}{\Delta \widehat{Y}_0}
\newcommand{\DZo}{\Delta Z_{\mathrm{initial}}}
\newcommand{\DWo}{\Delta W_{\mathrm{initial}}}
\newcommand{\DXo}{\Delta X_{\mathrm{initial}}}
\newcommand{\DYo}{\Delta Y_{\mathrm{initial}}}
\newcommand{\tDZo}{\widetilde{\Delta Z}_{\mathrm{initial}}}
\newcommand{\tDWo}{\widetilde{\Delta W}_{\mathrm{initial}}}
\newcommand{\tDXo}{\widetilde{\Delta X}_{\mathrm{initial}}}
\newcommand{\tDYo}{\widetilde{\Delta Y}_{\mathrm{initial}}}

%%%% OUTER SPACE %%%
\newcommand{\out}{\mathrm{sep}}
% Variables
\newcommand{\zOut}{z}
\newcommand{\zOutB}{\widetilde{z}}
\newcommand{\zuOut}{z^{\mathrm{u}}}
\newcommand{\zuOutB}{\widetilde{z}^{\mathrm{u}}}
\newcommand{\zsOut}{z^{\mathrm{s}}}
\newcommand{\zusOut}{z^{\mathrm{u,s}}}
\newcommand{\zdOut}{z^{\diamond}}
\newcommand{\wOut}{w}
\newcommand{\wOutB}{\widetilde{w}}
\newcommand{\wuOut}{w^{\mathrm{u}}}
\newcommand{\wuOutB}{\widetilde{w}^{\mathrm{u}}}
\newcommand{\wsOut}{w^{\mathrm{s}}}
\newcommand{\wusOut}{w^{\mathrm{u,s}}}
\newcommand{\wdOut}{w^{\diamond}}
\newcommand{\xOut}{x}
\newcommand{\xOutB}{\widetilde{x}}
\newcommand{\xuOut}{x^{\mathrm{u}}}
\newcommand{\xuOutB}{\widetilde{x}^{\mathrm{u}}}
\newcommand{\xsOut}{x^{\mathrm{s}}}
\newcommand{\xusOut}{x^{\mathrm{u,s}}}
\newcommand{\xdOut}{x^{\diamond}}
\newcommand{\yOut}{y}
\newcommand{\yOutB}{\widetilde{y}}
\newcommand{\yuOut}{y^{\mathrm{u}}}
\newcommand{\yuOutB}{\widetilde{y}^{\mathrm{u}}}
\newcommand{\ysOut}{y^{\mathrm{s}}}
\newcommand{\yusOut}{y^{\mathrm{u,s}}}
\newcommand{\ydOut}{y^{\diamond}}
% Diference variables
\newcommand{\dzOut}{\Delta z}
\newcommand{\dwOut}{\Delta w}
\newcommand{\dxOut}{\Delta x}
\newcommand{\dyOut}{\Delta y}
% Change of coordinates
\newcommand{\lauOut}{\lambda^{\mathrm{u}}}
\newcommand{\LauOut}{\Lambda^{\mathrm{u}}}

%%%% OUTER SPACE - INFINITE %%%
% Domains
\newcommand{\DuInfty}{{D}^{\mathrm{u},\infty}_{\rho_1}}
\newcommand{\DsInfty}{{D}^{\mathrm{s},\infty}_{\rho_1}}
\newcommand{\DdInfty}{{D}^{\diamond,\infty}_{\rho_1}}
\newcommand{\DuInftyRho}{{D}^{\mathrm{u},\infty}_{\rho_1}}
\newcommand{\DsInftyRho}{{D}^{\mathrm{s},\infty}_{\rho_1}}
\newcommand{\DdInftyRho}{{D}^{\diamond,\infty}_{\rho_1}}
\newcommand{\ballInftyDef}{B(\varrho)}
\newcommand{\ballInfty}{B(\varrho \de^3)}
%\newcommand{\DInfty}{{D}^{\infty}_{\rho_1}}
\newcommand{\rhoInfty}{\rho_1}
% Banach spaces
\newcommand{\XcalInfty}{\mathcal{X}^{\infty}}
\newcommand{\XcalInftyTotal}{\mathcal{X}^{\infty}_{\times}}
% Norms
\newcommand{\normInfty}[1]{\left\lVert#1\right\rVert^{\infty}}
\newcommand{\normInftySmall}[1]{\lVert#1\rVert^{\infty}}
\newcommand{\normInftyTotal}[1]{\left\lVert#1\right\rVert^{\infty}_{\times}}


%%%% OUTER SPACE - BOUNDED %%%
\newcommand{\ballOuterDef}{B(\varrho)}
\newcommand{\ballOuter}{B(\varrho \de^3)}
% Domains
\newcommand{\DuOut}{{D}_{\kappa,d_1,\rho_2}^{\mathrm{u, out}}}
\newcommand{\DuOutKappa}{{D}_{\kappa_1,d_1,\rho_2}^{\mathrm{u, out}}}
\newcommand{\DsOut}{{D}_{\kappa,d_1,\rho_2}^{\mathrm{s, out}}}
\newcommand{\DsOutKappa}{{D}_{\kappa_1,d_1,\rho_2}^{\mathrm{s, out}}}
\newcommand{\DusOut}{{D}_{\kappa,d_1,\rho_2}^{\mathrm{u/s, out}}}
\newcommand{\DdOut}{{D}_{\kappa,d_1,\rho_2}^{\diamond, \mathrm{out}}}
\newcommand{\DOut}{{D}_{\kappa,d_1, \rho_2}^{\mathrm{out}}}
\newcommand{\rhoOuter}{\rho_2}
\newcommand{\dOuter}{d_1}
\newcommand{\kappaOuter}{\kappa_1}
% Banach spaces
\newcommand{\XcalOut}{\mathcal{X}^{\mathrm{out}}}
\newcommand{\XcalOutTotal}{\mathcal{X}^{\mathrm{out}}_{\times}}
% Norms
\newcommand{\normOut}[1]{\left\lVert#1\right\rVert^{\mathrm{out}}}
\newcommand{\normOutSmall}[1]{\lVert#1\rVert^{\mathrm{out}}}
\newcommand{\normOutTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{out}}_{\times}}
\newcommand{\normOutTotalSmall}[1]{\lVert#1\rVert^{\mathrm{out}}_{\times}}

%%%% OUTER SPACE - TRANSITION %%%%%%
\newcommand{\normSup}[1]{\lVert#1\rVert_{\mathrm{sup}}}
\newcommand{\normSupBig}[1]{\left\lVert#1\right\rVert_{\mathrm{sup}}}
% Domain Boomerang
\newcommand{\DBoomerang}{{D}_{\kappa, d}}
\newcommand{\DBoomerangKappa}{{D}_{\kappa_0, d}}
\newcommand{\dBoomerang}{d}
\newcommand{\kappaBoomerang}{\kappa_0}
% Domain Outer Tilde
\newcommand{\DOuterTilde}{\widetilde{D}_{\kappa_2,d_2,d_3}^{\mathrm{u, out}}}
\newcommand{\DOuterTildeBig}{\widetilde{D}_{\tilde{\kappa}_2,\tilde{d}_2,\tilde{d}_3}^{\mathrm{u, out}}}
\newcommand{\dOuterA}{d_2}
\newcommand{\dOuterB}{d_3}
\newcommand{\kappaOuterTilde}{\kappa_2}
\newcommand{\dOuterABig}{\tilde{d}_2}
\newcommand{\dOuterBBig}{\tilde{d}_3}
\newcommand{\kappaOuterTildeBig}{\tilde{\kappa}_2}
\newcommand{\rhoOuterTilde}{\rho_3}
\newcommand{\YcalOuter}{\mathcal{Y}^{\mathrm{out}}}
\newcommand{\ballOuterTilde}{B(\varrho\de^2)}
\newcommand{\ballOuterTildeDef}{B(\varrho)}
% Domain Flow
\newcommand{\DFlow}{{D}_{\kappa_3, d_4}^{\mathrm{fl}}}
\newcommand{\dFlow}{d_4}
\newcommand{\kappaFlow}{\kappa_3}
% Domain Boomerang Tilde
\newcommand{\DBoomerangTilde}{\widetilde{D}_{\kappa, d}}
\newcommand{\DBoomerangTildeProp}{\widetilde{D}_{\kappa_4, d_5}}
\newcommand{\dBoomerangTilde}{d_5}
\newcommand{\kappaBoomerangTilde}{\kappa_4}
\newcommand{\YcalBoom}{\widetilde{\mathcal{Y}}}
\newcommand{\ballBoomerangTilde}{B(\varrho\de^2)}
% Funcions
\newcommand{\uOut}{\mathcal{U}}
\newcommand{\vOut}{\mathcal{V}}
\newcommand{\Gh}{\widehat{\Gamma}}
\newcommand{\Gu}{\Gamma^{\mathrm{u}}}
% Norms
\newcommand{\normFlow}[1]{\lVert#1\rVert^{\mathrm{fl}}}
\newcommand{\normFlowBig}[1]{\left\lVert#1\right\rVert^{\mathrm{fl}}}
\newcommand{\normFlowTotal}[1]{\lVert#1\rVert^{\mathrm{fl}}_{\times}}
\newcommand{\normFlowTotalBig}[1]{\left\lVert#1\right\rVert^{\mathrm{fl}}_{\times}}
% Banach Space
\newcommand{\XcalFlow}{\mathcal{X}^{\mathrm{fl}}}
\newcommand{\XcalFlowTotal}{\mathcal{X}^{\mathrm{fl}}_{\times}}
% Balls
\newcommand{\ballFlow}{B(\varrho\de^3)}
\newcommand{\ballFlowDef}{B(\varrho)}

%%%% MATCHING %%%
\newcommand{\mch}{\mathrm{mch}}
\newcommand{\kappaMch}{\kappa_6}
% Domains
\newcommand{\DuMchOut}{{D}_{\kappa}^{\mathrm{mch,u}}}
\newcommand{\DsMchOut}{{D}_{\kappa}^{\mathrm{mch,s}}}
\newcommand{\DdMchOut}{{D}_{\kappa}^{\mathrm{mch},\diamond}}
\newcommand{\DMchInn}{\mathcal{D}_{\kappa}^{\mathrm{mch}}}
\newcommand{\DuMchInn}{\mathcal{D}_{\kappa}^{\mathrm{mch,u}}}
\newcommand{\DsMchInn}{\mathcal{D}_{\kappa}^{\mathrm{mch,s}}}
\newcommand{\DdMchInn}{\mathcal{D}_{\kappa}^{\mathrm{mch},\diamond}}
\newcommand{\DusMchInn}{\mathcal{D}_{\kappa}^{\mathrm{mch,u,s}}}
% Variables Originals
\newcommand{\ZMchO}{Z}
\newcommand{\ZuMchO}{Z^{\mathrm{u}}}
\newcommand{\ZsMchO}{Z^{\mathrm{s}}}
\newcommand{\ZusMchO}{Z^{\mathrm{u,s}}}
\newcommand{\ZdMchO}{Z^{\diamond}}
\newcommand{\WMchO}{W}
\newcommand{\WuMchO}{W^{\mathrm{u}}}
\newcommand{\WsMchO}{W^{\mathrm{s}}}
\newcommand{\WusMchO}{W^{\mathrm{u,s}}}
\newcommand{\WdMchO}{W^{\diamond}}
\newcommand{\XMchO}{X}
\newcommand{\XuMchO}{X^{\mathrm{u}}}
\newcommand{\XsMchO}{X^{\mathrm{s}}}
\newcommand{\XusMchO}{X^{\mathrm{u,s}}}
\newcommand{\XdMchO}{X^{\diamond}}
\newcommand{\YMchO}{Y}
\newcommand{\YuMchO}{Y^{\mathrm{u}}}
\newcommand{\YsMchO}{Y^{\mathrm{s}}}
\newcommand{\YusMchO}{Y^{\mathrm{u,s}}}
\newcommand{\YdMchO}{Y^{\diamond}}
% Variables Diferencia
\newcommand{\ZMchU}{Z_1}
\newcommand{\ZuMchU}{Z_1^{\mathrm{u}}}
\newcommand{\ZsMchU}{Z_1^{\mathrm{s}}}
\newcommand{\ZusMchU}{Z_1^{\mathrm{u,s}}}
\newcommand{\ZdMchU}{Z_1^{\diamond}}
\newcommand{\WMchU}{W_1}
\newcommand{\WuMchU}{W_1^{\mathrm{u}}}
\newcommand{\WsMchU}{W_1^{\mathrm{s}}}
\newcommand{\WusMchU}{W_1^{\mathrm{u,s}}}
\newcommand{\WdMchU}{W_1^{\diamond}}
\newcommand{\XMchU}{X_1}
\newcommand{\XuMchU}{X_1^{\mathrm{u}}}
\newcommand{\XsMchU}{X_1^{\mathrm{s}}}
\newcommand{\XusMchU}{X_1^{\mathrm{u,s}}}
\newcommand{\XdMchU}{X_1^{\diamond}}
\newcommand{\YMchU}{Y_1}
\newcommand{\YuMchU}{Y_1^{\mathrm{u}}}
\newcommand{\YsMchU}{Y_1^{\mathrm{s}}}
\newcommand{\YusMchU}{Y_1^{\mathrm{u,s}}}
\newcommand{\YdMchU}{Y_1^{\diamond}}
% Banach Spaces
\newcommand{\XcalMch}{\mathcal{X}^{\mathrm{mch}}}
\newcommand{\XcalMchS}{\mathcal{X}^{\mathrm{mch,s}}}
\newcommand{\XcalMchU}{\mathcal{X}^{\mathrm{mch,u}}}
\newcommand{\XcalMchD}{\mathcal{X}^{\mathrm{mch},\diamond}}
\newcommand{\XcalMchUS}{\mathcal{X}^{\mathrm{mch,u/s}}}
\newcommand{\XcalMchTotal}{\mathcal{X}^{\mathrm{mch}}_{\times}}
\newcommand{\XcalMchUTotal}{\mathcal{X}^{\mathrm{mch,u}}_{\times}}
\newcommand{\XcalMchSTotal}{\mathcal{X}^{\mathrm{mch,s}}_{\times}}
\newcommand{\XcalMchDTotal}{\mathcal{X}^{\mathrm{mch},\diamond}_{\times}}
% Norms
\newcommand{\normMch}[1]{\left\lVert#1\right\rVert^{\mathrm{mch}}}
\newcommand{\normMchSmall}[1]{\lVert#1\rVert^{\mathrm{mch}}}
\newcommand{\normMchU}[1]{\left\lVert#1\right\rVert^{\mathrm{mch,u}}}
\newcommand{\normMchS}[1]{\left\lVert#1\right\rVert^{\mathrm{mch,s}}}
\newcommand{\normMchD}[1]{\left\lVert#1\right\rVert^{\mathrm{mch},\diamond}}
\newcommand{\normMchUTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{mch,u}}_{\times}}
\newcommand{\normMchSTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{mch,s}}_{\times}}
\newcommand{\normMchDTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{mch},\diamond}_{\times}}
\newcommand{\normMchTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{mch}}_{\times}}
\newcommand{\normMchTotalSmall}[1]{\lVert#1\rVert^{\mathrm{mch}}_{\times}}


%%%% DIFFERENCE %%%
\newcommand{\spl}{\mathrm{spl}}
\newcommand{\dzHat}{\Delta \Phi}
\newcommand{\dzHatO}{\Delta \Phi_0}
\newcommand{\dzHatU}{\Delta \Phi_1}
\newcommand{\dzOutO}{\Delta z_0}
\newcommand{\dwOutO}{\Delta w_0}
\newcommand{\dxOutO}{\Delta x_0}
\newcommand{\dyOutO}{\Delta y_0}
\newcommand{\dzOutU}{\Delta z_1}
\newcommand{\dwOutU}{\Delta w_1}
\newcommand{\dxOutU}{\Delta x_1}
\newcommand{\dyOutU}{\Delta y_1}
%Variables Inner domain
\newcommand{\DZInnC}{\Delta Z}
\newcommand{\DWInnC}{\Delta W}
\newcommand{\DXInnC}{\Delta X}
\newcommand{\DYInnC}{\Delta Y}
\newcommand{\DZInnU}{\Delta Z_1}
\newcommand{\DWInnU}{\Delta W_1}
\newcommand{\DXInnU}{\Delta X_1}
\newcommand{\DYInnU}{\Delta Y_1}
% Banach spaces
\newcommand{\XSpl}{\mathcal{X}^{\mathrm{spl}}}
\newcommand{\XSplTotal}{\mathcal{X}^{\mathrm{spl}}_{\times}}
% Norms
\newcommand{\normSpl}[1]{\left\lVert#1\right\rVert^{\mathrm{spl}}}
\newcommand{\normSplTotal}[1]{\left\lVert#1\right\rVert^{\mathrm{spl}}_{\times}}


%%%% CONSTANTS ARTICLE OUTER %%%
% Main: constant theoremes principals
\newcommand{\cttTheorem}{b_0}
% Main: Constants Existence
\newcommand{\cttOuterA}{b_1}
\newcommand{\cttOuterB}{b_2}
\newcommand{\cttOuterC}{b_3}
\newcommand{\cttOuterD}{b_4}
\newcommand{\cttOuterF}{b_5}
\newcommand{\cttOuterG}{b_6}
\newcommand{\cttOuterH}{b_7}
% Main: Constants Inner Derivation
\newcommand{\cttInnDerA}{c_1}
\newcommand{\cttInnDerAA}{\gamma_1}
\newcommand{\cttInnDerB}{c_2}
\newcommand{\cttInnDerBB}{\gamma_2}
\newcommand{\cttInnDerC}{b_8}
% Main: Constants Inner Computation
\newcommand{\cttInnExist}{b_{9}}
\newcommand{\cttInnDiff}{b_{10}}
% Main: Constants Matching
\newcommand{\cttMch}{b_{11}}
% Main: Constants Difference
\newcommand{\cttDiffA}{b_{12}}
\newcommand{\cttDiffB}{b_{13}}
% Proof Existence
\newcommand{\cttOutInftyA}{b_{14}}
\newcommand{\cttOutOutA}{b_{15}}
\newcommand{\cttOutOutB}{b_{16}}
\newcommand{\cttOutOutC}{b_{17}}
% Proof Matching
\newcommand{\cttMchA}{b_{18}}



% Main: Angles 
\newcommand{\betaBow}{\beta_0}
\newcommand{\betaOutA}{\beta_0}
\newcommand{\betaOutB}{\beta_1}
\newcommand{\betaInner}{\beta_0}
\newcommand{\betaMchA}{\beta_2}
\newcommand{\betaMchB}{\beta_3}

==> Article Outer/singularitiesOuter.tex <==


% In this section, we describe the analytical extension of the time 
% parameterization of the  separatrix of 
The unperturbed Hamiltonian 
\[
H_0(\la, \La, x,y) = 
H_{\pend}(\la, \La) + H_{\osc}(x,y)\]
(see \eqref{def:hamiltonianScalingH0}) possesses a saddle with two separatrices 
in the $(\la,\La)$-plane (see 
Figure~\ref{fig:separatrix}).
%
% In particular, since $H_0$ is decoupled, we only need to study ${H}_{\pend}$ 
% (see Proposition \ref{proposition:HamiltonianScaling}).
% The Hamiltonian ${H}_{\pend}(\la,\La)$ has $1$-degree of freedom and a saddle 
% at $(\la,\La)=(0,0)$ with two homoclinic connections or separatrices (see 
% Figure~\ref{fig:separatrix}). 
%
%From now on, we only consider the separatrix on the right; by symmetry, the results obtained below are analogous for the separatrix on the left. 
%
%We are interested in studying the analytic continuation of the time parametrization of this separatix.
%Let us only consider the separatrix on the right.
%
Let us consider the real-analytic time parametrization of the 
 separatrix with $\la\in (0,\pi)$,
\begin{equation}\label{eq:separatrixParametrization}
	\begin{split}
		\s:\reals &\to \torus \times \reals \\
		t &\mapsto \s(t)=(\la_h(t),\La_h(t)),
	\end{split}
\end{equation}
with initial condition $\s(0)=(\la_0,0)$ where $\la_0 =
\arccos\paren{\frac12-\sqrt{2}} \in \left(\frac{2}{3}\pi,\pi\right)$.
%
%\[
%\s(0)=(\la_0,0) \text{ where } \la_0 \in \left(\frac{2}{3}\pi,\pi\right).
%\]
%and satisfying the asymptotic condition
%$
%\lim_{t\to \pm \infty } \s(t) = (0,0).
%$
%
%

The following result (which encompass Theorem 2.2, Proposition 2.3 and 
Corollary~2.4 in \cite{articleInner})
gives the properties of the analytic extension of $\s(t)$ to the
domain 
\begin{equation}\label{def:dominiBow}
	\begin{split}	
		\Pi^{\mathrm{ext}}_{A, \beta} =& \claus{
			t \in \complexs \st 
			\vabs{\Im t} < \tan \beta \, \Re t + A }
		\cup \\
		&\claus{
			t \in \complexs \st 
			\vabs{\Im t} < -\tan \beta \, \Re t + A},
	\end{split}
\end{equation}
with $A$ as given in~\eqref{def:integralA} (see Figure~\ref{fig:dominiBow}).
%
\begin{figure} 
	\centering
	\begin{overpic}[scale=0.5]{dominiBow.png}
		\put(101,27.5){\footnotesize$\Re t$}
		\put(45.5,59){\footnotesize$\Im t$}
		\put(28,30){\footnotesize $\beta$}
		\put(42,45){\footnotesize $iA$}
		%\put(40,10){{$-iA$}}
		\put(70,32){$\Pi_{A,\beta}^{\mathrm{ext}}$}
	\end{overpic}
	\bigskip
	\caption{Representation of the domain $\Pi_{A,\beta}^{\mathrm{ext}}$ in~\eqref{def:dominiBow}.}
	\label{fig:dominiBow}
\end{figure}


\begin{theorem}\label{theorem:singularities}
The real-analytic time parametrization $\s$ defined 
in~\eqref{eq:separatrixParametrization} satisfies:
\begin{itemize}
\item There exists $0<\betaBow<\frac{\pi}{2}$ such that $\s(t)$ extends 
analytically to $\Pi_{A,\betaBow}$.
% as given in \eqref{def:dominiBow}.
%
\item $\s(t)$ has only two singularities on $\partial \Pi^{\mathrm{ext}}_{A, 
\betaBow}$ at $t=\pm iA$.
%
\item There exists $\upsilon>0$ such that,
for $t \in \complexs$ with $\vabs{t -iA}<\upsilon$ and $\arg(t -iA) \in (-\frac{3\pi}{2},\frac{\pi}{2})$, 
% $\s(t)=(\la_h(t),\La_h(t))$ can be expressed as
\begin{equation*}
%\label{eq:homoclinicaSingularities}
	\begin{split}
		&\la_h(t) =  \pi + 3\al_{+} (t- iA)^{\frac{2}{3}} + \OO(t- iA)^{\frac{4}{3}}, \\[0.5em]
		&\La_h(t) =  -\frac{ 2 \al_{+}}{3} \frac{1}{(t- iA)^{\frac{1}{3}}} + 
		\OO(t- iA)^{\frac{1}{3}}, 
	\end{split}
\end{equation*}
with $\al_{+} \in \complexs$ such that $\al_{+}^3=\frac{1}{2}$. 

An analogous result holds for $\vabs{t+iA}<\upsilon$, $\arg(t+iA) \in(-\frac{\pi}{2},\frac{3\pi}{2})$ and $\al_- = \conj{\al_+}$.
%
\item  $\La_h(t)$ has only one zero in $\ol{\Pi^{\mathrm{ext}}_{A, \betaBow}}$ at $t=0$.
\end{itemize}
\end{theorem}




==> Article Outer/undoChanges.tex <==

To prove Theorem \ref{theorem:mainTheorem} (and Remark \ref{remark:sectiontheta}) from Theorem \ref{theorem:mainTheoremPoincare} we need to ``undo'' the changes of coordinates $\phi_{\Poi}$ and $\phi_{\sca}$ and adjust the section from $\lambda=\text{constant}$ to $\theta=\text{constant}$.
%

First, we consider the change $\phi_{\sca}$ given by $(\la,L,\eta,\xi)=(\la,1+\de^2\La,\de x, \de y)$, (see \eqref{def:changeScaling}).
%
For $\la_* \in [\la_1,\la_2]$ we define
\begin{align}\label{proof:poincareEstimatesExistence}
	L^{\diamond}(\la_*;\de) = 1+\de^2 \La_*^{\diamond},
	\qquad
	\eta^{\diamond}(\la_*;\de) = \de x^{\diamond}_*, 
	\qquad
	\xi^{\diamond}(\la_*;\de) = \de y^{\diamond}_*,
	\quad
	\text{for } \diamond=\unstable,\stable.
\end{align}	
Then, by Theorem \ref{theorem:mainTheoremPoincare}, one has
\begin{equation}\label{proof:poincareEstimatesDifference}
\begin{split}	
	|\D L(\la_*;\de)| &= 
	|L^{\unstable}(\la_*;\de) - L^{\stable}(\la_*;\de) |
	= \OO \paren{\de^{\frac{10}3} e^{-\frac{A}{\de^2}}},
	\\
	|\D \eta(\la_*;\de)|
	&=
	|\eta^{\unstable}(\la_*;\de) - \eta^{\stable}(\la_*;\de)| 
	= 	\sqrt[6]{2} \,
\de^{\frac{4}{3}}  e^{-\frac{A}{\de^2}} 
	\boxClaus{ \vabs{\CInn}
	+ \OO\paren{\frac{1}{\vabs{\log \de}}}},\\
% 	\OO \paren{\de^{\frac{4}3} e^{-\frac{A}{\de^2}}},
	\qquad
	\D \xi(\la_*;\de) & = \conj{\D \eta(\la_*;\de)}.
	\end{split}	
\end{equation}

Next, we study the change $\phi_{\Poi}$. In the following result, we give a series expression of the polar coordinates with respect to the Poincar\'e elements. 
%
Its proof is a 
direct consequence of the definition of the Poincar\'e variables (see, for 
instance, Section 4.1 in 
\cite{articleInner}).

\begin{lemma}\label{lemma:seriesExpansionPoincare}
%
Fix $\varrho>0$.
%
Then, for $\vabs{(L-1,\eta,\xi)} \ll 1$ and $\vabs{\Im \la}\leq \varrho$, the 
polar  coordinates $(r,\tht,R,G)$ introduced  in \eqref{def:changePolars} satisfy
\begin{align*}
	r &= 1 +2(L-1)
	-\frac{e^{-i\la}}{\sqrt2}  \eta
	-\frac{e^{i\la}}{\sqrt2} \xi
	+ \OO(L-1,\eta,\xi)^2, 
	\\
	\tht &= \la + i\sqrt2 e^{-i\la}\eta -i \sqrt2 e^{i\la} \xi + \OO(L-1,\eta,\xi)^2, 
	\\
	R &= 
	{\frac{i e^{-i\la}}{\sqrt2}  \eta
	-
	\frac{i e^{i\la}}{\sqrt2} \xi}
	+
	\OO(L-1,\eta,\xi)^2,
	\qquad
	G = L - \eta \xi.
\end{align*}
\end{lemma}

%\begin{proof}
%The result for the angular momentum $G$ is straightforward by the definition of the Poincar\'e elements.
%%	
%\begin{align}
%	r=L^2(1-e\cos u), 
%	\qquad
%	\tht = \la + f-u + e \sin u,
%	\qquad
%	R = \frac{e \sin u}{L(1-e\cos u)}.
%\end{align}
%\end{proof}



%\begin{proof}
%%
%In this proof we use the formulae introduced in Section 2.1 in \cite{articleInner} for different orbital elements.
%%
%In the following, we apply the results regarding the eccentricity $e$, the mean anomaly $\ell$, the eccentric anomaly $u$ and the true anomaly $f$.
%
%\begin{itemize}
%	\item The result for the angular momentum $G$ is straightforward by the definition of the Poincar\'e elements.
%	\item The radius $r$ satisfies that $r=L^2(1-e\cos u)$. 
%	%
%	In Section 4.1 of \cite{articleInner}, it was seen that
%	\begin{equation}\label{eq:trigoU}
%		\begin{split}
%		e\cos u &= \frac{1}{\sqrt{2L}}
%		\paren{e^{-i\la}\eta+e^{i\la}\xi} 
%		%+ \frac{1}{2L} \paren{e^{-i\la}\eta-e^{i\la}\xi}^2 
%		+ \OO(e^{-i\la}\eta,e^{i\la}\xi)^2 \\
%		&= 
%		\frac{e^{-i\la}}{\sqrt{2}} \eta
%		+
%		\frac{e^{i\la}}{\sqrt{2}} \xi
%		+ \OO(L-1,\eta,\xi)^2
%		, \\
%		e\sin u &= 
%			\frac{i}{\sqrt{2L}} \paren{e^{-i\la}\eta-e^{i\la}\xi}
%			%+\frac{i}{2L} \paren{e^{-2i\la}\eta^2-e^{2i\la}\xi^2} 
%			+\OO(e^{-i\la}\eta,e^{i\la}\xi)^2
%		\\
%		&= 
%		\frac{i e^{-i\la}}{\sqrt{2}} \eta
%		-
%		\frac{i e^{i\la}}{\sqrt{2}} \xi
%		+ \OO(L-1,\eta,\xi)^2
%		, \\
%		\end{split}
%	\end{equation}
%	As a result, we obtain the asymptotic expression for $r$.
%	\item The angle $\tht$ satisfies that $\tht=\la + f-\ell$. 
%	%
%	Since the eccentric anomaly is given implicitly by $u-e \sin u = \ell$, we have that
%	\begin{align}\label{proof:thtDef}
%		\tht = \la + f-u + e \sin u.
%	\end{align} 
%	The true anomaly $f$ and the eccentricity $e$ satisfy that
%	\begin{align}\label{proof:trigfande}
%		\sin f = \frac{\sqrt{1-e^2}\sin u}{1-e\cos u},
%		\qquad
%		e^2 = 1-\frac{G^2}{L^2} = \eta\xi\frac{(2L-\eta \xi)}{L}.
%	\end{align}
%	Then, by \eqref{eq:trigoU},
%	\begin{align*}
%		\sin f &= \paren{1 + e\cos u} \sin u 
%		+ \OO(L-1,\eta,\xi)^2 \\
%		&= \sin(u+e\sin u) + \OO(L-1,\eta,\xi)^2.
%	\end{align*}
%	By \eqref{proof:thtDef} and using that $\vabs{\Im \la} \leq \varrho$, one obtains
%	$\tht = \la + 2 e \sin u + \OO(L-1,\eta,\xi)^2$, 
%	and applying \eqref{eq:trigoU} we obtain the 
%	corresponding asymptotic formula.
%%	\begin{align*}
%%		\tht = \la + 2 e \sin u + \OO(L-1,\eta,\xi)^2
%%		= \la + i \sqrt2 e^{-i\la} \eta 
%%		- i \sqrt2 e^{i\la}
%%		+ \OO(L-1,\eta,\xi)^2.
%%	\end{align*}
%	\item The linear momentum $R$ satisfies that
%	\[
%	-\frac{1}{2L^2}=\frac12\paren{R^2 + \frac{G^2}{r^2}}-\frac1{r}.
%	\]
%	%
%	Then, since $r=L^2(1-e\cos u)$ and, by \eqref{proof:trigfande}, $G^2=L^2(1-e^2)$, one obtains that
%	\begin{align*}
%		R^2 = \frac{(e \sin u)^2}{L^2(1-e\cos u)^2},
%	\end{align*}
%	and applying \eqref{eq:trigoU} we obtain the statement of the lemma.
%\end{itemize}
%\end{proof}

Since in Theorem \ref{theorem:mainTheoremPoincare} the distance is measured in the section $\la=\la_*$ whereas the Theorem \ref{theorem:mainTheorem}, and more generally Remark \ref{remark:sectiontheta}, measures it in the section  $\tht=\tht^*$, we must ``translate'' the estimates in 
% We need to compute the differences between invariant manifolds 
\eqref{proof:poincareEstimatesDifference} to the new section.
% , not in the section $\la=\la_*$, but in the polar coordinate section
%
By Lemma \ref{lemma:seriesExpansionPoincare}, let $g_{\tht}$ be the function such that $\tht=\la+g_{\tht}(\la,L,\eta,\xi)$.
%
Then, for $\diamond=\unstable,\stable$, we consider 
\[
F^{\diamond}(\la,\tht,\de) =\tht - \la + g_{\tht}\paren{\la,L^{\diamond}(\la;\de),\eta^{\diamond}(\la;\de),\xi^{\diamond}(\la;\de)}.
\]
Applying the Implicit Function Theorem, Lemma 
\ref{lemma:seriesExpansionPoincare} and that, by
\eqref{proof:poincareEstimatesExistence},
$L^{\diamond}(\la;0)=1$ and
$\eta^{\diamond}(\la;0) = 
\xi^{\diamond}(\la;0)=0$,
then there exist function 
$\wh\la^{\diamond}(\tht;\de)$ such that 
$F^{\diamond}(\wh\la^{\diamond}(\tht;\de),\tht,\de)=0$ and
% \textcolor{red}{.
\begin{equation}\label{proof:lausSerie}
\begin{split}	
\wh\la^{\diamond}(\tht;\de) =& \, \tht 
-i \sqrt2 e^{-i\tht}\wh\eta^{\diamond}(\tht;\de)	
+i \sqrt2 e^{i\tht}\wh\xi^{\diamond}(\tht;\de) \\
&+ \OO\paren{\wh L^{\diamond}(\tht;\de)-1,\wh \eta^{\diamond}(\tht;\de), 
\wh\xi^{\diamond}(\tht;\de)}^2,
\end{split}
\end{equation}
%
with 
$\wh\eta^{\diamond}(\tht;\de)=\eta^{\diamond}(\wh\la^{\diamond}(\tht;\de);\de)$, 
$\wh\xi^{\diamond}(\tht;\de)=\xi^{\diamond}(\wh\la^{\diamond}(\tht;\de);\de)$ 
and $\wh L^{\diamond}(\tht;\de)=L^{\diamond}(\wh\la^{\diamond}(\tht;\de);\de)$.
%
Notice that, by \eqref{def:estimatesInvMan} (plus Cauchy estimates for their 
derivatives) and \eqref{proof:poincareEstimatesExistence},
%
\begin{equation*}\label{proof:poincareEstimatesExistencelambda}
\wh\la^{\diamond}(\tht;\de) = \tht + \OO(\de^4).
\end{equation*}
Thus,  for any  $[\tht_1,\tht_2] \subset (0,\la_0)$ and $\delta$ small enough, 
there exists $[\lambda_1,\lambda_2] \subset (0,\la_0)$ such that, for $\tht \in 
[\tht_1,\tht_2]$ one has  $\wh\la^{\unstable,\stable}(\tht;\de) \in 
[\lambda_1,\lambda_2] $.
%
%
In addition,
\begin{equation}\label{proof:poincareEstimatesExistenceTheta}
\begin{aligned}	
\wh{L}^{\diamond}(\tht;\de) &= L^{\diamond}(\tht;\de) + \OO(\de^6) = 1 + \OO(\de^2),
\\ 
\wh\eta^{\diamond}(\tht;\de)
&= \eta^{\diamond}(\tht;\de) + \OO(\de^8)
= \OO(\de^4),
\\
\wh\xi^{\diamond}(\tht;\de)
&= \xi^{\diamond}(\tht;\de) + \OO(\de^8)
=\OO(\de^4).
\end{aligned}
\end{equation}
%
Then, since $\La^{\unstable,\stable}_*>0$, by \eqref{proof:poincareEstimatesExistence} one has that  $\wh{L}^{\unstable,\stable}(\tht;\de)>1$ for $\tht \in [\tht_1,\tht_2]$.
%
Moreover, by Lemma \ref{lemma:seriesExpansionPoincare} and taking $\de$ small enough, one has $r^{\unstable,\stable}(\tht)-1>0$.

The difference between the invariant manifolds in a section of fixed $\tht \in[\tht_1,\tht_2]$ is given by
%
\begin{align*}
	\D \wh\la(\tht;\de) =& \,
	\wh\la^{\unstable}(\tht;\de) -
	\wh\la^{\stable}(\tht;\de), 
	&
	\D \wh{L}(\tht;\de) =& \,  
	\wh{L}^{\unstable}(\tht;\de)-
	\wh{L}^{\stable}(\tht;\de), 
	\\
	\D \wh{\eta}(\tht;\de) =& \, 
	\wh\eta^{\unstable}(\tht;\de)-
	\wh\eta^{\stable}(\tht;\de), 
	&
	\D \wh{\xi}(\tht;\de) =& \, 
	\wh\xi^{\unstable}(\tht;\de)-
	\wh\xi^{\stable}(\tht;\de).
\end{align*}
%\begin{align*}
%	\D \wh\la(\tht;\de) =& \,
%	\wh\la^{\unstable}(\tht;\de) -
%	\wh\la^{\stable}(\tht;\de), 
%	&
%	\D \wh{L}(\tht;\de) =& \,  L^{\unstable}(\wh\la^{\unstable}(\tht;\de))-
%	L^{\stable}(\wh\la^{\stable}(\tht;\de)), 
%	\\
%	\D \wh{\eta}(\tht;\de) =& \, 
%\eta^{\unstable}(\wh\la^{\unstable}(\tht;\de))-
%	\eta^{\stable}(\wh\la^{\stable}(\tht;\de)), 
%	&
%	\D \wh{\xi}(\tht;\de) =& \, 
%\xi^{\unstable}(\wh\la^{\unstable}(\tht;\de))-
%	\xi^{\stable}(\wh\la^{\stable}(\tht;\de)).
%\end{align*}
% where the hats just denote that they are parameterized as graphs with respect to $\theta$ instead of $\lambda$.
Then, by \eqref{proof:lausSerie} and \eqref{proof:poincareEstimatesExistenceTheta}, one has that
\begin{align*}
\D \wh\la(\tht;\de) = 
-i\sqrt2 e^{-i\tht} \D\wh \eta(\tht;\de)
+i\sqrt2 e^{i\tht} \D\wh  \xi(\tht;\de)+
\OO\paren{\de^2 \D \wh{L}(\tht;\de),
\de^4 \D\wh \eta(\tht;\de),
\de^4\D \wh\xi(\tht;\de)}.
% +\OO(\de^{\frac{8}3} e^{-\frac{A}{\de^2}})
% =
% \OO(\de^{\frac43} e^{-\frac{A}{\de^2}}).
\end{align*} 
Moreover, by the mean value theorem,
\eqref{proof:poincareEstimatesDifference} and
\eqref{proof:poincareEstimatesExistenceTheta},
\begin{equation*}
%\label{proof:diffL}
\begin{split}	
\D \wh{L}(\tht;\de) =&\,
\D L(\wh\la^{\unstable}(\tht;\de);\de) +\wh 
L^\stable(\wh\la^{\unstable}(\tht;\de);\de)-\wh 
L^\stable(\wh\la^{\stable}(\tht;\de);\de)\\
% 
% \D \la(\tht;\de) \boxClaus{
% \int_0^1 \partial_{\la} L^{\stable}(t \la^{\unstable}(\tht;\de)+(1-t) \la^{\stable}(\tht;\de)) dt} \\
 =&\, \OO(\de^{\frac{10}3} e^{-\frac{A}{\de^2}})+\de^2\OO\left(\D \wh
\la(\tht;\de)\right).
\end{split}
\end{equation*}
Analogously,
\begin{equation*}
%\label{proof:diffetaxi}
\begin{split}	
	\D \wh{\eta}(\tht;\de) &= \D\eta(\wh\la^{\unstable}(\tht;\de);\de) + 
% \OO(\de^{\frac{7}3} e^{-\frac{A}{\de^2}}),
\de^ 4\OO\left(\D 
\wh\la(\tht;\de)\right) ,
	\\
	\D \wh{\xi}(\tht;\de) &= \conj{\D\eta(\la^{\unstable}(\tht;\de);\de)} +
	\de^ 4\OO\left(\D \wh
\la(\tht;\de)\right) .
% 	+ \OO(\de^{\frac{7}3} e^{-\frac{A}{\de^2}}).
\end{split}	
\end{equation*}
%and, applying Theorem \ref{theorem:mainTheoremPoincare},
%\begin{align*}
%\vabs{\D \wh{\eta}(\tht;\de)} = \sqrt[6]{2} \,
%\de^{\frac{4}{3}}  e^{-\frac{A}{\de^2}} 
%\boxClaus{ \vabs{\CInn}
%	+ \OO\paren{\frac{1}{\vabs{\log \de}}}}.
%\end{align*}
Therefore, using  \eqref{proof:poincareEstimatesDifference},  one can conclude 
that 
 \begin{align*}	
|\D \wh \la(\theta;\de)| &=  \OO \paren{\de^{\frac{4}3} 
e^{-\frac{A}{\de^2}}},
&
|\D\wh \eta(\theta;\de)|
&=\sqrt[6]{2} \,
\de^{\frac{4}{3}}  e^{-\frac{A}{\de^2}} 
\boxClaus{ \vabs{\CInn}
	+ \OO\paren{\frac{1}{\vabs{\log \de}}}},
\\
|\D \wh L(\theta;\de)| &=  \OO \paren{\de^{\frac{10}3} 
e^{-\frac{A}{\de^2}}},
&
\D\wh \xi(\theta;\de) & = \conj{\D \wh\eta(\theta;\de)}.
\end{align*}	
Once we have adjusted the transverse section, it only remains to apply  Lemma 
\ref{lemma:seriesExpansionPoincare}  to translate these differences 
% $\D\wh{L}(\tht,\de)$, 
% $\D\wh{\eta}(\tht,\de)$ and $\D\wh{\xi}(\tht,\de)$ 
to polar coordinates. That is,
%
% \textcolor{red}{(Repassar que estiguin b\'e les pot\`encies de $\de$.))}
% By, one has that
\begin{align*}
	r^{\unstable} - r^{\stable} 
	&= -\sqrt2 \cos \tht \, \Re \D \wh{\eta}(\tht;\de)
	-\sqrt2 \sin\tht \, \Im \D \wh{\eta}(\tht;\de)
	+ \OO(\de^{\frac{10}3} e^{-\frac{A}{\de^2}}), 
	\\
	R^{\unstable} - R^{\stable} 
	&= -\sqrt2 \cos \tht \, \Im \D \wh{\eta}(\tht;\de)
	+\sqrt2 \sin\tht \, \Re \D \wh{\eta}(\tht;\de)
	+ \OO(\de^{\frac{16}3} e^{-\frac{A}{\de^2}}),
	\\
	G^{\unstable} - G^{\stable} 
	&= \OO(\de^{\frac{10}3} e^{-\frac{A}{\de^2}}),
\end{align*}
which implies
% Then, by \eqref{proof:poincareEstimatesDifference},
\begin{align*}
\norm{(r^{\unstable},R^{\unstable},G^{\unstable})-(r^{\stable},R^{\stable},G^{\stable})}
=&\sqrt{2}
\vabs{\D \wh{\eta}(\tht;\de)}
+ \OO(\de^{\frac{10}3} e^{-\frac{A}{\de^2}}) \\
=&
\sqrt[3]{4} \, \de^{\frac43} e^{-\frac{A}{\de^2}} 
\boxClaus{\vabs{\CInn}+\OO\paren{\frac1{\vabs{\log \de}}}}.
\end{align*}
To conclude the proof of  Theorem 
\ref{theorem:mainTheorem}, it is enough to recall that $\de=\mu^{\frac14}$.

%%%%%%%%%%%%%%%%
 
%\begin{equation}\label{proof:inversetheta}
%\begin{split}	
%\tht &= g_{\tht}(\la,L,\eta,\xi)
%= \la + i\sqrt2 e^{-i\la}\eta -i \sqrt2 e^{i\la} \xi + \OO(L-1,\eta,\xi)^2,
%\\
%\la  &=  g_{\la}(\tht,L,\eta,\xi) 
%	= \tht - i \sqrt2 e^{-i\tht} \eta + 
%	i \sqrt2  e^{i\tht} \xi + \OO(L,\eta,\xi)^2.
%\end{split}
%\end{equation}
%Notice that, by \eqref{proof:poincareEstimatesExistence}, 
%$
%\vabs{(L^{\diamond}(\la_*)-1,\eta^{\diamond}(\la_*),
%	\xi^{\diamond}(\la_*))} \leq C \de \ll 1.
%$
%Therefore, we can apply the results in Lemma \ref{lemma:seriesExpansionPoincare} and \eqref{proof:inversetheta}. 
%%
%Then,
%\begin{align*}
%\la^{\diamond}(\tht_*) = 
%g_{\la}(\tht_*,L^*()) 
%\end{align*}
%




==> proofH-existenceTechnicalChangeuOut.tex <==
\subsection{Proof of Lemma~\ref{lemma:computationsRRRtransitionOuter}}
\label{subsubsection:ProofcomputationsRRRtransitionOuter}

\textcolor{red}{Es podria treure.}

%Let us recall operator $R$ as defined in~\eqref{def:operatorRRRtransition} is	
%$
%	R[\varphi](v) = \partial_w H_1^{\out}
%	\paren{v + \varphi(v), \zuOut(v+\varphi(v))},
%$
%with $\zuOut$ as given in Proposition~\ref{proposition:existenceComecocos} and the Hamiltonian $H_1^{\out}$ in \eqref{def:hamiltonianOuterSplit}.
%
%Then, we need to obtain estimates for $R[\varphi]$.

First, let us notice that, since $\DOuterTilde \subset \DuOut$, we have that $\YcalOuter \subset \XcalOut_{0,0}$ (see \eqref{def:XcalOut}).
%
Therefore, for $\al,\beta \in \reals$, if $\phiA \in \XcalOut_{\al,\beta}$ then $\phiA \in \YcalOuter$ and
\begin{equation*}%\label{proof:normesOutTilde}
	\normSup{\phiA} \leq C \normOut{\phiA}_{\al,\beta}.
\end{equation*}

Let $\phiA \in \YcalOuter$ such that $\normSup{\phiA}\leq \varrho \de^2$ and $v \in \DOuterTilde$
%
then, for $\de$ small enough, $v+\phiA(v) \in \DuOut$. 
%
As a result, we can apply the estimates of the derivatives of $H_1^{\out}$ obtained in the proof of Lemma \ref{lemma:computationsRRROut} to operator $R[\phiA]$ (see \eqref{def:operatorRRRtransition}).
%
Indeed, by \eqref{proof:estimatef1OutDCerivatives},
\begin{align*}
\normSup{R[\phiA]}
\leq
\normOut{\partial_w H_1^{\out}
\paren{\cdot, \zuOut}}_{1,-\frac{2}{3}}
\leq
C\de^2.
\end{align*}
Analogously, we can compute estimates for the derivative $DR[\phiA]$. Indeed, applying the results in Proposition \ref{proposition:existenceComecocos},
\eqref{proof:estimategOutDerivatives} and \eqref{proof:estimatef1OutDCerivatives}, we obtain
\begin{align*}
\normSup{DR[\phiA]} \leq&
\normOut{\partial_{uw} H_1^{\out}(\cdot,\zuOut)}_{1,\frac{1}{3}}
+
\normOut{\partial^2_{w} H_1^{\out}(\cdot,\zuOut)}_{0,-\frac{2}{3}}
	\normOut{\partial_u \wuOut}_{1,1} \\
	&+
	\normOut{\partial_{wx} H_1^{\out}(\cdot,\zuOut)}_{0,\frac53}
	\normOut{\partial_u \xuOut}_{0,\frac53}
	+
	\normOut{\partial_{wy} H_1^{\out}(\cdot,\zuOut)}_{1,-2}
	\normOut{\partial_u \yuOut}_{0,\frac{7}{3}} 
	\leq C \de^2.
%	\\
%	\leq&
%	C\de^2 + 
%	\frac{C}{\de^2} \normOut{\partial_{wx} H_1^{\out}(\cdot,\zuOut)}_{0,\frac{5}{3}}
%	+ 
%	\frac{C}{\de^2} \normOut{\partial_{wy} H_1^{\out}(\cdot,\zuOut)}_{0,\frac{5}{3}}
%	\leq C\de^2.
\end{align*}
\qed






==> proofH-existenceTechnicalFlow.tex <==
\subsection{Proof of Lemma~\ref{lemma:computationsRFlow}}
\label{subsubsection:ProofComputationsRFlow}

\textcolor{red}{Es podria treure.}

By the definition of $\RRR^{\flow}[\phiA]$ in \eqref{def:operatorRFlow}, we need to estimate  the derivatives of $H_1(\G_h(v)+\phiA(v);\de)$ and
\begin{align}\label{proof:functionTopertatorRflow}
T[\phiA_{\la}] = -V'(\la_h+\phiA_{\la}) +V'(\la_h)
+ V''(\la_h)\phiA_{\la},
\end{align}
where the potential $V$ is given in \eqref{def:potentialV}.

Let us consider $\phiA=(\phiA_{\la},\phiA_{\La},\phiA_x,\phiA_y) \in \XcalFlowTotal$ such that $\normFlowTotal{\phiA} \leq \varrho \de^3$.
%
%We define $\Phi=(\Phi_{\la},\Phi_{\La},\Phi_x,\Phi_y) = \G_h + \phiA$.
%%
By Theorem \ref{theorem:singularities}, for $v \in \DFlow$ and $\de$ small 
\begin{align}\label{proof:estimatesFlow}
\vabs{\la_h(v)+\phiA_{\la}(v)} < \pi, \quad
\vabs{\La_h(v)+\phiA_{\La}(v)} < C, \quad
\vabs{\phiA_{x}(v)} < C\de^3, \quad
\vabs{\phiA_{y}(v)} < C\de^3.
\end{align}
%
Then, by definition of $H_1$ in \eqref{def:hamiltonianScalingH1}, we have that
\begin{align*}
H_1(\G_h(v)+\phiA(v);\de) =& \,
H_1^{\Poi}\big(\la_h(v)+\phiA_{\la}(v),
1+\de^2(\La_h(v)+\phiA_{\La}(v)),
\de \phiA_x(v),\de \phiA_y(v);\de \big)  \\
&- V(\la_h(v)+\phiA_{\la}(v)) +
\frac{1}{\de^4} F_{\pend}(\de^2\La_h(v)+\de^2\phiA_{\La}(v)),
\end{align*}
where $H_1^{\Poi}$ is given in \eqref{def:hamiltonianPoincare1} and $F_{\pend}$ in \eqref{def:Fpend}, respectively.
%
(Recall that $F_{\pend}(s)=\OO(s^3)$).
%
By \eqref{proof:estimatesFlow} we have that $\vabs{(\de^2(\La_h(v)+\phiA_{\La}(v)),
\de \phiA_x(v), \de \phiA_y(v))} \ll 1$, 
for $\de$ small enough,  and
$\vabs{\la_h(v)+\phiA_{\la}(v)}<\pi$, as  a result, we can apply the results in Corollary \ref{corollary:seriesH1Poi}.
%
Indeed, for $v \in \DFlow$,
\begin{equation}\label{proof:flowA}
\begin{aligned}	
\vabs{\partial_{\la} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de^2, 
& \quad
\vabs{\partial_{x} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de,
\\
\vabs{\partial_{\La} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de^2, 
& \quad
\vabs{\partial_{y} H_1(\G_h(v)+\phiA(v);\de)} 
&\leq C \de,
\end{aligned}
\end{equation}	
and
\begin{equation}\label{proof:flowB}
\begin{split}
%\vabs{ \partial_{\la\La} H_1(\G_h(v)+\phiA(v);\de)}
%&\leq C \de^2
%\qquad
%\vabs{ \partial^2_{\La} H_1(\G_h(v)+\phiA(v);\de)}
%\leq C \de^2, 
%\\
\vabs{\partial_{i j} H_1(\G_h(v)+\phiA(v);\de)} &\leq C \de, 
\qquad \text{for } i,j \in \claus{\la,\La,x,y}.
\end{split}
\end{equation}

Then, it only remains to compute estimates for  $T[\phiA_{\la}]$.
%
By \eqref{proof:functionTopertatorRflow} and
\eqref{proof:estimatesFlow} we have that, for $v \in \DFlow$,
\begin{equation}\label{proof:flowC}
\begin{split}	
\vabs{T[\phiA](v)} \leq C \vabs{V''(\la_h(v))}
\vabs{\phiA_{\la}(v)} \leq C \de^2, \\
\vabs{D T[\phiA](v)} \leq C \vabs{V'''(\la_h(v))}
\vabs{\phiA_{\la}(v)} \leq C \de^2.
\end{split}
\end{equation}

Lastly, joining the estimates from \eqref{proof:flowA},
\eqref{proof:flowB} and \eqref{proof:flowC} we obtain the statement of the lemma. 

\qed

